Writing Reusable Digital Geometry Algorithms in a Generic Image Processing Framework

Digital Geometry software should reflect the generality of the underlying mathe- matics: mapping the latter to the former requires genericity. By designing generic solutions, one can effectively reuse digital geometry data structures and algorithms. We propose an image processing framework focused on the Generic Programming paradigm in which an algorithm on the paper can be turned into a single code, written once and usable with various input types. This approach enables users to design and implement new methods at a lower cost, try cross-domain experiments and help generalize results

==> share/ChangeLog <==
2012-02-21  Roland Levillain  <roland@lrde.epita.fr>

	Misc fixes in bib/sip.bib.

	* bib/sip.bib (cousty.09.iwcia): Remove useless field `series'.
	(itk.www): Protect the author's name.

2012-02-14  Roland Levillain  <roland@lrde.epita.fr>

	Bib: fixes.

	* bib/lang.bib (gosling.05.book): Fix title.
	Wrap long lines.
	* bib/sip.bib (pink.www): Fix case of authors.
	(rusinkiewicz.04.3dpvt):  Adjust whitespace.

2012-02-14  Roland Levillain  <roland@lrde.epita.fr>

	More bib entries in lang.bib and sip.bib.

	* bib/lang.bib (iso.08.fortran, ousterhout.09.book)
	(van-rossum.03.book)
	* bib/sip.bib (bradski.08.book, burger.08.book, dgtal.www)
	(eaton.02.book, froment.04.megawave, gandalf.www)
	(graphicsmagick.www, guenter.10.tr, hamey.07.dicta, imagej.www)
	(imagene.www, imlab.www, imlib3d.05.www, imview.www, itk.www)
	(leptonica.www, mamba.www, matlab.www, mathematica.www)
	(micromorph.www, octave.www, pil.www, qgar.www, sage.www)
	(scilab.www, still.05.book, vigra.www, vsipl++.11.spec)
	(wolfram.03.book, xip.www, yayi.www):
	New entries.

2012-02-13  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (rusinkiewicz.04.3dpvt): New entry.

2012-02-13  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lang.bib (gosling.05.book): New entry.

2012-02-12  Roland Levillain  <roland@lrde.epita.fr>

	Add bib entries for the latest ISO/IEC C and C++ standards.

	* bib/lang.bib (iso.11.c, iso.11.c++): New entries.

2012-02-14  Roland Levillain  <roland@lrde.epita.fr>

	New bib entries in compilation.bib, lang.bib and sip.bib.

	* bib/compilation.bib (lattner.04.cgo)
	* bib/lang.bib (beazley.96.usenix, gosling.05.book)
	* bib/sip.bib (cimg.www,numpy.11.ref,scipy.11.ref):
	New entries.

2012-02-14  Roland Levillain  <roland@lrde.epita.fr>

	Start a bibliography on parallel programming.

	* bib/parallel.bib: New.
	* Makefile (BIBS): Add parallel.bib.

2012-02-14  Roland Levillain  <roland@lrde.epita.fr>

	Start a bibliography on reproducible research.

	* bib/rr.bib: New.
	* Makefile (BIBS): Add rr.bib.

2012-01-31  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib, bib/mc.bib: Make neat.

2012-01-31  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (chedeau.12.tr): Protect the case of language names.

2012-01-30  Jonathan Fabrizio <jonathan@lrde.epita.fr>

	Fix spic2012 entry in lrde.bib

	* bib/lrde.bib: Fix spic2012 entry in lrde.bib
	* bib/make-bib.pl: Add 2012 in generation script

2012-01-31  Parutto Pierre  <parutto@lrde.epita.fr>

	* bib/mc.bib (duret.07.phd): new entry

2012-01-31  Didier Verna  <didier.verna@gmail.com>

	* bib/lrde.bib (chedeau.12.tr): New entry.

2011-12-14  Roland Levillain  <roland@lrde.epita.fr>

	Fix the install target.

	* Makefile (papers_DATA): s/README-lrde.bib/README-lrde-bib.txt/.

2011-12-01  Roland Levillain  <roland@lrde.epita.fr>

	Update the URL of Git share.

	* bin/git-submodules: s/git.lrde.org/git.lrde.epita.fr/.

2011-12-14  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (fabrizio.11.spic): New entry.

2011-12-14  Felix Abecassis  <abecassis@lrde.epita.fr>

	* bib/csi.bib: New entry.

2011-11-29  Roland Levillain  <roland@lrde.epita.fr>

	* bin/texi2dvi: Update from upstream.

2011-11-16  Roland Levillain  <roland@lrde.epita.fr>

	Support the generation of handouts containing notes.

	* make/handout.mk (%-notes.tex):
	(%-notes-2.pdf, %-notes-4.pdf, %-notes-6.pdf):
	New targets.

2011-11-16  Roland Levillain  <roland@lrde.epita.fr>

	Add support for 2-up handouts.

	* bin/beamer2handout: Here.
	* make/handout.mk (%-handout-2.pdf): New target.
	(CLEANFILES): Add *-handout-2.pdf.

2011-10-20  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (austern.99.book, musser.01.book): New entries.

2011-10-20  Roland Levillain  <roland@lrde.epita.fr>

	* bin/beamer2handout: Pass `--no-landscape' to pdfnup in 6-up mode.

2011-10-11  Roland Levillain  <roland@lrde.epita.fr>

	Fix bib/lrde.bib.

	* bib/lrde.bib: Fix `month' fields.
	Protect acronyms' case.
	Bib neat.

2011-10-11  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (duret.11.atva): Update with page numbers.

2011-09-30  Roland Levillain  <roland@lrde.epita.fr>

	Tidy bibliographies.

	* bib/csi.bib,
	* bib/gp.bib,
	* bib/sip.bib:
	Simplify the use of diacritics.
	* bib/lrde.bib: Likewise.
	(lazzara.11.icdar): Mark as published.
	(dolstra.10.jfp): Preserve the case of `Linux'.
	* bib/lang.bib,
	* bib/tiger.bib:
	Add a title.

2011-09-28  Akim Demaille  <Akim.Demaille@gmail.com>

	bin: sync with Gostai.
	* bin/texi2dvi: Sync with Gostai.
	* bin/xhtex: New.

2011-09-27  Roland Levillain  <roland@lrde.epita.fr>

	* make/dist.mk (distdir): Depend on $(data_DATA).

2011-09-27  Akim Demaille  <Akim.Demaille@gmail.com>

	share: AM_DEFAULT_VERBOSITY.
	* make/share.mk: here.

2011-09-27  Akim Demaille  <Akim.Demaille@gmail.com>

	mybabel: simplify switchlanguage.
	For some reason, in some cases, this works better.
	* styles/mybabel.hva: here.

2011-09-15  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (duret.11.vecos): Update.

2011-09-13  Roland Levillain  <roland@lrde.epita.fr>

	New bib entries used in my Ph.D. dissertation.

	* bib/gp.bib (veldhuizen.98.oomisec)
	* bib/sip.bib (beucher.79.iwip, bosc.03.phd)
	(cousty.09.iwcia,dias.11.dgci):
	New entries.

2011-09-13  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (levillain.11.gretsi): Mark as published.

2011-09-14  Akim Demaille  <Akim.Demaille@gmail.com>

	*.txt.
	* styles/README.txt: New.
	* styles/README: Remove.

2011-09-14  Akim Demaille  <Akim.Demaille@gmail.com>

	Sync with Gostai.
	* styles/myhyperref.sty, styles/myifthen.hva,
	* styles/myindex.sty, styles/mylistings.hva,
	* styles/mylistings.sty: here.

2011-09-14  Akim Demaille  <Akim.Demaille@gmail.com>

	UTF-8.
	* doc/hevea.txt, doc/share.txt, doc/svn.txt,
	* doc/update-lrde-bib.txt: here.

2011-09-14  Akim Demaille  <Akim.Demaille@gmail.com>

	Use *.txt for text files.
	* README-lrde-bib.txt: New.
	* README-lrde.bib: Remove.
	* README.txt: New.
	* README: Remove.
	* TODO.txt: New.
	* TODO: Remove.

2011-09-14  Akim Demaille  <Akim.Demaille@gmail.com>

	Sync with Gostai.
	* make/pdf-figs.mk, make/tex.mk: Here.

2011-09-14  Akim Demaille  <Akim.Demaille@gmail.com>

	Sync with Gostai.
	* bin/texloganalyser: New.
	* styles/headings.ist: New.
	* styles/ocaml.sty: Remove duplicate with styles/ldf/ocaml.sty.

2011-09-14  Akim Demaille  <Akim.Demaille@gmail.com>

	sync with gostai.
	* bin/texi2dvi: here.

2011-09-08  Akim Demaille  <Akim.Demaille@gmail.com>

	(partial) sync with Gostai.
	* styles/ldf/README.txt: Rename as...
	* styles/ldf/README: this.
	* styles/ldf/gdb.sty: New.
	* styles/ldf/ocaml.sty: New.
	* make/tex.mk, styles/ldf/bnf.sty, styles/ldf/c++.sty,
	* styles/ldf/urbiscript.sty: Sync.

2011-09-08  Didier Verna  <didier@lrde.epita.fr>

	* bib/lrde.bib (verna.11.onward, verna.11.tug): New entries.

2011-08-03  Roland Levillain  <roland@lrde.epita.fr>

	Augment gp.bib.

	* bib/gp.bib (koethe.98.gp): New entry.
	(dehnert.98.gp): Add editors.

2011-09-03  Roland Levillain  <roland@lrde.epita.fr>

	New entries in gp.bib and sip.bib.

	* bib/gp.bib (frigo.05.ieee, karmesin.98.iscope): New entries.
	(siek.98.iscope): Complete field `booktitle'.  Add a `publisher'
	field.
	* bib/sip.bib (pink.www): New entry.

2011-08-31  Akim Demaille  <Akim.Demaille@gmail.com>

	simpson: more of them.
	* styles/simpsons/burns.mf: New.
	* styles/simpsons/snpp.mf: New.

2011-07-29  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib: Clean up.

2011-07-29  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (heinzl.06.lcsd, spevak.06.lcsd): New entries.

2011-07-26  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (duret.11.vecos, duret.11.sumo): New entries.

2011-07-06  Roland Levillain  <roland@lrde.epita.fr>

	Clean up bibliographies with bibneat.

	* bib/csi.bib,
	* bib/gp.bib,
	* bib/lang.bib,
	* bib/lrde.bib,
	* bib/sip.bib:
	Here.

2011-07-06  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lang.bib (lang-bench.www): Fix field `howpublished'.

2011-07-06  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (lazzara.11.icdar): Update the abstract (again).

2011-07-04  Coddy Levi  <levi@lrde.epita.fr>

	* bib/csi.bib: Change abstract of levi.11.seminar

2011-07-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (lazzara.11.icdar): Update abstract.

2011-06-30  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (lazzara.11.icdar): Update title.

2011-06-29  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (duret.11.arxiv): New entry.

2011-06-27  Roland Levillain  <roland@lrde.epita.fr>

	Rename entry stroustrup.2007.hopl and move it into bib/lang.bib.

	* bib/compilation.bib (stroustrup.2007.hopl): Move entry...
	* bib/lang.bib (stroustrup.07.hopl): ...here.

2011-06-24  Roland Levillain  <roland@lrde.epita.fr>

	New entries in gp.bib, lang.bib and sip.bib.

	* bib/gp.bib (garcia.07.jfp)
	* bib/lang.bib (lang-bench.www)
	* bib/sip.bib (dobie.91.prl):
	New entries.

2011-06-23  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (duret.11.atva): New entry.

2011-06-23  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (bensalem.11.sumo): Update.

2011-06-28  Pierre Parutto  <parutto@lrde.epita.fr>

	Debugged nameclash on ifpdf package

	* share/styles/semann.cls
	Removed ifpdf inclusion/definition

	* share/styles/semplan.cls
	Removed ifpdf inclusion/definition

2011-06-20  Roland Levillain  <roland@lrde.epita.fr>

	Use a uniform syntax for authors in bibliographies.

	* bib/gp.bib
	(abrahams.04.metaprog, dosreis.06.popl, gregor.05.ijpp):
	Separate authors with `and'.
	(dosreis.06.popl, gregor.06.oopsla):
	Protect Gabriel Dos Reis' name.

2011-06-15  Julien Marquegnies  <marquegnies@lrde.epita.fr>

	* bib/csi.bib: New entry. Bib neat.

2011-06-13  Akim Demaille  <Akim.Demaille@gmail.com>

	EBNF.
	* styles/ldf/bnf.sty: Restore, for bw compat.

2011-06-13  Akim Demaille  <Akim.Demaille@gmail.com>

	Fix typo.
	* make/tex.mk (rev.sty): here.

2011-06-13  Akim Demaille  <Akim.Demaille@gmail.com>

	svn-grep.
	* bin/svn-grep: New.

2011-06-13  Guillaume Fiette  <fiette@lrde.epita.fr>

	* bib/csi.bib: Change title of fiette.11.seminar.

2011-06-13  Akim Demaille  <Akim.Demaille@gmail.com>

	More silent-rules support.
	* make/dist.mk: Space changes.
	* make/handout.mk: Here to.
	* make/tex.mk: Remove support for obsolete rev.tex.

2011-06-13  Guillaume Fiette  <fiette@lrde.epita.fr>

	* bib/csi.bib: Change title of fiette.11.seminar

2011-06-13  Guillaume Fiette  <fiette@lrde.epita.fr>

	* bib/csi.bib: New entry. Bib neat.

2011-06-12  Coddy Levi  <levi@lrde.epita.fr>

	* bib/csi.bib: New entry. Bib neat.

2011-06-12  Sylvain Lobry  <lobry@lrde.epita.fr>

	* bib/csi.bib: New entry. Bib neat.

2011-06-12  Felix Abecassis  <abecassis@lrde.epita.fr>

	* bib/csi.bib: New entry. Bib neat.

2011-06-08  Roland Levillain  <roland@lrde.epita.fr>

	Complete myhyperref.sty w.r.t. the LNCS style.

	* styles/myhyperref.sty: Define \chapterautorefname and
	\subfigureautorefname resp. to `Chap.' and `Fig.' in LNCS style.

2011-06-06  Roland Levillain  <roland@lrde.epita.fr>

	* bib/csi.bib: Bib neat.

2011-06-06  Roland Levillain  <roland@lrde.epita.fr>

	New bib entries.

	* bib/sip.bib (ibanez.05.book, morph-m.www): Here.
	(gil.www): Remove the year.

2011-06-06  Roland Levillain  <roland@lrde.epita.fr>

	Protect values assigned to local variables in svn-externals.

	* bin/svn-externals (svn_youngest, svn_externals_update_stream):
	Here.

2011-05-31  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/mc.bib (manna.87.podc, ehlers.10.spin, tsay.11.tacas):
	New entries.

2011-06-01  Roland Levillain  <roland@lrde.epita.fr>

	Check more files with `make neat'.

	* Makefile (BIBS): Add gp.bib, lang.bib, olena.bib and tiger.bib.
	* bib/gp.bib,
	* bib/lang.bib,
	* bib/olena.bib,
	* bib/tiger.bib:
	Bib-neat them.

2011-06-01  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib, bib/mc.bib, bib/sip.bib: Bib neat.

2011-06-01  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (geraud.10.livre): Fix field `editor'.

2011-06-01  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (lazzara.11.icdar): New entry.

2011-06-01  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (levillain.11.gretsi): Fix field `urllrde'.

2011-05-20  Roland Levillain  <roland@lrde.epita.fr>

	Fix mylistings.

	* styles/mylistings.hva: Do not include the non-existing
	ldf/ocaml.sty.

2011-05-20  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lang.bib (iso.06.eiffel): New entry.

2011-05-19  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (bensalem.11.sumo): New entry.

2011-05-16  Roland Levillain  <roland@lrde.epita.fr>

	Tag GRETSI symposia as national conferences.

	* bib/lrde.bib (baillard.07.gretsi, levillain.11.gretsi): Here.

2011-05-16  Roland Levillain  <roland@lrde.epita.fr>

	* bin/make-bib.pl: Cover publications of 2011.

2011-05-16  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (levillain.11.gretsi): New entry.

2011-05-09  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (bracha.90.sigplan): New entry.

2011-05-09  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (angulo.10.chapter): New entry.

2011-05-02  Roland Levillain  <roland@lrde.epita.fr>

	New entries in bib.gp and lang.gp.

	* bib/gp.bib (cleary.05.staticassert, gregor.05.ijpp)
	(klarer.04.staticassert, siek.99.msthesis)
	* bib/lang.bib (stawiaski.08.phd, ta.08.eccv):
	New entries.

2011-05-02  Roland Levillain  <roland@lrde.epita.fr>

	Fix some bibliographical entries.

	* bib/gp.bib (czarnecki.00.book): Do not protect title.
	Add missing year.
	(meyers.00.cuj): Fix journal name.
	* bib/lang.bib (iso.0x.c++): Use a correct month abbreviation.

2011-04-20  Roland Levillain  <roland@lrde.epita.fr>

	Remove the year from the ConceptGCC Web site reference.

	* bib/gp.bib (conceptgcc.07.www): Rename as...
	(conceptgcc.www): ...this.
	Remove the year.

2011-04-19  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lang.bib (iso.05.ada): New entry.

2011-04-13  Roland Levillain  <roland@lrde.epita.fr>

	More references in lang.bib and gp.bib.

	* bib/lang.bib (alexandrescu.10.d,  budd.95.leda,  budd.95.leda)
	* bib/gp.bib (czarnecki.98.phd, pooma.www):
	New entries.
	(boost.08.www): Rename as...
	(boost.www): ...this.
	Remove the year.

2011-05-19  Akim Demaille  <Akim.Demaille@gmail.com>

	Sunc with Gostai.
	* styles/ldf/bnf.sty, styles/ldf/urbiscript.sty,
	* styles/ldf/yacc.sty, styles/mycxx.sty,
	* styles/mylistings.hva: Sync.
	* styles/ocaml.sty: New.

2011-05-19  Akim Demaille  <Akim.Demaille@gmail.com>

	compilation.bib.
	* bib/compilation.bib (conway.63.jacm, lewis.68.jacm): New.

2011-04-28  Roland Levillain  <roland@lrde.epita.fr>

	Typo in lang.bib.

	* bib/lang.bib (atskinson.78.acm): Rename entry as...
	(atkinson.78.acm): ...this.

2011-04-07  Akim Demaille  <Akim.Demaille@gmail.com>

	curve: update to 1.16.
	* curve.cls: From 1.10.

2011-04-05  Roland Levillain  <roland@lrde.epita.fr>

	* doc/share.txt: Typo.

2011-04-05  Roland Levillain  <roland@lrde.epita.fr>

	* Makefile: Aesthetic change.

2011-04-04  Roland Levillain  <roland@lrde.epita.fr>

	New entries in bib.gp.

	* bib/gp.bib (unruh.94.tr, veldhuizen.03.tr, veldhuizen.95.www):
	New entries.

2011-03-29  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (musser.94.spe): New entry.

2011-03-28  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/mc.bib (dallien.06.aejm, geldenhuys.06.spin, heiner.08.sfm)
	(loding.01.ipl, pyarali.00.lctes): New references.  Also fix
	Springer/Spring-Verlag usage: all LNCS volumes >= 3130 are
	published by Springer, all LNCS volumes < 3130 are published by
	Springer-Verlag.
	* bib/csi.bib: Run bibneat.

2011-03-24  Roland Levillain  <roland@lrde.epita.fr>

	New bib entries in gp.bib.

	* bib/gp.bib (lorusso.www, plauger.00.book, sgi.stl)
	(stevens.95.ddj, stepanov.95.tr): New entries.

2011-03-22  Roland Levillain  <roland@lrde.epita.fr>

	Add language definition of CLU for listings package.

	* styles/ldf/clu.sty: New file.
	Include it...
	* styles/mylistings.hva: ...here.

2011-03-22  Roland Levillain  <roland@lrde.epita.fr>

	New bib entries.

	* bib/lang.bib (atskinson.78.acm, liskov.93.hopl)
	* bib/sip.bib (berti.00.phd, koethe.00.phd):
	Here.

2011-03-22  Roland Levillain  <roland@lrde.epita.fr>

	Move ellis.90.arm from gp.bib to lang.bib.

	* bib/gp.bib (ellis.90.arm): Move entry...
	* bib/lang.bib: ...here.

2011-03-24  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (sutter.09.blog): New entry.

2011-03-17  Roland Levillain  <roland@lrde.epita.fr>

	Have texi2dvi honor Automake's silent rules.

	* make/tex.mk (AM_DEFAULT_VERBOSITY): Set to 1 by default, so as
	to keep the compatibility with Makefiles not generated by
	Automake (1.11).
	(texi2dvi_verbose, texi2dvi_verbose_, texi2dvi_verbose_0): New.
	(TEXI2DVIFLAGS): Append $(texi2dvi_verbose).

2011-03-15  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (dehnert.98.gp, jazayeri.98.report): New entries.

2011-03-15  Roland Levillain  <roland@lrde.epita.fr>

	Create a bibliography for programming languages.

	* bib/transformers.bib (iso.98.c++, iso.03.c, iso.99.c)
	(iso.0x.c++): Move entries...
	* bib/lang.bib: ...here (new file).

2011-03-11  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (ellis.90.arm, stroustrup.89.cs): New entries.

2011-03-07  Roland Levillain  <roland@lrde.epita.fr>

	Remove obsolete language definitions.

	* styles/ldf/lstgrammar.sty: Remove (service already provided by
	styles/ldf/bnf.sty and styles/ldf/sdf.sty).
	* styles/ldf/ocaml.sty: Remove (was a duplicate of the
	built-in Objective Caml style).

2011-02-23  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (veldhuizen.98.iscope): New entry.

2011-02-23  Roland Levillain  <roland@lrde.epita.fr>

	* bib/olena.bib (olena.www): Remove field `year'.

2011-02-04  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (karvonen.02.pp): Fix title and URL.

2011-02-04  Roland Levillain  <roland@lrde.epita.fr>

	Add new entries to bib/gp.bib.

	* bib/gp.bib (pirkelbauer.08.sac, pirkelbauer.10.scp)
	(stepanov.09.book, veldhuizen.95.c++a): New entry.
	(veldhuizen.95.c++): Rename as...
	(veldhuizen.95.c++b): ...this.

2011-02-04  Roland Levillain  <roland@lrde.epita.fr>

	Fix and augmented entries related to ``C++ Gems''.

	* bib/gp.bib (myers.96.cppgems, veldhuizen.96.cppgemsa):
	New entries.
	(veldhuizen.98.cppgems): Rename entry as...
	(veldhuizen.96.cppgemsb): ...this.
	(coplien.96.cppgems,veldhuizen.96.cppgemsb): Use @InCollection
	entry types.
	Instead of citing it, inline fields booktitle, editor and
	publisher from...
	(cppgems): ...this entry.
	Fix editor's name and year.

2011-01-24  Roland Levillain  <roland@lrde.epita.fr>

	Fix bib entries.

	* bib/lrde.bib (levillain.09.ismm): Complete entry.
	(levillain.10.wadgmm): Add an `url' field.
	* bib/gp.bib (siek.01.bgl): Use an abbreviation in field `month'.

2011-01-22  Akim Demaille  <Akim.Demaille@gmail.com>

	More bison directives.
	* styles/ldf/asf.sty: Minor change.
	* styles/ldf/yacc.sty: Support for directives.

2011-01-17  Roland Levillain  <roland@lrde.epita.fr>

	* bib/olena.bib (olena.www): s/library/platform/.

2010-12-13  Roland Levillain  <roland@lrde.epita.fr>

	* bib/mc.bib (tabakov.10.rv): Typo.

2010-12-13  Roland Levillain  <roland@lrde.epita.fr>

	Update Springer's LNCS style.

	* styles/llncs.cls: Update to version 2.17.

2010-12-13  Roland Levillain  <roland@lrde.epita.fr>

	Fix some address fields.

	* bib/compilation.bib (kuipers.03.scp)
	* bib/sensor-networks.bib (verifsn1)
	* bib/sip.bib (berti.06.fgcs, goutsias.00.fi, meijster.04.phd)
	* bib/transformers.bib (cordy.06.scp):
	Here.

2010-12-10  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/mc.bib (cichon.09.depcos, dax.07.atva, tabakov.10.rv): New
	entries.
	(rozier.07.spin): Protect {LTL}.

2010-12-09  Roland Levillain  <roland@lrde.epita.fr>

	beamer2handout: Catch up with the current interface of pdfnup.

	* bin/beamer2handout: Use option `--landscape' (resp. nothing)
	instead of `--orient landscape' (resp. `--orient portrait').

2010-12-08  Roland Levillain  <roland@lrde.epita.fr>

	Fix `.id' to `.pdf' conversions.

	* make/pdf-figs.mk (%.pdf): Here.

2010-12-08  Akim Demaille  <Akim.Demaille@gmail.com>

	More about the LR paper.
	* bib/transformers.bib: here.

2010-11-24  Akim Demaille  <Akim.Demaille@gmail.com>

	yacc: fix comments.
	* styles/ldf/yacc.sty: here.

2010-11-24  Roland Levillain  <roland@lrde.epita.fr>

	* make/pdf-figs.mk (%.png): Help Dia select the output type.

2010-11-24  Akim Demaille  <Akim.Demaille@gmail.com>

	tex.mk: ensure target dir.
	WARNING: You might need to change your *_FLAGS.
	* make/tex.mk: Rename all *_FLAGS into *FLAGS, as per
	Make standards.
	Use ENSURE_TARGET_DIR to make sure we output in an existing
	dir.

2010-11-24  Akim Demaille  <Akim.Demaille@gmail.com>

	share: update.

2010-11-24  Akim Demaille  <Akim.Demaille@gmail.com>

	pdf-figs.mk: support silent-mode.
	* make/pdf-figs.mk: here.

2010-11-02  Roland Levillain  <roland@lrde.epita.fr>

	Add Nicolas Pierron's paper on NixOS.

	* bib/lrde.bib (dolstra.10.jfp): New entry.

2010-11-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib: Make it neat.

2010-10-26 Jonathan Fabrizio <jonathan@lrde.epita.fr>

	* bib/lrde.bib: Add minetto.10.icip

2010-10-22  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (siek.05.pldi): New entry.

2010-10-22  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (rozenfeld.66.jacm): New entry.

2010-10-18  Roland Levillain  <roland@lrde.epita.fr>

	* styles/bilan.hva, styles/bilan.sty: Convert to UTF-8.

2010-10-06  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (levillain.10.icip): Add page numbers.

2010-10-05  Didier Verna  <didier@lrde.epita.fr>

	* bib/lrde.bib: Added verna.10.tug.

2010-10-04  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (levillain.10.icip): Set status as published.

2010-09-21  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (couprie.09.pami): Add lrdedoc field.

2010-09-21  Thierry GERAUD  <thierry.geraud@lrde.epita.fr>

	* bib/lrde.bib (geraud.10.livre): Fix pages.

2010-09-16  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (couprie.01.jei): New entry.

2010-09-14  Roland Levillain  <roland@lrde.epita.fr>

	* bin/make-bib.pl: Handle book chapters properly.

2010-09-14  Roland Levillain  <roland@lrde.epita.fr>

	Fix book chapters entries.

	* bib/lrde.bib (duflot.06.book, geraud.10.book, geraud.10.livre):
	Here.

2010-09-14  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib: Make it neat.

2010-09-14  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (linard.10.acsd): New entry.

2010-09-14  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (levillain.10.wadgmm): Add page numbers.

2010-09-09  Thierry GERAUD  <thierry.geraud@lrde.epita.fr>

	* bib/lrde.bib (geraud.10.book): Fix pages.

2010-09-08  Thierry GERAUD  <thierry.geraud@lrde.epita.fr>

	* bib/lrde.bib (geraud.10.livre): New entry.
	(geraud.10.book): New entry.

2010-09-03  Roland Levillain  <roland@lrde.epita.fr>

	* bib/csi.bib: Make it neat.

2010-09-03  Roland Levillain  <roland@lrde.epita.fr>

	* bib/csi.bib: Do not use extended characters.

2010-09-03  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (dasilva.04.workcomp-sul): New entry.

2010-09-03  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (dornellas.04.workcomp-sul): New entry.

2010-09-01  Roland Levillain  <roland@lrde.epita.fr>

	* styles/lrde-bulletin.sty: Use `mathpazo' instead of `mathpple'.

2010-08-30  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (levillain.10.wadgmm): Set status as published.

2010-08-30  Roland Levillain  <roland@lrde.epita.fr>

	Update Springer's LNCS style.

	* styles/llncs.cls: Update to version 2.16.
	* styles/splncs03.bst: New.

2010-07-05  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (gil.www): New entry.

2010-07-05  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (ritter.90.cvgip): New entry.

2010-06-09  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/csi.bib: Do not enclose titles with {{...}}.

2010-06-01  Felix Abecassis  <abecassis@lrde.epita.fr>

	* bib/csi.bib: Swap abstract and resume.

2010-06-17  Roland Levillain  <roland@lrde.epita.fr>

	Properly escape some words (or not).

	* bib/lrde.bib (geraud.08.mpool): Remove superfluous parentheses
	around ``MPOOL''.
	(levillain.10.icip) Protect ``Milena'' with parentheses.

2010-05-26  Akim Demaille  <Akim.Demaille@gmail.com>

	tikz-qtree 1.1.
	http://tug.ctan.org/pkg/tikz-qtree
	* styles/pgfsubpic.sty: New.
	* styles/pgfsubpic.tex: New.
	* styles/pgftree.sty: New.
	* styles/pgftree.tex: New.
	* styles/tikz-qtree-compat.sty: New.
	* styles/tikz-qtree.sty: New.
	* styles/tikz-qtree.tex: New.

2010-05-26  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib: Add page numbers for some entries.

2010-05-26  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (levillain.10.icip): New entry.

2010-05-11  Roland Levillain  <roland@lrde.epita.fr>

	* bib/csi.bib: Tidy with `make neat'.

2010-05-11  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (levillain.10.wadgmm): New entry.

2010-05-10  Didier Verna  <didier@lrde.epita.fr>

	* bib/lrde.bib (verna.10.els): Add.

2010-05-05  Roland Levillain  <roland@lrde.epita.fr>

	Prevent name clashes with current LaTeX distributions.

	* styles/texi.hva (\acronym): Rename as...
	(\myacronym): ...this, to avoid a name clash with acronym.sty.
	* styles/lrde-bulletin.sty (\nohyphens): Rename as
	(\mynohyphens): ...this, to avoid a name clash with hyphenat.sty.

2010-05-05  Roland Levillain  <roland@lrde.epita.fr>

	Have make-bib.pl process all projects.

	* bin/make-bib.pl (@project): Add project "Verification".

2010-05-05  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib: Add a missing comma.

2010-05-05  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (hamez.08.atpn): Mark as published.

2010-05-03  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (bertrand.07.chapter): Add field `lrdedoc'.

2010-05-03  Roland Levillain  <roland@lrde.epita.fr>

	Fix make-bib.pl.

	* bin/make-bib.pl (display_help): Here.

2010-04-14  Didier Verna  <didier@lrde.epita.fr>

	* bib/lrde.bib (verna.10.jucs): Update.

2010-04-20  Julien Marquegnies  <marquegnies@lrde.epita.fr>

	* bib/csi.bib (marquegnies.10.seminar): New entry.

2010-04-20  Edwin Carlinet  <carlinet@lrde.epita.fr>

	* bib/csi.bib (carlinet.10.seminar): New entry.

2010-04-20  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (geraud.08.mpool): Complete title.

2010-04-19  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (dornellas.01.phd): New entry.

2010-04-19  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (whitehead.39.lms): New entry.

2010-04-19  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (levillain.09.ismm): Honor the 2-letter initials rule.

2010-04-15  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (couprie.09.pami): Protect case.

2010-04-07  Akim Demaille  <Akim.Demaille@gmail.com>

	update share.

2010-04-07  Akim Demaille  <Akim.Demaille@gmail.com>

	update share.

2010-04-07  Akim Demaille  <Akim.Demaille@gmail.com>

	LDF: update.
	* styles/ldf/dot.sty: New.
	* styles/ldf/urbi.sty: Rename as...
	* styles/ldf/urbiscript.sty: this.
	Complete.
	* styles/ldf/yacc.sty: Update.
	* styles/mylistings.hva: Adjust.

2010-04-07  Akim Demaille  <Akim.Demaille@gmail.com>

	texi: bbr and cronym.
	* styles/texi.hva: Add them.

2010-04-07  Akim Demaille  <Akim.Demaille@gmail.com>

	styles: catch up.
	* styles/misc.hva: here.

2010-04-07  Akim Demaille  <Akim.Demaille@gmail.com>

	myhyperref: Title case.
	* styles/myhyperref.sty: Use the Title Case for all the autoref
	names.
	Be compatible with ENTCS style.

2010-04-07  Akim Demaille  <Akim.Demaille@gmail.com>

	pdf-figs: fixes.
	* make/pdf-figs.mk: Prefer && to ;.

2010-04-07  Akim Demaille  <Akim.Demaille@gmail.com>

	pdf-figs.mk: improve.
	Catch up with Gostai's document-aux.
	* make/pdf-figs.mk: Use variable names instead of hard coded
	names.
	Create the destination directory if it does not exist.
	Work with a tmp file to avoid broken files when the process is
	interrupted.

2010-04-07  Akim Demaille  <Akim.Demaille@gmail.com>

	Avoid accents in *.sty.
	* styles/myhyperref.sty: here.
	This way we are compatible with UTF-8 and Latin 1.

2010-03-17  Akim Demaille  <Akim.Demaille@gmail.com>

	Remove Project macro names.
	* styles/lrde-bulletin.sty: Here.
	Use share/style/misc.sty instead.

2010-03-17  Akim Demaille  <Akim.Demaille@gmail.com>

	adr: remove boxedverbatim.
	* styles/lrde-bulletin.sty ({boxedverbatim}): Remove, we use
	lstlisting.

2010-03-17  Akim Demaille  <Akim.Demaille@gmail.com>

	adr: fix utf-8 conversion.
	* styles/lrde-bulletin.sty: Do not require utf8 inputenc
	inside the very macro that features utf-8 text: load it before.

2010-03-17  Akim Demaille  <Akim.Demaille@gmail.com>

	lrde-bulletin: UTF-8.
	* styles/lrde-bulletin.sty: here.

2010-03-05  Roland Levillain  <roland@lrde.epita.fr>

	Prevent name clashes between gettext.sty and translator.sty.

	* styles/gettext.sty (\newtranslation): Rename command as...
	(\newtranslationstring): ...this.

2010-02-09  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (wilson.92.ipi): New entry.

2010-02-09  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (stroustrup.2007.hopl): New entry.

2010-02-09  Roland Levillain  <roland@lrde.epita.fr>

	Add acronyms.

	* styles/myacronym.sty (ip, floss): Here.

2010-01-27  Roland Levillain  <roland@lrde.epita.fr>

	Use developed first names instead of just initials.

	* bib/lrde.bib (cadilhac.06.avocs, chekroun.06.iciar)
	(dehak.09.interspeech, dehak.09.interspeechb, lesage.06.isvc)
	(perrot.06.nist): Here.

2010-01-27  Roland Levillain  <roland@lrde.epita.fr>

	Add missing diacritics in lrde.bib.

	* bib/lrde.bib (darbon.05.eusipco, lesage.06.isvc): Here.

2010-01-29  Vincent Ordy  <ordy@lrde.epita.fr>

	Add report numbers to csi.bib.
	* bib/csi.bib: here.

2010-01-20  Roland Levillain  <roland@lrde.epita.fr>

	Install products with write permissions for the group.

	* Makefile (install): Here.
	Suggested by Geoffroy Fouquier <geoffroy.fouquier@lrde.epita.fr>.

2010-01-18  Roland Levillain  <roland@lrde.epita.fr>

	Fix instantiate-template.sh w.r.t. submodule `share'.

	* bin/instantiate-template.sh: Here.

2010-01-17  Roland Levillain  <roland@lrde.epita.fr>

	Have git-submodules handle submodules in subdirectories.

	* bin/git-submodules (git_submodules_subscribe): Include the
	subdirectory in the path of the submodule.

2010-01-17  Roland Levillain  <roland@lrde.epita.fr>

	Have instantiate-template.sh work with Git.

	* bin/instantiate-template.sh: Here.

2010-01-13  Roland Levillain  <roland@lrde.epita.fr>

	Add support for Git share.

	* make/share-am.mk (git-share-up, git-share-push):
	New (phony) targets.

2010-01-13  Roland Levillain  <roland@lrde.epita.fr>

	Have git-submodules pin existing submodules to HEAD on re-subscription.

	* bin/git-submodules (git_submodules_subscribe): Here.

2010-01-11  Roland Levillain  <roland@lrde.epita.fr>

	Update the IEEE style file for SPS Conferences (ICASSP, ICIP).

	* styles/spconf.sty: Here.
	Downloaded from
	https://www.securecms.com/ICIP2010/Papers/PaperFormat/spconf.sty.

2010-01-11  Roland Levillain  <roland@lrde.epita.fr>

	Fix the test on the number of arguments in instantiate-template.sh.

	* bin/instantiate-template.sh: Here.

2010-01-06  Akim Demaille  <Akim.Demaille@gmail.com>

	simpsons/simpsons.sty.
	Taken from http://tug.ctan.org/tex-archive/usergrps/uktug/baskervi/4_4/
	* styles/simpsons/bart.mf: New.
	* styles/simpsons/homer.mf: New.
	* styles/simpsons/lisa.mf: New.
	* styles/simpsons/maggie.mf: New.
	* styles/simpsons/marge.mf: New.
	* styles/simpsons/simpsons.mf: New.
	* styles/simpsons/simpsons.sty: New.

2010-01-05  Roland Levillain  <roland@lrde.epita.fr>

	Add #-style comments to the BNF language definition file.

	* styles/ldf/bnf.sty: Here.

2010-01-04  Roland Levillain  <roland@lrde.epita.fr>

	Add a listings language definition for Treecc.

	* styles/ldf/treecc.sty: New file.
	Use it...
	* styles/mylistings.hva: ...here.

2010-01-04  Roland Levillain  <roland@lrde.epita.fr>

	More references on Treecc.

	* bib/compilation.bib (treecc, weatherley.02.www): New entries.

2009-12-27  Guillaume Sadegh  <sadegh@lrde.epita.fr>

	* bib/csi.bib (sadegh.seminar.10): New entry.

2009-12-14  Didier Verna  <didier@lrde.epita.fr>

	* bib/lrde.bib (verna.09.jucs): New.

2009-12-10  Roland Levillain  <roland@lrde.epita.fr>

	Add git-submodules, a helper script to manipulate Git submodules.

	* bin/git-submodules: New.
	Inspired from bin/svn-externals.

2009-11-30  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bin/make-bib.pl (output): Do not call svn, it prevents this
	script from running from the git repository.
	* bib/lrde.bib: Remove the empty entry added by Reda (hiss!)

2009-11-16  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (duret.09.atva): Update page and volume.

2009-10-16  Florent DHalluin  <d-halluin@lrde.epita.fr>

	Add d-halluin.10.seminar.
	* bib/csi.bib(d-halluin.10.seminar): Add this entry.

2009-10-15  Vincent Ordy  <ordy@lrde.epita.fr>

	Add ordy.10.seminar.
	* bib/csi.bib (ordy.10.seminar): New.

2009-10-05  Thierry Geraud  <thierry.geraud@lrde.epita.fr>

	Update some LRDE logos.

	* figs/lrde-red.png,
	* figs/logo_lrde-green.png: Update to the without-tongue
	versions.

2009-09-16  Roland Levillain  <roland@lrde.epita.fr>

	Update the link to the PDF version of cousty.09.ismm in /lrde/doc/.

	* bib/sip.bib: Here.

2009-09-15  Roland Levillain  <roland@lrde.epita.fr>

	Have instantiate-template.sh be callable from everywhere.

	* bin/instantiate-template.sh: Accept an explicit template
	directory path as optional fourth parameter.

2009-09-15  Roland Levillain  <roland@lrde.epita.fr>

	Fix string substitutions in bin/instantiate-template.sh.

	* bin/instantiate-template.sh: s,vcs/locale,vcs/local.rb,.

2009-09-15  Roland Levillain  <roland@lrde.epita.fr>

	Update IEEE Transactions style and bibliography files.

	* styles/IEEEtran.cls: Update to version 1.7a.
	* styles/IEEEtranN.bst,
	* styles/IEEEtranSA.bst,
	* styles/IEEEtranSN.bst:
	New files.
	* styles/IEEEtran.bst, styles/IEEEtranS.bst,
	* bib/IEEEabrv.bib, bib/IEEEexample.bib, bib/IEEEfull.bib:
	Update to version 1.12.

2009-08-31  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (levillain.09.ismm): Mark it published.

2009-08-31  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib: Rename couprie.08.pami to couprie.09.pami.

2009-06-30  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/mc.bib (loding.98.diplom, cormen.01.algo, emerson.87.scp,
	safra.89.stoc): New entries.

2009-06-23  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (duret.09.atva): Add urllrde.

2009-06-23  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (duret.09.atva): Typo.

2009-06-23  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (duret.09.atva): New entry.
	* bib/csi.bib, bib/sip.bib: Make neat.

2009-06-29  Roland Levillain  <roland@lrde.epita.fr>

	Fix bib entry bertrand.08.chapter.

	* bib/sip.bib (bertrand.08.chapter): Remove extra introductory
	words at the beginning of field `title'.

2009-06-10  Didier Verna  <didier@lrde.epita.fr>

	* bib/lrde.bib (verna.08.lncs): New entry.

2009-06-03  Florent DHalluin  <d-halluin@lrde.epita.fr>

	csi.bib: Update d-halluin.09.seminar
	* bib/csi.bib: Update according to the report v2.

2009-06-01  Warren Seine  <soow@lrde.epita.fr>

	Add some missing "number" fields.
	* bib/csi.bib: Do that.

2009-06-01  Warren Seine  <soow@lrde.epita.fr>

	Add new entry in GP bibliography (dosreis.06.popl).
	* bib/gp.bib: New entry.
	* bib/transformers.bib: Fix C++0x draft URL.

2009-05-30  Warren Seine  <soow@lrde.epita.fr>

	Update C++0x draft date.
	* bib/transformers.bib: May 2008 -> March 2009.

2009-05-30  Warren Seine  <soow@lrde.epita.fr>

	Fix seine.09.seminar bibliography.
	* csi.bib: Improve according to RL's review.
	* gp.bib: Add year field to entry.

2009-05-28  Roland Levillain  <roland@lrde.epita.fr>

	* styles/mylistings.sty: Remove dead code.

2009-05-28  Roland Levillain  <roland@lrde.epita.fr>

	Allow user-defined distribution hooks in Makefiles.

	* make/dist.mk (dist-hook): New (empty) rule.
	Invoke it at the end of...
	(distdir): ...this rule.
	(.PHONY): Add dist-hook.

2009-05-22  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (dornellas.03.ijprai): New entry.

2009-05-20  Vincent Ordy  <ordy@lrde.epita.fr>

	Update Otto picture.
	* figs/lrde-big.png: Update to the version without tongue.

2009-05-19  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (veldhuizen.97.iscope): Fix and supplement entry.

2009-05-19  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (poincarre.99.rcmp): New entry.

2009-05-19  Roland Levillain  <roland@lrde.epita.fr>

	Turn reference cousty.09.ismm into a published entry.

	* bib/sip.bib (cousty.09.ismm): Here.
	Add missing fields.

2009-05-04  Vincent Ordy  <ordy@lrde.epita.fr>

	Adjust texi2dvi flags to be backward compatible with tildes.
	See http://lists.gnu.org/archive/html/bug-texinfo/2009-05/msg00005.html
	* make/tex.mk: Add -~ to texi2dvi flags.

2009-05-04  Akim Demaille <demaille@gostai.com>

	texi2dvi: fix spurious invocation of tex4ht.
	* bin/texi2dvi (run_tex4ht): tex4ht is not needed to create DVI
	files.

2009-05-04  Akim Demaille <demaille@gostai.com>

	texi2dvi: remote spurious $0.
	* bin/texi2dvi (run_tex): Remove duplicate $0 display.

2009-04-29  Vincent Ordy  <ordy@lrde.epita.fr>

	Give mylistings package options to listing package.
	* styles/mylistings.hva: here.

2009-04-29  Jérôme Galtier  <jerome.galtier@lrde.epita.fr>

	Fixes from Daniela.
	* bib/csi.bib: Typos in damota.09.seminar, carlinet.09.seminar and
	folio.09.seminar.

2009-04-29  Akim Demaille  <akim@lrde.epita.fr>

	Update texi2dvi from master.
	* bin/texi2dvi: here.

2009-04-27  Vincent Ordy  <ordy@lrde.epita.fr>

	Fixes from Daniela.
	* bib/csi.bib: Fix galtier.09, lefortier.09 and sadegh.09.

2009-04-20  Akim Demaille  <akim@lrde.epita.fr>

	Help tex4ht.
	* styles/myenumerate.sty: itemautorefname is sometimes
	defined, sometimes not.  So use \def.

2009-04-15  Akim Demaille  <akim@lrde.epita.fr>

	Update texi2dvi from master.
	* bin/texi2dvi: here.

2009-04-14  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib: Bib-neat again.

2009-04-14  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib: Partial spell-check.

2009-04-14  Roland Levillain  <roland@lrde.epita.fr>

	Bib-neat bib/sip.bib.

	* bib/sip.bib: Here.
	* Makefile (BIBS): Add sip.bib.

2009-04-14  Roland Levillain  <roland@lrde.epita.fr>

	* bib/csi.bib: Bib-neat it.

2009-04-14  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (levillain.09.ismm): New entry.

2009-04-14  Roland Levillain  <roland@lrde.epita.fr>

	Handle 6-up handouts.

	* make/handout.mk (%-handout-6.pdf): New target.
	(CLEANFILES): Add *-handout-6.pdf.

2009-04-09  Warren Seine  <soow@lrde.epita.fr>

	Change seine.09.seminar.
	* bib/csi.bib: Do that (was the old one).

2009-04-08  Roland Levillain  <roland@lrde.epita.fr>

	Add bibliographical entries related to digital topology.

	* bib/sip.bib (cornea.07.tvcg, lam.92.pami, lamy.07.cmpb,
	(lobregt.80.pami): New entries.

2009-04-08  Akim Demaille  <akim@lrde.epita.fr>

	Name fix.
	* bib/lrde.bib: Watch the case.

2009-04-07  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (kong.89.cvgip): Honor capitals in title.

2009-04-01  Thierry Geraud  <thierry.geraud@lrde.epita.fr>

	Remove Otto's tongue in lrde_epita.png.

	* figs/lrde_epita.png: Remove Otto's tongue.

2009-04-01  Akim Demaille  <akim@lrde.epita.fr>

	Protect acronyms in titles.
	* bib/lrde.bib (dehak.08.nist): Here.

2009-03-31  Roland Levillain  <roland@lrde.epita.fr>

	Augment and clean up bib/sip.bib.

	* bib/sip.bib (bertrand.95.cras, bertrand.06.iwcia)
	(bertrand.07.chapter, bertrand.07.cras, couprie.08.pami)
	(kong.89.cvgip, ronse.88.dam): New entries.

2009-03-31  Roland Levillain  <roland@lrde.epita.fr>

	Start a math style.

	* styles/math.sty: New.

2009-03-31  Didier Verna  <didier@lrde.epita.fr>

	Set status of verna.08.jucs to `published'.

	* bib/lrde.bib (verna.08.jucs): Remove `note' field.

2009-03-30  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bin/bibneat (bib_file_clean): Fix the regex for deleting
	empty fields.

2009-03-30  Didier Verna  <didier@lrde.epita.fr>

	Set status of verna.09.ilc to `published'.

	* bib/lrde.bib (verna.09.ilc): Remove `note' field.

2009-03-26  Florent DHalluin  <d-halluin@lrde.epita.fr>

	Fix d-halluin.09.seminar
	* bib/csi.bib: .

2009-03-24  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (gagnon.98.tools): Protect SableCC.

2009-03-23  Roland Levillain  <roland@lrde.epita.fr>

	Set status demaille.09.sac to `published'.

	* bib/lrde.bib (demaille.09.sac): Remove field `note'.

2009-03-23  Vincent Ordy  <ordy@lrde.epita.fr>

	[bin/abstract] Fix for dash in BibTeX keys.
	* bin/abstract: (getbibentries) Allow user to have a dash in is
	entry key (d-halluin, van-noppen).

2009-03-21  Vincent Ordy  <ordy@lrde.epita.fr>

	Add an option to bin/abstract to construct wiki content from
	BibTex entries.
	* bin/abstract: here.

2009-03-20  Vincent Ordy  <ordy@lrde.epita.fr>

	Take Roland's comment into account.
	* bib/csi.bib:
	(folio.09)	Add french title.
	(abraham.09)	textit -> emph.
	(ordy.09)	it -> emph.

2009-03-20  Jerome Galtier  <jerome.galtier@lrde.epita.fr>

	Take Roland's comment into account for galtier.09.seminar.
	* bib/csi.bib: Do not protect Vaucanson when unnecessary.

2009-03-20  Benoit Sigoure  <tsunanet@gmail.com>

	Make generate-rev-sty Git-friendly.
	* bin/generate-rev-sty: If svn info fails, try to use git log, just
	in case.

2009-03-19  Roland Levillain  <roland@lrde.epita.fr>

	Add a class for SIGPLAN conference proceedings.

	* styles/sigplanconf.cls: New.

2009-03-19  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (flex.07.manual): New entry.

2009-03-18  Loic Denuziere  <denuziere@lrde.epita.fr>

	Reformulate seminar abstract.
	* bib/csi.bib: Reformulate denuziere.09.seminar abstract.

2009-03-18  Florent DHalluin  <d-halluin@lrde.epita.fr>

	Add d-halluin.09.seminar to csi.bib
	* bib/csi.bib: Add d-halluin.09.seminar.

2009-03-18  Loic Denuziere  <denuziere@lrde.epita.fr>

	Reformulate seminar abstract.
	* bib/csi.bib: Reformulate denuziere.09.seminar.

2009-03-18  Edwin Carlinet  <carlinet@lrde.epita.fr>

	Add edwin's seminar entry.
	* bib/csi.bib: Add my seminar entry.

2009-03-18  Jerome Galtier  <jerome.galtier@lrde.epita.fr>

	Add galtier.09.seminar to csi.bib.
	* bib/csi.bib: Add galtier.09.seminar.

2009-03-17  Loic Denuziere  <denuziere@lrde.epita.fr>

	Update seminar abstract.
	* bib/csi.bib: Add url information to denuziere.09.seminar.

2009-03-17  Loic Denuziere  <denuziere@lrde.epita.fr>

	Add abstract to csi.bib.
	* bib/csi.bib: Add abstract.

2009-03-17  Vincent Ordy  <ordy@lrde.epita.fr>

	Add ordy.09.seminar to csi.bib.
	* bib/csi.bib: Do that + make neat.

	* bib/lrde.bib,
	* bib/mc.bib: make neat.

2009-03-17  Samuel Da Mota  <da-mota@lrde.epita.fr>

	* bib/csi.bib: add damota.09.seminar

2009-03-12  Vincent Ordy  <ordy@lrde.epita.fr>

	Fix "Dennis" in README.
	* doc/share.txt: here.

2009-03-05  Roland Levillain  <roland@lrde.epita.fr>

	* bib/transformers.bib (cordy.06.scp): New entry.

2009-02-26  Roland Levillain  <roland@lrde.epita.fr>

	New blue EPITA logo with English caption.

	* figs/epita-blue-en.png: New.

2009-02-20  Reda Dehak  <reda@lrde.epita.fr>

	* bib/lrde.bib: add dehak.08.nist and dehak.09.icassp.

2009-02-19  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (meyer.91.afcet): Fixme field `booktitle'.

2009-02-18  Roland Levillain  <roland@lrde.epita.fr>

	Typo in publisher's field of darbon.02.ismm.

	* bib/lrde.bib (darbon.02.ismm): s/Sciro/CSIRO/.

2009-02-18  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (cousty.08.dgci, meyer.91.afcet): New entries.

2009-02-18  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (bertrand.99.dgci, bertrand.08.chapter)
	(edmonds.60.nams): New entries.

2009-02-15  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (cousty.09.pami): New entry.

2009-02-15  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib: Tidy.

2009-02-15  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (enficiaud.07.phd): New entry.

2009-02-15  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (yoo.04.book): New entry.

2009-02-15  Roland Levillain  <roland@lrde.epita.fr>

	* bib/olena.bib (olena.www): Udate year.

2009-02-15  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (van-droogenbroeck.96.prl): New entry.

2009-02-15  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (van-herk.92.prl): New entry.

2009-02-09  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (gerlach.03.appt): New entry.

2009-02-09  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (berti.06.fgcs): New entry.

2009-02-06  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (alcoverro.08.3dtv): New entry.

2009-02-04  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (musser.89.issac): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (kapoor.00.tr): Don not use extended characters.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (kapoor.00.tr): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (koethe.00.cppr): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (koethe.98.hcva): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (koethe.01.dig): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (kettner.98.scg): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (berti.00.tmpw): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/acronyms.bib (ismm): Refine definition.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (meyer.07.ismm): Precise book title.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (vincent.92.chapter): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (vincent.91.pami): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (cousty.09.ismm): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (lomenie.08.prl): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (meyer.07.ismm): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (vincent.89.sp): New entry.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (vincent.91.sp): Add an `lrdedoc' field.

2009-02-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (vincent.91.sp): New entry.

2009-01-28  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/mc.bib (rauchhenzinger.96.swat): Protect Streett.

2009-01-27  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/mc.bib: s/LTL/{LTL}/.

2009-01-20  Roland Levillain  <roland@lrde.epita.fr>

	* styles/myacronym.sty (wst): New acronym.

2009-01-19  Roland Levillain  <roland@lrde.epita.fr>

	Add a alternate ISO C++ language definition for listings.

	* styles/ldf/c++.sty: New.
	Include this file...
	* styles/mylistings.hva: ...here.

2009-01-19  Roland Levillain  <roland@lrde.epita.fr>

	* styles/myacronym.sty (rag): New acronym.

2009-01-19  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (heijmans.92.chapter): New entry.

2009-01-19  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib (goutsias.00.fi): New entry.

2009-01-13  Didier Verna  <didier@lrde.epita.fr>

	* bib/lrde.bib (verna.09.ilc): New entry.

2009-01-07  Akim Demaille  <akim@lrde.epita.fr>

	generate-rev-sty.
	* bin/generate-rev-sty: New.
	* make/tex.mk (rev.sty): Use it.

2009-01-05  Nicolas Ballas  <ballas@lrde.epita.fr>

	Fix some typos in the CSI abstracts.

	* bib/csi.bib: Update.

2008-12-29  Roland Levillain  <roland@lrde.epita.fr>

	* bib/csi.bib: Bibneat it.

2008-12-29  Roland Levillain  <roland@lrde.epita.fr>

	Correct the French abstracts of the January 2009 CSI Seminars.

	* bib/csi.bib: Typos, missing punctuation, case-related errors,
	etc.

2008-12-22  Roland Levillain  <roland@lrde.epita.fr>

	styles/myacronym.sty: Help LaTeX with the hyphenation of Programming.

	* styles/myacronym.sty: Help LaTeX with the hyphenation of
	``Programming'' in GP.

2008-12-22  Roland Levillain  <roland@lrde.epita.fr>

	* bib/strategoxt.bib (BKVV08): Protect project name.

2008-12-21  Akim Demaille  <akim@lrde.epita.fr>

	decl is a scool keyword.
	* styles/ldf/scool.sty: And sort.

2008-12-21  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (liskov.74.vhll): New entry.

2008-12-21  Akim Demaille  <akim@lrde.epita.fr>

	Load all the defined languages.
	* styles/mylistings.hva (d, nemerle, scool): Load them.

2008-12-21  Akim Demaille  <akim@lrde.epita.fr>

	More project macros.
	* styles/misc.hva: Here.

2008-12-21  Akim Demaille  <akim@lrde.epita.fr>

	Bib formatting changes.
	* bib/gp.bib, bib/transformers.bib: Formatting changes.
	* bib/transformers.bib (vaucanson.www): Remove.
	(veldhuizen.99.tr): Move to...
	* bib/gp.bib: Here.

2008-12-20  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (veldhuizen.97.iscope): New entry.

2008-12-17  Maxime van Noppen  <yabo@lrde.epita.fr>

	Fix (again) abstract.
	* csi.bib: Here.

2008-12-17  Maxime van Noppen  <yabo@lrde.epita.fr>

	Fix abstract.
	* bib/csi.bib: Here.

2008-12-17  Maxime van Noppen  <yabo@lrde.epita.fr>

	Add the abstract for van-noppen.09.seminar.
	* csi.bib: here.

2008-12-17  Alexandre Abraham  <abraham@lrde.epita.fr>

	Add abraham.09.seminar in csi.bib.

	* bib/csi.bib: Add abraham.09.seminar in csi.bib.

2008-12-16  Jimmy Ma  <jimmy.ma@lrde.epita.fr>

	Add ma.09.seminar in csi.bib.
	* bib/csi.bib: update.

2008-12-16  Nicolas Ballas  <ballas@lrde.epita.fr>

	Add ballas.09.seminar in csi.bib.

	* bib/csi.bib: update.

2008-12-15  Maxime van Noppen  <yabo@lrde.epita.fr>

	Move styles to a better location.
	* ldf/d.sty: New.
	* ldf/grammar.sty: Merge grammar styles.
	* ldf/lstgrammar.sty: New.
	* ldf/nemerle.sty: New.
	* ldf/ocaml.sty: New.
	* ldf/scool.sty: New.
	* lstd.sty: Remove.
	* lstgrammar.sty: Remove.
	* lstnemerle.sty: Remove.
	* lstocaml.sty: Remove.
	* lstscool.sty: Remove.

2008-12-12  Roland Levillain  <roland@lrde.epita.fr>

	* styles/myacronym.sty (OO): Add an hyphen in definition.

2008-12-09  Florian Lesaint  <florian.lesaint@lrde.epita.fr>

	Add bib entrey for Student Report No. 0833.
	* csi.bib: Here.

2008-11-26  Akim Demaille  <akim@lrde.epita.fr>

	\nolinkurl.
	* styles/lrde-bulletin.sty (\urlnote): Use nolinkurl instead
	of url so that a single hyperlink be output (currently there
	are two, pointing to the same url).

2008-11-25  Maxime van Noppen  <yabo@lrde.epita.fr>

	Add a bib entry for a paper of Stroustrup (IAP 04).
	* transformers.bib: Here.

2008-11-25  Roland Levillain  <roland@lrde.epita.fr>

	* styles/myacronym.sty (bgl, gnu, tweast, tweasts): New acronyms.

2008-11-19  Maxime van Noppen  <yabo@lrde.epita.fr>

	Add some listing styles.

	Supported languages : D, Nermele, OCaml, Scool.
	There is also a style for pseudo-grammar code.
	Don't forget you're welcome to improve them ;-)

	* lstd.sty: New.
	* lstgrammar.sty: New.
	* lstnemerle.sty: New.
	* lstocaml.sty: New.
	* lstscool.sty: New.

2008-11-18  Maxime van Noppen  <yabo@lrde.epita.fr>

	Add the Scool macro.
	* lrde-bulletin.sty: Here.

2008-11-06  Roland Levillain  <roland@lrde.epita.fr>

	Alternate ACM copyright header for personal copy.

	* styles/mysig-alternate.cls: Allow the user to produce a header
	suitable for a personal copy (as required by the ACM) by defining
	\personalcopy.

2008-11-05  Akim Demaille  <akim@lrde.epita.fr>

	Use &contents.
	* bin/abstract: Formatting changes.
	* bin/deacronym (&contents): New, use it.
	* bin/update-cite: Use "die" on errors.

2008-11-04  Akim Demaille  <akim@lrde.epita.fr>

	deacronym.
	* bin/deacronym: New.
	* doc/share.txt: Doc it.
	* styles/myacronym.sty: Ditto.

2008-10-29  Akim Demaille  <akim@lrde.epita.fr>

	Update ENTCS files.
	* styles/entcs.cls: Update from master.
	* styles/entcsmacro.sty: Ditto.

2008-10-27  Akim Demaille  <akim@lrde.epita.fr>

	vaucanson-g-to-tikz.
	* bin/vaucanson-g-to-tikz: New.
	Imported from thl, where it was used to convert all the VaucansonG
	figures into TikZ figures.

2008-10-16  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (demaille.08.kex): New entry.

2008-10-15  Akim Demaille  <akim@lrde.epita.fr>

	Formatting changes.
	* styles/lrde-bulletin.sty: here.
	I don't know what I must do so that I need not avoid to put an
	empty line after \maketitle, please help me.  If I leave an
	empty line, then I waste one line after the title.

2008-10-15  Didier Verna  <didier@lrde.epita.fr>

	* bib/lrde.bib (verna.08.els)
	(verna.08.jucs): New entries.

2008-10-15  Akim Demaille  <akim@lrde.epita.fr>

	colorframe.
	* styles/mylistings.sty (colorframe, lightpink): New.
	Taken from demaille.09.sac.

2008-10-15  Akim Demaille  <akim@lrde.epita.fr>

	Improve the generation of the bib tables.
	* bin/make-bib.pl: Formatting changes in the output.

2008-10-14  Roland Levillain  <roland@lrde.epita.fr>

	* bin/make-bib.pl: Include year 2009 in the list of publications.

2008-10-14  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (demaille.09.sac): New entry.

2008-10-10  Roland Levillain  <roland@lrde.epita.fr>

	More program-transformation and code-generation-related entries.

	* bib/compilation.bib (baxter.04.icse, gagnon.98.tools)
	(hildum.90.tse,partsch.83.csur): New entries.

2008-10-09  Roland Levillain  <roland@lrde.epita.fr>

	* bib/strategoxt.bib (FV04.retrofit): Typo.

2008-10-09  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (schwartzbach.08.cc): Remove field `crossref'.

2008-10-08  Akim Demaille  <akim@lrde.epita.fr>

	Capitalize urls in foot notes.
	* styles/lrde-bulletin.sty: Remove obsolete comments.
	(\urlnote): Use \MakeUppercase on the first letter.

2008-10-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (ucla-cg.05.jtb): New entry.

2008-10-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (schwartzbach.08.cc): New entry.

2008-09-19  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* styles/vaucanson-g.sty: Fix pstricks' version check.
	Reported by Reuben Thomas <rtt@sc3d.org>.

2008-09-17  Vincent Ordy  <ordy@lrde.epita.fr>

	Revert "share/ r3123: Rename bib keys".
	* bib/ciaa-04.bib,
	* bib/codegen.bib,
	* bib/compilation.bib,
	* bib/compilation.clement.bib,
	* bib/csi.bib,
	* bib/cwi.bib,
	* bib/gp.bib,
	* bib/lrde.bib,
	* bib/mc.bib,
	* bib/model-checking.bib,
	* bib/olena.bib,
	* bib/pp.bib,
	* bib/rivf-06.bib,
	* bib/rivf-07.bib,
	* bib/saga.bib,
	* bib/sip.bib,
	* bib/tiger.bib,
	* bib/transformers.bib,
	* bib/vaucanson.bib: Do that.

2008-09-17  Akim Demaille  <akim@lrde.epita.fr>

	\var in \tt\it.
	* styles/texi.hva (\var): Change.

2008-09-10  Vincent Ordy  <ordy@lrde.epita.fr>

	Rename bib keys.
	* bib/ciaa-04.bib,
	* bib/codegen.bib,
	* bib/compilation.bib,
	* bib/compilation.clement.bib,
	* bib/csi.bib,
	* bib/cwi.bib,
	* bib/gp.bib,
	* bib/lrde.bib,
	* bib/mc.bib,
	* bib/model-checking.bib,
	* bib/olena.bib,
	* bib/pp.bib,
	* bib/rivf-06.bib,
	* bib/rivf-07.bib,
	* bib/saga.bib,
	* bib/sip.bib,
	* bib/tiger.bib,
	* bib/transformers.bib,
	* bib/vaucanson.bib: Do that.

2008-09-03  Akim Demaille  <akim@lrde.epita.fr>

	styles/README.
	* doc/share.txt: Point to it.
	* styles/README: New.

2008-09-02  Akim Demaille  <demaille@gostai.com>

	Add first names.
	* bib/compilation.bib: To Appel.

2008-09-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (stroustrup.08.faq): New entry.

2008-09-02  Akim Demaille  <demaille@gostai.com>

	Add missing author to tiger docs.
	* bib/tiger.bib: here.

2008-09-02  Akim Demaille  <akim@lrde.epita.fr>

	Fix keys.
	* bib/transformers.bib: here.

2008-09-02  Akim Demaille  <akim@lrde.epita.fr>

	More bibtex quotes.
	* bib/gp.bib: there.

2008-09-02  Roland Levillain  <roland@lrde.epita.fr>

	Have entry boost.08.www behave with natbib.

	* bib/gp.bib (boost.08.www): Have the authors (The Boost Project)
	be a single entity.

2008-09-02  Roland Levillain  <roland@lrde.epita.fr>

	* styles/myacronym.sty: Define acronym BGL, FP and RAII.

2008-09-02  Roland Levillain  <roland@lrde.epita.fr>

	Add a bibliographical entry for the May 2008 C++0x Working Draft.

	* bib/transformers.bib (iso.0x.c++): New entry.

2008-09-02  Akim Demaille  <akim@lrde.epita.fr>

	Fix/complete some BibTeX entries.
	* bib/compilation.bib, bib/tiger.bib: here.

2008-08-29  Akim Demaille  <akim@lrde.epita.fr>

	OOL and zendra.97.siglplan.
	* bib/compilation.bib, styles/myacronym.sty: here.

2008-08-29  Akim Demaille  <akim@lrde.epita.fr>

	Fix yacc.ldf.
	* styles/ldf/README: New.
	* styles/ldf/yacc.sty: Add dummy keyword.

2008-08-29  Akim Demaille  <akim@lrde.epita.fr>

	Beware of special chars.
	It is not easy to pass a literal string to perl via the
	command line, do it via the environment.
	* bin/instantiate-template.sh: Use the env to pass args to perl.

2008-08-23  Roland Levillain  <roland@lrde.epita.fr>

	Fix some bibliographical entries.

	* bib/compilation.bib (kuipers.03.scp): Fix title and journal
	name.
	* bib/strategoxt.bib (Vis04.strategoxt): Fix publisher name.

2008-07-28  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (demaille.08.iticse): Add urllrde field.

	* bib/lrde.bib, bib/csi.bib: Do not use \textsc for XML and FSMXML.

	* bib/csi.bib (ma.08.seminar): Typo.

	* bib/lrde.bib (demaille.08.fsmnlp): Update the abstract to match
	the final version of the paper.

2008-07-24  Akim Demaille  <akim@lrde.epita.fr>

	bilan.sty: A maketitle for articles.
	* styles/bilan.sty (\maketitle): New implementation for
	article.cls.

2008-07-24  Akim Demaille  <akim@lrde.epita.fr>

	bibtex.sty.
	* styles/ldf/bibtex.sty: New.
	* styles/mylistings.hva: Use it.
	Define LaTeX as a new language.

2008-07-19  Roland Levillain  <roland@lrde.epita.fr>

	Add a bibliography for the Tiger project.

	* bib/tiger.bib: New bibliography.
	(tiger.2007.assignments, tiger.2007.tcrm): New entries.
	* bib/transformers.bib (tiger.www): Move entry...
	* bib/tiger.bib: ...here.

2008-07-16  Jimmy Ma  <jimmy.ma@lrde.epita.fr>

	Update abstract in ma.08.seminar.
	* csi.bib: Here.

2008-07-08  Akim Demaille  <akim@lrde.epita.fr>

	Fix references to floats that are in enumerations.
	* styles/myenumerate.sty: Load enumerate.sty *after* Didier's trick.

2008-07-08  Akim Demaille  <akim@lrde.epita.fr>

	Fix textsc use.
	* bib/lrde.bib: here.
	Thanks to Roland Levillain.

2008-07-08  Akim Demaille  <akim@lrde.epita.fr>

	lrde.bib: Minor style changes.
	* bib/lrde.bib: here.

2008-07-07  Roland Levillain  <roland@lrde.epita.fr>

	Fix the previous patch.

	* styles/myacronym.sty: Provide correct acronyms for HIR and LIR.

2008-07-07  Roland Levillain  <roland@lrde.epita.fr>

	Add acronyms HIR and LIR.

	* styles/myacronym.sty (hir, lir): New acronyms.

2008-07-04  Roland Levillain  <roland@lrde.epita.fr>

	lrde.bib cleanup.

	* bib/lrde.bib (demaille.08.fsmnlp, geraud.08.mpool,
	(ricou.07.eceg, ricou.08.eceg): Preserve capitals in titles.
	(demaille.08.iticse, geraud.08.mpool): Remove the `note' field.

2008-07-04  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (demaille.08.fsmnlp): New entry.

2008-07-04  Akim Demaille  <akim@lrde.epita.fr>

	rev.hva.
	* styles/rev.hva: New.

2008-07-04  Akim Demaille  <akim@lrde.epita.fr>

	Update texi2dvi.
	* bin/texi2dvi: From master.

2008-07-04  Akim Demaille  <akim@lrde.epita.fr>

	Fix qcm.sty.
	* styles/qcm.sty (qcm): Use linewidth, not textwidth,
	to work properly when in multicol.

2008-07-01  Roland Levillain  <roland@lrde.epita.fr>

	Add EPITA's gray logo.

	* figs/epita-gray.pdf: New logo, copied from
	https://svn.lrde.epita.fr/svn/lrde-communication/trunk/logos/epita/2007/EPITA%20Ingenieur_metal%202007-2.pdf
	* figs/epita.pdf: New symlink.

2008-06-24  Roland Levillain  <roland@lrde.epita.fr>

	Fix some more BibTeX entries.

	* bib/olena.bib (olena.www): Use a more canonical form for the
	field `author'.
	* bib/lrde.bib (burrus.03.mpool): Do not use an acronym in field
	`booktitle'.
	(duret.00.gcse): Typo in field `title'.
	* bib/gp.bib (cgal.08.www): Properly escape the contents of the
	field `author'.
	(canning.89.fpca, chiba.95.oopsla, dosreis.05.lcsd)
	(garcia.03.oopsla, gregor.06.oopsla, jarvi.06.pldi):
	Remove years from conference acronyms when they are superfluous.
	(stroustrup.05.lcsd): Likewise.
	Add a field `address'.
	(veldhuizen.99.tech): Rename entry as...
	(veldhuizen.99.techrep): ...this.
	Fix field `institution'.

2008-06-23  Roland Levillain  <roland@lrde.epita.fr>

	Fix some entries of bib/gp.bib.

	* bib/gp.bib (abrahams.01.tmpw, boost.08.www, garcia.03.oopsla)
	(gregor.06.oopsla, jarvi.06.pldi):
	Preserve capitals and remove useless escapes.

2008-06-23  Vincent Ordy  <ordy@lrde.epita.fr>

	Change seminar title.
	* styles/semann.cls,
	* styles/semplan.cls:
	Change "Seminaire" to "Seminaire des etudiants-chercheurs"

2008-06-18  Akim Demaille  <akim@lrde.epita.fr>

	texi2dvi: update.
	* bin/texi2dvi: From master.

2008-06-16  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	A script to construct abstract/resume documents
	automatically from BibTeX entries.

	* bin/abstract: New file.
	* doc/share.txt: Mention it.

2008-06-16  Akim Demaille  <akim@lrde.epita.fr>

	Update texi2dvi.
	* bin/texi2dvi: From master.

2008-06-16  Akim Demaille  <akim@lrde.epita.fr>

	FiNK.
	* styles/fink.sty: New.

2008-06-11  Akim Demaille  <demaille@gostai.com>

	texi2dvi: Sort functions.
	* bin/texi2dvi: Sort functions.

2008-06-11  Akim Demaille  <demaille@gostai.com>

	texi2dvi --help.
	* bin/texi2dvi: Document -I's behavior.

2008-06-11  Akim Demaille  <demaille@gostai.com>

	texi2dvi: avoid.
	It is virtually impossible to find a safe means to use
	echo with \n in it.  So use cat and here docs.
	* bin/texi2dvi ($usage): Remove, replaced by...
	(usage): this function.

2008-06-11  Akim Demaille  <demaille@gostai.com>

	texi2dvi: Fix the fix.
	* bin/texi2dvi: One cannot just call absolute_filenames, since
	always add ".:" in front, which results in invalid -I ".:/foo:/bar"
	passed to the various tools.
	(list_concat_dirs): New.
	Currently most a copy of absolute_filenames, but the latter
	is scheduled for removal.
	Use list_concat_dirs for -I support.
	(--I*): Remove, not documented anywhere, and too accepting.

2008-06-10  Alexandre Abraham  <abraham@lrde.epita.fr>

	Fix typos.

	* bib/csi.bib: Fix typos.

2008-06-06  Vincent Ordy  <ordy@lrde.epita.fr>

	Add wiki link checker.
	* bin/bibtex-check: Add link checker.

	* bib/csi.bib,
	* bib/lrde.bib:
	make neat

2008-06-06  Vincent Ordy  <ordy@lrde.epita.fr>

	Fix a texi2dvi bug.
	* bin/texi2dvi: Fix the path expansion of multiple directories.

2008-06-06  Akim Demaille  <demaille@gostai.com>

	bnf.sty, and rename ldf/*.ldf to ldf/*.sty.
	* styles/ldf/asf.ldf, styles/ldf/asn1.ldf,
	* styles/ldf/aterm.ldf, styles/ldf/box.ldf,
	* styles/ldf/grammar.ldf, styles/ldf/hir.ldf,
	* styles/ldf/leopard.ldf, styles/ldf/lex.ldf,
	* styles/ldf/mips.ldf, styles/ldf/parse-testsuite.ldf,
	* styles/ldf/prism.ldf, styles/ldf/reactive-modules.ldf,
	* styles/ldf/rtg.ldf, styles/ldf/sdf.ldf, styles/ldf/stl.ldf,
	* styles/ldf/stratego.ldf, styles/ldf/tiger.ldf,
	* styles/ldf/vaucanson.ldf, styles/ldf/yacc.ldf:
	Rename as...
	* styles/ldf/asf.sty, styles/ldf/asn1.sty,
	* styles/ldf/aterm.sty, styles/ldf/box.sty,
	* styles/ldf/grammar.sty, styles/ldf/hir.sty,
	* styles/ldf/leopard.sty, styles/ldf/lex.sty,
	* styles/ldf/mips.sty, styles/ldf/parse-testsuite.sty,
	* styles/ldf/prism.sty, styles/ldf/reactive-modules.sty,
	* styles/ldf/rtg.sty, styles/ldf/sdf.sty, styles/ldf/stl.sty,
	* styles/ldf/stratego.sty, styles/ldf/tiger.sty,
	* styles/ldf/vaucanson.sty, styles/ldf/yacc.sty:
	these.
	* styles/ldf/bnf.sty: New.
	* styles/mylistings.hva: Adjust.

2008-05-30  Vincent Ordy  <ordy@lrde.epita.fr>

	Create missing wiki pages; update URLs.
	* share/bib/csi.bib: update.

2008-05-30  Vincent Ordy  <ordy@lrde.epita.fr>

	Fix accents in ag.bib.
	* bib/ag.bib: Fix accents.

2008-05-29  Vincent Ordy  <ordy@lrde.epita.fr>

	Fix/add some urllrde.
	* bib/csi.bib: update.

2008-05-29  Roland Levillain  <roland@lrde.epita.fr>

	Fix LRDE URLs in the LRDE Bibliography.

	* bib/lrde.bib (darbon.05.phd, darbon.06.tr): Fix field `urllrde'.

2008-05-29  Roland Levillain  <roland@lrde.epita.fr>

	Remove invalid characters from the LRDE bibliography.

	* bib/lrde.bib (demaille.08.iticse): Remove invalid characters
	from field `address'.

2008-05-28  Roland Levillain  <roland@lrde.epita.fr>

	Update the LRDE bibliography.

	* bin/make-bib.pl (@project): Add Tiger.
	* bib/lrde.bib (baillard.07.gretsi, berger.07.icip)
	(chekroun.06.iciar, verna.06.ijcs, verna.06.imecs)
	(verna.06.practex, verna.07.imecs):
	Remove the ``Accepted'' status for published papers.
	(demaille.05.iticse): Set field note to ``Tiger''.
	(demaille.08.iticse): Aesthetic changes.
	(geraud.08.mpool): Likewise.
	Don't use non standard LaTeX commands in title.
	(laplante.06.tocl): Rename as...
	(laplante.07.tocl): ...this
	Add missing information since the publication.

2008-05-26  Florian Lesaint  <florian.lesaint@lrde.epita.fr>

	Add url and urllrde in lesaint.08.seminar.
	* bib/csi.bib: Here.

2008-05-26  Cedric Raud  <spycam@lrde.epita.fr>

	Add the url to raud.08.seminar.
	* csi.bib: Added : 200807-Seminar-Raud

2008-05-26  Vincent Ordy  <ordy@lrde.epita.fr>

	update URLLRDE in ordy.08.seminar.
	* bib/csi.bib: update.

2008-05-26  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (geraud.08.mpool): New entry.

2008-05-26  Nicolas Ballas  <ballas@lrde.epita.fr>

	update URLLRDE in ballas.08.seminar.

	* bib/csi.bib: update.

2008-05-26  Jimmy Ma  <jimmy.ma@lrde.epita.fr>

	Clean up in ma.08.seminar.
	* bib/csi.bib: remove traces of previous conflict.

2008-05-26  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib: Fix field `author' of demaille.08.iticse.

2008-05-26  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (demaille.08.iticse): New entry.

2008-05-26  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (boost.08.www.gp): New entry.

2008-05-26  Jimmy Ma  <jimmy.ma@lrde.epita.fr>

	Add url and urllrde in ma.08.seminar.
	* bib/csi.bib: here.

2008-05-24  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib: Add entry meyer.86.sigplan.

2008-05-22  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (hemon.08.sagt): Add french title and abstract.

2008-05-22  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/csi.bib: Corrections from Daniella.

2008-05-22  Florian Lesaint  <florian.lesaint@lrde.epita.fr>

	Typo in lesaint.08.seminar.
	* csi.bib: Typo.

2008-05-21  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/csi.bib (delmon.08.seminar): Typo.

2008-05-21  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/csi.bib: Fix usage of {{...}} in titles, and a couple
	of other small typos.

2008-05-21  Cedric Raud  <spycam@lrde.epita.fr>

	Fix typo in raud.08.seminar.
	* csi.bib: Fix typo

2008-05-21  Nicolas Ballas  <ballas@lrde.epita.fr>

	Add a french title in csi.bib .

	* bib/csi.bib: .

2008-05-21  Caroline Vigouroux  <vigour_c@epita.fr>

	Add french title.
	* csi.bib: Add french title.

2008-05-19  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (stroustrup.05.lcsd): New entry.

2008-05-18  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (geraud.06.scoop-pres): Remove duplicate entry.
	This entry is already present in bib/olena.bib, and is not an
	official publication of the LRDE.

2008-05-18  Roland Levillain  <roland@lrde.epita.fr>

	* bib/olena.bib: Typo.

2008-05-18  Roland Levillain  <roland@lrde.epita.fr>

	Miscellaneous updates in some bibliographies.

	* bib/olena.bib: State the topic of this bibliography.
	Set the spell-checker language to American English.
	* bib/gp.bib: Likewise.
	(boost.07.www, cgal.07.www): Rename as...
	(boost.08.www, cgal.08.www): ...these.
	Add an ``author'' field.
	Update field ``year''.

2008-05-14  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/csi.bib, bib/lrde.bib: Run "make neat", fix a missing comma
	and remove two accents.

2008-05-06  Akim Demaille  <akim@lrde.epita.fr>

	Avoid using graphicspath, use qualified file names.
	* make/tex.mk: Pass -I <path to share/> to texi2dvi.
	* styles/bilan.sty: here.

2008-04-06  Roland Levillain  <roland@lrde.epita.fr>

	Fix entry johnson.79 in bib/transformers.bib.

	* bib/transformers.bib (johnson.79): Remove empty field `series'.

2008-04-05  Florian Lesaint  <florian.lesaint@lrde.epita.fr>

	Update csi.bib.
	* bib/csi.bib {lesaint.07.seminar}: Here.
	Add abstract and resume.

2008-04-05  Akim Demaille  <demaille@gostai.com>

	Fix csi.bib.
	* bib/csi.bib (raud.08.seminar): Here.
	Remove "oldkeys" entries for keys that never existed.

2008-04-05  Akim Demaille  <demaille@gostai.com>

	phenix.
	* bib/transformers.bib (phenix.08.svn): New.

2008-04-04  Akim Demaille  <demaille@gostai.com>

	Add more consistent file names.
	* figs/logo_lrde-blue.mask.jpg: New.
	* figs/logo_lrde.mask.jpg: New.

2008-04-04  Cedric Raud  <spycam@lrde.epita.fr>

	Fix raud.08.seminar.centaur.
	* csi.bib: Optimized english and title added.

2008-04-04  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	Make sure we can run "make csi.pdf".

	* bib/csi.bib (moulard.08.seminar): Do not use the undefined macro
	\Scoop.
	* bin/make-bib.pl (output): Do not hardcode lrde.bib, use the
	script's argument.

2008-04-04  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/csi.bib: Run "make neat" to add missing commas.

2008-04-03  Jimmy Ma  <jimmy.ma@lrde.epita.fr>

	Fix lazzara.07.seminar.
	* bib/csi.bib: Add abstract and resume to lazzara.07.seminar.

2008-04-03  Akim Demaille  <demaille@gostai.com>

	Various csi.bib fixes.
	* bib/csi.bib: Fix typos.
	Prefer \texttt and so forth to \tt.

2008-04-02  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/lrde.bib (cadilhac.06.avocs, darbon.05.eusipco,
	darbon.05.ispa, denise.06.rt, duflot.04.avocs, lesage.06.isvc):
	These papers are no longer "To appear", so remove the note
	and complete the reference when possible.
	(hamez.08.atpn): This one is, so note it.

2008-04-02  Matthieu Garrigues  <garrigues@lrde.epita.fr>

	* bib/csi.bib: Fix garrigues.08.seminar.fllt.

2008-04-02  Maxime van Noppen  <maxime.van-noppen@lrde.epita.fr>

	Fix in seminar resume
	* csi.bib: Here.

2008-04-01  Caroline Vigouroux  <vigour_c@epita.fr>

	Add vigouroux.08.seminar to csi.bib.
	* bib/csi.bib: .

2008-03-31  Etienne FOLIO  <folio@lrde.epita.fr>

	Fixes.
	* bib/csi.bib: Fixes.

2008-03-31  Damien Lefortier  <dam@lrde.epita.fr>

	Add lefortier.08.seminar to csi.bib.
	* bib/csi.bib: Here.

2008-03-31  Etienne FOLIO  <folio@lrde.epita.fr>

	Abstract corrections.
	* bib/csi.bib: Abstract corrections.

2008-03-31  Etienne FOLIO  <folio@lrde.epita.fr>

	New entry for Etienne Folio's abstract.
	* bib/csi.bib: New abstract.

2008-03-31  Antoine Legrand  <legrand@lrde.epita.fr>

	Add legrand.08.seminar to csi.bib.
	* csi.bib: Here.

2008-03-31  Florian Queze  <Florian.Queze@lrde.epita.fr>

	Add queze.08.seminar to csi.bib
	* bib/csi.bib: .

2008-03-31  Alexandre Abraham  <abraham@lrde.epita.fr>

	Adding abstract to csi.bib.

	* bib/csi.bib: Add abraham.08.seminar.

2008-03-31  Guillaume SADEGH  <guillaume.sadegh@lrde.epita.fr>

	Add sadegh.08.seminar to csi.bib.
	* csi.bib: Here.

2008-03-31  Roland Levillain  <roland@lrde.epita.fr>

	* bib/csi.bib: Misc. fixes in van-noppen.08.seminar.

2008-03-31  Maxime van Noppen  <yabo@lrde.epita.fr>

	Add van-noppen.08.seminar to csi.bib
	* csi.bib: Here.

2008-03-31  Roland Levillain  <roland@lrde.epita.fr>

	* bib/csi.bib: Fix English and French abstracts of
	ballas.08.seminar.

2008-03-31  Roland Levillain  <roland@lrde.epita.fr>

	* bib/csi.bib: Fix English and French abstracts of
	jardonnet.08.seminar.

2008-03-31  Caroline Vigouroux  <vigour_c@epita.fr>

	Add vigouroux.08.seminar.fllt to csi.bib.
	* csi.bib: Add vigouroux.08.seminar.fllt to csi.bib.

2008-03-31  Cedric Raud  <spycam@lrde.epita.fr>

	Add raud.08.seminar.centaur to csi.bib.
	* csi.bib: Here.

2008-03-31  Caroline Vigouroux  <vigour_c@epita.fr>

	add abstract.
	* csi.bib: added abstract.

2008-03-31  Vincent Ordy  <vincent.ordy@lrde.epita.fr>

	Add ordy.08.seminar to csi.bib.
	* bib/csi.bib: Here.

2008-03-31  Matthieu Garrigues  <garrigues@lrde.epita.fr>

	* bib/csi.bib: Add garrigues.08.seminar.fllt to csi.bib.

2008-03-31  Jerome Galtier  <jerome.galtier@lrde.epita.fr>

	Add galtier.08.seminar to csi.bib.
	* bib/csi.bib: Here.

2008-03-29  Florian Lesaint  <florian.lesaint@lrde.epita.fr>

	Fix title of lesaint.08.seminar in csi.bib.
	* bib/csi.bib: Here.

2008-03-29  Florent DHalluin  <d-halluin@lrde.epita.fr>

	Add entry in csi.bib for d-halluin.08.seminar
	* csi.bib: There.

2008-03-29  Florian Lesaint  <florian.lesaint@lrde.epita.fr>

	Add lesaint.08.seminar to csi.bib.
	* bib/csi.bib: Here.

2008-03-28  Jimmy Ma  <jimmy.ma@lrde.epita.fr>

	Add ma.08.seminar to csi.bib.
	* bib/csi.bib: Here.

2008-03-27  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* bib/mc.bib (rozier.07.spin): New entry.
	* bib/csi.bib, lrde/lrde.bib: Cleanup.

2008-03-26  Roland Levillain  <roland@lrde.epita.fr>

	* styles/lrde-bulletin.sty (\ladr): New command.

2008-03-25  Akim Demaille  <akim@lrde.epita.fr>

	Update texi2dvi.
	* bin/texi2dvi: From master.

2008-03-19  Alexandre Hamez <alexandre.hamez@lip6.fr>

	Updated lrde.bib
	* bib/lrde.bib: Added entry hamez.08.atpn

2008-03-14  Akim Demaille  <akim@lrde.epita.fr>

	Fixes.
	* bib/lrde.bib: Fix LaTeX errors.

2008-03-12  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (darbon.08.iwcia): Preserve capitals.

2008-02-28  Roland Levillain  <roland@lrde.epita.fr>

	Fix entry round.06.quiz.

	* bib/compilation.bib (round.06.quiz): Turn the field `url' into a
	field `howpublished', so that Beamer displays it in the
	references.

2008-02-28  Roland Levillain  <roland@lrde.epita.fr>

	Add commands to typeset D (the language).

	* styles/mycxx.sty (\DTeX, \D, \DHR): New commands.

2008-02-28  Akim Demaille  <akim@lrde.epita.fr>

	Catch up with master.
	* bin/texi2dvi: here.

2008-02-20  Akim Demaille  <akim@lrde.epita.fr>

	Add demaille.08.ldta and le-quoc.08.ispec.
	* bib/lrde.bib: here.

2008-01-28  Guillaume Duhamel  <guillaume.duhamel@lrde.epita.fr>

	Update csi.bib.
	* bib/csi.bib: Add duhamel.08.seminar.

2008-01-28  Matthieu Garrigues  <garrigues@lrde.epita.fr>

	* share/bib/csi.bib: Add en entrie for my report.

2008-01-28  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	Allow the simple checks of bibtex-check to be run against
	individual bibtex files.

	* Makefile (neat): Run bibtex-check after bibneat.
	* bib/lrde.bib: Run through bibneat and fix accents.
	* bin/bibtex-check: Accept bibtex files as arguments.
	(check_bib): Rename as ...
	(check_char): ... this.
	(check_bib): New function to gather basic checks.
	(check_perms_or_student, check_all): Adjust to use check_bib.

2008-01-24  Akim Demaille  <akim@lrde.epita.fr>

	qcm.cls.
	* styles/qcm.cls: New.
	Based on Didier Verna's qcm.cls, but with s/question/qcm/g
	to avoid conflicts, just like in qcm.sty.
	Renaming will be needed to comply with the license.

2008-01-18  Roland Levillain  <roland@lrde.epita.fr>

	Add commands to typeset C# (the language).

	* styles/mycxx.sty (\CsTeX, \Cs, \CsHR): New commands.

2008-01-18  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib: Add a `lrdedoc' key to dewar.08.crosstalk.

2008-01-18  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib: Add dewar.08.crosstalk.

2008-01-18  Renaud Durlin  <renaud.durlin@lrde.epita.fr>

	Fix asf coloration.
	* styles/ldf/asf.ldf: Here.

2008-01-17  Roland Levillain  <roland@lrde.epita.fr>

	Introduce \emphdfn.

	* styles/texi.hva (\emphdfn): New.
	Provide back the service of the previous (Texinfo-like) \dfn
	command: highlighting a term without indexing it.

2008-01-16  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Add missing commas in lrde.bib.
	* lrde.bib: here.

2008-01-16  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Add a year field for demaille.08.ldta.
	* bib/lrde.bib(demaille.08.ldta): Add the year 2008 to the article.

2008-01-15  Daniela Becker  <daniela@lrde.epita.fr>

	<complete publis>
	* lrde.bib: Add abstracts, full names, urllrde.

2008-01-14  Akim Demaille  <akim@lrde.epita.fr>

	Fixes.
	* bib/lrde.bib: Run make neat.

2008-01-14  Daniela Becker  <daniela@lrde.epita.fr>

	<update lrde.bib>
	* bib/lrde.bib: Add darbon.08.iwcia.

2008-01-11  Akim Demaille  <akim@lrde.epita.fr>

	bibtex-check.
	* bin/bibtex-check: New.
	* Makefile: Use it.

2008-01-10  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* Makefile (BIBS): Add mc.bib.
	* bib/csi.bib, bib/lrde.bib, bib/mc.bib: Run "make neat".
	* doc/share.txt (mc.bib): Document.

2008-01-10  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* mc.bib: New file.

2008-01-09  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Use bibtool if it is installed.
	* bin/extract_bliblio.sh: Test if bibtool is in the path then use
	it otherwise use the previous sed script to extract bibtex
	keys. Change the help message to expand the $0 and change the
	pattern to use.  Now '.*\(-------\).*' is automatically added over
	the pattern.

2008-01-07  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Add missing comma.
	* bib/lrde.bib(geraud.06.scoop-pres): After the project name.

2008-01-03  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Fix previous patch.
	* bin/extract_bliblio.sh: Remove debug option.

2008-01-03  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Add a script to extract Bibtex entries from a list of bibtex files.
	* bin/extract_bliblio.sh: New.

2008-01-03  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Fill the french abstract of the last report from Nicolas Neri.
	* bib/csi.bib (neri.07.seminar.SMALLSUBJECT -> neri.08.seminar):
	Rename the entry and add a french abstract extracted from
	"Seminar-2008-01-16".

2008-01-03  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Update accent in the abstracts of "hocquet.08.seminar".
	* bib/csi.bib (hocquet.08.seminar): Remove UTF-8 and replace by the
	abstract found here:
	http://www/cgi-bin/twiki/view/Publications/Seminar-2008-01-16
	and use latin2tex to escape accents.

2008-01-02  Thierry Geraud  <thierry.geraud@lrde.epita.fr>

	Add geraud.06.scoop-pres in bib/lrde.bib.

	* bib/lrde.bib (geraud.06.scoop-pres): New.

2008-01-02  Akim Demaille  <akim@lrde.epita.fr>

	Fix csi.bib partially.
	* bin/latin2tex: More chars.
	* bib/csi.bib: Run latin2tex.

2008-01-02  Akim Demaille  <demaille@gostai.com>

	urbi.sty.
	* styles/ldf/urbi.sty: New.
	* styles/mylistings.hva: Use it.

2007-12-20  Roland Levillain  <roland@lrde.epita.fr>

	Update semann.cls.

	* styles/semann.cls: Use package `mybabel' instead of `babel'.
	Use packages `amsfonts', `multicol', `myacronym' and `mycxx'.
	(\projet, \bibpresentation): New commands.

2007-12-20  Roland Levillain  <roland@lrde.epita.fr>

	Add styles and images used to generate CSI Seminar posters
	and outlines.

	* styles/semann.cls, styles/semplan.cls:
	New styles.
	* figs/logo_lrde.png, figs/logo_lrde-blue.png,
	* figs/logo_lrde-green.png, figs/logo_lrde-red.png:
	New images.

2007-12-18  Roland Levillain  <roland@lrde.epita.fr>

	Sort entries in csi.bib.

	* bib/csi.bib: Do it.

2007-12-18  Roland Levillain  <roland@lrde.epita.fr>

	Start fixing entries in csi.bib.

	* bib/csi.bib (charron.08.seminar, leroi.07.seminar.synch)
	(moulard.07.seminar.scoop, querol.07.seminar)
	(z.07.seminar.smallsubject): Add missing
	entries, where applicable: English and French titles, English and
	French abstracts.
	Reindent.
	(leroi.07.seminar.synch, moulard.07.seminar.scoop)
	(querol.07.seminar, z.07.seminar.smallsubject): Rename as...
	(leroi.08.seminar.synch, moulard.08.seminar)
	(querol.08.seminar, lazzara.08.seminar): ...these.
	(deledalle.08.seminar, hocquet.08.seminar): Fix year.
	(pierron.07.seminar, pierron.08.seminar): Fix entries.
	(pierron.07.seminar): Remove duplicate entry.
	(garcia-ballester.08.seminar): New entry.

2007-12-12  mefyl  <mefyl@gruntech.net>

	Sort entries alphabetically.
	* bib/csi.bib: Here.

2007-12-12  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Add Abstract.
	* bib/csi.bib: here.

2007-12-12  Benoit Sigoure  <tsuna@lrde.epita.fr>

	Add my abstract for my 1st seminar.
	* bib/csi.bib (sigoure.06.seminar): Here.

2007-12-12  Quentin Hocquet  <mefyl@lrde.epita.fr>

	Add entry for my third seminar.
	* csi.bib: Here.

2007-12-12  Renaud Durlin  <renaud.durlin@lrde.epita.fr>

	Add abstract and resume for my seminars.
	* bib/csi.bib: Here.

2007-12-12  Benoit Sigoure  <tsuna@lrde.epita.fr>

	Add sigoure.08.seminar.
	* csi.bib: Here.

2007-12-10  Akim Demaille  <akim@lrde.epita.fr>

	Fix check-wiki.
	* Makefile: Add missing var name.

2007-12-07  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* styles/mylistings.sty (verylightgray): Define as rgb, not gray.
	Not all installations of LaTeX support the latter.

2007-12-07  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Fix typo.
	* bib/lrde.bib: Remove comma and add comma.

2007-12-07  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Add demaille.08.ldta in lrde.bib.
	* bib/lrde.bib: Add the entry for demaille.08.ldta.

2007-12-07  Akim Demaille  <akim.demaille@free.fr>

	Be more alsolanguage friendly.
	* styles/ldf/asf.ldf: Use "morekeywords" rather than "keywords"
	so that we can mix it with other languages such as sdf.

2007-12-07  Akim Demaille  <akim.demaille@free.fr>

	More pretty-printing.
	* styles/ldf/stratego.ldf: More literate symbols.
	More symbols.
	* styles/ldf/sdf.ldf ([ag]sdf): Derive from Stratego too.

2007-12-07  Akim Demaille  <akim.demaille@free.fr>

	Capitalize.
	* bib/lrde.bib: one letter.

2007-12-07  Renaud Durlin  <renaud.durlin@lrde.epita.fr>

	Add Bibtex entry for SDF reference manual.
	* bib/transformers.bib: Here.

2007-12-06  Akim Demaille  <akim@lrde.epita.fr>

	Make \Cxx more robust.
	* styles/mycxx.sty (\CxxTeX, \CTeX, \CxxHR, \CHR): New.

2007-12-06  Akim Demaille  <demaille@gostai.com>

	Sort acronyms.
	* styles/myacronym.sty: Here.
	Write nondeterministic, not non-deterministic.

2007-12-05  Akim Demaille  <demaille@gostai.com>

	More languages for listings.
	Based on work by Renaud Durlin.
	* styles/ldf/asf.ldf: New.
	* styles/mylistings.hva: Load it.
	* styles/ldf/sdf.ldf, styles/ldf/stratego.ldf: Complete.

2007-12-05  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Fix the problem of capitalized letter of "Programming" in references.
	* bib/transformers.bib: here.

2007-12-05  Guillaume Leroi  <guillaume.leroi@lrde.epita.fr>

	Add seminar report entry.
	* csi.bib: Add entry for December 2007 report on synchronized
	transducer.

2007-12-04  Benoit Sigoure  <tsuna@lrde.epita.fr>

	Improve a BiBTeX entry.
	* bib/pp.bib (jonge-pp-2002): Here.  Using information from ACM
	portal and citeseer.

2007-12-04  Benoit Sigoure  <tsuna@lrde.epita.fr>

	Remove a duplicate BiBTeX entry.
	* bib/strategoxt.bib (Jon00): Remove.
	* bib/pp.bib (jonge-pp-2002): Complete with the extra information of
	Jon00.

2007-12-04  Akim Demaille  <demaille@gostai.com>

	Let texi2dvi keep the trailing //.
	* bin/texi2dvi ($space, $tab): New.
	($IFS): Use them to be robust to zealous white space cleanups.
	(absolute): Preserve the trailing slashes.
	(tex_envvars): Add MPINPUTS, MFINPUTS, and TFMFONTS.

2007-12-02  Akim Demaille  <akim@lrde.epita.fr>

	Do not require to load french.
	* styles/gettext.sty (\translation): Accept a third arg.
	* styles/mybabel.hva (\BabelRequireLanguage): New.

2007-12-02  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Update URLs for UU-AG.
	* bib/ag2.bib: here.

2007-12-01  Akim Demaille  <akim@lrde.epita.fr>

	switchlanguage.
	* share/styles/mybabel.hva: New.

2007-12-01  Akim Demaille  <akim@lrde.epita.fr>

	gettext.sty.
	I faced a name conflict on \translate.
	* styles/translate.sty: Rename as...
	* styles/gettext.sty: this.

2007-12-01  Akim Demaille  <akim@lrde.epita.fr>

	More todo in texi.sty.
	* styles/texi.sty: Add more things to do here.

2007-12-01  Akim Demaille  <akim@lrde.epita.fr>

	More tyla entries.
	* bib/compilation.bib: here.

2007-11-30  Akim Demaille  <akim@lrde.epita.fr>

	Tidy bib.
	* bib/transformers.bib: Use our key style.
	Prefer braces to quotes.

2007-11-29  Renaud Durlin  <renaud.durlin@lrde.epita.fr>

	Fix ASF acronym.
	* styles/myacronym.sty: Fix ASF acronym.

2007-11-21  Roland Levillain  <roland@lrde.epita.fr>

	* doc/svn.txt: Typo.

2007-11-21  Akim Demaille  <akim@lrde.epita.fr>

	mycxx options.
	* styles/mycxx.sty: Support options "normal", and "sf" defaulting
	to the first one.
	Some reviewers dislike the "sf" version, so make "normal" the
	default.

2007-11-20  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* doc/share.txt: Mention bibneat.

2007-11-20  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* Makefile (%.tex, %.txt, %-private.tex): Make the generated
	output read-only to prevent accidental editions.
	* bin/make-bib.pl (verbose): Fix prototype.

2007-11-20  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	* hevea.txt: Typos.
	* svn.txt: Some rewording.
	* update-lrde-bib.txt: Mention "make neat".

2007-11-16  Akim Demaille  <akim@lrde.epita.fr>

	Fix broken command.
	* bib/lrde.bib: Remove a spurious space.

2007-11-14  Alexandre Duret-Lutz  <adl@lrde.epita.fr>

	introduce bibneat and cleanup csi.bib and lrde.bib

	* Makefile (neat, check-style): New targets.
	(check): Run check-style.
	(check-bib): Really abort on error.
	* bib/csi.bib, bib/lrde.bib: bibneatify, and fix some uses of
	double-quotes.
	* bib/strategoxt.bib, bib/visser.bib: Update from master.
	* bin/bibneat: New file.
	* bin/update-bib (strategoxt.bib): s/Benoit/Beno{^i}t/ on the fly.

2007-11-13  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Add a paper in Transformers.bib.
	* bib/transformers.bib: The added paper explaions a bit how
	they have handle include with AG.

2007-11-08  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Fix r2426.
	* bib/transformers.bib: Fix entry of rodeh.99.

2007-11-07  Akim Demaille  <akim@lrde.epita.fr>

	Bash 3.2 portability.
	* make/tex.mk: here.

2007-11-07  Akim Demaille  <akim@lrde.epita.fr>

	\sectionframe.
	* styles/beamerthemeKremlinBicetre.sty (\sectionframe)
	(\subsectionframe): New.
	Use them.

2007-11-07  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Add Bibtex entry for "Finding circular attribute in AGs".
	* bib/transformers.bib: Add an old printed article.

2007-11-07  Akim Demaille  <akim@lrde.epita.fr>

	Put the logo on the right.
	* styles/beamerthemeKremlinBicetre.sty (\maketitle): As sometimes
	we want longer titles.
	This is not enough though, the placement should be absolute, or from
	the bottom.

2007-11-07  Akim Demaille  <akim@lrde.epita.fr>

	Fix ricou.07.adass.
	* bib/lrde.bib: Fill the entry.
	Use correct separator for authors.
	Protect acronyms in the title.
	Sort properly.
	Add missing comma.

2007-11-05  Akim Demaille  <akim@lrde.epita.fr>

	Don't specify the bibstyle.
	* styles/beamerthemeKremlinBicetre.sty: here.

2007-11-05  Akim Demaille  <akim@lrde.epita.fr>

	Fix.
	* bin/instantiate-template.sh: Fix.

2007-11-05  Akim Demaille  <akim@lrde.epita.fr>

	\bibliographyframe.
	* styles/beamerthemeKremlinBicetre.sty (\bibliographyframe): New.

2007-10-29  Guillaume Lazzara  <z@lrde.epita.fr>

	Update LRDE URL in bib entry
	* bib/csi.bib: here.

2007-10-29  Guillaume Lazzara  <z@lrde.epita.fr>

	Add bib entry for "Boosting Vaucanson's genericity" techrep.
	* bib/csi.bib: here.

2007-10-26  Akim Demaille  <akim@lrde.epita.fr>

	qcm.sty.
	* styles/qcm.sty: New.
	Based on Didier Verna's QCM 2.1, but with several additions/changes:
	- question renamed qcm to avoid conflicts
	- support for beforeqcm and beforeqcmbody
	- pass [t] to the minipage so that the question number is next to
	  the beginning of the question.
	- definition {correction} only if it is not defined

2007-10-26  Roland Levillain  <roland@lrde.epita.fr>

	Automate the update of some more bibliographic styles.

	* Makefile (GASTEX_STYLES, FR_BIB_STYLES): New.
	(update-styles): Use them.
	Add download actions of French bibliographic styles to this
	rule.

2007-10-26  Akim Demaille  <akim@lrde.epita.fr>

	Fixes.
	* bib/lrde.bib: Wrap long lines.
	Fix % uses.
	Remove spurious spaces.
	Add a comma to every end of field.

2007-10-25  Daniela Becker  <daniela@lrde.epita.fr>

	Fix entries
	* bib/lrde.bib: Fix entries.

2007-10-19  Roland Levillain  <roland@lrde.epita.fr>

	Fix bib/compilation.clement.bib.

	* bib/compilation.clement.bib: A lot of syntactic corrections,
	thanks to Emacs' `M-x bibtex-validate'.

2007-10-19  Roland Levillain  <roland@lrde.epita.fr>

	Preserve capitals in titles of BibTeX entries.

	* bib/compilation.bib,
	* bib/csi.bib,
	* bib/gp.bib,
	* bib/kernighan.bib,
	* bib/lrde.bib,
	* bib/strategoxt.bib,
	* bib/tom.bib,
	* bib/transformers.bib:
	Preserve capitals of words C, C++, ConceptC++, GNU, Java, ML,
	SCOOP, Scool, Tom and UNIX.

2007-10-19  Roland Levillain  <roland@lrde.epita.fr>

	Fix fields `booktitle' of InProceedings entries.

	* bib/ag.bib, bib/gp.bib: s/In the Proceedings/Proceedings/.

2007-10-19  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (cgal.07.www): Add a field `key' to make
	citations look nicer (when using natbib, for instance).

2007-10-19  Roland Levillain  <roland@lrde.epita.fr>

	Add French versions of frequently used BibTeX styles.

	* styles/abbrv-fr.bst,
	* styles/abbrvnat-fr.bst,
	* styles/alpha-fr.bst,
	* styles/apalike-fr.bst,
	* styles/ieeetr-fr.bst,
	* styles/plain-fr.bst,
	* styles/plainnat-fr.bst,
	* styles/siam-fr.bst,
	* styles/unsrt-fr.bst,
	* styles/unsrtnat-fr.bst: New files.
	Imported from http://www.lsv.ens-cachan.fr/~markey/bibla.php.
	* doc/share.txt: Mention them.

2007-10-18  Roland Levillain  <roland@lrde.epita.fr>

	Fix Makefile's `clean' target.

	* Makefile (CLEANFILES): Don't remove bib/lrde.bib nor
	README-lrde.bib.

2007-10-18  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Add missing keywords in LDF for Stratego and SDF(AG).
	* styles/ldf/sdf.ldf: Add some Stratego keywords.
	* styles/ldf/stratego.ldf: Add missing Stratego keywords.

2007-10-17  Akim Demaille  <akim@lrde.epita.fr>

	myindex.hva.
	* styles/myindex.hva: New.
	Really too poor, but I don't know how to make this work
	with HeVeA.
	* styles/texi.hva: Remove debugging information.
	* vaucanson.sty: Remove.
	Has nothing to do there.

2007-10-17  Akim Demaille  <akim@lrde.epita.fr>

	myifthen.sty.
	* styles/myifthen.sty: New.

2007-10-17  Akim Demaille  <akim@lrde.epita.fr>

	More HeVeA compat.
	* styles/myhyperref.hva, styles/bilan.hva, styles/misc.hva:
	HeVeA now (1.10) supports \RequirePackage.
	* styles/mybabel.hva: Move portable definitions to...
	* styles/mybabel.sty: here.
	(\og, \fg): Now supported by HeVeA.
	(\voeu, \voeux): New.
	* styles/myifthen.sty: Rename as...
	* styles/myifthen.hva: this.
	* sytles/myifthen.sty: New.
	* styles/texi.hva (\mailto): Fix to work properly with HeVeA.

2007-10-16  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib: Add fact.www.

2007-10-16  Roland Levillain  <roland@lrde.epita.fr>

	Fix veldhuizen.99.tech.

	* bib/gp.bib (veldhuizen.99.tech): Rename field `url' as
	`howpublished', so that natbib-style citations can work
	properly.

2007-10-16  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib: Add myrnyy.04.cit.

2007-10-15  Thierry Geraud  <thierry.geraud@lrde.epita.fr>

	Fix jerome's 06 entries in lrde.bib.

	* bib/lrde.bib (konukoglu.06.itip): Rename as...
	(yoruk.06.itip): ...this.
	(darbon.06.jmiv, darbon.06.jmivb.pdf): Fix title.
	Add volume, number, and pages fields.
	Remove 'note' field.

2007-10-13  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (karvonen.02.pp): Fix title.

2007-10-13  Akim Demaille  <akim@lrde.epita.fr>

	colorbox.
	* styles/mylistings.sty (colorbox): New style.

2007-10-13  Roland Levillain  <roland@lrde.epita.fr>

	* styles/myacronym.sty (\acrodef{oop}):
	s/Object Oriented/Object-Oriented/.

2007-10-12  Akim Demaille  <akim@lrde.epita.fr>

	Prefer svnw, fix bib title.
	* bib/gp.bib: Protect from lower casing.
	* make/share-am.mk (SVN): Look for svn-wrapper first.

2007-10-12  Akim Demaille  <akim@lrde.epita.fr>

	More about JJForester.
	* bib/compilation.bib: Here.
	And sort.

2007-10-12  Akim Demaille  <akim@lrde.epita.fr>

	lrdedoc.
	* bib/compilation.bib: For visser.01.sigplan.

2007-10-12  Akim Demaille  <akim@lrde.epita.fr>

	tom.bib.
	* bib/tom.bib: New.
	* bin/update-bib: Fetch it.

2007-10-12  Akim Demaille  <akim@lrde.epita.fr>

	update-bib.
	* bin/update-bib: Fix.
	* bib/strategoxt.bib: Update.

2007-10-12  Akim Demaille  <akim@lrde.epita.fr>

	update-bib.
	* bin/update-bib: New.
	Based on...
	* Makefile (update-bib): This.
	* bib/strategoxt.bib, bib/kernighan.bib, bib/visser.bib: Update.

2007-10-12  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib: Add meyers.96.morec++.

2007-10-12  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib: Add karvonen.02.pp.

2007-10-12  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib: Add vanrossum.06.python.

2007-10-12  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib: Add ben-kiki.05.yaml.

2007-10-12  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib: Add shopyrin.06.ieeesoft.

2007-10-11  Akim Demaille  <akim@lrde.epita.fr>

	Fix update-cite.
	* bin/update-cite: Group where needed.
	* bib/gp.bib: Fix a key.

2007-10-10  Akim Demaille  <akim@lrde.epita.fr>

	bagge.03.scam.
	* bib/transformers.bib (bagge.03.scam): New.

2007-10-10  Akim Demaille  <akim@lrde.epita.fr>

	bagge.03.rule.
	* bib/transformers.bib: Add it.
	Normalize and sort the file.

2007-10-10  Akim Demaille  <akim@lrde.epita.fr>

	Fixes.
	* Makefile: Fix the dependencies on make-bib.pl.
	* bin/make-bib.pl: Up to 2008.
	* styles/misc.sty: \defined does not exist.

2007-10-05  Akim Demaille  <akim@lrde.epita.fr>

	myindex.
	* styles/lrde-bulletin.sty, styles/misc.sty, styles/myhyperref.sty:
	Use myifthen.
	Reported by Michael Cadilhac.
	* styles/myindex.sty: New.
	* styles/texi.hva: Use it.

2007-10-05  Akim Demaille  <akim@lrde.epita.fr>

	myifthen, \dfn.
	* styles/myifthen.sty: New.
	* styles/texi.hva (\dfn): Now also introduces the defined term
	in the index.
	(\hyperpagebf): New.
	Not used yet, as we need to teach xindy that this is markup.

2007-10-01  Akim Demaille  <akim@lrde.epita.fr>

	\coeur.
	* styles/mybabel.hva: Define a few \oe words.
	* styles/mybabel.sty: Include it.

2007-10-01  Akim Demaille  <akim@lrde.epita.fr>

	Update.
	* bin/texi2dvi: From Master.

2007-09-27  Akim Demaille  <akim.demaille@free.fr>

	Kill a few warnings.
	* styles/misc.sty: Don't require myhyperref, since that prevents
	passing it options.  Rather, use its features if available.
	* styles/myhyperref.sty (\gf): A local definition avoiding PDF
	warnings.

2007-09-25  Akim Demaille  <akim@lrde.epita.fr>

	Bulletin changes
	* styles/lrde-bulletin.sty (\chapter): Have a bigger subtitle.
	Remove tricks to squeeze the room here: that's the wrong
	approach, rather play with \@plus etc. in \@startsection.

2007-09-19  Akim Demaille  <akim.demaille@free.fr>

	volumetitle use
	* styles/lrde-bulletin.sty: Put it in \huge in the title page,
	and use it in the headers.

2007-09-19  Roland Levillain  <roland@lrde.epita.fr>

	Start a bibliography for Olena.

	* bib/lrde.bib (geraud.06.scoop-pres, olena.www): Move these
	entries...
	* bib/olena.bib: ...here (new file).

2007-09-19  Thierry Geraud  <thierry.geraud@lrde.epita.fr>

	Add URL in an lrde.bib entry.

	* bib/lrde.bib (geraud.06.scoop-pres): Add urllrde.

2007-09-19  Didier Verna  <didier@lrde.epita.fr>

	* styles/lrde-bulletin.sty (\titlepage): Use babel's \No macro.

2007-09-19  Akim Demaille  <akim@lrde.epita.fr>

	Update Vaucanson-g again
	* Makefile (update-styles): Fetch Vcn where it lives.
	* styles/vaucanson-g.sty: Update.

2007-09-19  Akim Demaille  <akim@lrde.epita.fr>

	Update Vaucanson-G
	* styles/FinalStateVar.tex: New.
	* styles/VCPref-beamer.tex: New.
	* styles/VCPref-gastex.tex: New.
	* styles/VCPref-main.tex: New.
	* styles/VCPref-slides.tex: New.
	* styles/VCpatch-pstricks-1-10.tex: New.
	* styles/Vaucanson-G.tex, styles/vaucanson-g.sty: Update from upstream.

2007-09-17  Akim Demaille  <demaille@gostai.com>

	\inputarticle
	* share/styles/lrde-bulletin.sty: Well, not new, existed
	already!
	(inputenc, mybabel): Require them.
	For some reason it doesn't appear to be working properly:
	the "N^o" part of the title page comes out badly. Didier?

2007-09-17  Akim Demaille  <demaille@gostai.com>

	\gf
	* styles/mybabel.hva, styles/mybabel.sty (\gf): New.
	Don't use \g which is reported to be defined by "some"
	package.

2007-09-17  Akim Demaille  <akim@lrde.epita.fr>

	Fix key style
	* bib/lrde.bib: Use the style defined in the README.

2007-09-17  Reda Dehak  <reda@lrde.epita.fr>

	* bib/lrde.bib: add dehak.08a.odyssey, dehak.08b.odyssey and
	kenny.08b.odyssey.

2007-09-14  Akim Demaille  <demaille@gostai.com>

	Update lrde-bulletin.sty
	* styles/lrde-bulletin.sty (myhyperref, wrapfig): Require them,
	we use them.
	(\chapter): Use \huge instead of \Huge.

2007-09-07  Akim Demaille  <akim@lrde.epita.fr>

	More compact.
	* styles/mysig-alternate.cls (\leftmargini): Redefine.

2007-09-07  Akim Demaille  <akim@lrde.epita.fr>

	Comments.
	* styles/mysig-alternate.cls: Fix command definitions.

2007-08-31  Akim Demaille  <akim@lrde.epita.fr>

	seminarTimeTable.
	* styles/lrde-bulletin.sty (seminarTimeTable, seminarSession):
	New.

2007-08-30  Roland Levillain  <roland@lrde.epita.fr>

	Fix instantiate-template.sh.

	* bin/instantiate-template.sh: Have Perl regexp be robust to
	quotes (') and at (@).

2007-08-06  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (conceptgcc.07.www): New entry.

2007-08-06  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (boost.07.www): New entry..

2007-08-06  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (chiba.95.oopsla): New entry.

2007-08-06  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (cgal.07.www): New entry.

2007-08-04  Roland Levillain  <roland@lrde.epita.fr>

	Protect upper case letters in gp.bib.

	* bib/gp.bib (gil.07.www, jarvi.01.tmpw, lumsdaine.01.itl)
	(siek.98.iscope, siek.98.poosc, siek.00.bccl, siek.01.bgl)
	(stepanov.00.book): Protect upper case letters.

2007-08-01  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib (zolyomi.03.gpce): New.
	(jarvi.03.gpce, zolyomi.04.gpce): Add acronym GPCE to `booktitle'.

2007-07-31  Roland Levillain  <roland@lrde.epita.fr>

	More entries in gp.bib (cont.).

	* bib/gp.bib (dosreis.05.lcsdm, siek.00.bccl, zolyomi.04.gpce):
	New entries.
	(gurtovoy.04.mpl): Write the full first names of authors.
	Rename field `conflocation' as `address'.
	Typo in `publisher' field.
	* bib/lrde.bib (duret.00.gcse): Typo in `booktitle' field.

2007-07-30  Roland Levillain  <roland@lrde.epita.fr>

	Even more entries in gp.bib.

	* bib/gp.bib (garcia.03.oopsla): Fix the `author' field.
	(siek.00.tmpw): Add a `lrdedoc' field.
	(veldhuizen.99.tech): Turn entry into a technical report.
	Complete entry.
	(abrahams.01.tmpw, jarvi.03.gpce, jarvi.06.pldi, lumsdaine.01.itl)
	(powell.00.cuj, siek.98.iscope, siek.98.poosc, siek.98.siamoo)
	(weiser.00.tmpw): New entries.
	* bib/lrde.bib (geraud.06.scoop-pres): Use \url in `howpublished'
	field.
	(olena.www): Rename field `url' as `howpublished'.

2007-07-27  Roland Levillain  <roland@lrde.epita.fr>

	More entries in gp.bib.

	* bib/gp.bib (coplien.96.cppgems): Fix title.
	(abrahams.04.metaprog, myers.95.cppr): Protect the case of `C++'.
	(gil.07.www, siek.01.bgl): More entries.

2007-07-26  Roland Levillain  <roland@lrde.epita.fr>

	Fix BibTeX entry abrahams.04.metaprog.

	* bib/gp.bib (abrahams.04.metaprog): Move URL from field
	`note' to field `annote'.

2007-07-26  Roland Levillain  <roland@lrde.epita.fr>

	Remove duplicate entry olena.www.

	* bib/gp.bib, bib/transformers.bib (olena.www): Move entry...
	* bib/lrde.bib (olena.www): ...here.

2007-07-26  Roland Levillain  <roland@lrde.epita.fr>

	Update gp.bib.

	* bib/gp.bib (abrahams.04.metaprog): New entry.
	(gurtovoy.02.boost): Update entry and rename it as...
	(gurtovoy.04.mpl): ...this.

2007-07-23  Akim Demaille  <akim@lrde.epita.fr>

	Update texi2dvi, myenumerate
	* bin/texi2dvi: Update from master.
	* styles/myenumerate.sty: New.

2007-07-17  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib: Add geraud.06.scoop-pres.

2007-07-09  Roland Levillain  <roland@lrde.epita.fr>

	* styles/fixme.sty: Update to FiXme 3.2.

2007-07-06  Roland Levillain  <roland@lrde.epita.fr>

	Add/update the ACM SIG Proceedings Templates.
	(From http://www.acm.org/sigs/pubs/proceed/template.html.)

	* styles/acm_proc_article-sp.cls: New (ACM LaTeX2e Style File
	V3.1SP (June 2007)).
	* styles/sig-alternate.cls: Update (Alternate ACM LaTeX2e
	Style File V2.3 (June 2007)).

2007-06-27  Akim Demaille  <akim@lrde.epita.fr>

	Fix csi.bib.
	* doc/share.txt: More about csi.bib.
	* bib/csi.bib: Fix keys and other mistakes.

2007-06-26  Charles-Alban Deledalle  <deledalle@lrde.epita.fr>

	Add deledalle report reference.

	* bib/csi.bib: .

2007-06-25  Benoit Sigoure  <tsuna@lrde.epita.fr>

	* bib/csi.bib: Add revCPP report.

2007-06-21  Akim Demaille  <akim@lrde.epita.fr>

	* bin/instantiate-template.sh: Also instantiate the ignores..

2007-06-21  Akim Demaille  <akim@lrde.epita.fr>

	Fixes.
	* bib/lrde.bib: Pay attention to upper case letters in titles.

2007-06-21  Akim Demaille  <akim@lrde.epita.fr>

	\warn.
	* styles/mylistings.sty (\warn): Protect again multiple definitions.
	* styles/beamerthemeKremlinBicetre.sty (\warn): New.

2007-06-18  Akim Demaille  <akim@lrde.epita.fr>

	Clean lrde.bib.
	* bib/lrde.bib: A few fixes.
	 (geraud.06.ivc): Remove.

2007-06-15  Akim Demaille  <akim@lrde.epita.fr>

	Check csi.bib.
	* Makefile (BIBS): New.
	Use to check several *.bib instead of just lrde.bib.
	* bib/csi.bib: Fix some errors.
	Sort.

2007-06-14  Maxime van Noppen  <maxime.van-noppen@lrde.epita.fr>

	Add seminar
	* csi.bib: Add seminar.

2007-06-14  Florian Queze  <Florian.Queze@lrde.epita.fr>

	Add entry for my seminar
	* csi.bib: Add entry for my repport.

2007-06-14  Florian Lesaint  <florian.lesaint@lrde.epita.fr>

	Add entry for seminar
	* bib/csi.bib: Here.

2007-06-14  Antoine Leblanc  <leblanc@lrde.epita.fr>

	Report 0745 SMALLSUBJECT updated
	* bib/csi.bib: SMALLSUBJECT updated.

2007-06-08  Antoine Leblanc  <leblanc@lrde.epita.fr>

	Report 0745 added in csi.bib
	* bib/csi.bib: Report 0745 added.

2007-06-07  Roland Levillain  <roland@lrde.epita.fr>

	Add baillard.07.gretsi to bib/lrde.bib.

	* bib/lrde.bib: Add entry baillard.07.gretsi.

2007-06-06  Akim Demaille  <akim@lrde.epita.fr>

	More Svn info.
	* TODO: New.
	* make/tex.mk: Pass all the infos.

2007-05-30  Roland Levillain  <roland@lrde.epita.fr>

	styles/gretsi.cls.

	* styles/gretsi.cls: New.

2007-05-30  Roland Levillain  <roland@lrde.epita.fr>

	Add style file for Signal Processing Society Conferences
	(ICASSP, ICIP).

	* styles/spconf.sty: New.

2007-05-30  Roland Levillain  <roland@lrde.epita.fr>

	Add package newalg.

	* styles/newalg.sty: New.

2007-05-22  Akim Demaille  <akim@lrde.epita.fr>

	Missing tags.
	* bib/lrde.bib: More transformers.

2007-05-22  Akim Demaille  <akim@lrde.epita.fr>

	Fix attribution.
	* bib/lrde.bib: Properly tag vcn papers.

2007-05-22  Akim Demaille  <akim@lrde.epita.fr>

	* bin/texi2dvi: Update DVIPSHEADERS so that dvips finds its
	special headers.

2007-05-22  Akim Demaille  <akim@lrde.epita.fr>

	Add Gastex.
	* Makefile (update-styles): New.
	* styles/gastex.pro: New.
	* styles/gastex.sty: New.

2007-05-21  Roland Levillain  <roland@lrde.epita.fr>

	* bib/sip.bib: Fix the previous patch.

2007-05-14  Roland Levillain  <roland@lrde.epita.fr>

	* bib/gp.bib: Add siek.04.clfpg.

2007-05-03  Roland Levillain  <roland@lrde.epita.fr>

	* styles/lrde-bulletin.sty: Have a bigger space between a title
	and an article.

2007-05-03  Thierry Geraud  <thierry.geraud@lrde.epita.fr>

	Update lrde.bib.

	* bib/lrde.bib (berger.07.icip): Update status.
	Add urllrde.

2007-04-27  Akim Demaille  <akim@lrde.epita.fr>

	Fix lrde.bib.
	* bin/make-bib.pl: Minor changes.
	* bib/lrde.bib: Add missing comma.
	* Makefile: Use perl to invoke make-bib.pl.

2007-04-25  Olivier Ricou <ricou@lrde.epita.fr>

	* bib/lrde.bib: Add ricou.07.eceg

2007-04-24  Didier Verna  <didier@lrde.epita.fr>

	* bib/lrde.bib (verna.06.ijcs): New.

2007-04-23  Daniela Becker  <daniela@lrde.epita.fr>

	Add itemTotal
	* styles/facture.cls (\itemTotal): New.
	Use it.

2007-04-23  Roland Levillain  <roland@lrde.epita.fr>

	Add a listings language style file for Leopard.

	* styles/ldf/leopard.ldf: New file.
	* styles/mylistings.hva: Include it.

2007-04-19  Roland Levillain  <roland@lrde.epita.fr>

	* styles/llncs.cls: Update to version 2.14.

2007-04-17  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (cardelli.96.csur): Fix the entry.

2007-04-17  Roland Levillain  <roland@lrde.epita.fr>

	More on cardelli.96.csur.

	* bib/compilation.bib (cardelli.96.acmcs): Rename as...
	(cardelli.96.csur): ...this.
	Fix title.
	Use the long form of the title of the journal.
	Add a WWW URL and a location in LRDE's documentation repository.

2007-04-17  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (ieee.98.float, goldberg.91.csur): New
	citations.

2007-04-16  Roland Levillain  <roland@lrde.epita.fr>

	Fix update-cite.

	* bin/update-cite (learn_from_bib): Use `!' as separator for the
	substitution command instead of `<' and `>', since it tends to mix
	up with the `<' of the f of the `(?<=[{, ])' pattern.
	* bib/compilation.bib (aiken.96.sigplan): s/Sigplan/SIGPLAN/.
	(automake.www) Add `automake' to `oldkeys'.
	(visser.01.sigplan): New entry.

2007-04-04  Akim Demaille  <akim.demaille@free.fr>

	* styles/myhyperref.sty (\subfigureautorefname): New.

2007-04-02  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (edwards.03.ln): Add `edwardsln' to oldkeys.

2007-03-28  Akim Demaille  <akim@lrde.epita.fr>

	eta.bib.
	* bib/eta.bib: New.
	Courtesy from Jacques Sakarovitch.

2007-03-27  Akim Demaille  <akim@lrde.epita.fr>

	Bib changes.
	* bib/gp.bib (iso.98.cpp): Remove, duplicates...
	* bib/transformers.bib (iso.98.c++): this.
	Complete these entries.
	* bib/vaucanson.bib: Add years to produce nicer bibliographies, and
	nicer keys.
	(thompson.68.cacm): New.

2007-03-27  Akim Demaille  <akim@lrde.epita.fr>

	More for automata.
	* styles/myacronym.sty (stl): New.
	* bib/ciaa-04.bib: New.

2007-03-19  Thierry Geraud  <thierry.geraud@lrde.epita.fr>

	Fix ambiguity about Rejected papers.

	* doc/update-lrde-bib.txt: Fix text on 'Rejected' papers.
	* bib/lrde.bib (geraud.06.lcsd-abstract): Remove.

2007-03-15  Akim Demaille  <akim@lrde.epita.fr>

	Fixes.
	* bib/lrde.bib (hamez.07.pohll): Fix.
	* Makefile (check): Run all the checks.

2007-03-15  Akim Demaille  <akim@lrde.epita.fr>

	* bib/lrde.bib: Add le-quoc.07.ntms..

2007-03-15  Akim Demaille  <akim@lrde.epita.fr>

	* styles/splncs.bst: New.

2007-03-14  Roland Levillain  <roland@lrde.epita.fr>

	Fix the `-s, --share' option in bin/update-cite.

	* bin/update-cite (parse_options): Do it.

2007-03-12  Akim Demaille  <akim.demaille@free.fr>

	* bin/update-cite: Strengthen the RE.

2007-03-05  Akim Demaille  <akim@lrde.epita.fr>

	More history.

	* bib/compilation.bib: More history entries.

2007-03-05  Akim Demaille  <akim@lrde.epita.fr>

	Beware of local implementation as a function.

	* bin/texi2dvi: Don't rely on non-IFS splitting when using local.
	Maybe we should just not use local at all.
	Or never use it to assign at the same time: declare, then assign.

2007-03-05  Akim Demaille  <akim@lrde.epita.fr>

	More compilation.bib.

	* bib/compilation.bib: Extend it.

2007-03-02  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Add student reports 0702.
	* bib/csi.bib: here.

2007-03-02  Akim Demaille  <akim@lrde.epita.fr>

	* bib/ciaa-05.bib: New.

2007-03-01  Akim Demaille  <demaille@gostai.com>

	Fixes
	* bin/update-cite: Fixes.
	* make/dist.mk (DISTDIR): Rename as...
	(distdir): this.

2007-02-28  Akim Demaille  <akim@lrde.epita.fr>

	Fixes.
	* styles/beamerthemeKremlinBicetre.sty: Include misc instead of
	defining again \lrde etc.
	Don't rely on the graphpath.
	* styles/myhyperref.sty: Do not change the link colors when
	using Beamer.  One bad result was the use of blue over... blue
	for the internal links, such as the short title in each bottom
	line (which in Beamer is a link to the toc).

2007-02-28  Roland Levillain  <roland@lrde.epita.fr>

	Move geraud.06.lcsd-abstract to lrde/papers/rejected/.

	* bib/lrde.bib (geraud.06.lcsd-abstract): Tag as rejected.

2007-02-27  Akim Demaille  <akim@lrde.epita.fr>

	Enable the disabling of local tocs.
	* styles/beamerthemeKremlinBicetre.sty: Check whether \NoSectionToc
	or \NoSubsectionToc are defined.
	Maybe there are means to pass arguments to themes?

2007-02-26  Akim Demaille  <akim@lrde.epita.fr>

	Title fixes.
	* bib/lrde.bib (borghi.06.crossroads): here.

2007-02-23  Akim Demaille  <akim@lrde.epita.fr>

	Fix the size of the references.
	* styles/facture.cls: here.

2007-02-20  Nicolas Pierron  <nicolas.pierron@lrde.epita.fr>

	Add paper: Strategic Graph Rewriting -- Transforming and
	Traversing Terms with References
	* transformers.bib: Add paper.

2007-02-14  Akim Demaille  <akim@lrde.epita.fr>

	rivf-07.bib.
	* bib/rivf-07.bib: New.
	* bib/lrde.bib: Fix/complete.

2007-02-12  Akim Demaille  <akim@lrde.epita.fr>

	One more simplification.
	* bib/lrde.bib: here.

2007-02-12  Akim Demaille  <akim@lrde.epita.fr>

	Bib fixes.
	* bin/latin2tex: Beware of "c,".
	* bib/rivf-06.bib: Remove useless braces.
	* Makefile: Let the checks be more explicit.

2007-02-09  Akim Demaille  <akim@lrde.epita.fr>

	rivf-06.bib.
	* bib/rivf-06.bib: New.

2007-02-09  Akim Demaille  <akim@lrde.epita.fr>

	More lrde.bib checks.
	* Makefile (check-urllrde, check-wiki, maintainer-check): New.

2007-02-08  Akim Demaille  <akim@lrde.epita.fr>

	Typos.
	* bib/lrde.bib: Complete first names, protect upper cases in
	titles.

2007-02-08  Akim Demaille  <akim@lrde.epita.fr>

	{CLOS}.
	* bib/lrde.bib: Use braces to protect upper cases.

2007-02-08  Akim Demaille  <akim@lrde.epita.fr>

	Simple fixes.
	* styles/misc.sty: We need hyperref for \texorpdfstring.
	* bib/lrde.bib: Add a missing volume.
	* bib/IEEEfull.bib, bib/IEEEabrv.bib: White spaces changes.

2007-02-05  Akim Demaille  <akim@lrde.epita.fr>

	* styles/texi.hva (\mailto, \http): New.
	(\email): Use for former.

2007-01-31  Akim Demaille  <akim@lrde.epita.fr>

	More builtins in KB.
	* styles/beamerthemeKremlinBicetre.sty (xspace, eurosym): Use.
	(\csi, \epita, \lrde): New.

2007-01-30  Roland Levillain  <roland@lrde.epita.fr>

	* styles/rotating.hva: New.
	Dummy header, to pacify HeVeA.

2007-01-29  Akim Demaille  <akim@lrde.epita.fr>

	make -k.
	* Makefile (check-warning): New.

2007-01-29  Akim Demaille  <akim@epita.fr>

	* bib/lrde.bib: RIVF cannot claim to be IEEE.
	Use isbn instead of annote to store isbn numbers.
	(berger.07.icip): Sort properly.
	(darbon.07.mirage): Add.

2007-01-26  Akim Demaille  <akim@lrde.epita.fr>

	Improve HeVeA's \og & \fg.
	* styles/mybabel.hva: Using xspace and ~.

2007-01-26  Roland Levillain  <roland@lrde.epita.fr>

	* styles/atbeginend.sty: New style (imported).
	* doc/share.txt: Document it.

2007-01-26  Roland Levillain  <roland@lrde.epita.fr>

	Add an IEEE bibliography style and its abbreviated version.

	* styles/IEEEbib.bst, styles/IEEEbib-abrv.bst: New.
	* doc/share.txt: Document them.

2007-01-26  Roland Levillain  <roland@lrde.epita.fr>

	* README: Document the use of acronyms in bibliographies.
	Typos.

2007-01-25  Roland Levillain  <roland@lrde.epita.fr>

	Start a bibliography on Signal and Image Processing in share,
	from contents.bib files from /lrde/doc.

	* bib/lrde.bib: Have French first names starting with `Ch' and
	`Th' keep the `h' when abbreviated.
	* bib/sip.bib,
	* bib/acronyms.bib, bib/acronyms-abrv.bib: New.
	* doc/share.txt: Mention them.

2007-01-24  Akim Demaille  <akim@lrde.epita.fr>

	waddington.05.ldta.
	* doc/share.txt: One more example, to highlight the use of the
	file extension.
	* bib/transformers.bib (waddington.05.ldta): New.
	* Makefile (update): Remove write permissions from download bibs.

2007-01-24  Akim Demaille  <akim@lrde.epita.fr>

	lrde/doc.
	* doc/share.txt: s,/mnt,/lrde,g.
	Introduce the "lrdedoc" field in BibTeX entries.
	* bib/gp.bib (gamma.95.gp): Be an example.

2007-01-24  Akim Demaille  <akim@lrde.epita.fr>

	Fix kernighan.bib.
	* bib/kernighan.bib: Add many missing commas.
	* Makefile (update): Do this automatically in the future.

2007-01-24  Akim Demaille  <akim@lrde.epita.fr>

	/lrde/doc.
	* Makefile: Adjust paths.

2007-01-22  Akim Demaille  <akim@lrde.epita.fr>

	Update IEEEtran.cls.
	* styles/IEEEtran.cls: Version 1.7, from upstream.
	* doc/share.txt: Update location of doc.

2007-01-22  Didier Verna  <didier@lrde.epita.fr>

	* bib/lrde.bib (verna.07.imecs): New.

2007-01-22  Thierry GERAUD  <theo@tegucigalpa.lrde.epita.fr>

	* bib/lrde.bib (fouquier.07.icassp): Fix entry.
	* bib/lrde.bib (berger.07.icip): New.

2007-01-22  Roland Levillain  <roland@lrde.epita.fr>

	Add support for PBM and PPM files for PDF.

	* make/pdf-figs.mk (SHARE_EXTS_TO_PDF): Add pbm and ppm.
	(%.pdf): New rule to create PDF files from PBM and PPM images.

2007-01-19  Akim Demaille  <akim@lrde.epita.fr>

	Aleluia, hevea now supports xspace.
	This is hevea 1.09.
	* styles/misc.hva, styles/misc.sty: Include the package xspace
	for hevea too.

2007-01-16  Akim Demaille  <akim@lrde.epita.fr>

	Sync with master.
	* bin/texi2dvi: here.

2007-01-16  Akim Demaille  <akim@lrde.epita.fr>

	remove hevea trailing spaces.
	* bin/texi2dvi (run_hevea): here.

2007-01-15  Akim Demaille  <akim@lrde.epita.fr>

	\acr.
	* styles/myacronym.sty (\acr, \acrp): New.
	* doc/share.txt: Doc them.

2007-01-10  Akim Demaille  <akim@lrde.epita.fr>

	Don't include figs/ by default.
	* make/tex.mk(TEXI2DVI_FLAGS): Don't pass -I figs.
	It is safer to use qualified file names with includegraphics etc.
	Besides, that make DVI work easier (dvips and xdvi don't have -I figs,
	but if the file name is qualified, they will find the files).

2007-01-09  Akim Demaille  <akim.demaille@free.fr>

	Add eps support to pdf-figs.mk
	* make/pdf-figs.mk: here.
	This is messy, Q&D, but I need that now :(

2007-01-08  Akim Demaille  <akim@lrde.epita.fr>

	mysig-alternate.
	* styles/mysig-alternate.cls: New.
	* doc/share.txt: Doc it.

2007-01-08  Akim Demaille  <akim@lrde.epita.fr>

	More precise entries.
	* bib/compilation.bib: here.

2007-01-08  Akim Demaille  <akim@lrde.epita.fr>

	Fix dist.
	* make/dist.mk: Don't use pipes to avoid hiding failures.

2007-01-05  Roland Levillain  <roland@lrde.epita.fr>

	Add support for PGM files.

	* make/pdf-figs.mk (SHARE_EXTS_TO_PDF): Add pgm.
	(%.pdf): New rule to convert PGM images to PDF files.

2007-01-05  Akim Demaille  <akim@lrde.epita.fr>

	Complete bibs.
	* bib/lrde.bib, bib/compilation.bib: Complete entries, to
	please picky reviewers.

2007-01-05  Akim Demaille  <akim@lrde.epita.fr>

	Use the long title.
	* styles/beamerthemeKremlinBicetre.sty (\maketoc): here.

2007-01-05  Akim Demaille  <akim@lrde.epita.fr>

	Fix share-up.
	* make/share-am.mk: here.

2007-01-05  Akim Demaille  <akim@lrde.epita.fr>

	More pdf output.
	* make/pdf-figs.mk: Add support for GNU Plot files output in
	PDF + TeX parts.
	Workaround fig2dev portability issues.
	* doc/share.txt: Update.

2006-12-18  Akim Demaille  <akim@lrde.epita.fr>

	Fix share-up.
	* make/share-am.mk: Here.

2006-12-18  Akim Demaille  <akim@lrde.epita.fr>

	grammar.ldf.
	* styles/ldf/grammar.ldf: New.
	* styles/mylistings.hva: Use it.
	* doc/share.txt: Doc it.
	* make/share-am.mk: Initialize CLEANFILES for real.

2006-12-11  Akim Demaille  <akim.demaille@free.fr>

	camlp4.manual
	* bib/transformers.bib: New.

2006-12-11  Valentin David  <valentin@ii.uib.no>

	Add a space after arrows in SDF syntax
	* styles/ldf/sdf.ldf: Add a space.

2006-12-11  Akim Demaille  <akim.demaille@free.fr>

	Don't use courier, it's real ugly
	* styles/myentcs.cls: here.

2006-12-11  Akim Demaille  <akim.demaille@free.fr>

	Use rightarrow in SDF
	* styles/ldf/sdf.ldf: Here.

2006-12-11  Akim Demaille  <akim.demaille@free.fr>

	Found the quotes!
	* styles/ldf/stratego.ldf: Finally found the right way to
	type set the Stratego quotes.

2006-12-11  Akim Demaille  <akim@lrde.epita.fr>

	Fix SDF definition.
	* styles/ldf/sdf.ldf: context and free are not keywords,
	context-free is.

2006-12-11  Akim Demaille  <akim@lrde.epita.fr>

	Improve Stratego style.
	* styles/ldf/stratego.ldf: Don't highlight {}.
	- is valid in identifiers.

2006-12-11  Akim Demaille  <akim@lrde.epita.fr>

	Candy for |[]|.
	* styles/ldf/stratego.ldf: here.

2006-12-11  Akim Demaille  <akim@lrde.epita.fr>

	|[ ]|.
	* styles/ldf/stratego.ldf: Add candy for quotes.

2006-12-11  Valentin David  <valentin@ii.uib.no>

	Add a SAGA bibtex file.
	* bib/saga.bib: New.

2006-12-11  Akim Demaille  <akim@lrde.epita.fr>

	More oldkeys, fix update-cite.
	* bin/update-cite: Don't match too easily.
	* bib/transformers.bib, bib/cwi.bib: Add missing oldkeys.

2006-12-08  Akim Demaille  <akim@lrde.epita.fr>

	More transformer.bib.
	* doc/share.txt: Use zzzref for cross-refs.
	* bib/transformers.bib (zook.04.gpce): New.
	Rekey some entries.

2006-12-08  Akim Demaille  <akim@lrde.epita.fr>

	psbbox: Fix gs invocation.
	* bin/psbbox: Pass - to gs.

2006-12-08  Akim Demaille  <akim@lrde.epita.fr>

	psbbox --pages.
	* bin/psbbox: Support --pages.
	(&backup): Copy instead of moving.

2006-12-06  Akim Demaille  <akim@lrde.epita.fr>

	myentcs.
	* styles/myentcs.cls: New.
	* doc/share.txt: Doc it.

2006-12-06  Akim Demaille  <akim@lrde.epita.fr>

	Remove anisko.05.ldta.
	* bib/lrde.bib: Was rejected anyway.

2006-12-06  Akim Demaille  <akim@lrde.epita.fr>

	Update foreign bibs.
	* make/share-am.mk (update): Remove.
	* Makefile (update): New.
	* bib/strategoxt.bib: Update.
	* bib/kernighan.bib: Update.
	* bib/dmr.bib: Rename as...
	* bib/richie.bib: this.
	Update.

2006-12-06  Akim Demaille  <akim@lrde.epita.fr>

	Clean transformers.bib and csi.bib.
	* bib/transformers.bib, bib/csi.bib: Run reformat.
	Move student reports from the former to the latter.
	Sort.

2006-12-06  Akim Demaille  <akim@lrde.epita.fr>

	Fix bib entry key.
	* bib/lrde.bib (bellot.07.rivf): Rename as...
	(le-quoc.07.rivf): this.

2006-12-06  Akim Demaille  <akim@lrde.epita.fr>

	Fix an urllrde.
	* bib/lrde.bib (bellot.07.rivf): here.

2006-12-04  Akim Demaille  <akim@lrde.epita.fr>

	bellot.07.rivf.
	* bib/lrde.bib: New.
	Run Emacs' reformatting.

2006-12-04  Akim Demaille  <akim@lrde.epita.fr>

	Typo in previous checkin.
	* make/dload.mk: Check whether there is something to install,
	not whether there is a place for it to be installed.

2006-12-04  Akim Demaille  <akim@lrde.epita.fr>

	dload.mk: also handle lrde/papers.

	* make/dload.mk: .

2006-12-04  Akim Demaille  <akim@lrde.epita.fr>

	Add phony.
	* make/dload.mk: here.

2006-12-04  Akim Demaille  <akim@lrde.epita.fr>

	Update ENTCS style.
	* styles/entcs.cls: Updated from http://www.entcs.org/prelim.html.
	* styles/prentcsmacro.sty: Remove, as this file is
	specific to each conference, it should not be shared.

2006-12-04  Akim Demaille  <akim@lrde.epita.fr>

	Fix entcsmacro.sty.
	* styles/entcsmacro.sty: What are they waiting for to update
	their url?

2006-12-04  Akim Demaille  <akim@lrde.epita.fr>

	entsmacro.
	* styles/entcsmacro.sty: New.

2006-11-29  mefyl  <mefyl@lrde.epita.fr>

	Add Hocquet and Moulard techreps to csi.bib.
	* bib/csi.bib: Add Hocquet and Moulard techreps.

2006-11-28  Christophe Berger  <christophe.berger@lrde.epita.fr>

	Fix seminar techrep name (introduced in rev 1713).

	* bib/csi.bib: Fix the name.

2006-11-28  Akim Demaille  <akim@lrde.epita.fr>

	Display the keys of the papers in the private version.
	* bin/make-bib.pl: Do that.
	* bib/lrde.bib (geraud.06.lcsd_abstract): Rename as...
	(geraud.06.lcsd-abstract): this, to avoid LaTeX issues with _.

2006-11-28  Akim Demaille  <akim@lrde.epita.fr>

	compactemize -> compactitemize.
	* styles/beamerthemeKremlinBicetre.sty: here.

2006-11-28  Akim Demaille  <akim@lrde.epita.fr>

	Remove a spurious period.
	* styles/lrde-bst.sty: here.

2006-11-28  Akim Demaille  <akim@lrde.epita.fr>

	Fixes in lrde.bib.
	* bib/lrde.bib (konukoglu.0X.itip): Complete and rename as
	(konukoglu.06.itip): this.
	(geraud.04.iccvg): Fix the year (my bad).

2006-11-27  Christophe Berger  <christophe.berger@lrde.epita.fr>

	Add seminar techreps to csi.bib.

	* bib/csi.bib: Add 0517 and 0603 seminar techreps.

2006-11-27  Akim Demaille  <akim@lrde.epita.fr>

	Issue the total of publications.
	* bin/make-bib.pl: Generate the total.
	Put the submissions before.
	* Makefile: Don't use >$@, that's dangerous.

2006-11-27  Akim Demaille  <akim@lrde.epita.fr>

	Prepare lrde.bib to be online.
	* bib/lrde.bib: Comment changes.
	* Makefile: Install it.

2006-11-27  Akim Demaille  <akim@lrde.epita.fr>

	lrde-private.pdf.
	* Makefile: It can appear in /mnt/doc/papers/lrde.

2006-11-27  Akim Demaille  <akim@lrde.epita.fr>

	Enumerate the publications.
	* bin/make-bib.pl (&section_by_key): Use &bibliography.
	(&bibliography): Use {enumerate}.

2006-11-27  Akim Demaille  <akim@lrde.epita.fr>

	pgfdeclare logos.
	* styles/beamerthemeKremlinBicetre.sty (lrde-logo-mask, lrde-logo)
	(lrde-logo-red): New pgf images.

2006-11-23  Roland Levillain  <roland@lrde.epita.fr>

	Fix bin/pdfbook.

	* bin/pdfbook (work_dir): New.  Use it to define...
	(in_ps, book_ps): ...these.
	Pass an output filename as second argument to ps2pdf14, instead of
	writing the standard output of ps2psd14 to this file.

2006-11-22  Akim Demaille  <akim@lrde.epita.fr>

	Add \photo.
	* styles/lrde-bulletin.sty: here.
	With help from Didier Verna.

2006-11-18  Akim Demaille  <akim.demaille@free.fr>

	Update svn-externals
	* bin/svn-externals: Support arguments: directories to update.
	* make/share-am.mk: Use that feature.

2006-11-18  Akim Demaille  <akim.demaille@free.fr>

	Changes in KB style
	* styles/beamerthemeKremlinBicetre.sty: Use dynamic uncovering scheme.
	* styles/numberslides.sty: Fix comment.

2006-11-16  Akim Demaille  <akim.demaille@free.fr>

	Beamer things
	* figs/lrde-red.png, figs/lrdemask.jpg: New.
	* styles/numberslides.sty: Also include the instution.

2006-11-16  Akim Demaille  <akim.demaille@gmail.com>

	prism.ldf
	* styles/ldf/prism.ldf: New.
	From Benoit Sigoure.
	* styles/mylistings.hva: Use it.
	* doc/share.txt: Adjust.

2006-11-10  Akim Demaille  <akim@lrde.epita.fr>

	More ps tools.
	* bin/pdfbook: Don't optimize PS for speed.
	* bin/psfit: Use better margin default values.
	Document the a2ps binding.
	($verbose): Rename as...
	($verbose_p): this.
	Use the latest psbbox interface.
	* bin/psbbox: More TODO.

2006-11-09  Akim Demaille  <akim@lrde.epita.fr>

	Fix psfit, improve psbbox.
	* bin/psbbox: Support -e, -c, -f.
	* bin/psfit: Fix the computation of odd side inner margins.

2006-11-08  Akim Demaille  <akim@lrde.epita.fr>

	darbon.07.ei.
	* bib/lrde.bib (darbon.07.ei): New.
	Sort entries.

2006-11-06  Akim Demaille  <akim@lrde.epita.fr>

	lrde.bib fixes.
	* bib/lrde.bib (herault.06.qest): Year is 2006.
	(verna.06.ecoop): Flag as best paper.

2006-11-03  Akim Demaille  <akim@lrde.epita.fr>

	Use rich frames for tocs.
	* styles/beamerthemeKremlinBicetre.sty: Don't pass [plain] to
	toc frames.

2006-11-03  Akim Demaille  <akim@lrde.epita.fr>

	Don't use AtEndDocumentation.
	* styles/beamerthemeKremlinBicetre.sty: For some reason, the
	toc is not issued, but there is a empty slide.

2006-11-01  Akim Demaille  <akim@lrde.epita.fr>

	Also install the README.
	* Makefile: install README-lrde.bib to keep up to date.

2006-11-01  Akim Demaille  <akim@lrde.epita.fr>

	Move the checkin machinery of lrde.bib into share.
	* doc/update-lrde-bib.txt: New.
	* README-lrde.bib: New.
	* Makefile: Merge in, and adjust, what was in lrde-publis.

2006-11-01  Akim Demaille  <akim@lrde.epita.fr>

	Fix entry.
	* bib/lrde.bib (darbon.06b.jmiv): Rename as.
	(darbon.06.jmivb)

2006-11-01  Akim Demaille  <akim@lrde.epita.fr>

	Protect from bibtex.
	* bib/lrde.bib: The use of \LaTeX.

2006-11-01  Akim Demaille  <akim@lrde.epita.fr>

	Update svn-externals.

	* bin/svn-externals: More aliases.
	Simplify some checks.
	More assertions.
	* make/share-am.mk (SVN): New, use it.
	Upgrade the svn-externals invocation.

2006-10-30  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (bordeleau.03)
	* bib/model-checking.bib (arora, hightower): Remove extended
	characters to please BibTeX.

2006-10-30  Akim Demaille  <akim@lrde.epita.fr>

	Updates.
	* styles/lrde-bst.sty: New.
	* styles/misc.sty (\CurVe): New.
	* bin/make-bib.pl: --verbose.
	* bib/lrde.bib: Typo.

2006-10-30  Akim Demaille  <akim@lrde.epita.fr>

	Update lrde.bib.
	* bib/lrde.bib (darbin.06.tr): New.
	I found this definition in /mnt/doc.  It was not checked in.

2006-10-30  Akim Demaille  <akim@lrde.epita.fr>

	More styles for talks.
	* styles/numberslides.sty: New.
	* styles/beamerthemeKremlinBicetre.sty: New.
	* doc/share.txt: Adjust.

2006-10-27  Akim Demaille  <akim@lrde.epita.fr>

	Upgrades.
	* bin/psfit: Support -d/-i.
	Does not work as cleanly as expected :(
	* bin/svn-externals: Support -S, -U, -u, and recursive aliases.

2006-10-23  Akim Demaille  <akim.demaille@free.fr>

	Pass -p to fig2dev
	* make/pdf-figs.mk: to keep it landscape.

2006-10-22  Akim Demaille  <akim.demaille@free.fr>

	update svn-externals
	* bin/svn-externals: More aliases.
	More options.

2006-10-20  Akim Demaille  <akim@lrde.epita.fr>

	Trailing spaces.
	* styles/IEEEtranS.bst: Kill them.

2006-10-20  Akim Demaille  <akim@lrde.epita.fr>

	dos2unix.
	* styles/IEEEtran.bst: Do that.
	Kill trailing spaces.

2006-10-20  Akim Demaille  <akim@lrde.epita.fr>

	pdffig support.
	* make/pdf-figs.mk: Support pdffig.

2006-10-12  Akim Demaille  <akim@lrde.epita.fr>

	dload.mk.
	* make/dload.mk: New.
	* doc/share.txt: Document it.

2006-10-12  Akim Demaille  <akim@lrde.epita.fr>

	Upgrade psfit and psbbox.
	* bin/psfit, bin/psbbox: Accept more options.
	Accept - for input and output.

2006-10-11  Akim Demaille  <akim@lrde.epita.fr>

	psbbox: work also as a filter.
	* bin/psbbox: Implement that.
	The support for --help is tbd.

2006-10-09  Akim Demaille  <akim@lrde.epita.fr>

	Update svn-externals.

	* bin/svn-externals (usage): New.
	Don't expect sed to be nice, OSX is out there.
	Simplify the handling of aliases.

2006-10-09  Akim Demaille  <akim@lrde.epita.fr>

	psfit todo.

	* bin/psfit: Add some.

2006-10-06  Akim Demaille  <akim@lrde.epita.fr>

	Fix psfit.

	* styles/facture.cls: Add some useful comments I found somewhere.
	* bin/psfit: Support --margin, 24pt by default.
	Use correct A4 dimensions, not Letter ;)

2006-10-06  Akim Demaille  <akim@lrde.epita.fr>

	psfit.

	* doc/share.txt: Update.
	* bin/pdfbook: Pass -optimizeForSpeed.
	Support PS/PDF output.
	* bin/psfit: New.
	* bin/psbbox: Keep %%Page DSCs.

2006-10-04  Akim Demaille  <akim@lrde.epita.fr>

	Leave room for the bill key.

	* styles/facture.cls: Do that.

2006-10-04  Akim Demaille  <akim@lrde.epita.fr>

	Support *.tiff.

	* make/pdf-figs.mk: Do that.

2006-10-04  Akim Demaille  <akim@lrde.epita.fr>

	pdf-figs.

	* doc/share.txt: Typo.
	* doc/svn.txt: About not checking in products.
	* make/pdf-figs.mk: Support EXTS_TO_PDF and EXTS_TO_PNG.

2006-10-04  Akim Demaille  <akim@lrde.epita.fr>

	Fix svn-externals.

	* bin/svn-externals: Variables changes in pipes don't affect the
	environment...
	(svn_externals_update_stream): New.
	(svn_externals_update): Adjust.

2006-10-04  Akim Demaille  <akim@lrde.epita.fr>

	svn-externals.

	* doc/hevea.txt: New, extracted from...
	* README: here.
	Rename as...
	* make/share-am.mk: this.
	* README: New symlink.
	* doc/share.txt: New.
	* doc/README.svn: Rename as...
	* doc/svn.txt: this.

	* bin/update-share: Remove.
	* bin/svn-externals: New.

2006-09-29  Akim Demaille  <akim@lrde.epita.fr>

	Add README.svn.

	* doc: New.
	* doc/README.svn: New.
	* README: Update.

2006-09-27  Florent Terrones  <terron_f@lrde.epita.fr>

	* bib/vaucanson.bib: Add some misc urls.
	* bib/lrde.bib: Add the 2004 XML proposal.

2006-09-27  Roland Levillain  <roland@lrde.epita.fr>

	Adjust lrde.bst.

	* styles/lrde.bst (output.urllrde): Use `write$' instead of `output'.
	(output.note): New function.
	(output.etc): New function.
	(article, book, booklet, inbook, incollection, inproceedings)
	(manual, mastersthesis, misc, phdthesis, proceedings, techreport):
	Use it.
	From Akim Demaille.

2006-09-27  Roland Levillain  <roland@lrde.epita.fr>

	* bib/lrde.bib (lesage.06.isvc): Remove dummy entries.

2006-09-25  Akim Demaille  <akim@lrde.epita.fr>

	Merge lrde.bst and lrde-bulletin.bst.

	* styles/lrde-bulletin.bst: Remove.
	* styles/lrde.bst: Merge its features in here.
	(format): New, to factor.
	* README: Adjust.

2006-09-22  Akim Demaille  <akim@lrde.epita.fr>

	Don't output the key.

	* styles/lrde-bulletin.bst (\urllrdekey, \urllrdeyear): New.
	(\urltitlelrde): Rename as...
	(\lrdebibtitle): this.

2006-09-22  Akim Demaille  <akim@lrde.epita.fr>

	Add lrde-bulletin.bst.

	* styles/lrde-bulletin.bst: New.
	* bib/lrde.bib (verna.06.practex): Add a volume.

2006-09-21  Roland Levillain  <roland@lrde.epita.fr>

	Fix the previous patch.

	* bib/lrde.bib (darbon.06.iccp): Add a missing coma.

2006-09-21  Roland Levillain  <roland@lrde.epita.fr>

	Add darbon.06.iccp.

	* bib/lrde.bib (darbon.06.iccp): New entry.

2006-09-21  Roland Levillain  <roland@lrde.epita.fr>

	Fix cadilhac.06.avocs key.

	* bib/lrde.bib (cadilhac.06.avoics): Rename as...
	(cadilhac.06.avocs): ...this.
	* README: Typo.

2006-09-21  Akim Demaille  <akim@lrde.epita.fr>

	dmr.bib.

	* bib/dmr.bib: New.
	* README: Update.

2006-09-20  Michaël Cadilhac  <michael.cadilhac@lrde.epita.fr>

	* bib/lrde.bib: Add AVoCS 2006 Cadilhac et al paper..

2006-09-20  Akim Demaille  <akim@lrde.epita.fr>

	Add urls.

	* bib/csi.bib (sigoure.06.seminar.xrm): Add url.

2006-09-20  SIGOURE Benoit  <sigoure.benoit@lrde.epita.fr>

	Add Benoit Sigoure's techrep 0620.

	* bib/csi.bib: Here.

2006-09-20  Akim Demaille  <akim@lrde.epita.fr>

	Add wsn.

	* styles/myacronym.sty (wsn): New.

2006-09-20  Akim Demaille  <akim@lrde.epita.fr>

	Remove the definition of \CurVe.

	* bib/lrde.bib: as it breaks some tools (e.g., bibentry.sty).

2006-09-19  Akim Demaille  <akim@lrde.epita.fr>

	lrde.bib: Make it self contained.

	* bib/lrde.bib (\CurVe): Define.

2006-09-19  Akim Demaille  <akim@lrde.epita.fr>

	Fixes in lrde.bib.

	* bib/lrde.bib: Fixes and formatting changes.

2006-09-19  Akim Demaille  <akim@lrde.epita.fr>

	More lrde.bib.

	* bib/lrde.bib (baillard.05.adass, geraud.06.lcsd_abstract)
	(lesage.06.isvc, verna.06.practex): New.

2006-09-19  Akim Demaille  <akim@lrde.epita.fr>

	Nolimips Listing support.

	* styles/ldf/mips.ldf ([Nolimips]Assembler): New.

2006-09-18  Didier Verna  <didier@lrde.epita.fr>

	* styles/misc.hva (\etc): Fix typesetting.

2006-09-14  Akim Demaille  <akim@lrde.epita.fr>

	and fix it.

	* bib/lrde.bib: do it.

2006-09-14  Akim Demaille  <akim@lrde.epita.fr>

	Add urllrde.

	* bib/lrde.bib: Do it.

2006-09-14  Akim Demaille  <akim@lrde.epita.fr>

	Don't force the definition of DISTDIR.

	* make/dist.mk: nor that of TARBALL.

2006-09-14  Akim Demaille  <akim@lrde.epita.fr>

	More citations.

	* bib/lrde.bib (cadilhac.06.XX): Needs to be completed.
	* bib/gp.bib (veldhuizen.95.c++): New.
	* bib/csi.bib: Normalize.
	* bib/sensor-networks.bib: Remove junk.
	* README: Document csi.bib.

2006-09-13  Didier Verna  <didier@lrde.epita.fr>

	* styles/misc.hva (\clos): New macro.

2006-09-08  Akim Demaille  <akim@lrde.epita.fr>

	More SIGCSE.

	* bib/compilation.bib (mead.06.sigcse, werner.03.jcsc): New.

2006-09-08  Akim Demaille  <akim@lrde.epita.fr>

	Move Gamma.

	* bib/compilation.bib (gamma.95.dp): Move to...
	* bib/gp.bib: here (was duplicate).
	Fix other entries.

2006-09-08  Akim Demaille  <akim@lrde.epita.fr>

	More bib.

	* bib/compilation.bib (appelbe.78.sigcse, haynes.98.sigcse): New.

2006-09-08  Akim Demaille  <akim@lrde.epita.fr>

	Fix style of gp.bib.

	* bib/gp.bib: Do it.
	(onela.net, oonumerics.net, mpl): Rename as...
	(onela.www, oonumerics.www, gurtovoy.02.boost): these.

2006-09-08  Akim Demaille  <akim@lrde.epita.fr>

	Add hyphenation.

	* styles/myacronym.sty (oop): Do it.

2006-09-08  Akim Demaille  <akim@lrde.epita.fr>

	* styles/texi.sty, styles/texi.hva (\dfn, \var): Simplify them,
	since LaTeX actually already provides these services.
	(\email): Don't define it if already defined.

2006-09-07  Akim Demaille  <akim@lrde.epita.fr>

	* style/myacronyms.sty (cisc, il, ir, mips, risc, treecc): New.

2006-09-06  Akim Demaille  <akim@lrde.epita.fr>

	* make/share-am.mk (CLEANFILES): Initialize so that we can include
	these files last, instead of first.
	* bib/compilation.bib (aiken.96.sigplan): An article.
	(briggs.92.phd): Complete.

2006-09-06  Akim Demaille  <akim@lrde.epita.fr>

	* bin/update-cite: New.
	* README: Document.
	* bin/latin2tex: Implement --help.
	* bib/compilation.bib: Equip with oldkeys.
	(diwan.04.jeric, guimar.84.sigcse, shapiro.76.sigcse)
	(waite.06.iticse): New.

2006-09-05  Akim Demaille  <akim@lrde.epita.fr>

	* bib/lrde.bib (borghi.06.crossroads): Fix references.
	(darbon.XX.jmiv, darbon.XXb.jmiv): Rename and complete as...
	(darbon.06.jmiv, darbon.06b.jmiv): these.
	(demaille.06.isola): Accepted.

2006-08-11  Roland Levillain  <roland@lrde.epita.fr>

	Fix transformers.bib.

	* bib/transformers.bib (jastadd-url, uuag.www): Please BibTeX.

2006-07-25  Akim Demaille  <akim@lrde.epita.fr>

	texi: Prefix internal command names.

	* styles/texi.sty: Do it.
	This fixes a problem where a use of \var{} in a LaTeX document
	using an index would produce a failing index.  There is probably
	a name clash, I don't know which, we (with Micha) renamed them all.

2006-07-25  Akim Demaille  <akim@lrde.epita.fr>

	Add \strong.

	* styles/texi.hva: Do it.
	* README: Doc it.

2006-07-20  Akim Demaille  <akim@lrde.epita.fr>

	Add pdf-figs.mk.

	* make/pdf-figs.mk: New.
	* README: Document it.

2006-07-19  Akim Demaille  <akim@lrde.epita.fr>

	Don't ship .svn files.

	Reported by Valentin David.
	* make/dist.mk (DIST_IGNORE): New.
	Include .svn and +commited files.
	(distdir): Use it.

2006-07-19  Akim Demaille  <akim@lrde.epita.fr>

	Fix accents in bibtex files, add david.06.iccp.

	* bib/lrde.bib (david.06.iccp): New.

	* bin/latin2tex: New.
	* bib/transformers.bib, bib/ag.bib, bib/vaucanson.bib,
	* bib/compilation.clement.bib, bib/model-checking.bib,
	* bib/compilation.bib, bib/csi.bib: Normalize using latin2tex.
	* README, Makefile: Update.

2006-07-19  Akim Demaille  <akim@lrde.epita.fr>

	updates and IEEE completion.

	* styles/IEEEtranS.bst: New.
	* bib/IEEEfull.bib: New.
	* bib/IEEEbcpat.bib: New.
	* bib/IEEEabrv.bib: New.
	* bib/IEEEexample.bib: New.
	* bin/texi2dvi: Try to run bibtex for hevea.
	It does not work currently, as LaTeX (the real one) must
	be run to generate the aux file.
	* make/dist.mk (dist): Use cp, not tar, to preserve subdirectories.

2006-07-18  SIGOURE Benoit  <sigoure.benoit@lrde.epita.fr>

	Add some bib entry.

	* bib/strategoxt.bib: Here.
	* bib/model-checking.bib: And here.

2006-07-13  Akim Demaille  <akim@lrde.epita.fr>

	Black links.

	* styles/myhyperref.sty: Use \IsAFinal.
	* README: Explain.

2006-07-13  Akim Demaille  <akim@lrde.epita.fr>

	More doc.

	* README: for latex8.

2006-07-13  Akim Demaille  <akim@lrde.epita.fr>

	Kill trailing spaces.

	* styles/latex8.sty: Do it.

2006-07-13  Akim Demaille  <akim@lrde.epita.fr>

	Add dist.mk.

	* make/dist.mk: New.
	* README: Update.

2006-07-07  Robert Bigaignon  <robert.bigaignon@lrde.epita.fr>

	Add csi techrep bib (to be completed).

	* bib/csi.bib: New. Add bib entries for some CSI students
	technical reports.

2006-06-28  Akim Demaille  <akim@lrde.epita.fr>

	Bib normalization.

	* bib/compilation.bib (briggs92): Rename as...
	(briggs.92): this.

2006-06-27  Akim Demaille  <akim@lrde.epita.fr>

	Update texi2dvi.

	* bin/texi2dvi: from master.

2006-06-27  Akim Demaille  <akim@lrde.epita.fr>

	s/update/share-up/.

	* make/share-am.mk: Do it.
	* README: Doc it.
	* bin/texi2dvi: Update.

2006-06-27  Akim Demaille  <akim@lrde.epita.fr>

	Update texi2dvi.

	* bin/texi2dvi: Update from master.

2006-06-27  Akim Demaille  <akim@lrde.epita.fr>

	$(ChangeLog).

	* make/tex.mk (ChangeLog): New.
	Use it.
	* README: Doc it.

2006-06-26  Akim Demaille  <akim@lrde.epita.fr>

	Updates.

	* styles/myacronym.sty (burg, yacc): New.
	* bin/texi2dvi: Update from master.
	* make/share-am.mk (share_dir): Take $(srcdir) into account.

2006-06-21  Akim Demaille  <akim@lrde.epita.fr>

	Add isola.

	* bib/lrde.bib (demaille.06.isola): New.

2006-06-21  Akim Demaille  <akim@lrde.epita.fr>

	Remove citeseer url.

	* bib/model-checking.bib (kwiatkowska.02.tacas): Remove url.

2006-06-21  Akim Demaille  <akim@lrde.epita.fr>

	Bind mostlyclean to clean.

	* make/share.mk (clean): Depends on mostlyclean.

2006-06-20  Akim Demaille  <akim@lrde.epita.fr>

	Fix accent.

	* bib/lrde.bib: Fix latin 1 accent.
	* Makefile: New.

2006-06-20  Akim Demaille  <akim@lrde.epita.fr>

	Bib renaming.

	* bib/model-checking.bib (ggfirst): Remove, part of lrde.bib.
	(reactive): Rename as...
	(alur.96.lics): this.
	(webapmc): Rename as...
	(apmc.www): this.

2006-06-20  Akim Demaille  <akim@lrde.epita.fr>

	Fix cross-refs.

	* bib/model-checking.bib (vmcai): Rename as...
	(herault.04.vmcai): this.
	(DBLP:conf/vmcai/2004): Rename as...
	(xxxref.04.vmcai): this to please bibtex (and alphabetical sorting).

2006-06-20  Akim Demaille  <akim@lrde.epita.fr>

	New bibs: sensor networks, and model checking.

	* bib/model-checking.bib: New.
	* bib/sensor-networks.bib: New.

2006-06-19  Akim Demaille  <akim@lrde.epita.fr>

	Fix kernighan.bib.

	* styles/myacronym.sty (ratfor): New.
	* bib/kernighan.bib: Add missing `,'.
	Reformat.

2006-06-19  Akim Demaille  <akim@lrde.epita.fr>

	Add kerighan.bib.

	* bib/kernighan.bib: New.

2006-06-19  Akim Demaille  <akim@lrde.epita.fr>

	Update texi2dvi.

	* bin/texi2dvi: From master.

2006-06-19  Akim Demaille  <akim@lrde.epita.fr>

	More acronyms.

	* styles/myacronym.sty (prism): New.

2006-06-16  Akim Demaille  <akim@lrde.epita.fr>

	PCTL in XRM.

	* styles/ldf/reactive-modules.ldf (XRM): Add PCTL features.

2006-06-15  Akim Demaille  <akim@lrde.epita.fr>

	More RM languages.

	* styles/mylistings.hva (Underline): New.
	* styles/ldf/reactive-modules.ldf ([M4] {Reactive Modules}): New.

2006-06-14  Akim Demaille  <akim@lrde.epita.fr>

	More XRM.

	* styles/ldf/reactive-modules.ldf: More keywords.

2006-06-14  Michaël Cadilhac  <michael.cadilhac@lrde.epita.fr>

	* styles/myacronym.sty: Add Vaucanson related acronyms.

2006-06-14  Akim Demaille  <akim@lrde.epita.fr>

	ctmcs are ctmcs.

	* styles/myacronym.sty (ctmc): Typo.

2006-06-14  Akim Demaille  <akim@lrde.epita.fr>

	More xrm.

	* styles/myacronym.sty (ctmc, xrm): New.
	* styles/ldf/reactive-modules.ldf: Fix missing `;'.
	* bin/update-share: Disable set -x at the end.

2006-06-13  Michaël Cadilhac  <michael.cadilhac@lrde.epita.fr>

	* styles/ldf/vaucanson.ldf: Update. Change for_each to for_all.

2006-06-13  Akim Demaille  <akim@lrde.epita.fr>

	More RM keywords.

	* styles/mylistings.sty: Define the style for keywords[2].
	* styles/ldf/reactive-modules.ldf: More keywords.
	* bin/update-share: Prompt the user to check in the host project.
	* make/share-am.mk (share-ci): New.

2006-06-13  Akim Demaille  <akim@lrde.epita.fr>

	More Reactive Modules.

	* styles/ldf/reactive-modules.ldf (reactivemodules): Rename as...
	(Reactive Modules): this.
	([Extended] Reactive Modules): New.

2006-06-13  Akim Demaille  <akim@lrde.epita.fr>

	Typo.

	* styles/mylistings.sty (\lstnewenvironment): takes two args.

2006-06-12  Akim Demaille  <akim@lrde.epita.fr>

	Add IEEEtran and rev.tex.

	* styles/IEEEtran.bst: New.
	* styles/IEEEtran.cls: New.
	* styles/mylistings.sty: Decode and use \latexofthepoor.
	Preliminary.
	* make/tex.mk (rev.tex, CLEANFILES): New.
	* README: Complete.

2006-06-12  Akim Demaille  <akim@lrde.epita.fr>

	Initialize CLEANFILES, fix handouts.

	* make/share-am.mk (CLEANFILES): New.
	* make/handout.mk: No longer change the PATH.
	Fix the location of beamer2handout.

2006-06-07  Akim Demaille  <akim@epita.fr>

	* bib/lrde.bib (denise.06.rt, lassaigne.06.qest): Fix the authors.

2006-06-07  Akim Demaille  <akim@epita.fr>

	* bib/lrde.bib (denise.06.rt, lassaigne.06.qest): New.

2006-06-05  Roland Levillain  <roland@lrde.epita.fr>

	Remove styles/GRASSnews.sty.

	* styles/GRASSnews.sty: Remove.
	* README: Update.

2006-06-05  Akim Demaille  <akim@lrde.epita.fr>

	Don't output submissions.

	* share/bin/make-bib.pl: Support --with-submitted.
	(&output): New.

2006-06-05  Akim Demaille  <akim@lrde.epita.fr>

	share should not check out lrde.bib.

	* bin/update-share, make/tex.mk: lrde.bib lives here.

2006-06-05  Akim Demaille  <akim@lrde.epita.fr>

	Add lrde.bst.

	* styles/lrde.bst: New.
	From lrde-publis.

2006-06-05  Akim Demaille  <akim@epita.fr>

	share/bib/lrde.bib becomes the master.
	2006-06-05  Didier Verna  <didier@lrde.epita.fr>

	* lrde.bib: (verna.06.ecoop): Accepted.

	2006-05-23  Akim Demaille  <akim@epita.fr>

	* lrde.bib (chekroun.06.iciar): Accepted.
	Add urllrde.

	2006-05-02  Didier Verna  <didier@lrde.epita.fr>

	* lrde.bib (verna.06.ecoop): Add (Submitted).

	2006-05-02  Didier Verna  <didier@lrde.epita.fr>

	* lrde.bib (verna.06.imecs): Add (accepted).

	2006-04-01  Thierry GERAUD  <theo@tegucigalpa.lrde.epita.fr>

	* darbon.05.phd.pdf: New entry.
	* contents.bib (chekroun.06.iciar): Add fake entry for
	make to work.
	Update.

	2006-01-23  Thierry GERAUD  <theo@tegucigalpa.lrde.epita.fr>

	* darbon.06.siam.pdf: Change format to pdf.
	* lrde.bib: Commit Jerome's changes.
	* lrde.txt: Likewise.

	2006-01-18  Jerome Darbon  <jerome@epita.fr>

	* lrde.bib (darbon.06.siam): add
	* lrde.bib (lesage.06.icpr): add (submission)

	2005-12-19  Akim Demaille  <akim@epita.fr>,
	    Daniela Becker  <daniela@lrde.epita.fr>

	* lrde.bib: Complete urllrdes.

	2005-12-16  Akim Demaille  <akim@epita.fr>

	* lrde.bib: Fix a couple of syntactic errors.
	(duflot.05.sttt): Remove.

	2005-12-15  Louis-Noel Pouchet  <louis-noel.pouchet@lrde.epita.fr>

	* lrde.bib (claveirole.05.ciaa): Add LNCS references.
	(lombardy.04.tcs): Add urllrde.

	2005-12-15  Akim Demaille  <akim@epita.fr>

	* lrde.bib (maes.03.dpcool): Add the abstract.

	2005-11-21  Akim Demaille  <akim@lrde.epita.fr>

	Fix rivf'06.

	* lrde.bib (demaille.06.rivf): Accepted.

	2005-11-21  Akim Demaille  <akim@epita.fr>

	* lrde.bib (darbon.XX.jmiv, darbon.XXb.jmiv): Update.
	(demaille.06.rivf): Update.

	2005-11-07  Roland Levillain  <roland@lrde.epita.fr>

	* lrde.bib (levillain.05.olenaposter): New entry.
	* lrde.tex: Regen.

	2005-11-07  Roland Levillain  <roland@lrde.epita.fr>

	* lrde.bib (levillain.05.tigerposter): New entry.

	2005-10-26  Akim Demaille  <akim@epita.fr>

	* lrde.bib: Adjust several url.
	Sort out the Carlier case.
	Sort out the SUD case.
	Remove incorrect fixmes.

	2005-10-25  Documentaliste  <doc@nostromo.lrde.epita.fr>

	* lrde.bib (bloch.03.ai): Change urllrde.

	2005-10-25  Reda Dehak  <reda@lrde.epita.fr>

	* lrde.bib: Update dehak.05.pami

	2005-10-25  Akim Demaille  <akim@epita.fr>,
	    Daniela Becker <daniela@lrde.epita.fr>

	* lrde.bib: Add the urls.

	2005-10-24  Akim Demaille  <akim@epita.fr>

	* lrde.bib (demaille.05.iticse): With urllrde.

	2005-10-24  Akim Demaille  <akim@epita.fr>

	* lrde.bib (demaille.06.rivf): New.

	2005-10-24  Akim Demaille  <akim@epita.fr>

	* lrde.bib (borghi.06.crossroads): New.

	2005-09-21  Thierry Geraud  <theo@lrde.epita.fr>

	* lrde.bib (geraud.06.ivc): New.

	2005-07-12  Akim Demaille  <akim@epita.fr>

	* lrde.bib (darbon.05.isvc, duflot.06.book): New.
	(laplante.0X.tocl): Rename as...
	(laplante.06.tocl): this.

	2005-05-31  Akim Demaille  <akim@epita.fr>

	* lrde.bib (lombardy.04.tcs): New.

	2005-05-26  Akim Demaille  <akim@epita.fr>

	* lrde.bib (claveirole.05.ciaa): New.

	2005-05-25  Akim Demaille  <akim@epita.fr>

	Support category = national for conferences.

	* lrde.bib (geraud.00.rfia, geraud.99.gretsi): Flag as national.

	2005-05-24  Akim Demaille  <akim@epita.fr>

	* lrde.bib (david.05.sud, gournet.05.sud, pouillard.05.sud):
	Fix.
	Reformatting.

	2005-05-23  Akim Demaille  <akim@epita.fr>

	* lrde.bib: Fix typos.

	2005-05-23  Sylvain Peyronnet  <peyronnet@lrde.epita.fr>

	* lrde.bib (guirado.05.pdmc): Update


	2005-05-23  Jerome Darbon  <jerome@epita.fr>

	* lrde.bib (darbon.04.tr): Update
	* lrde.bib (darbon.05.tr): Update

	2005-05-23  Akim Demaille  <akim@epita.fr>

	* lrde.bib (duret.01.ae): Fix the project.

2006-06-05  Roland Levillain  <roland@lrde.epita.fr>

	* styles/lrde-bulletin.sty: Fix the previous patch.

2006-06-05  Roland Levillain  <roland@lrde.epita.fr>

	Create the lrde-bulletin package from the GRASSnews package.

	* styles/GRASSnews.sty: Copy as...
	* styles/lrde-bulletin.sty: ...this.
	Adjust names.
	(makesubtitle, section, inputarticle, newfootnote, thefootnote)
	(urlnote, Href, legend, seminardate, Vauc, Tfers, Mkv, Oln): New
	commands (imported from L'air de rien 4.0 and 5.0).

2006-06-05  Akim Demaille  <akim@lrde.epita.fr>

	Start merging lrde-publis with share.

	* bin/svndiff: bin/make-bib.pl, bin/svnci: New.
	From lrde-publis/bin.
	* README: Update.

2006-06-05  Roland Levillain  <roland@lrde.epita.fr>

	Don't display null subvolume numbers in GRASSnews.

	* styles/GRASSnews.sty: Don't display the subvolume number in
	the complete volume number if it is null.

2006-06-05  Roland Levillain  <roland@lrde.epita.fr>

	Add a subvolume command to the GRASSnews package.

	* styles/GRASSnews.sty (subvolume): New command.
	Use it to define a complete volume number (following the
	volume.subvolume scheme), used in headers.

2006-06-05  Roland Levillain  <roland@lrde.epita.fr>

	Resolve GRASSnews.sty's dependency on the array package.

	* styles/GRASSnews.sty: Require the array package.

2006-05-31  Roland Levillain  <roland@lrde.epita.fr>

	Clean up handout support.

	* make/tex.mk (%-handout-4.pdf): Remove rule.
	* make/handout.mk (clean, handout-clean): Likewise.
	(CLEANFILES): Append *-handout-4.pdf.
	* make/share.mk: Remove $(CLEANFILES) when invoked.
	* README: Update.

2006-05-30  Akim Demaille  <akim@lrde.epita.fr>

	Update texi2dvi.

	* bin/texi2dvi: Update from master.

2006-05-30  Akim Demaille  <akim@lrde.epita.fr>

	Update facture.cls.

	* styles/facture.cls: Update the main phone number.
	Use the same font for "facture" and its reference.

2006-05-30  Akim Demaille  <akim@lrde.epita.fr>

	PHONY targets.

	* styles/facture.cls: Provide a more informative error message.
	* make/share-am.mk, make/tex.mk, make/share.mk: Declare the phony
	targets.

2006-05-24  Akim Demaille  <akim@lrde.epita.fr>

	Add lrde.bib.

	* bib/lrde.bib: New.
	Add it, there are too many problems with this approach.
	Currently, the original is still in another repository.

2006-05-24  Akim Demaille  <akim@lrde.epita.fr>

	Include lrde.bib in the tex dependencies.

	* make/tex.mk (share_tex_dependencies): Include lrde.bib.
	This ensures that it is checked out *before* we try to
	use it (something that using "all" only is not enforced).

2006-05-23  Akim Demaille  <akim@lrde.epita.fr>

	More update-share fixes.

	* bin/update-share: Protect the cd using a sub-shell.
	* make/tex.mk (lrde.bib): Use the relative path to update-share.

2006-05-23  Akim Demaille  <akim@lrde.epita.fr>

	Fix update-share again.

	* bin/update-share, make/tex.mk: Fix them so that update-share
	is always invoked from the host directory.

2006-05-23  Robert Bigaignon  <robert.bigaignon@lrde.epita.fr>

	Fix update-share.

	* bin/update-share: Fix change of directory.

2006-05-23  Akim Demaille  <akim@lrde.epita.fr>

	share_share -> share.

	* make/tex.mk: Fix stupid typo.

2006-05-23  Akim Demaille  <akim@lrde.epita.fr>

	Fix update-share interface.

	* bin/update-share: When --lrde.bib is passed on the command
	line, don't also process it as a directory name.

2006-05-23  Akim Demaille  <akim@lrde.epita.fr>

	Compile LaTeX to info/txt.

	* bin/texi2dvi (run_to_html): Rename as...
	(run_hevea): this.
	Accept $1: the destination language.
	Extend the getarg loop to accept --info and --text (currently
	hidden).
	* make/tex.mk (.txt, .info): New targets from tex and ltx.

2006-05-23  Roland Levillain  <roland@lrde.epita.fr>

	* bin/beamer-handout: Remove.

2006-05-23  Akim Demaille  <akim@lrde.epita.fr>

	/!\ Renaming directory variables.

	This change might require adjustments in your Makefiles.
	* make/share-am.mk, make/tex.mk, make/share.mk
	(bib_dire, style_dir, make_dir): Rename as...
	(share_bib_dire, share_style_dir, share_make_dir): Rename as...

	* bin/beamer2handout: Diagnose a missing pdfnup.

2006-05-22  Roland Levillain  <roland@lrde.epita.fr>

	Add beamer2handout.

	* bin/beamer2handout: New (imported script).
	* make/handout.mk (%-handout-4.pdf),
	* make/tex.mk (%-handout-4.pdf): Use beamer2handout instead of
	beamer-handout.
	* README: Mention beamer2handout.

2006-05-19  Akim Demaille  <akim@lrde.epita.fr>

	Fix texi.sty.

	* styles/texi.sty: Don't reproduce texinfo.tex's code, using LaTeX
	features suffices.
	* make/tex.mk (share_tex_dependencies): New.

2006-05-19  Akim Demaille  <akim@epita.fr>

	* make/share-am.mk: New, contains most of the former contents
	of...
	* make/share.mk: this file.
	Now includes the previous one and defines clean and mostlyclean.
	* make/tex.mk: Adjust.
	* README: Adjust.

2006-05-19  Akim Demaille  <akim@epita.fr>

	* make/tex.mk (mostlyclean-local): New alias for mostlyclean to
	hook Automake's mostlyclean target.

2006-05-19  Akim Demaille  <akim@epita.fr>

	* styles/mybabel.hva: Load the real babel with the right
	language.
	* styles/mybabel.sty: Don't load it.
	* bin/update-share: Put the cd in a sub shell.
	* make/tex.mk, make/share.mk: Fix the invocation of update-share.

2006-05-16  Akim Demaille  <akim@epita.fr>

	* styles/hevea.sty: New.
	* styles/texi.sty: Make it robust to \ttsl not existing.

2006-05-16  Akim Demaille  <akim@lrde.epita.fr>

	* bin/texi2dvi: Update.

2006-05-16  Akim Demaille  <akim@lrde.epita.fr>

	* bib/transformers.bib (ekman.04): Fix title.

2006-05-13  Akim Demaille  <akim@lrde.epita.fr>

	* style/curve.cls: new.

2006-05-12  Akim Demaille  <akim@lrde.epita.fr>

	* styles/latex8.bst: New.

2006-05-11  Akim Demaille  <akim@lrde.epita.fr>

	* styles/latex8.sty: New.
	* make/tex.mk (all): Hook lrde.bib to it.
	It should no longer be required to mention it.
	* README: Update.

2006-05-09  Akim Demaille  <akim@lrde.epita.fr>

	* bin/update-share: Support --lrde.bib.
	* make/tex.mk: Provide a means to generate lrde.bib if missing.
	* make/tex.mk, make/share.mk (all): New.
	To make sure our targets don't get promoted as default target (in
	Make the default target is the first to appear in the list, it
	does not default to "all").

2006-05-05  Akim Demaille  <akim@lrde.epita.fr>

	* styles/GRASSnews.sty (\volumetitle): New.
	Use it.

2006-05-05  Akim Demaille  <akim@lrde.epita.fr>

	* styles/misc.sty: Add it for real.

2006-05-05  Akim Demaille  <akim@lrde.epita.fr>

	* styles/misc.sty, styles/misc.hva: Fix the inclusion of xspace.

2006-05-05  Akim Demaille  <akim@lrde.epita.fr>

	* styles/mylistings.hva (darkorange, darkgreen, default style):
	Move...
	* styles/mylistings.sty: here.
	* styles/mybabel.hva: New.
	* styles/mybabel.sty: Load it.
	* styles/bilan.hva: Loadf inputenc, mybabel, myhyperref, misc.
	* styles/bilan.sty: Load it.
	* styles/misc.sty: Load the following file, since it now contains
	most of the definitions.
	* src/misc.hva: new.
	More definitions.

2006-04-30  Akim Demaille  <akim@lrde.epita.fr>

	* styles/ldf/stl.ldf, styles/ldf/vaucanson.ldf: New.

2006-04-28  Akim Demaille  <akim@lrde.epita.fr>

	* styles/vaucanson.sty: New, symlink to vaucanson-g.sty.

2006-04-13  Roland Levillain  <roland@lrde.epita.fr>

	Fix bin/pdfbook.

	* bin/pdfbook: Work around Adobe Reader's deficiencies w.r.t to
	its standard input/output.

2006-04-07  Akim Demaille  <akim@lrde.epita.fr>

	* styles/GRASSnews.sty (\titlepage): Use a tabular to typeset the
	logo and the title.

2006-04-06  Akim Demaille  <akim@lrde.epita.fr>

	* styles/GRASSnews.sty: Include the number in the title.
	Squeese some vertical spaces after the title.
	Update version number.

2006-04-04  Akim Demaille  <akim@lrde.epita.fr>

	* styles/GRASSnews.sty (\email): Remove, defined by texi.sty.
	Comment out a large batch of TeX code that duplicates the features
	of texi.sty, rather, require the latter.  Note that some bits of
	the commented out section seem to be a better implementation of
	texi.sty, we might want to use them in the future.
	(\acronym): Disable, conflicts with acronym.sty.

2006-04-03  Akim Demaille  <akim@lrde.epita.fr>

	* share/bib/compilation.bib (havm, helloworld, historycomputing):
	Rename as...
	(havm.www, helloworld.www, historycomputing.www): this.

2006-03-28  Akim Demaille  <akim@lrde.epita.fr>

	* bib/compilation.bib (tanenbaum.04.linux, mohr.04.370): New.

2006-03-17  Akim Demaille  <akim@lrde.epita.fr>

	* bib/compilation.bib (guy.71.ladybird, time.83.computer)
	(watchmen.www, apple-history.www): New.

2006-03-16  Akim Demaille  <akim@lrde.epita.fr>

	* bib/compilation.bib (huggins.06.hopper, maccarthy.www): New.

2006-03-15  Akim Demaille  <akim@lrde.epita.fr>

	* styles/asn1.ldf: New.
	* styles/mylistings.hva: Use it.
	(\warn): New.
	Should provide a beamer-less version.

2006-03-08  Akim Demaille  <akim@lrde.epita.fr>

	* styles/mylistings.hva (\warn): New, for the sake of the ttcolor
	style.
	* styles/ldf/tiger.ldf: primitive is also an added keyword.

2006-03-08  Akim Demaille  <akim@lrde.epita.fr>

	* bin/beamer-handout: Catch errors.
	Don't pass -expand to acroread, as sometimes it triggers a weird
	behavior.

2006-03-08  Akim Demaille  <akim@lrde.epita.fr>

	* styles/GRASSnews.sty: Fix the header :(

2006-03-07  Akim Demaille  <akim@lrde.epita.fr>

	* bib/compilation.bib (automake): Rename as...
	(automake.www): this.
	(autoconf.www, duret-lutz.06.autotools): New.

2006-03-06  Akim Demaille  <akim@lrde.epita.fr>

	* styles/mybabel.sty: Require 2004/11/20 to avoid `:' issues.
	* styles/myhyperref.sty: Similarly, require 2003/11/30.
	* styles/bilan.sty: We no longer use varioref.

2006-03-06  Roland Levillain  <roland@lrde.epita.fr>

	* bin/pdfbook: Remove options confusing Adobe Reader's output.

2006-03-06  Akim Demaille  <akim@lrde.epita.fr>

	* styles/GRASSnews.sty: Provide odd/even footer/header.
	* bin/update-share: Set LC_ALL globally.
	Fix the error reporting.

2006-03-06  Akim Demaille  <akim@lrde.epita.fr>

	* styles/ldf/lex.ldf: New.
	* styles/ldf/yacc.ldf (Bison): Handle @s.
	* styles/mylistings.hva: Use it.
	(darkorange, darkgreen): New colors.
	(ttcolor): Use them.

2006-03-03  Akim Demaille  <akim@lrde.epita.fr>

	* styles/facture.cls: New.
	Modified to support the \kind command.
	* styles/bilan.sty (\maketitle): Display the author.

2006-02-28  Akim Demaille  <akim@lrde.epita.fr>

	* bib/compilation.bib (smith.06, spacewar.www): New.

2006-02-28  Didier Verna  <didier@lrde.epita.fr>

	* styles/GRASSnews.sty: Use 'Numero' instead of 'Version'.

2006-02-26  Akim  <akim@sulaco.lrde.epita.fr>

	* bib/compilation.bib (owen.03.wwww, wbg.06.www, zuse.04)
	(lohr.02.goto): New.

2006-02-23  Akim Demaille <akim@lrde.epita.fr>

	* styles/supertabular.hva, styles/multicol.hva: New.

2006-02-07  Akim Demaille  <akim@lrde.epita.fr>

	Make myhyperref more robust.

	* styles/ldf/reactive-modules.ldf: New.
	* styles/mylistings.hva: Adjust.
	* styles/myhyperref.sty: Use \def to define the autorefnames,
	so that we are robust to defined/undefined autorefnames.

2006-01-27  Akim Demaille  <akim@lrde.epita.fr>

	HeVeA adjustments.

	* styles/texi.sty: Require hevea.
	* styles/bilan.hva: Don't include mylistings: the sty file doesn't.

2006-01-27  Akim Demaille  <akim@lrde.epita.fr>

	More HeVeA support.

	* styles/mylistings.hva: New.
	* styles/mylistings.sty: Use it.
	* styles/texi.hva: New.
	* styles/texi.sty: Use it.
	* styles/bilan.hva: New.
	* styles/ldf/tiger.ldf: Define the dialect first, to avoid
	warnings.
	* styles/myhyperref.hva: New.
	* bin/texi2dvi (run_to_html): Pass the original directory as a -I.
	* make/tex.mk: Provide tex -> html rules.

2006-01-26  Akim Demaille  <akim@lrde.epita.fr>

	texi: enable hevea use.

	* styles/texi.sty: Be `\input'able for hevea.
	* bin/texi2dvi: Upgrade.

2006-01-24  Akim Demaille  <akim@lrde.epita.fr>

	figurename.

	* styles/myhyperref.sty: Add figure autorefname.

2006-01-24  Akim Demaille  <akim@lrde.epita.fr>

	Fix bilan.sty.

	* styles/bilan.sty: Do not include varioref after hyperref.
	(\maketitle): Make a bigger title.
	* make/tex.mk: Also support the *.ltx extension.
	* make/share.mk (share_dir): Be a default value.

2006-01-23  Akim Demaille  <akim@lrde.epita.fr>

	Adjust bilan.sty.

	* styles/bilan.sty (\lrde): Is the acronym too.
	* styles/myhyperref.sty (appendix): New autoref name.

2006-01-23  Akim Demaille  <akim@lrde.epita.fr>

	Prepare the `bilan LRDE'.

	* styles/mybabel.sty: Warn if hyperref is loaded after.
	* styles/bilan.sty: New.
	* styles/myhyperref.sty: More translations.
	* make/tex.mk (TEXI2PDF_FLAGS): New.
	Use it.

2006-01-20  Akim Demaille  <akim@lrde.epita.fr>

	Prepare l'air de rien 2.

	* styles/GRASSnews.sty: Bulletin -> aleastriel.
	Leave no space between the subtitle and the author name.

2006-01-20  Didier Verna  <didier@lrde.epita.fr>

	* styles/misc.sty: New. Various useful macros.

2006-01-19  Roland Levillain  <roland@lrde.epita.fr>

	Add references compiled by Clement Vasseur.

	* bin/list2bib: New.
	* bib/compilation.clement.bib: New (generated).

2006-01-18  Akim Demaille  <akim@lrde.epita.fr>

	Complete/normalize compilation.bib.

	* bib/compilation.bib: Complete and normalize the keys.

2006-01-18  Akim Demaille  <akim@lrde.epita.fr>

	Add prooftree, complete mylisting & compilation.bib.

	* styles/mylistings.sty: Use the unused languages.
	* styles/prooftree.sty: New.
	* bib/compilation.bib (sebesta.02, wikipedia): New.
	* README: Complete.

2006-01-18  Akim Demaille  <akim@lrde.epita.fr>

	Add texi.sty.

	* styles/texi.sty: New.
	* README: Update.

2006-01-13  Akim Demaille  <akim@lrde.epita.fr>

	Add menhir.www.

	* bib/compilation.bib (menhir.www): New.
	(yaxx): Fix and rename as...
	(yaxx.www): this.

2006-01-13  Akim Demaille  <akim@epita.fr>

	* styles/ldf/yacc.ldf: More symbols.

2006-01-13  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (leung.96.prop): New entry.

2006-01-10  Akim Demaille  <akim@lrde.epita.fr>

	Create codegen.bib.

	* bib/codegen.bib: New.
	* bib/compilation.bib (fraser.91, fraser92engineering): Remove.
	(mono): Rename as...
	(mono.www): this.
	(parr.95.spe): New.

2006-01-10  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (mono): New.

2006-01-10  Akim Demaille  <akim@lrde.epita.fr>

	Fixes.

	* bib/compilation.bib: Do it.

2006-01-10  Akim Demaille  <akim@lrde.epita.fr>

	Add waite.06.sigcse.

	* bib/compilation.bib: Do it.

2006-01-10  Roland Levillain  <roland@lrde.epita.fr>

	* bib/compilation.bib (aho.89.acmtpls, cattell.80.acmtpls)
	(fraser.91): New.

2006-01-10  Akim Demaille  <akim@lrde.epita.fr>

	Complete yacc.ldf.

	* styles/ldf/yacc.ldf: Add some symbols.

2006-01-10  Akim Demaille  <akim@lrde.epita.fr>

	vollmar.06.sigcse.

	* bib/compilation.bib (vollmar.06.sigcse): New.

2006-01-10  Akim Demaille  <akim@lrde.epita.fr>

	listings: No color with box style.

	* styles/mylistings.sty: Use sffamily instead.

2006-01-10  Roland Levillain  <roland@lrde.epita.fr>

	* bin/update-share: Don't rely on the current locale when invoking
	`svn info'.

2006-01-09  Roland Levillain  <roland@lrde.epita.fr>

	Add weatherley.02 in compilation.bib.

	* bib/compilation.bib (weatherley.02): New.

2006-01-09  Akim Demaille  <akim@lrde.epita.fr>

	Update sig-alternate and compilation.bib.

	* styles/sig-alternate.cls: Version 1.8.
	* bib/compilation.bib (matz03, aycock.1995.mbl, Debray2002)
	(Baldwin2003): Rename as...
	(matz.03, aycock.95.mbl, debray.02.sigcse, baldwin.03.sigcse):
	these.

2006-01-06  Akim Demaille  <akim@lrde.epita.fr>

	Add Bison extinct.

	*  share/bib/compilation.bib (Aycock2003): Rename as...
	(aycock.03.sigplan): This.
	(aycock.02.crossroads): New.

2006-01-06  Akim Demaille  <akim@lrde.epita.fr>

	Don't require babel.

	* styles/mybabel.sty: Check that sig-alternate was not loaded.
	* styles/myhyperref.sty (mybabel): Don't require it.
	Change the definition of the autorefname to work whether
	babel is used or not.

2006-01-05  Akim Demaille  <akim@lrde.epita.fr>

	cfg/cfl.

	* styles/myacronym.sty: Define them.

2006-01-04  Akim Demaille  <akim@lrde.epita.fr>

	Add compilation.bib & sig-alternate.cls.

	* styles/sig-alternate.cls: New.
	* bib/compilation.bib: New.

2006-01-03  Akim Demaille  <akim@lrde.epita.fr>

	Used sed instead of grep -v.

	* bin/update-share: Do that.

2006-01-03  Akim Demaille  <akim@lrde.epita.fr>

	update texi2dvi.

	* bin/texi2dvi: Update.
	* figs/lrde-big.png: New.
	* make/tex.mk: Use bearmer-handsout.
	* make/share.mk (clean): Bind mostly-clean.

2005-12-19  Akim Demaille  <akim@lrde.epita.fr>

	Update texi2dvi.

	* bin/texi2dvi: From master.

2005-12-15  Akim Demaille  <akim@lrde.epita.fr>

	Add llncs.cls.

	* styles/llncs.cls: New.

2005-12-15  Akim Demaille  <akim@lrde.epita.fr>

	Add projects.bib.

	* bib/projects.bib: New.

2005-12-15  Akim Demaille  <akim@lrde.epita.fr>

	Replace c++.bib with gp.bib from burrus.03.mpool.

	* bib/gp.bib: New.
	* bib/c++.bib: Remove.

2005-12-13  Akim Demaille  <akim@lrde.epita.fr>

	Add garcia.03.oopsla.

	* bib/c++.bib: Do it.

2005-12-13  Akim Demaille  <akim@lrde.epita.fr>

	More listing styles.

	* styles/mylistings.sty (box): New style.
	(HIR): Move to...
	* styles/ldf/hir.ldf: this new file.
	* styles/myacronym.sty (fsml): Use textsc for at&t..
	* bib/vaucanson.bib: Use \acf{fsml}.
	* make/tex.mk (clean): Bind to mostly-clean.

2005-12-12  Akim Demaille  <akim@lrde.epita.fr>

	Various fixes.

	* styles/mycxx.sty: Make them usable in PDF strings.
	* styles/myacronym.sty (lgpl, liafa, enst): New.
	* styles/myhyperref.sty: Allow links to be broken.
	* make/tex.mk: Complete dependencies.

2005-12-12  Akim Demaille  <akim@lrde.epita.fr>

	gp/scoop.

	* styles/myacronym.sty (gp, scoop): New.

2005-12-12  Akim Demaille  <akim@lrde.epita.fr>

	mybabel, vaucanson.bib.

	* styles/mybabel.sty: New.
	This is used to make sure we can rely on babel being used.
	* styles/myhyperref.sty: Use it.
	* styles/myacronym.sty: Use it.
	(fsm, fsml, swig): New.
	* bib/vaucanson.bib: New.

2005-12-12  Akim Demaille  <akim@lrde.epita.fr>

	Add pdfbook.

	* bin/pdfbook: New.

2005-12-07  Akim Demaille  <akim@lrde.epita.fr>

	GRASSnews changes.

	* styles/GRASSnews.sty: Vol -> Ver.
	Point to the bulletin's web page.

2005-12-06  Akim Demaille  <akim@lrde.epita.fr>

	Don't impose the English language.

	* styles/myhyperref.sty: .

2005-12-06  Akim Demaille  <akim@lrde.epita.fr>

	GRASSnews: Catch empty lines.

	* styles/GRASSnews.sty: Catch bad empty lines.

2005-12-06  Akim Demaille  <akim@lrde.epita.fr>

	Be picky.

	* bin/update-share: Be picky.

2005-12-06  Olivier Ricou <ricou@lrde.epita.fr>

	ajout de par devant l'auteur

	* styles/GRASSnews.sty: ajout de par devant l'auteur

2005-12-06  Akim Demaille  <akim@lrde.epita.fr>

	More ldf files.

	* styles/ldf/yacc.ldf: New.
	* styles/ldf/mips.ldf: New.
	* styles/mylistings.sty: Extracted from here.
	(tiger): Remove, defined elsewhere.

2005-12-06  Akim Demaille  <akim@lrde.epita.fr>

	More weird LaTeX style files.

	* styles/algorithmic.sty: New.
	* styles/Vaucanson-G.tex: New.
	* styles/vaucanson-g.sty: New.
	* styles/algorithm.sty: New.
	* make/tex.mk (%.dvi: %.tex): New.
	* README: Complete a bit.

2005-12-05  Akim Demaille  <akim@lrde.epita.fr>

	Acronyms for APMC.

	* styles/myacronym.sty (apmc, csl, dtmc, fpras, ltl):
	(pts, rm): New.

2005-12-01  Akim Demaille  <akim@lrde.epita.fr>

	Lst styles, abbrev.

	* styles/mylistings.sty (sdf, tiger): Move to...
	* styles/ldf/sdf.ldf: here...
	* styles/ldf/tiger.ldf: and here.
	* styles/myacronym.sty (gpl): New.

2005-12-01  Akim Demaille  <akim@lrde.epita.fr>

	More bib, more acronyms.

	* styles/myacronym.sty (dsel): New.
	* bib/transformers.bib (knuth.65.ic): New.

2005-11-30  Akim Demaille  <akim@lrde.epita.fr>

	Volume -> Version.

	* styles/GRASSnews.sty: Volume -> Version.

2005-11-30  Akim Demaille  <akim@lrde.epita.fr>

	Add GRASSnews.sty.

	* styles/myhyperref.sty: Use hypersetup.
	* styles/GRASSnews.sty: New.

2005-11-29  Akim Demaille  <akim@lrde.epita.fr>

	Better use of sortunder.

	* styles/myhyperref.sty (subsubection): Handle it.
	* bib/strategoxt.bib, bib/transformers.bib, bib/cwi.bib:
	Better use of sortunder.

2005-11-29  Akim Demaille  <akim@lrde.epita.fr>

	Name conventions.

	* bib/transformers.bib (uuag-url): Rename as...
	(uuag.www): this.

2005-11-28  Akim Demaille  <akim@lrde.epita.fr>

	More acronyms.

	* styles/myacronym.sty (cpp, asf+sdf): New.

2005-11-24  Akim Demaille  <akim@lrde.epita.fr>

	Add cwi.bib.

	* bib/transformers.bib: Move some entries to...
	* bib/cwi.bib: here.

2005-11-24  Akim Demaille  <akim@lrde.epita.fr>

	Add cwi.bib.

	* bib/transformers.bib (brand.2003.entcs): Move to...
	* bib/cwi.bib (brand.03.entcs): here.
	* make/tex.mk (clean, mostly-clean): New.
	* make/share.mk: Idem.

2005-11-24  Akim Demaille  <akim@lrde.epita.fr>

	Create share/make.

	* make: New.
	* make/tex.mk: New.
	* make/handout.mk: New.
	* make/share.mk: New.

2005-11-23  Akim Demaille  <akim@lrde.epita.fr>

	add beamer-handout.

	* bin/update-share: Let lrde.bib be writable when needed.
	* bin/beamer-handout: New.
	* bin/psbbox: New.

2005-11-21  Akim Demaille  <akim@lrde.epita.fr>

	Compatibility bw hyperref and entcs.

	* styles/mycxx.sty: New.
	* styles/transformers.sty: Adjust.
	* styles/myhyperref.sty: Beware of entcs.cls.
	* styles/myacronym.sty (EPITA): New.
	* bib/transformers.bib: Naming convention change.

2005-11-21  Akim Demaille  <akim@lrde.epita.fr>

	* styles/bibunits.sty: New.
	* bin/texi2dvi: Update.

2005-11-21  Akim Demaille  <akim@lrde.epita.fr>

	Now lrde.bib is always up to date.

	* bin/update-share: Checkout lrde.bib.
	* bib: Adjust.
	* bib/lrde.bib: Remove.

2005-11-18  Akim Demaille  <akim@lrde.epita.fr>

	More bibs.

	* bib/ag.bib: New.
	* bib/c++.bib: New.
	* bib/pp.bib: New.

2005-11-18  Akim Demaille  <akim@lrde.epita.fr>

	* styles/entcs.bst: New.
	* styles/mycomment.sty: New.

2005-11-18  Akim Demaille  <akim@lrde.epita.fr>

	Fixes.

	* styles/myhyperref.sty: Fix.
	* styles/myacronym.sty: Fix.
	* bib/strategoxt.bib: No anonymous entries.

2005-11-18  Akim Demaille  <akim@lrde.epita.fr>

	* styles/myhyperref.sty (\defautorefname): New.
	From Michael Cadilhac & Didier Verna.
	Use it.

2005-11-18  Akim Demaille  <akim@lrde.epita.fr>

	Fix inclusion of hyperref.

	* styles/transformers.sty: Include myhyperref last.
	* styles/myhyperref.sty: Define the subsection autorefname.
	* bib/lrde.bib: Fix again.

2005-11-17  Akim Demaille  <akim@lrde.epita.fr>

	* bib/lrde.bib: Fix link.

2005-11-17  Akim Demaille  <akim@lrde.epita.fr>


	* bin/update-share: Trace.
	* bib/lrde.bib: New.

2005-11-17  Akim Demaille  <akim@lrde.epita.fr>

	* styles/prentcsmacro.sty: New.

2005-11-17  Akim Demaille  <akim@lrde.epita.fr>

	More shared items.

	* styles/fixme.sty: New.
	* styles/myhyperref.sty: Depend upon the language.
	* styles/entcs.cls: New.
	* vcs: New.
	* README: New.

2005-11-17  Akim Demaille  <akim@epita.fr>

	* README: New.


==> share/bin/beamer2handout <==
#!/bin/bash
# beamer2handout is just a small convenient interface to pdfnup
# (http://www2.warwick.ac.uk/fac/sci/statistics/staff/academic/firth/software/pdfjam/)
#
# beamer2handout creates 4up or 6up a4-sized pdf docs of your
# input pdf (intented for and tested with latex-beamer docs)
# $Id: beamer2handout 604 2005-04-27 11:00:56Z adam $
# by Arthur van dam, useful hints by David Firth and Eelco Dolstra.

# Customize this to your own needs:
pdfnup="pdfnup";
addArgs="";

if ! ($pdfnup --help) >/dev/null 2>&1; then
  echo >&2 "$0: pdfnup not found.  On Debian or with the MacPorts, install pdfjam."
  exit 1
fi

usagetext=\
"Usage:
  $ beamer2handout (input.pdf) [(2up|4up|6up) [output.pdf]]"

helptext=\
"beamer2handout converts a (latex-beamer) pdf file to A4-sized handouts.
One can choose for either four (default) or six slides on one page.
$usagetext"

if test -n "${1}"; then
	case "${1}" in
		*".pdf");;
		"--help") echo "$helptext";
			  exit 0;;
		*) echo "beamer2handout: first argument must be input pdf filename.";
		   echo "$usagetext";
		   exit 1;;
	esac
	inFile=${1};
else
	echo "beamer2handout: Missing arguments";
    echo "$usagetext";
	exit 1;
fi
if test -n "${2}"; then
	case "${2}" in
		"2up") nup="1x2"; landscape="--no-landscape";;
		"4up") nup="2x2"; landscape="--landscape";;
		"6up") nup="2x3"; landscape="--no-landscape";;
		*) nup="2x2"; landscape="--landscape";
		   echo "beamer2handout warning: ignoring invalid 2nd argument '${2}'.
			 Defaulting to 2x2.";;
	esac
else
	nup="2x2"; landscape="--landscape";
fi
if test -n "${3}"; then
	case "${3}" in
		*".pdf") addArgs="$addArgs --outfile ${3}";;
		*) echo "beamer2handout: Third argument (when used) should be output pdf filename.";
		   echo "$usagetext";
		   exit 1;;
	esac
fi

# Use array instead of string for nupCmd, to allow argvalues with spaces.
nupCmd=\
($pdfnup $inFile --paper a4paper --nup $nup $landscape \
--noautoscale false --scale 0.95 --delta "3mm 3mm" --frame true \
$addArgs);

# Now run it!
echo "beamer2handout: calling pdfnup:
${nupCmd[@]}";

"${nupCmd[@]}";


==> share/bin/bibneat <==
#! /bin/bash
# bibneat - Call a number of tools in order to clean a bib file.

# Name of the program, and a function to report problems.
me=$(basename $0)
warn ()
{
  echo "$me:" "$@" >&2
}

# Tmp dir
tmpdir=${TMPDIR:-/tmp}/bneat$$
debug=:
# By default, keep the comments
kill=false

# The version/usage strings
version="bibneat 0.1"

usage="\
Usage: $me [OPTIONS] FILES
Each BibTeX FILE is backed up, and various reformating are performed.

Options:
 -h, --help        display this help and exit
 -v, --version     display version information and exit
 -k, --kill        kill comments in the Bib source
 -q, --quiet       don't print informational messages"

help="Try \`$me --help' for more information."

# Parse command line arguments.
option_without_arguments='vhsqkD'

# Push a token among the arguments that will be used to notice when
# we ended options/arguments parsing.
arg_sep="$$--$$"
set dummy "${1+"$@"}" "$arg_sep"
shift
while test "x$1" != "x$arg_sep"; do

  # Handle --option=value by splitting apart and putting back on argv.
  case "$1" in
    --*=*)
      opt=`echo "$1" | sed -e 's/=.*//'`
      val=`echo "$1" | sed -e 's/[^=]*=//'`
      shift
      set dummy "$opt" "$val" "${1+"$@"}"
      shift
      ;;

    -[$option_without_arguments]?*)
      # Prefix $1 with x to avoid running `echo -na' for instance.
      opt=`echo "x$1" | sed -e 's/x-\(.\).*/-\1/'`
      rest=`echo "x$1" | sed -e 's/x-.\(.*\)/-\1/'`
      shift
      set dummy "$opt" "$rest" "${1+"$@"}"
      shift
      ;;

    # This case needs to be protected so that the case `-??*' does
    # not split long options without arguments
    --*)
      ;;

    # This is an option with argument.  Split apart and put back on argv.
    -??*)
      opt=`echo "x$1" | sed -e 's/x-\(.\).*/-\1/'`
      arg=`echo "x$1" | sed -e 's/x-.\(.*\)/\1/'`
      shift
      set dummy "$opt" "$arg" "${1+"$@"}"
      shift
      ;;
  esac

  # Now, handle the options.  $1 is the option *only*.  If it has an
  # argument, it is now necessarily in $2 etc.  Remember to shift
  # when fetching an argument.
  case "$1" in
    -v | --v*) echo "$version"; exit 0;;
    -h | --h*) echo "$usage"; exit 0;;
    -q | -s | --s* | --q*) verbose=:;;
    -k | --k* ) kill=:;;
    # Delay debugging so that options parsing does not appear
    -D | --debug)  debug=echo ;;

    --) # What remains are not options.
      shift
      while test "x$1" != "x$arg_sep"; do
        set dummy "${1+"$@"}" "$1"
        shift
	shift
      done
      break;;

    -*)
      echo "$program: Unknown or ambiguous option \`$1'." >&2
      echo "$program: Try \`--help' for more information." >&2
      exit 1;;
    *) set dummy "${1+"$@"}" "$1"
       shift
       ;;
   esac
   shift
done
# Pop the token
shift


if test -n "`$debug true`"; then
  # Set -x now if debugging
  set -x
else
  # Temp dir.  Get ready not to leave junk (if not debugging)
  trap "/bin/rm -rf $tmpdir" 0 1 2 3 13 15
fi

if (bibtool </dev/null) >/dev/null 2>&1; then :; else
  echo "$0: bibtool is not installed" 1>&2
  (exit 1); exit 1
fi

mkdir $tmpdir

# Clean the bib file $1, and save the result in $2.
# $1 and $2 can safely be the same path.
bib_file_clean ()
{
  tmp=$tmpdir/$(basename $2)
  (
    # Get the heading comments of the file, since bibtool looses all
    # comments.  (The convoluted sed script remove empty lines before
    # the first @-line.  this is because bibtool already adds one
    # empty line at the top of the file.)
    $kill || sed -n '/^[ ]*@/{x;1!P;Q};/./!H;/./{x;1!p};' "$1"
    # bibtool has this bad habit of leaving empty fields.
    # Option -O is documented to do this, but is refused by the executable.
    # Beware that grep may exit 1
    bibtool -s "$1" | (egrep -v '\{\},?$'; true) |
      sed "/month/{s/{[jJ]anuary}/jan/;
                   s/{[jJ]anvier}/jan/;
                   s/{[jJ]an\.\?}/jan/;
                   s/{[fF]ebruary}/feb/;
                   s/{[fF]eb\.\?}/feb/;
                   s/{[fF].*vrier}/feb/;
                   s/{[fF].*v\.\?}/feb/;
                   s/{[mM]arch}/mar/;
                   s/{[mM]ars}/mar/;
                   s/{[mM]ar\.\?}/mar/;
                   s/{[aA][pv]ril}/apr/;
                   s/{[aA][pv]r\.\?}/apr/;
                   s/{[mM]a[yi]}/may/;
                   s/{[jJ]une}/jun/;
                   s/{[jJ]un\.\?}/jun/;
                   s/{[jJ]uin}/jun/;
                   s/{[jJ]uly}/jul/;
                   s/{[jJ]u[il]\.\?}/jun/;
                   s/{[jJ]uil.*}/jul/;
                   s/{[aA]ugust}/aug/;
                   s/{[aA]ug\.\?}/aug/;
                   s/{[aA].*ut}/aug/;
                   s/{[sS]eptember}/sep/;
                   s/{[sS]eptembre}/sep/;
                   s/{[sS]ept\?\.\?}/sep/;
                   s/{[oO]ctober}/oct/;
                   s/{[oO]ctobre}/oct/;
                   s/{[oO]ct\.\?}/oct/;
                   s/{[nN]ovember}/nov/;
                   s/{[nN]ovembre}/nov/;
                   s/{[nN]ov\.\?}/nov/;
                   s/{[dD]ecember}/dec/;
                   s/{[dD]ecembre}/dec/;
                   s/{[dD]ec\.\?}/dec/; }"
    # Get the heading trailing comments of the file.
    $kill || sed 1,`sed -n '/^}/=' "$1" | tail -n 1`d "$1"
  ) > $tmp

  mv $tmp $2
}

set -e

for src in "$@"
do
  # We don't trust ourselves
  cp -bf --backup=numbered "$src" "$src"

  bib_file_clean "$src" "$src"

  warn "$src: cleaned"
done

exit 0


==> share/bin/bibtex-check <==
#! /bin/sh

case $VERBOSE in
  x) set -x;;
esac

papers_dir=/lrde/doc/lrde/papers
share_dir=$(dirname $(dirname "$PWD/$0"))
share_bib_dir=$share_dir/bib

test "X$AM_COLOR_TESTS" != Xno &&		\
test "X$TERM" != Xdumb &&			\
{						\
  test "X$AM_COLOR_TESTS" = Xalways ||	\
  {						\
    test -t 1 2>/dev/null &&			\
    tput bold 1 >/dev/null 2>&1 &&		\
    tput setaf 1 >/dev/null 2>&1 &&		\
    tput sgr0 >/dev/null 2>&1;			\
  }						\
} &&						\
{						\
  red=$(tput setaf 1);				\
  grn=$(tput setaf 2);				\
  lgn=$(tput bold)$(tput setaf 2);		\
  blu=$(tput setaf 4);				\
  std=$(tput sgr0);				\
}


stderr ()
{
  local i
  for i
  do
    echo >&2 "$0: $i"
  done
}

# Indent, and put in red
red ()
{
  sed >&2 -e "s/.*/  ${red}&${std}/" "$@"
}

msg_checking ()
{
  msg_checking_msg_=$1
  echo >&2
  stderr "*** Checking $msg_checking_msg_"
}

msg_result ()
{
  stderr "$msg_checking_msg_: $(truth $1)"
  echo >&2
  msg_checking_msg_=
}


truth()
{
  local sta=$?
  if test $# -eq 1; then
    sta=$1
  fi
  case $sta in
    0) echo "${grn}OK${std}";;
    1) echo "${red}KO${std}";;
    *) echo "${red}KO ($?)${std}";;
  esac
}


check_char ()
{
  msg_checking "for invalid characters"
  local fail=0
  LC_ALL=C grep '[^[:print:][:blank:]]' "$@" && fail=1
  msg_result $fail
}

check_style ()
{
  msg_checking "for double-quotes"
  local b
  local fail=0
  for b
  do
    LC_ALL=C grep '=[	 ]*"' $b /dev/null && fail=1
  done
  msg_result $fail
}

# AS_TMPDIR([bibtex-check])
my_mktemp ()
{
  # Create a (secure) tmp directory for tmp files.
  : ${TMPDIR=/tmp}
  {
    tmp=`(umask 077 && mktemp -d "$TMPDIR/bibtex-checkXXXXXX") 2>/dev/null` &&
    test -n "$tmp" && test -d "$tmp"
  }  ||
  {
    tmp=$TMPDIR/bibtex-check$$-$RANDOM
    (umask 077 && mkdir "$tmp")
  } ||
  {
     echo "$me: cannot create a temporary directory in $TMPDIR" >&2
     { (exit 1); exit 1; }
  }
  echo $tmp
}


# check_pdf BIBFILE DIRECTORY
# ---------------------------
# Check that the papers in BIBFILE are also available in DIRECTORY.
check_pdf ()
{
  msg_checking "for BibTeX/PDF correspondance"
  local bib=$1
  local dir=$2
  local fail=0
  (cd $dir && ls -1 *.pdf) |
     grep -Ev '^lrde(-private)?\.pdf$' |
     sed -e 's/\.pdf$//' |
     sort >/tmp/list.pdf
  sed -ne '/^@.*{[ \t]*/{s///;s/,//;p}' $bib |
     sort >/tmp/list.bib
  if cmp -s /tmp/list.pdf /tmp/list.bib; then :; else
    echo "Files in $dir not in $bib:"
    comm -23 /tmp/list.pdf /tmp/list.bib | red
    echo
    echo "Files in $bib not in $dir:"
    comm -13 /tmp/list.pdf /tmp/list.bib | red
    echo
    fail=1
  fi
  msg_result $fail
}

check_urllrde ()
{
  msg_checking "for urllrde in $@"
  local fail=0
  local b
  for b
  do
    bib2bib -q -c 'not urllrde : "."' -oc check.bib $b >/dev/null
    if test -s check.bib; then
      stderr "$b: entries that lack an urllrde field:"
      red check.bib
      fail=1
    fi &&
    rm -f check.bib
  done
  msg_result $fail
}

check_wikilinks ()
{
  local i=0
  local regexp='s,.*<a href="\(http://www.lrde.epita.fr/dload/[^"]*\)".*,\1,p'
  local urls=$(sed -ne "$regexp" "$1")
  for url in $urls 'X'; do
    if test $url = 'X'; then
      test $i -eq 0 && echo >&2 "${red}WARNING${std}: no URL given in $u"
      continue
    fi
    i=1
    if ! wget -q -O /dev/null $url; then
      echo >&2 "${red}WARNING${std}: $url is invalid"
    fi
  done
}

check_wiki ()
{
  msg_checking "for existence of the urllrde page"
  local fail=0
  dir=$(my_mktemp)
  echo >&2 "$dir"
  local b
  for b
  do
    sed -ne 's/.*urllrde.*{\(.*\)\}.*/\1/p' $b |
      while read u;
      do
	printf >&2 "    $u... "
        if wget -q -O $dir/$u http://publis.lrde.epita.fr/$u; then
	  echo >&2 "${grn}PASS${std}"
          check_wikilinks "$dir/$u"
	else
	  echo >&2 "${red}FAIL${std}"
          fail=1
        fi
      done
  done
  rm -rf $dir
  
  msg_result $fail
}


# check_bib BIBFILES...
# ---------------------
# Basic checks for bibtex files.
check_bib()
{
  check_char  "$@"
  check_style "$@"
}

# check_perms_or_student BIBFILE DIRECTORY
# ----------------------------------------
# More elaborate checks for bibtex files about our own papers.
check_perms_or_student ()
{
  local bib=$1
  local dir=$2
  check_bib     $bib
  check_pdf     $bib $dir
  check_urllrde $bib
  check_wiki    $bib
}

check_perms ()
{
  check_perms_or_student $share_bib_dir/lrde.bib /lrde/doc/lrde/papers
}

check_students ()
{
  check_perms_or_student $share_bib_dir/csi.bib /lrde/doc/lrde/student-reports
}

check_all ()
{
  check_char     "$@"
  check_perms
  check_students
}

case $1 in
  -h|--help)
     echo "$0 [perms | csi | all | FILES...]"
     echo
     echo "Run a number of sanity check on bib files."
     ;;
  perms) check_perms;;
  csi)   check_students;;
  all)   check_all $share_bib_dir/*.bib;;
  *)     check_bib "$@"
esac


==> share/bin/deacronym <==
#! /usr/bin/perl -w

# Usage: deacronym FILE...
#
# Looks for \acrodef in the *.{tex,sty} files all the subdirectories,
# and replaces the various forms of \ac with the proper inlined
# expansion in the FILEs.  The original FILEs will be backed up as
# FILE.bak.  This is useful when a LaTeX must be delivered with little
# dependencies.
#
# Bugs:
#
# Of course it has limitations: it is "static" instead of "dynamic",
# i.e., instead of using the full form for the first \ac to be
# expanded, it will expanded the first *occurrence* of \ac.  This is
# usually what one wants.
#
# Besides it will obviously be wrong if \ac is used in macros.
#
# You will still have to remove possible definition of in the TeX
# files and to remove the inclusion of acronym.sty.

use strict;
use IO::File;
use File::Find;

# key -> short.
my %short;
# key -> long.
my %long;
# key -> 1 if already expanded, undefined otherwise.
my %done;

# contents ($FILE_NAME)
# ---------------------
sub contents ($)
{
  my ($file) = @_;
  local $/;			# Turn on slurp-mode.
  my $f = new IO::File "< $file" or die "$file";
  my $contents = $f->getline or die "$file";
  $f->close;
  return $contents;
}

# Learn from the current file, if a *.{sty,tex} file.
sub learn
{
  my ($file) = $File::Find::name;
  return
      unless $file =~ /\.(sty|tex)$/;
  print STDERR "Checking $file\n";
  # Learn about all the occurrences of \acrodef{key}[SHORT]{LONG}.
  my $contents = contents($file);
  # When spanning several lines, not supported.
  $contents =~ s(\\acrodef\{(\w+)\}\[(.*?)\]\{(.*)\}$)
                ($short{$1} = $2; $long{$1} = $3; ""; )gme;
}

# handle MACRO, KEY
# -----------------
sub handle ($$)
{
  my ($macro, $key) = @_;

  my $long = $long{$key};
  my $short = $short{$key};

  # If plural, "LONGs (SHORTs)".
  if ($macro =~ /p/)
    {
      $short .= 's';
      $long  .= 's';
    }

  # If reversed, "SHORT (LONG)".
  my $full = ($macro =~ /r/
              ? "$short ($long)"
              : "$long ($short)");

  my $res;
  # If long, or short, don't consider the acronym is defined.
  if ($macro =~ /s/)
    {
      # Short, just the acronym.
      $res = $short;
    }
  elsif ($macro =~ /l/)
    {
      # Long, just the long.
      $res = $long;
    }
  elsif ($macro =~ /f/)
    {
      # Full, the full version, even if defined already.
      $res = $full;
      $done{$key} = 1;
    }
  else
    {
      # Not full nor short, provide the full version only if first
      # occurrence.
      $res = defined $done{$key} ? $short : $full;
      $done{$key} = 1;
    }

  print STDERR "\\$macro\{$key\} -> $res\n";
  return $res;
}

# deacronym ($FILE)
# -----------------
# "Inline" uses of \ac* in $FILE.
sub deacronym ($)
{
  my ($file) = @_;
  my ($bak) = "$file.bak";
  rename ($file, $bak) or die;
  my $contents = contents ($bak);
  # Perform all the sustitutions.
  $contents =~ s(\\(ac[lprs]*)\{(.*?)\})
                ( handle($1, $2); )ge;
  my $out = new IO::File(">$file") or die;
  print $out $contents;
}

## ------ ##
## Main.  ##
## ------ ##

File::Find::find ({wanted => \&learn, no_chdir => 1 }, '.');
for my $key (sort keys %short)
{
  print STDERR "$key -> $short{$key}, $long{$key}\n";
}
for my $file (@ARGV)
{
  deacronym($file);
}

### Setup "GNU" style for perl-mode and cperl-mode.
## Local Variables:
## perl-indent-level: 2
## perl-continued-statement-offset: 2
## perl-continued-brace-offset: 0
## perl-brace-offset: 0
## perl-brace-imaginary-offset: 0
## perl-label-offset: -2
## cperl-indent-level: 2
## cperl-brace-offset: 0
## cperl-continued-brace-offset: 0
## cperl-label-offset: -2
## cperl-extra-newline-before-brace: t
## cperl-merge-trailing-else: nil
## cperl-continued-statement-offset: 2
## End:


==> share/bin/generate-rev-sty <==
#! /usr/bin/perl -w

use strict;

my $changelog = $ARGV[0];
#-f $changelog || die "no such file: $changelog";

$ENV{'LC_ALL'} = 'C';

my %info;

my $svn_info = `svn info $changelog 2>/dev/null ||
git log -n 1 --pretty=format:'Revision: %h
Last Changed Author: %an
Last Changed Date: %ai' $changelog`;
$svn_info =~
  s{^([\w\s]+):\s+(.*)$}
   {
     my $val = $2;
     (my $key = $1) =~ s| ||g;
     $info{$key} = $val;
   }exmg;

# Translate the date into something nicer to read.
# Last Changed Date: 2008-06-04 17:37:38 +0200 (Wed, 04 Jun 2008)
$info{LastChangedDate} =~
    m/^(\d+)-(\d+)-(\d+) (\d+):(\d+):(\d+) ([+\d]+)(?: \((.*)\))?$/;
$info{LastChangedYear} = $1;
$info{LastChangedMonth} = $2;
$info{LastChangedDay} = $3;
$info{LastChangedHour} = $4;
$info{LastChangedMinute} = $5;
$info{LastChangedSecond} = $6;
$info{LastChangedTimeZone} = $7;
$info{LastChangedTimeShortDate} = $8 || '';

# Be sure to define at least SvnRev, even if to nothing.
$info{Rev} = $info{Revision} || '';

for my $k (sort keys %info)
{
  print "\\newcommand{\\Svn$k}{$info{$k}}\n";
}


==> share/bin/git-submodules <==
#! /bin/sh

# Avoid locale-related differences in the output (e.g., space before
# colons).
export LC_ALL=C

set -e

me=$(basename $0)

## BEGIN
#    git-submodules [OPTIONS] [DIRS]
#
# Handle the Git submodules of the DIRS (by default ".").
#
# Options:
#   -h, --help, -h      display this message and exit
#   -u, --update=DIR    upgrade the pinned externals directory DIR to the
#                       newest version, and upgrade.
#                       "all" means all the submodules
#   -U, --update-all    same as --update=all
#   -s, --subscribe=URL add a pinned external on URL, under the same directory
#                       name.  If there was already a dependency, pin it.
#   -n, --dry-run       display the commands, don't run them
#
# URL aliases:
#   share     git@git.lrde.epita.fr:lrde-publis-share
#
## END

## --------------------- ##
## Standard components.  ##
## --------------------- ##


stderr ()
{
    echo >&2 "$me: $@"
}

fatal ()
{
    stderr "$@"
    exit 1
}

usage ()
{
  # BSD sed is real piece of s.*t.
  sed -n '/^## BEGIN/,/^## END/{s/^#$/# /;s/^# //;/^#/!p;}' $0
}


## --------------------- ##
## Business components.  ##
## --------------------- ##

# url_aliases URL
# ---------------
# Decode the address URL, which might use other URL aliases.
# Aliases are read from the usage notice, the big comment
# at the start of this script.
url_aliases ()
{
  case $1 in
    http* | ssh* )
      echo "$1";;
    *)
      local alias=$1
      local url=$(usage |
		  sed -n "/^URL aliases:/,/^# *\$/{
			     /^ *$alias *\\([^ ].*\\)/{s//\1/;p;q;};
			 }")
      echo "$url"
      ;;
  esac
}


# git_submodules_update HOST-DIR PINNED-DIR
# -----------------------------------------
# Update all the pinned Git submodules to the most recent version.
git_submodules_update ()
{
  (
    set -e
    cd "$1"
    (
      set -e
      cd "$2"
      $run git pull
    )
    $run git add "$2"
  )
}


# git_submodules_subscribe DIR URL MODDIR
# ---------------------------------------
# Subscribe directory DIR/MODDIR to submodule at URL.  If there is
# already a module named MODDIR, ensure the passed URL matches its URL
# and pin it to the HEAD of the remote submodule.
git_submodules_subscribe ()
{
  url="$2"
  moddir="$1/$3"

  git_url_key="submodule.$moddir.url"
  if old_url=$(git config --get "$git_url_key"); then
    test "x$old_url" = "x$url" \
      || fatal "existing submodule $moddir subscribed to a different URL."
    # Pin an existing submodule.
    $run git submodule update
    (
      set -e
      $run cd "$moddir"
      $run git checkout master
      $run git pull
    )
  else
    # New subscription.
    $run git submodule add "$url" "$moddir"
    $run git submodule init
  fi
}



## ------ ##
## Main.  ##
## ------ ##

# List of upgrades.
upgrades=
# List of subscriptions.
subscriptions=
# List of directories to process.
dirs=

while test $# != 0
do
  case $1 in
    # Handle --option=value by splitting apart and putting back on argv.
    --*=*)
      opt=`echo "$1" | sed -e 's/=.*//'`
      val=`echo "$1" | sed -e 's/[^=]*=//'`
      shift
      set dummy "$opt" "$val" ${1+"$@"}; shift
      ;;

    # Handle --update-all as --update "all"
    -U | --update-all | --upgrade-all )
      shift
      set dummy --update "all" ${1+"$@"}; shift
      ;;
  esac

  case $1 in
      -h | --help )
	  usage
	  exit 0
	  ;;
      -u | --update | --upgrade )
	  if test x$2 = xall; then
	    git submodule status | while read sha1 dir ref; do
	      updates="$updates $dir"
	    done
	  else
	    updates="$updates $2"
	  fi
	  shift
	  ;;
      -s | --subscribe )
	  subscriptions="$subscriptions $2"
	  shift
	  ;;
      -n | --dry-run )
	  run=stderr
	  ;;
      -*)
	  fatal "invalid option: $1"
	  ;;
      *)
	  dirs="$dirs $1"
	  ;;
  esac
  shift
done

test -n "$dirs" || dirs=.

for d in $dirs
do
  # Did the process trigger any update?
  update=false

  for s in $subscriptions
  do
    git_submodules_subscribe "$d" $(url_aliases "$s") "$s"
    update=true
  done

  for u in $updates
  do
    git_submodules_update "$d" "$u"
    update=true
  done

  if $update; then
    stderr "You should commit, submodules were updated."
  fi
done


==> share/bin/latin2tex <==
#! /bin/sh

# Change all the latin 1 accents to TeX accents.  We don't use recode,
# because we don't want to convert { into \{ and so forth.

recode_lower=$(echo "
s/á/\\'a/g;
s/à/\\\`a/g;
s/â/\\^a/g;
s/ä/\\\"a/g;
s/ã/\\~a/g;
s/ß/\\ss{}/g;
s/é/\\'e/g;
s/è/\\\`e/g;
s/ê/\\^e/g;
s/ë/\\\"e/g;
s/î/\\^i/g;
s/ï/\\\"i/g;
s/ó/\\'o/g;
s/ô/\\^o/g;
s/ö/\\\"o/g;
s/ø/\\o{}/g;
s/ü/\\\"u/g;
s/û/\\^u/g;
s/ù/\\\`u/g;
s/ç/\\,c{}/g;
" | sed -e 's/[\\`"]/\\&/g')

recode_upper=$(echo "$recode_lower" |
	       sed -e 's/\"/\\\"/g' |
	       tr '[:lower:]' '[:upper:]' |
	       sed 's/^S/s/g;s/G;$/g;/g')

recode_one_file ()
{
  local file=$1

  sed -i~ -e "$recode_lower" -e "$recode_upper" $file
}

for opt
do
  case $opt in
  -h | --help)
     cat <<-EOF
	$0 [OPTIONS] FILES

	Convert the latin 1 accents in the BibTeX FILES to be 7
	bit clean.  Recode cannot be used, as it changes the special
	characters ({, } etc.) too.  A backup is left with ~ appended.

	Options:
	  -h, --help        Display this message and exit successfully
EOF
     exit 0
     ;;
  -*)
     echo >&2 "unknown option: $opt"
     exit 1
     ;;

  *)
     recode_one_file "$opt"
     ;;
  esac
done


==> share/bin/list2bib <==
#! /usr/bin/env python

# usage: list2bib <file.list >file.bib

# This script was written for a specific purpose (converting a
# bibliography in a personal/non-standard format to a BibTeX file),
# but it might serve as a basis for other scripts.
#
#
# The input follows this layout:
#
#   # A comment.
#   # Another comment.
#
#   # A title.
#   Compiler construction bibliography
#
#   
#   *** A section.
#
#   http://www.an.url.org
#    A title.
#    An author.
#    A year.
#
#
# Hence, entries are formated like this:
#
#   http://citeseer.ist.psu.edu/briggs92register.html
#    Register Allocation via Graph Coloring
#    Preston Briggs
#    1992


import sys, re

# Read a line, removing white space and comments
def read_line (input):
  line = input.readline ()
  while line:
    line = line.lstrip ()
    # Strip white space and comments.
    if not line or line[0] in ['\n', '\r', '#', '*']:
      line = input.readline ()
    else:
      break
  # Remove trailing \n and \r.
  return line.rstrip ("\n\r")

# Wrap a line.
def wrap (s, width, indent_char = '{'):
  # Look for the first occurrence of INDENT_CHAR to get the level of
  # indentation.
  indent = s.find (indent_char) + 1
  pieces = s.split(' ')
  output = ""
  line = pieces.pop (0)
  sep = " "
  while pieces:
    piece = pieces.pop (0)
    if len (line) + len (sep) + len (piece) > width:
      # "Flush" the current line, and start a new one.
      output += line + "\n"
      line = " " * indent + piece
    else:
      line += sep + piece
  output += line
  return output

class Entry:
  """A BibTeX entry."""

  def __init__(self, title, author, year, url):
    self.title = title
    self.author = self.gen_author (author)
    self.year = year
    self.url = url
    self.key = self.gen_key (author, year)

  def __str__ (self):
    return "@Article{" + self.key + "\n" + \
           wrap ("  title =        {" + self.title + "}", 75) + "\n" + \
           wrap ("  author =       {" + self.author + "}", 75)  + "\n" + \
           "  year =         {" + self.year + "}\n" + \
           "  url =          {" + self.url + "}\n" + \
           "}\n"

  def gen_author (self, author):
    as = author.split (',')
    authors = [a.strip () for a in as]
    return " and ".join (authors)

  def gen_key (self, author, year):
    authors = author.split (',')
    names = authors[0].split (" ")
    lastname = names[-1].lower ()
    digits = str (year)[-2:]
    return lastname + "." + digits

# Tag proper nouns as verbatim.
def verbatimize (s):
  proper_nouns = ["ANSI", "Bison", "BURS", "C", "CISC", "DAGs", "Flex",
                  "Forth", "GCC", "HARE", "IA-64", "Impact-I", "Intel",
                  "Java", "MBURG", "RISC", "RTL", "sigma-SSA", "SSA", "SELF"]
  verb = s
  for n in proper_nouns:
    verb = re.sub ("\\b" + n + "\\b", "{" + n + "}", verb);
  return verb

# Driver.
input = sys.stdin
line = read_line (input)
entries = []
# Skip header.
if line == "Compiler construction bibliography":
  line = read_line (input)
while line:
  url = line
  title = verbatimize (read_line (input))
  author = read_line (input)
  year = read_line (input)
  e = Entry (title, author, year, url)
  entries.append (e)
  # Next.
  line = read_line (input)
entries.sort (lambda x, y: cmp(x.key, y.key))
for e in entries:
  print (e)


==> share/bin/psbbox <==
#! /usr/bin/perl -w

use strict;
use diagnostics;
use IO::File;

# How to invoke gs so that it prints the effective bboxes of a file.
my $gs_bbox = "gs -q -dBATCH -sDEVICE=bbox -dNOPAUSE";

sub display_help ()
{
  print <<EOF;
usage: $0 [OPTIONS] [INPUT] [OUTPUT]

Fix the BoundingBox Document Structuring Comments in a PostScript file.

Options:
  -h, --help       display this help and exit
  -v, --verbose    display debugging date
  -q, --quiet      don\'t display informational messages

  -f, --fix        fix the input file\'s bounding boxes
  -c, --claimed    display claimed bounding boxes
  -e, --effective  display effective bounding boxes

  -a, --pages=SEL  select the set of pages to sample [-]
                   SEL   ::= RANGE (, RANGE)*
                   RANGE ::= PAGE | [PAGE] - [PAGE]

If INPUT is unspecified, or equal to \`-\', then it stands for the
standard input.  If OUTPUT to \`-\', it stands for standard output.

If INPUT is specified but OUTPUT is not, then INPUT is fixed in place
and a copy of the original is left as INPUT.bak.

Todo:
  - don\'t use all the page, just sample some of them using psselect,
    as the gs invocation is really longuish.
    Find a nice sampling scheme
  - do not duplicate code between psbbox and psfit.
  - do not backup when not needed, or remove the back up file if useless
EOF
  exit 0;
}

sub stderr ($)
{
  print STDERR @_, "\n";
}

my $verbose_p = 1;

sub verbose ($)
{
  stderr @_
    if $verbose_p;
}




sub set_min (\$$)
{
  my ($ref, $val) = @_;
  $$ref = $val
    unless (defined $$ref && $$ref < $val);
}

sub set_max (\$$)
{
  my ($ref, $val) = @_;
  $$ref = $val
    unless (defined $$ref && $$ref > $val);
}

sub set_union (\@@)
{
  my ($bbox, @new) = @_;
  set_min ($$bbox[0], $new[0]);
  set_min ($$bbox[1], $new[1]);
  set_max ($$bbox[2], $new[2]);
  set_max ($$bbox[3], $new[3]);
}



=item C<bbox ($input)>
Compute the bbox and high res bbox for C<$input>, and return them in
a hash with keys (if available) C<BoundingBox> and C<HiResBoundingBox>,
and array as values (left, bottom, right, top).
=cut

sub bbox ($)
{
  my ($input) = @_;
  my $in = new IO::File ($input) or die;
  my $res = ();

  while ($_ = $in->getline)
    {
      if (/%%((?:HiRes)?BoundingBox): ([\d.]+) ([\d.]+) ([\d.]+) ([\d.]+)/)
	{
	  set_union (@{$res->{$1}}, $2, $3, $4, $5);
	}
    }
  return $res;
}


sub print_bbox ($\%)
{
  my ($msg, $bbox) = @_;
  foreach my $k (sort keys %$bbox)
    {
      print "$msg $k: @{$bbox->{$k}}\n";
    }
}


=item C<save_stdin ()>
Save the standard input in a temporary file, and return its name.
=cut

sub save_stdin ()
{
  use File::Temp qw/ tempfile /;
  my ($fh, $filename) = tempfile();
  my $line;
  for (;;)
    {
      undef $!;
      unless (defined( $line = <> ))
	{
	  die $! if $!;
	  last; # reached EOF
	}
      print $fh $line;
    }
  return $filename;
}


=item C<backup ($file)>
Rename C<$file> with a back up extensions, and return this name.
=cut

sub backup ($)
{
  my ($file) = @_;
  use File::Copy;
  my $SIMPLE_BACKUP_SUFFIX = $ENV{'SIMPLE_BACKUP_SUFFIX'} || '~';

  # Back up and install the new one.
  my $backup = "$file$SIMPLE_BACKUP_SUFFIX";
  copy ($file, $backup)
    or die "cannot backup $file: $!";
  return $backup;
}


=item C<psbbox ($file, $out, %bbox)>
Fix the claimed bounding boxed of C<$file> to be the effective values
C<%bbox>, and save the result in the file handle C<$out>.
=cut

sub psbbox ($$\%)
{
  my ($file, $out, $bbox) = @_;

  my $in = new IO::File ($file) or die;
  while ($_ = $in->getline ())
    {
      # FIXME: Maybe we should fix all the PageBoundingBoxes?
      if (/%%((?:Page)?((?:HiRes)?BoundingBox))/)
	{
	  print $out "%%$1: @{$bbox->{$2}}\n";
	}
      else
	{
	  print $out $_;
	}
    }
}

## ------ ##
## Main.  ##
## ------ ##

my $fix_p = 0;
my $claimed_p = 0;
my $effective_p = 0;
# Page ranges to print, in psselect/a2ps syntax.  By default, all.
my $pages = "-";

use Getopt::Long;
Getopt::Long::GetOptions
  (
   'v|verbose'    => \$verbose_p,
   'q|quiet'      => sub { $verbose_p = 0; },
   'f|fix'        => \$fix_p,
   'c|claimed'    => \$claimed_p,
   'e|effective'  => \$effective_p,
   'h|help'       => \&display_help,
   'a|pages'      => \$pages,
   )
  or exit 1;

die "incorrect number of arguments"
  unless 0 <= $#ARGV && $#ARGV <= 2;


# ---------------------------- #
# Compute $input and $output.  #
# ---------------------------- #

my $input = $ARGV[0];
my $output = $ARGV[1];

# Always save the input.  When we just want the claimed bboxes, this
# is overkill, but this is rare enough to be ignored.
if (!defined $input || $input eq "-")
{
  # We really need a file, cannot work with stdin.
  $input = save_stdin;
  $output = "-";
}
elsif (!defined $output)
{
  # There is no output set: backup the input, and set the output to the
  # original file name.
  $output = $input;
  $input = backup ($input);
}


# --------- #
# Process.  #
# --------- #

# A pipe to select $pages from the input file.
my $psselect = ($pages ? "psselect -q -p$pages <" : "cat") . " \"$input\"";

my $claimed = bbox ("$psselect |");
print_bbox "Claimed", %$claimed
  if $claimed_p;

my $effective = bbox ("$psselect | $gs_bbox - 2>&1 >/dev/null |");
stderr "$effective";

print_bbox "Effective", %$effective
  if $effective_p;

if ($fix_p)
{
  my $out;
  if ($output eq "-")
    {
      $out = *STDOUT;
    }
  else
    {
      $out = new IO::File (">$output") or die;
    }
  psbbox $input, $out, %$effective
}


### Setup "GNU" style for perl-mode and cperl-mode.
## Local Variables:
## perl-indent-level: 2
## perl-continued-statement-offset: 2
## perl-continued-brace-offset: 0
## perl-brace-offset: 0
## perl-brace-imaginary-offset: 0
## perl-label-offset: -2
## cperl-indent-level: 2
## cperl-brace-offset: 0
## cperl-continued-brace-offset: 0
## cperl-label-offset: -2
## cperl-extra-newline-before-brace: t
## cperl-merge-trailing-else: nil
## cperl-continued-statement-offset: 2
## End:


==> share/bin/psfit <==
#! /usr/bin/perl -w

use strict;

# Margin apply on the four borders.
my $margin = 20;
my $inner  = 12;
my $duplex = 0;

=item C<display_help>
Display help and exit
=cut

sub display_help ()
{
  print <<EOF;
usage: $0 [OPTIONS] [INPUT] [OUTPUT]

Scale the PostScript INPUT file to fit in the A4 paper.  Save the
result in OUTPUT.  The BoundingBox comments on FILE are fixed as a
side effect.

The processing is long.

Options:
  -h, --help               display this help and exit
  -v, --verbose            display debugging date
  -q, --quiet              do not display informational messages
  -m, --margin=SIZE        margin in PostScript points  [$margin]
                           applies to bottom, top, left, and right.
  -i, --inner-margin=SIZE  inner margin for binding [$inner]
                           (added to the whole margin)
  -d, --duplex             inner margin side depends on parity of the page

If INPUT is unspecified, or equal to \`-\', then it stands for the
standard input.  If OUTPUT to \`-\', it stands for standard output.

If INPUT is specified but OUTPUT is not, then INPUT is scaled in place
and a copy of the original is left as INPUT.bak.

Use with a2ps:
  Using psfit to print booklets proves to be both extremely useful, and
  very slow.  I use another user option: \`bookf\'.  To use it, put
  the following in your ~/.a2ps/a2psrc:

    # Use acroread as a pdf -> ps filter.
    Variable: del.acroread \\
       acroread -toPostScript

    # When delegating to acrobat, apply n-uping and page selection on
    # the output.
    Delegation: Acrobat pdf:ps \\
       #{del.acroread} < '\$f' | #{del.psselnup}

    # Invoke psfit before launching the stock psbook sequence.
    Variable: lp.hook.book.fit \\
       psfit --duplex | #{lp.hook.book}

    # Define a user option `-=bookf'.  Use `book' if you want
    # to override the default `-=book' user option.
    UserOption: bookf \\
      -1Dlp.hook=#{lp.hook.book.fit} -s1

  and run \`a2ps -=bookf foo.ps bar.pdf\'.

Todo:
  - fix the resulting BoundingBox (why psresize does not do it?)
  - support various output formats
  - do not duplicate code between psbbox and psfit.
    actually, there are so similar, that they could be a single program
    maybe under two names (or a default mode).
EOF
  exit 0;
}


my $verbose_p = 0;

sub verbose ($)
{
  print STDERR @_, "\n"
      if $verbose_p;
}

=item C<save_stdin ()>
Save the standard input in a temporary file, and return its name.
=cut

sub save_stdin ()
{
  use File::Temp qw/ tempfile /;
  my ($fh, $filename) = tempfile();
  my $line;
  for (;;)
    {
      undef $!;
      unless (defined( $line = <> ))
	{
	  die $! if $!;
	  last; # reached EOF
	}
      print $fh $line;
    }
  return $filename;
}


=item C<backup ($file)>
Rename C<$file> with a back up extensions, and return this name.
=cut

sub backup ($)
{
  my ($file) = @_;
  use File::Copy;
  my $SIMPLE_BACKUP_SUFFIX = $ENV{'SIMPLE_BACKUP_SUFFIX'} || '~';

  # Back up and install the new one.
  my $backup = "$file$SIMPLE_BACKUP_SUFFIX";
  move ($file, $backup)
    or die "cannot backup $file: $!";
  return $backup;
}



sub min ($$)
{
  my ($a, $b) = @_;
  return ($a < $b) ? $a : $b;
}


sub psfit ($$$)
{
  my ($in, $out, $margin) = @_;

  # We must know the right bounding box, so compute it.
  # We don't need to fix the file though.
  my $cmd = "psbbox -e $in /dev/null " . ($verbose_p ? "--verbose" : "--quiet");
  my $psbbox_log = `$cmd` ;
  die "psbbox returned nothing"
    unless $psbbox_log;
  chomp $psbbox_log;
  verbose "LOG: $psbbox_log";
  my $bbox;
  # Prefer the high res bbox if available.
  foreach my $dsc ("HiResBoundingBox", "BoundingBox")
    {
      ($bbox) = ($psbbox_log =~ m/.*Effective $dsc: ([\d.\s]*).*/s);
      last
	if $bbox;
    }
  verbose "BBOX: $bbox";

  # Input dimensions: left bottom right top
  my @idims = split ' ', $bbox;
  # Output dimensions: paper size
  my @odims = split ' ', "0 0 595 842";

  # Input width and height.
  my $iw = $idims[2] - $idims[0];
  my $ih = $idims[3] - $idims[1];

  # Output width and height.
  my $ow = $odims[2] - $odims[0];
  my $oh = $odims[3] - $odims[1];

  # Maximum width and height scales, taking into account margins.
  my $ratio_w = ($ow - 2 * $margin - $inner) / $iw;
  my $ratio_h = ($oh - 2 * $margin) / $ih;

  verbose "RATIO: $ratio_w, $ratio_h";

  # The common scale.
  my $scale = min ($ratio_h, $ratio_w);

  verbose "SCALE: $scale";

  # Effective final width and height.
  my $ew = $iw * $scale;
  my $eh = $ih * $scale;

  verbose "EFFECTIVE: $ew, $eh";

  # Output width and height margins (well, halves).
  my $owm = ($ow - $ew - $inner) / 2;
  my $ohm = ($oh - $eh) / 2;

  verbose "MARGINS: w = $owm (i = $inner), h = $ohm";

  # Offset before applying the scale
  my $woff = ($odims[0] - $idims[0]) * $scale + $owm;
  my $even_woff = $woff + $inner;
  my $odd_woff = $woff + ($duplex ? 0 : $inner);
  my $hoff = ($odims[1] - $idims[1]) * $scale + $ohm;

  my $request =
    sprintf ("2:0\@%.3f(%.3f,%.3f),1\@%.3f(%.3f,%.3f)",
	     $scale, $even_woff, $hoff,
	     $scale, $odd_woff,  $hoff);
  verbose "REQUEST: $request";

  if ($out eq "-")
    {
      system ("pstops", $request, $in) == 0
	or die;
    }
  else
    {
      system ("pstops", $request, $in, $out) == 0
	or die;
    }
}

## ------ ##
## Main.  ##
## ------ ##

use Getopt::Long;
Getopt::Long::GetOptions
  (
   'v|verbose'  => sub { $verbose_p = 1; },
   'q|quiet'    => sub { $verbose_p = 0; },
   'h|help'     => \&display_help,
   'm|margin=s' => \$margin,
   'i|inner=s'  => \$inner,
   'd|duplex'   => \$duplex,
   )
  or exit 1;

my $input = $ARGV[0];
my $output = $ARGV[1];

if (!defined $input || $input eq "-")
{
  # We really need a file, cannot work with stdin.
  $input = save_stdin;
  $output = "-";
}
elsif (!defined $output)
{
  # There is no output set: backup the input, and set the output to the
  # original file name.
  $output = $input;
  $input = backup ($input);
}

psfit $input, $output, $margin;



### Setup "GNU" style for perl-mode and cperl-mode.
## Local Variables:
## perl-indent-level: 2
## perl-continued-statement-offset: 2
## perl-continued-brace-offset: 0
## perl-brace-offset: 0
## perl-brace-imaginary-offset: 0
## perl-label-offset: -2
## cperl-indent-level: 2
## cperl-brace-offset: 0
## cperl-continued-brace-offset: 0
## cperl-label-offset: -2
## cperl-extra-newline-before-brace: t
## cperl-merge-trailing-else: nil
## cperl-continued-statement-offset: 2
## End:


==> share/bin/svn-externals <==
#! /bin/sh

# Avoid locale-related differences in the output (e.g., space before
# colons).
export LC_ALL=C

set -e

me=$(basename $0)

## BEGIN
#    svn-externals [OPTIONS] [DIRS]
#
# Handle the svn:externals dependencies of the DIRS (by default ".").
#
# Options:
#   -h, --help, -h      display this message and exit
#   -u, --update=DIR    upgrade the pinned externals directory DIR to the
#                       newest version, and upgrade.
#                       "all" means all the externals
#   -U, --update-all    same as --update=all
#   -s, --subscribe=URL add a pinned external on URL, under the same directory
#                       name.  If there was already a dependency, pin it.
#   -n, --dry-run       display the commands, don't run them
#
# URL aliases:
#   gostai    https://svn.gostai.com/svn
#   common      gostai/common
#   jpeg           common/libjpeg-6b/jpeg-6b
#   baux           common/project-template/trunk/build-aux
#   libport        common/project-template/trunk/libport
#   lurbi       gostai/liburbi-cpp/trunk
#   uobj           lurbi/src/liburbi/uobject
#   share     https://svn.lrde.epita.fr/svn/lrde-publis/trunk/share
#
# An svn:externals dependency is "pinned" if it has an explicit
# revision number.
## END

## --------------------- ##
## Standard components.  ##
## --------------------- ##


stderr ()
{
    echo >&2 "$me: $@"
}

fatal ()
{
    stderr "$@"
    exit 1
}

usage ()
{
  # BSD sed is real piece of s.*t.
  sed -n '/^## BEGIN/,/^## END/{s/^#$/# /;s/^# //;/^#/!p;}' $0
}


## --------------------- ##
## Business components.  ##
## --------------------- ##

# url_aliases URL
# ---------------
# Decode the address URL, which might use other URL aliases.
# Aliases are read from the usage notice, the big comment
# at the start of this script.
url_aliases ()
{
  case $1 in
    http* )
      echo "$1";;
    *)
      local loc=$1
      local alias=$(echo "$loc" | sed 's,/.*,,')
      local ext=$(echo   "$loc" | sed -n 's,^[^/]*/\(.*\),\1,p')
      local url=$(usage |
		  sed -n "/^URL aliases:/,/^# *\$/{
			     /^ *$alias *\\([^ ].*\\)/{s//\1/;p;q;};
			 }")
      url=$(url_aliases "$url")
      if test x"$ext" != x; then
	url=$url/$ext
      fi
      echo "$url"
      ;;
  esac
}

# svn_youngest URL
# ----------------
# Return the youngest revision of repository URL.
svn_youngest ()
{
  # Beware not to ignore the failure: pipes are not good.
  local info="$(svn info "$1")"
  test -n "$info" ||
    fatal "cannot get youngest revision number"
  echo "$info" | sed -n '/Revision: /{s///;p;q;}'
}


# svn_externals_update_stream [DIR]
# ---------------------------------
# Upgrade the pinned svn:externals corresponding to DIR in STDIN, and
# pass to STDOUT.  If DIR is empty, do it for all the directories.
svn_externals_update_stream ()
{
  # "all" means, any directory here.
  local request=$1
  test x"$request" != xall ||
    request=""

  while read e
  do
    case $e in
    # Keep comments.
    '' | '#'*)
      echo "$e"
      ;;

    # With revision.
    *' -r '[0-9]*)
      # Decode the svn:externals.
      # % svn pg svn:externals .
      # share -r 1569 https://svn.lrde.epita.fr/svn/lrde-publis/trunk/share
      dir=$(echo "$e" | sed 's/ .*//')
      if test -z "$request" || test "$request" = "$dir"; then
	rev=$(echo "$e" | sed -n 's/.*-r \([0-9][0-9]*\) *.*/\1/p')
	url=$(echo "$e" | sed -n 's/.* \(http\)/\1/p')
	test -n "$url" ||
	  fatal "cannot fetch the URL of $e"
	new_rev=$(svn_youngest "$url")
	test -n "$new_rev" ||
	  fatal "cannot fetch the revision of $url"
	echo "$dir -r $new_rev $url"
      else
	echo "$e"
      fi
      ;;

    # Without revision.
    *)
      echo "$e"
      ;;
    esac
  done
}


# svn_externals_update HOST-DIR PINNED-DIR
# ----------------------------------------
# Update all the pinned svn:externals to the most recent version.
svn_externals_update ()
{
  local externals="$(svn propget svn:externals "$1" |
		    svn_externals_update_stream "$2")"
  $run svn propset svn:externals "$externals" "$1"
}


# svn_externals_subscribe DIR URL
# -------------------------------
svn_externals_subscribe ()
{
  local host=$1
  local url=$2
  local dir=$(echo "$url" | sed -e 's,/$,,;s,.*/,,')
  local rev=$(svn_youngest "$url")
  externals=$(svn propget svn:externals "$host" |
	      sed -e "/^$dir /d")
  externals="$externals
$dir -r $rev $url"
  $run svn propset svn:externals "$externals" "$host"
}



## ------ ##
## Main.  ##
## ------ ##

# List of upgrades.
upgrades=
# List of subscriptions.
subscriptions=
# List of directories to process.
dirs=

while test $# != 0
do
  case $1 in
    # Handle --option=value by splitting apart and putting back on argv.
    --*=*)
      opt=`echo "$1" | sed -e 's/=.*//'`
      val=`echo "$1" | sed -e 's/[^=]*=//'`
      shift
      set dummy "$opt" "$val" ${1+"$@"}; shift
      ;;

    # Handle --update-all as --update "all"
    -U | --update-all | --upgrade-all )
      shift
      set dummy --update "all" ${1+"$@"}; shift
      ;;
  esac

  case $1 in
      -h | --help )
	  usage
	  exit 0
	  ;;
      -u | --update | --upgrade )
	  updates="$updates $2"
	  shift
	  ;;
      -s | --subscribe )
	  subscriptions="$subscriptions $2"
	  shift
	  ;;
      -n | --dry-run )
	  run=stderr
	  ;;
      -*)
	  fatal "invalid option: $1"
	  ;;
      *)
	  dirs="$dirs $1"
	  ;;
  esac
  shift
done

test -n "$dirs" || dirs=.

for d in $dirs
do
  # Should we run svn up at the end?
  update=false

  for s in $subscriptions
  do
    svn_externals_subscribe "$d" $(url_aliases "$s")
    update=true
  done

  for u in $updates
  do
    svn_externals_update "$d" "$u"
    update=true
  done

  if $update; then
    $run svn up
    stderr "You should checkin $d, externals were updated."
  fi
done

exit 0


==> share/bin/svn-grep <==
#! /bin/sh

# svngrep PATTERNS...
# PATTERNS are based to grep, so they can include options.

svnls ()
{
  # Performing status on external item at 'tests'
  #               510      510 demaille     tests
  # M             510       43 roussel      tests/AUTHORS
  # A             510      464 nottale      tests/wrapper.in
  #               510      501 demaille     tests/uob
  #              1482      556 demaille     libport/escape.cc
  svn st -vq |
    perl -n -e '/^.*\s+\d+\s+\d+\s+\w+\s+(.+)$/ && print "$1\n";'
}

svnls | xargs grep --color=auto "$@"


==> share/bin/svndiff <==
#!/bin/sh

{
  svn info | sed -n '/^URL: /{s///;p;q;}'
  echo
  svn diff --diff-cmd "`which diff`" -x "-w -u" $@ >$$.diffs
  # Don't fail if missing.
  diffstat $$.diffs 2>/dev/null
  echo
  sed $$.diffs -e "# do not try this at home !
/^Index: .*ChangeLog\$/{
n
N
N
N
N
s/.*\n.*\n.*\n.*[0-9]*-[0-9]*-[0-9]*/from/
n
:chlg
/^\+/b db
s/^.//
n
\${
g
s/^\n//
q
}
/^Index: /!b chlg
b continue
:db
/^\+/{
s/^.//
n
b db
}
N
s/.*\n//
\${
g
s/^\n//
q
}
/^Index: /!b db
:continue
x
s/^\n//
G
:finish
/^==*\$/{
N
s/^==*\n//
}
n
\$q
b finish
}
/^==*\$/d
\${
x
s/^\n//
p
g
p
}
H
d"
} | tee diffs.patch

rm $$.diffs


==> share/bin/texi2dvi <==
#! /bin/sh
# texi2dvi --- produce DVI (or PDF) files from Texinfo (or (La)TeX) sources.
# $Id: texi2dvi,v 1.167 2011/10/21 18:42:37 karl Exp $
#
# Copyright 1992, 1993, 1994, 1995, 1996, 1997, 1998, 1999, 2001, 2002, 2003,
# 2004, 2005, 2006, 2007, 2008, 2009, 2010, 2011 Free Software Foundation, Inc.
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 3 of the License,
# or (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program.  If not, see <http://www.gnu.org/licenses/>.
#
# Originally written by Noah Friedman.
#
# Please send bug reports, etc. to bug-texinfo@gnu.org.
# If possible, please send a copy of the output of the script called with
# the `--debug' option when making a bug report.

test -f /bin/ksh && test -z "$RUNNING_KSH" \
  && { UNAMES=`uname -s`; test "x$UNAMES" = xULTRIX; } 2>/dev/null \
  && { RUNNING_KSH=true; export RUNNING_KSH; exec /bin/ksh $0 ${1+"$@"}; }
unset RUNNING_KSH

# No failure shall remain unpunished.
set -e

# This string is expanded automatically when this file is checked out.
rcs_revision='$Revision: 1.167 $'
rcs_version=`set - $rcs_revision; echo $2`
program=`echo $0 | sed -e 's!.*/!!'`

build_mode=${TEXI2DVI_BUILD_MODE:-local}
build_dir=${TEXI2DVI_BUILD_DIRECTORY:-.}

# Initialize variables for option overriding and otherwise.
# Don't use `unset' since old bourne shells don't have this command.
# Instead, assign them an empty value.
action=compile
batch=false     # interact normally
catcode_special=maybe
debug=false
escape="\\"
expand=false    # true for expansion via makeinfo
includes=
line_error=true # pass --file-line-error to TeX
max_iters=-1    # keep going forever
oname=          # --output
out_lang=dvi
quiet=false     # let the tools' message be displayed
recode=false
set_language=
src_specials=
shell_escape=
latex2html=hevea  # or set to tex4ht
textra=         # Extra TeX commands to insert in the input file.
txiprereq=19990129 # minimum texinfo.tex version with macro expansion
verb=false      # true for verbose mode
translate_file= # name of charset translation file
recode_from=    # if not empty, recode from this encoding to @documentencoding

orig_pwd=`pwd`

# We have to initialize IFS to space tab newline since we save and
# restore IFS and apparently POSIX allows stupid/broken behavior with
# empty-but-set IFS.
# http://lists.gnu.org/archive/html/automake-patches/2006-05/msg00008.html
# We need space, tab and new line, in precisely that order.  And don't leave
# trailing blanks.
space=' '
tab='	'
newline='
'
IFS="$space$tab$newline"

# In case someone pedantic insists on using grep -E.
: ${EGREP=egrep}

# Systems which define $COMSPEC or $ComSpec use semicolons to separate
# directories in TEXINPUTS -- except for Cygwin et al., where COMSPEC
# might be inherited, but : is used.
if test -n "$COMSPEC$ComSpec" \
   && uname | $EGREP -iv 'cygwin|mingw|djgpp' >/dev/null; then
  path_sep=";"
else
  path_sep=":"
fi

# Pacify verbose cds.
CDPATH=${ZSH_VERSION+.}$path_sep

# If $TEX is set to a directory, don't use it.
test -n "$TEX" && test -d "$TEX" && unset TEX

# 
## --------------------- ##
## Auxiliary functions.  ##
## --------------------- ##

# In case `local' is not supported by the shell, provide a function
# that simulates it by simply performing the assignments.  This means
# that we must not expect `local' to work, i.e., we must not (i) rely
# on it during recursion, and (ii) have two local declarations of the
# same variable.  (ii) is easy to check statically, and our test suite
# does make sure there is never twice a static local declaration of a
# variable.  (i) cannot be checked easily, so just be careful.
#
# Note that since we might use a function simulating `local', we can
# no longer rely on the fact that no IFS-splitting is performed.  So,
# while
#
# foo=$bar
#
# is fine (no IFS-splitting), never write
#
# local foo=$bar
#
# but rather
#
# local foo="$bar"
(
  foo=bar
  test_local () {
    local foo=foo
  }
  test_local >/dev/null 2>&1
  test $foo = bar
) || eval '
local () {
  case $1 in
    *=*) eval "$1";;
  esac
}
'


# cd_orig
# -------
# Return to the original directory.
cd_orig ()
{
  # In case $orig_pwd is on a different drive (for DOS).
  cd /

  # Return to the original directory so that
  # - the next file is processed in correct conditions
  # - the temporary file can be removed
  cd "$orig_pwd" || exit 1
}

# func_dirname FILE
# -----------------
# Return the directory part of FILE.
func_dirname ()
{
  dirname "$1" 2>/dev/null \
  || { echo "$1" | sed 's!/[^/]*$!!;s!^$!.!'; }
}


# noexit FILE
# -----------
# Return FILE with one extension remove.  foo.bar.baz -> foo.bar.
noext ()
{
  echo "$1" | sed -e 's/\.[^/.][^/.]*$//'
}


# absolute NAME -> ABS-NAME
# -------------------------
# Return an absolute path to NAME.
absolute ()
{
  case $1 in
   [\\/]* | ?:[\\/]*)
      # Absolute paths don't need to be expanded.
      echo "$1"
      ;;
   *) local slashes
      slashes=`echo "$1" | sed -n 's,.*[^/]\(/*\)$,\1,p'`
      local rel
      rel=$orig_pwd/`func_dirname "$1"`
      if test -d "$rel"; then
        (cd "$rel" 2>/dev/null &&
         local n
         n=`pwd`/`basename "$1"`"$slashes"
         echo "$n")
      else
        error 1 "not a directory: $rel"
      fi
      ;;
  esac
}


# ensure_dir DIR1 DIR2...
# -----------------------
# Make sure the directories exist.
ensure_dir ()
{
  for dir
  do
    # Beware that in parallel builds we may have several concurrent
    # attempts to create the directory.  So fail only if "mkdir"
    # failed *and* the directory still does not exist.
    test -d "$dir" \
      || mkdir "$dir" \
      || test -d "$dir" \
      || error 1 "cannot create directory: $dir"
  done
}


# error EXIT_STATUS LINE1 LINE2...
# --------------------------------
# Report an error and exit with failure if EXIT_STATUS is non null.
error ()
{
  local s="$1"
  shift
  report "$@"
  if test "$s" != 0; then
    exit $s
  fi
}


# findprog PROG
# -------------
# Return true if PROG is somewhere in PATH, else false.
findprog ()
{
  local saveIFS="$IFS"
  IFS=$path_sep  # break path components at the path separator
  for dir in $PATH; do
    IFS=$saveIFS
    # The basic test for an executable is `test -f $f && test -x $f'.
    # (`test -x' is not enough, because it can also be true for directories.)
    # We have to try this both for $1 and $1.exe.
    #
    # Note: On Cygwin and DJGPP, `test -x' also looks for .exe.  On Cygwin,
    # also `test -f' has this enhancement, but not on DJGPP.  (Both are
    # design decisions, so there is little chance to make them consistent.)
    # Thusly, it seems to be difficult to make use of these enhancements.
    #
    if  { test -f "$dir/$1"     && test -x "$dir/$1"; } ||
        { test -f "$dir/$1.exe" && test -x "$dir/$1.exe"; }; then
      return 0
    fi
  done
  return 1
}

# report LINE1 LINE2...
# ---------------------
# Report some information on stderr.
report ()
{
  for i in "$@"
  do
    echo >&2 "$0: $i"
  done
}


# run COMMAND-LINE
# ----------------
# Run the COMMAND-LINE verbosely, and catching errors as failures.
run ()
{
  verbose "Running $@"
  "$@" 2>&5 1>&2 ||
     error 1 "$1 failed"
}


# usage
# -----
# Display usage and exit successfully.
usage ()
{
  # We used to simply have `echo "$usage"', but coping with the
  # changing behavior of `echo' is much harder than simply using a
  # here-doc.
  #
  #             echo '\noto'   echo '\\noto'   echo -e '\\noto'
  # bash 3.1      \noto           \\noto          \noto
  # bash 3.2       %oto           \noto           -e \noto
  #
  # where % denotes the eol character.
  cat <<EOF
Usage: $program [OPTION]... FILE...
  or:  texi2pdf [OPTION]... FILE...
  or:  pdftexi2dvi [OPTION]... FILE...

Run each Texinfo or (La)TeX FILE through TeX in turn until all
cross-references are resolved, building all indices.  The directory
containing each FILE is searched for included files.  The suffix of FILE
is used to determine its language ((La)TeX or Texinfo).  To process
(e)plain TeX files, set the environment variable LATEX=tex.

In order to make texi2dvi a drop-in replacement of TeX/LaTeX in AUC-TeX,
the FILE may also be composed of the following simple TeX commands.
  \`\\input{FILE}'     the actual file to compile
  \`\\nonstopmode'     same as --batch

When invoked as \`texi2pdf' or \`pdftexi2dvi', or given the option --pdf
or --dvipdf, generate PDF output.  Otherwise, generate DVI.

General options:
  -b, --batch         no interaction
  -D, --debug         turn on shell debugging (set -x)
  -h, --help          display this help and exit successfully
  -o, --output=OFILE  leave output in OFILE (implies --clean);
                        only one input FILE may be specified in this case
  -q, --quiet         no output unless errors (implies --batch)
  -s, --silent        same as --quiet
  -v, --version       display version information and exit successfully
  -V, --verbose       report on what is done

TeX tuning:
  -@                         use @input instead of \input for preloaded Texinfo
  -e, -E, --expand           force macro expansion using makeinfo
  -I DIR                     search DIR for Texinfo files
  -l, --language=LANG        specify LANG for FILE, either latex or texinfo
      --no-line-error        do not pass --file-line-error to TeX
  -r, --recode               call recode before TeX to translate input
      --recode-from=ENC      recode from ENC to the @documentencoding
      --shell-escape         pass --shell-escape to TeX
      --src-specials         pass --src-specials to TeX
  -t, --command=CMD          insert CMD in copy of input file
   or --texinfo=CMD          multiple values accumulate
      --translate-file=FILE  use given charset translation file for TeX

Output format:
      --dvi     output a DVI file [default]
      --dvipdf  output a PDF file via DVI (using dvipdf)
      --html    output an HTML file; run HeVeA for LaTeX files
      --info    output an Info file; run HeVeA for LaTeX files
  -p, --pdf     use pdftex or pdflatex for processing
      --ps      output a PostScript file via DVI (using dvips)
      --text    output a plain text file.  Use HeVeA for LaTeX files

Build modes:
  --build=MODE         specify the treatment of auxiliary files [$build_mode]
      --tidy           same as --build=tidy
  -c, --clean          same as --build=clean
      --build-dir=DIR  specify where the tidy compilation is performed;
                         implies --tidy;
                         defaults to TEXI2DVI_BUILD_DIRECTORY [$build_dir]
  --mostly-clean       remove the auxiliary files and directories
                         but not the output
  --max-iterations=N   don't process files more than N times

The MODE specifies where the TeX compilation takes place, and, as a
consequence, how auxiliary files are treated.  The build mode
can also be set using the environment variable TEXI2DVI_BUILD_MODE.

Valid MODEs are:
  \`local'      compile in the current directory, leaving all the auxiliary
               files around.  This is the traditional TeX use.
  \`tidy'       compile in a local *.t2d directory, where the auxiliary files
               are left.  Output files are copied back to the original file.
  \`clean'      same as \`tidy', but remove the auxiliary directory afterwards.
               Every compilation therefore requires the full cycle.

Using the \`tidy' mode brings several advantages:
  - the current directory is not cluttered with plethora of temporary files.
  - clutter can be even further reduced using --build-dir=dir: all the *.t2d
    directories are stored there.
  - clutter can be reduced to zero using, e.g., --build-dir=/tmp/\$USER.t2d
    or --build-dir=\$HOME/.t2d.
  - the output file is updated after every succesful TeX run, for
    sake of concurrent visualization of the output.  In a \`local' build
    the viewer stops during the whole TeX run.
  - if the compilation fails, the previous state of the output file
    is preserved.
  - PDF and DVI compilation are kept in separate subdirectories
    preventing any possibility of auxiliary file incompatibility.

On the other hand, because \`tidy' compilation takes place in another
directory, occasionally TeX won't be able to find some files (e.g., when
using \\graphicspath): in that case, use -I to specify the additional
directories to consider.

The values of the BIBTEX, DVIPDF, DVIPS, HEVEA, LATEX, MAKEINDEX,
MAKEINFO, PDFLATEX, PDFTEX, T4HT, TEX, TEX4HT, TEXINDEX, and THUMBPDF
environment variables are used to run those commands, if they are set.
Any CMD strings are added after @setfilename for Texinfo input, or in
the first line for LaTeX input.

Report bugs to bug-texinfo@gnu.org,
general questions and discussion to help-texinfo@gnu.org.
GNU Texinfo home page: <http://www.gnu.org/software/texinfo/>
General help using GNU software: <http://www.gnu.org/gethelp/>
EOF
  exit 0
}


# verbose WORD1 WORD2
# -------------------
# Report some verbose information.
verbose ()
{
  if $verb; then
    echo >&2 "$0: $@"
  fi
}


# version
# -------
# Display version info and exit succesfully.
version ()
{
  cat <<EOF
texi2dvi (GNU Texinfo 4.13+dev) $rcs_version

Copyright (C) 2011 Free Software Foundation, Inc.
License GPLv3+: GNU GPL version 3 or later <http://gnu.org/licenses/gpl.html>
This is free software: you are free to change and redistribute it.
There is NO WARRANTY, to the extent permitted by law.
EOF
  exit 0
}


## ---------------- ##
## Handling lists.  ##
## ---------------- ##


# list_append LIST-NAME ELEM
# --------------------------
# Set LIST-NAME to its former contents, with ELEM appended.
list_append ()
{
  local la_l="$1"
  shift
  eval set X \$$la_l "$@"
  shift
  eval $la_l=\""$@"\"
}


# list_concat_dirs LIST-NAME DIR-LIST
# -----------------------------------
# Append to LIST-NAME all the components (included empty) from
# the $path_sep separated list DIR-LIST.  Make the paths absolute.
list_concat_dirs ()
{
  local lcd_list="$1"
  # Empty path components are meaningful to tex.  We rewrite them as
  # `EMPTY' so they don't get lost when we split on $path_sep.
  # Hopefully no one will have an actual directory named EMPTY.
  local replace_EMPTY="-e 's/^$path_sep/EMPTY$path_sep/g' \
                       -e 's/$path_sep\$/${path_sep}EMPTY/g' \
                       -e 's/$path_sep$path_sep/${path_sep}EMPTY:/g'"
  save_IFS=$IFS
  IFS=$path_sep
  set x `echo "$2" | eval sed $replace_EMPTY`; shift
  IFS=$save_IFS
  local dir
  for dir
  do
    case $dir in
      EMPTY)
       list_append $lcd_list ""
       ;;
      *)
       if test -d $dir; then
          dir=`absolute "$dir"`
         list_append $lcd_list "$dir"
       fi
       ;;
    esac
  done
}


# list_prefix LIST-NAME SEP -> STRING
# -----------------------------------
# Return a string that is composed of the LIST-NAME with each item
# preceded by SEP.
list_prefix ()
{
  local lp_p="$2"
  eval set X \$$1
  shift
  local lp_res
  for i
  do
    lp_res="$lp_res \"$lp_p\" \"$i\""
  done
  echo "$lp_res"
}

# list_infix LIST-NAME SEP -> STRING
# ----------------------------------
# Same as list_prefix, but a separator.
list_infix ()
{
  eval set X \$$1
  shift
  local la_IFS="$IFS"
  IFS=$path_sep
  echo "$*"
  IFS=$la_IFS
}

# list_dir_to_abs LIST-NAME
# -------------------------
# Convert the list to using only absolute dir names.
# Currently unused, but should replace absolute_filenames some day.
list_dir_to_abs ()
{
  local ld_l="$1"
  eval set X \$$ld_l
  shift
  local ld_res
  for dir
  do
    dir=`absolute "$dir"`
    test -d "$dir" || continue
    ld_res="$ld_res \"$dir\""
  done
  set X $ld_res; shift
  eval $ld_l=\"$@\"
}


## ------------------------------ ##
## Language auxiliary functions.  ##
## ------------------------------ ##


# out_lang_set LANG
# -----------------
out_lang_set ()
{
  case $1 in
    dvi|dvipdf|html|info|pdf|ps|text) out_lang=$1;;
    *) error 1 "invalid output format: $1";;
  esac
}


# out_lang_tex
# ------------
# Return the tex output language (DVI or PDF) for $OUT_LANG.
out_lang_tex ()
{
  case $out_lang in
    dvi | ps | dvipdf ) echo dvi;;
    pdf ) echo $out_lang;;
    html | info | text ) echo $out_lang;;
    *)    error 1 "invalid out_lang: $1";;
  esac
}


# out_lang_ext
# ------------
# Return the extension for $OUT_LANG.
out_lang_ext ()
{
  case $out_lang in
    dvipdf ) echo pdf;;
    dvi | html | info | pdf | ps | text ) echo $out_lang;;
    *)    error 1 "invalid out_lang: $1";;
  esac
}


## ------------------------- ##
## TeX auxiliary functions.  ##
## ------------------------- ##

# Save TEXINPUTS so we can construct a new TEXINPUTS path for each file.
# Likewise for bibtex and makeindex.
tex_envvars="BIBINPUTS BSTINPUTS DVIPSHEADERS INDEXSTYLE MFINPUTS MPINPUTS \
TEXINPUTS TFMFONTS"
for var in $tex_envvars; do
  eval ${var}_orig=\$$var
  export $var
done


# absolute_filenames TEX-PATH -> TEX-PATH
# ---------------------------------------
# Convert relative paths to absolute paths, so we can run in another
# directory (e.g., in tidy build mode, or during the macro-support
# detection).  Prepend ".".
absolute_filenames ()
{
  # Empty path components are meaningful to tex.  We rewrite them as
  # `EMPTY' so they don't get lost when we split on $path_sep.
  # Hopefully no one will have an actual directory named EMPTY.
  local replace_empty="-e 's/^$path_sep/EMPTY$path_sep/g' \
                       -e 's/$path_sep\$/${path_sep}EMPTY/g' \
                       -e 's/$path_sep$path_sep/${path_sep}EMPTY:/g'"
  local res
  res=`echo "$1" | eval sed $replace_empty`
  save_IFS=$IFS
  IFS=$path_sep
  set x $res; shift
  res=.
  for dir
  do
    case $dir in
      EMPTY)
        res=$res$path_sep
        ;;
      *)
        if test -d "$dir"; then
          res=$res$path_sep`absolute "$dir"`
        else
          # Even if $dir is not a directory, preserve it in the path.
          # It might contain metacharacters that TeX will expand in
          # turn, e.g., /some/path/{a,b,c}.  This will not get the
          # implicit absolutification of the path, but we can't help that.
          res=$res$path_sep$dir
        fi
        ;;
    esac
  done
  echo "$res"
}


# output_base_name FILE
# ---------------------
# The name of FILE, possibly renamed to satisfy --output.
# FILE is local, there is no directory part.
output_base_name ()
{
  case $oname in
    '') echo "$1";;
     *) local out_noext
        out_noext=`noext "$oname"`
        local file_ext
        file_ext=`echo "$1" | sed 's/^.*\.//'`
        echo "$out_noext.$file_ext"
      ;;
  esac
}


# destdir
# -------
# Return the name of the directory where the output is expected.
destdir ()
{
  case $oname in
    '')  echo "$orig_pwd";;
    *)   dirname "$oname";;
  esac
}


# move_to_dest FILE...
# --------------------
# Move FILE to the place where the user expects it.  Truly move it, that
# is, it must not remain in its build location unless that is also the
# output location.  (Otherwise it might appear as an extra file in make
# distcheck.)
#
# FILE can be the principal output (in which case -o directly applies), or
# an auxiliary file with the same base name.
move_to_dest ()
{
  # If we built in place, there is nothing to install, leave.
  case $tidy:$oname in
    false:) return;;
  esac

  local destfile
  local destdir
  local destbase
  local sourcedir
  local sourcebase

  for file
  do
    test -f "$file" ||
      error 1 "no such file or directory: $file"
    case $tidy:$oname in
      true:)  destdir=$orig_pwd
              destfile=$destdir/$file;;
      *:*)    destfile=`output_base_name "$file"`
              destdir=`dirname "$destfile"`;;
    esac
    # We want to compare the source location and the output location,
    # and if they are different, do the move.  But if they are the
    # same, we must preserve the source.  Since we can't assume
    # stat(1) or test -ef is available, resort to comparing the
    # directory names, canonicalized with pwd.  We can't use cmp -s
    # since the output file might not actually change from run to run;
    # e.g., TeX DVI output is timestamped to only the nearest minute.
    destdir=`cd "$destdir" && pwd`
    destbase=`basename "$destfile"`

    sourcedir=`dirname "$file"`
    sourcedir=`cd "$sourcedir" && pwd`
    sourcebase=`basename "$file"`

    if test "$sourcedir/$sourcebase" != "$destdir/$destbase"; then
      verbose "Moving $file to $destfile"
      rm -f "$destfile"
      mv "$file" "$destfile"
    fi
  done
}


## --------------------- ##
## Managing xref files.  ##
## --------------------- ##

# aux_file_p FILE
# ---------------
# Return with success if FILE is an aux file.
aux_file_p ()
{
  test -f "$1" || return 1
  case $1 in
    *.aux) return 0;;
    *)     return 1;;
  esac
}

# bibaux_file_p FILE
# ------------------
# Return with success if FILE is an aux file containing citation
# requests.
bibaux_file_p ()
{
  test -s "$1" || return 1
  if (grep '^\\bibstyle[{]' "$1"   \
      && grep '^\\bibdata[{]' "$1" \
      ## The following line is suspicious: fails when there
      ## are citations in sub aux files.  We need to be
      ## smarter in this case.
      ## && grep '^\\citation[{]' "$f"
      ) >&6 2>&1;
  then
    return 0
  fi
  return 1
}

# index_file_p FILE
# -----------------
# Return with success if FILE is an index file.
index_file_p ()
{
  test -f "$1" || return 1
  case $in_lang:$latex2html:`out_lang_tex`:`sed '1q' "$1"` in
    # When working with TeX4HT, *.idx are created by LaTeX.  They must
    # be processed to produce *.4ix, *.4dx files.  The *.4dx file is
    # passed to makeindex to produce the *.ind file.  This sequence is
    # handled by run_index, so we are only interested in the *.idx
    # files, which have each "\indexentry" preceded by a
    # "\beforeentry".
    latex:tex4ht:html:"\\beforeentry {"*) return 0;;

    # When index.sty is used, there is a space before the brace.
    latex:*:*:"\\indexentry{"*|latex:*:*:"\\indexentry {"*) return 0;;

    texinfo:*:*:"\\entry{"*) return 0;;

    *) return 1;;
  esac
}

# xref_file_p FILE
# ----------------
# Return with success if FILE is an xref file (indexes, tables and lists).
xref_file_p ()
{
  test -f "$1" || return 1
  # If the file is not suitable to be an index or xref file, don't
  # process it.  It's suitable if the first character is a
  # backslash or right quote or at, as long as the first line isn't
  # \input texinfo.
  case `sed '1q' "$1"` in
    "\\input texinfo"*) return 1;;
    [\\''@]*)           return 0;;
           *)           return 1;;
  esac
}


# generated_files_get FILENAME-NOEXT [PREDICATE-FILTER]
# -----------------------------------------------------
# Return the list of files generated by the TeX compilation of FILENAME-NOEXT.
generated_files_get ()
{
  local filter=true
  if test -n "$2"; then
    filter=$2
  fi

  # Gather the files created by TeX.
  (
    if test -f "$1.log"; then
      sed -n -e "s,^\\\\openout.* = \`\\(.*\\)'\\.,\\1,p" "$1.log"
    fi
    echo "$1.log"
  ) |
  # Depending on these files, infer outputs from other tools.
  while read file; do
    echo $file
    case $in_lang in
      texinfo)
        # texindex: texinfo.cp -> texinfo.cps
       if index_file_p $file; then
         echo ${file}s
       fi
       ;;
      latex)
        if aux_file_p $file; then
          # bibtex: *.aux -> *.bbl and *.blg.
          echo $file | sed 's/^\(.*\)\.aux$/\1.bbl/'
          echo $file | sed 's/^\(.*\)\.aux$/\1.blg/'
          # -recorder: .fls
          echo $file | sed 's/^\(.*\)\.aux$/\1.fls/'
       fi
       ;;
    esac
  done |
  # Filter existing files matching the criterion.
  #
  # With an input file name containing a space, this produces a
  # "command not found" message (and filtering is ineffective).
  # The situation with a newline is presumably even worse.
  while read file; do
    if $filter "$file"; then
      echo $file
    fi
  done |
  sort |
  # Some files are opened several times, e.g., listings.sty's *.vrb.
  uniq
}


# xref_files_save
# ---------------
# Save the xref files.
xref_files_save ()
{
  # Save copies of auxiliary files for later comparison.
  xref_files_orig=`generated_files_get "$in_noext" xref_file_p`
  if test -n "$xref_files_orig"; then
    verbose "Backing up xref files: $xref_files_orig"
    # The following line improves `cp $xref_files_orig "$work_bak"'
    # by preserving the directory parts.  Think of
    # cp chap1/main.aux chap2/main.aux $work_bak.
    #
    # Users may have, e.g., --keep-old-files.  Don't let this interfere.
    # (Don't use unset for the sake of ancient shells.)
    TAR_OPTIONS=; export TAR_OPTIONS
    tar cf - $xref_files_orig | (cd "$work_bak" && tar xf -)
  fi
}


# xref_files_changed
# ------------------
# Whether the xref files were changed since the previous run.
xref_files_changed ()
{
  # LaTeX (and the package changebar) report in the LOG file if it
  # should be rerun.  This is needed for files included from
  # subdirs, since texi2dvi does not try to compare xref files in
  # subdirs.  Performing xref files test is still good since LaTeX
  # does not report changes in xref files.
  if grep "Rerun to get" "$in_noext.log" >&6 2>&1; then
    return 0
  fi

  # If old and new lists don't at least have the same file list,
  # then one file or another has definitely changed.
  xref_files_new=`generated_files_get "$in_noext" xref_file_p`
  verbose "Original xref files = $xref_files_orig"
  verbose "New xref files      = $xref_files_new"
  if test "x$xref_files_orig" != "x$xref_files_new"; then
    return 0
  fi

  # Compare each file until we find a difference.
  for this_file in $xref_files_new; do
    verbose "Comparing xref file `echo $this_file | sed 's|\./||g'` ..."
    # cmp -s returns nonzero exit status if files differ.
    if cmp -s "$this_file" "$work_bak/$this_file"; then :; else
      verbose "xref file `echo $this_file | sed 's|\./||g'` differed ..."
      if $debug; then
        diff -u "$work_bak/$this_file" "$this_file"
      fi
      return 0
    fi
  done

  # No change.
  return 1
}



## ----------------------- ##
## Running the TeX suite.  ##
## ----------------------- ##



# run_tex ()
# ----------
# Run TeX as "$tex $in_input", taking care of errors and logs.
run_tex ()
{
  case $in_lang:$latex2html:`out_lang_tex` in
    latex:*:dvi|latex:tex4ht:html)
        tex=${LATEX:-latex};;
    latex:*:pdf)
        tex=${PDFLATEX:-pdflatex};;
    texinfo:*:dvi)
        # MetaPost also uses the TEX environment variable.  If the user
        # has set TEX=latex for that reason, don't bomb out.
        case $TEX in
          *latex) tex=tex;; # don't bother trying to find etex
               *) tex=$TEX
        esac;;
    texinfo:*:pdf) tex=$PDFTEX;;

    *) error 1 "$out_lang not supported for $in_lang";;
  esac

  # do the special catcode trick for ~ in filenames only for Texinfo,
  # not LaTeX.
  if test x"$in_lang" = xtexinfo && test $catcode_special = maybe; then
    catcode_special=true
  else
    catcode_special=false
  fi

  # Beware of aux files in subdirectories that require the
  # subdirectory to exist.
  case $in_lang:$tidy in
    latex:true)
       sed -n 's|^[ ]*\\include{\(.*\)/.*}.*|\1|p' "$in_input" |
       sort -u |
       while read d
       do
         ensure_dir "$work_build/$d"
       done
       ;;
  esac

  # Note that this will be used via an eval: quote properly.
  local cmd="$tex"

  # If possible, make TeX report error locations in GNU format.
  if $line_error; then
    if test "${tex_help:+set}" != set; then
      # Go to a temporary directory to try --help, since old versions that
      # don't accept --help will generate a texput.log.
      tex_help_dir=$t2ddir/tex_help
      ensure_dir "$tex_help_dir"
      tex_help=`cd "$tex_help_dir" >&6 && $tex --help </dev/null 2>&1 || true`
    fi
    # The mk program and perhaps others want to parse TeX's
    # original error messages.
    case $tex_help in
      *file-line-error*) cmd="$cmd --file-line-error";;
    esac
  fi

  # Tell TeX about TCX file, if specified.
  test -n "$translate_file" && cmd="$cmd --translate-file=$translate_file"

  # Tell TeX to make source specials (for backtracking from output to
  # source, given a sufficiently smart editor), if specified.
  test -n "$src_specials" && cmd="$cmd $src_specials"

  # Tell TeX to allow running external executables
  test -n "$shell_escape" && cmd="$cmd $shell_escape"

  # Tell TeX to be batch if requested.
  if $batch; then
    # \batchmode does not show terminal output at all, so we don't
    # want that.  And even in batch mode, TeX insists on having input
    # from the user.  Close its stdin to make it impossible.
    cmd="$cmd </dev/null '${escape}nonstopmode'"
  fi

  # we'd like to handle arbitrary input file names, especially
  # foo~bar/a~b.tex, since Debian likes ~ characters.
  if $catcode_special; then
    # $normaltilde is just to reduce line length in this source file.
    # The idea is to define \normaltilde as a catcode other ~ character,
    # then make the active ~ be equivalent to that, instead of the plain
    # TeX tie.  Then when the active ~ appears in the filename, it will
    # be expanded to itself, as far as \input will see.  (This is the
    # same thing that texinfo.tex does in general, BTW.)
    normaltilde="${escape}catcode126=12 ${escape}def${escape}normaltilde{~}"
    cmd="$cmd '$normaltilde${escape}catcode126=13 ${escape}let~\normaltilde '"
  fi
  # Other special (non-active) characters could be supported by
  # resetting their catcodes to other on the command line and changing
  # texinfo.tex to initialize everything to plain catcodes.  Maybe someday.

  # append the \input command.
  cmd="$cmd '${escape}input'"

  # TeX's \input does not (easily or reliably) support whitespace
  # characters or other special characters in file names.  Our intensive
  # use of absolute file names makes this worse: the enclosing directory
  # names may include white spaces.  Improve the situation using a
  # symbolic link to the filename in the current directory, in tidy mode
  # only.  Do not alter in_input.
  #
  # The filename is almost always tokenized using plain TeX conventions
  # (the exception would be if the user made a texinfo.fmt file).  Not
  # all the plain TeX special characters cause trouble, but there's no
  # harm in making the link.
  #
  case $tidy:`func_dirname "$in_input"` in
    true:*["$space$tab$newline\"#\$%\\^_{}~"]*)
      _run_tex_file_name=`basename "$in_input"`
      if test ! -f "$_run_tex_file_name"; then
        # It might not be a file, clear it.
        run rm -f "$_run_tex_file_name"
        run ln -s "$in_input"
      fi
      cmd="$cmd '$_run_tex_file_name'"
      ;;

    *)
      cmd="$cmd '$in_input'"
      ;;
  esac

  verbose "$0: Running $cmd ..."
  if eval "$cmd" >&5; then
    case $out_lang in
      dvi | pdf ) move_to_dest "$in_noext.$out_lang";;
    esac
  else
    error 1 "$tex exited with bad status, quitting."
  fi
}

# run_bibtex ()
# -------------
# Run bibtex on current file.
# - If its input (AUX) exists.
# - If some citations are missing (LOG contains `Citation').
#   or the LOG complains of a missing .bbl
#
# Don't try to be too smart:
#
# 1. Running bibtex only if the bbl file exists and is older than
# the LaTeX file is wrong, since the document might include files
# that have changed.
#
# 3. Because there can be several AUX (if there are \include's),
# but a single LOG, looking for missing citations in LOG is
# easier, though we take the risk to match false messages.
run_bibtex ()
{
  case $in_lang in
    latex)   bibtex=${BIBTEX:-bibtex};;
    texinfo) return;;
  esac

  # "Citation undefined" is for LaTeX, "Undefined citation" for btxmac.tex.
  # The no .aux && \bibdata test is also for btxmac, in case it was the
  # first run of a bibtex-using document.  Otherwise, it's possible that
  # bibtex would never be run.
  if test -r "$in_noext.aux" \
     && test -r "$in_noext.log" \
     && ((grep 'Warning:.*Citation.*undefined' "$in_noext.log" \
          || grep '.*Undefined citation' "$in_noext.log" \
          || grep 'No file .*\.bbl\.' "$in_noext.log") \
          || (grep 'No \.aux file' "$in_noext.log" \
              && grep '^\\bibdata' "$in_noext.aux")) \
        >&6 2>&1; \
  then
    for f in `generated_files_get "$in_noext" bibaux_file_p`
    do
      run $bibtex "$f"
    done
  fi
}

# run_index ()
# ------------
# Run texindex (or makeindex or texindy) on current index files.  If
# they already exist, and after running TeX a first time the index
# files don't change, then there's no reason to run TeX again.  But we
# won't know that if the index files are out of date or nonexistent.
run_index ()
{
  local index_files
  index_files=`generated_files_get $in_noext index_file_p`
  test -n "$index_files" ||
    return 0

  : ${MAKEINDEX:=makeindex}
  : ${TEXINDEX:=texindex}
  : ${TEXINDY:=texindy}

  local index_file
  local index_noext
  case $in_lang:$latex2html:`out_lang_tex` in
    latex:tex4ht:html)
      for index_file in $index_files
      do
        index_noext=`noext "$index_file"`
        run tex \
            '\def\filename{{'"$index_noext"'}{idx}{4dx}{ind}}
             \input idxmake.4ht'
        run $MAKEINDEX -o $index_noext.ind $index_noext.4dx
      done
      ;;

    latex:*)
      if $TEXINDY --version >&6 2>&1; then
        run $TEXINDY $index_files
      else
        run $MAKEINDEX $index_files
      fi
      ;;

    texinfo:*)
      run $TEXINDEX $index_files
      ;;
  esac
}


# run_tex4ht ()
# -------------
# Run the last two phases of TeX4HT: tex4ht extracts the HTML from the
# instrumented DVI file, and t4ht converts the figures and installs
# the files when given -d.
#
# Because knowing exactly which files are created is complex (in
# addition the names are not simple to compute), which makes it
# difficult to install the output files in a second step, it is much
# simpler to install directly the output files.
run_tex4ht ()
{
  case $in_lang:$latex2html:`out_lang_tex` in
    latex:tex4ht:html)
      : ${TEX4HT:=tex4ht} ${T4HT:=t4ht}
      run "$TEX4HT" "-f/$in_noext"
      # Do not remove the / after the destdir.
      run "$T4HT" "-d`destdir`/" "-f/$in_noext"
      ;;
  esac
}


# run_thumbpdf ()
# ---------------
run_thumbpdf ()
{
  if test `out_lang_tex` = pdf \
     && test -r "$in_noext.log" \
     && grep 'thumbpdf\.sty'  "$in_noext.log" >&6 2>&1; \
  then
    thumbpdf=${THUMBPDF:-thumbpdf}
    thumbcmd="$thumbpdf $in_dir/$in_noext"
    verbose "Running $thumbcmd ..."
    if $thumbcmd >&5; then
      run_tex
    else
      report "$thumbpdf exited with bad status." \
             "Ignoring its output."
    fi
  fi
}


# run_dvipdf FILE.dvi
# -------------------
# Convert FILE.dvi to FILE.pdf.
run_dvipdf ()
{
  # Find which dvi->pdf program is available.
  if test -z "$dvipdf"; then
    for i in "$DVIPDF" dvipdfmx dvipdfm dvipdf dvi2pdf dvitopdf;
    do
      if findprog $i; then
        dvipdf=$i
      fi
    done
  fi
  # These tools have varying interfaces, some 'input output', others
  # 'input -o output'.  They all seem to accept 'input' only,
  # outputting using the expected file name.
  run $dvipdf "$1"
  if test ! -f `echo "$1" | sed -e 's/\.dvi$/.pdf/'`; then
    error 1 "cannot find output file"
  fi
}

# run_tex_suite ()
# ----------------
# Run the TeX tools until a fix point is reached.
run_tex_suite ()
{
  # Move to the working directory.
  if $tidy; then
    verbose "cd $work_build"
    cd "$work_build" || exit 1
  fi

  # Count the number of cycles.
  local cycle=0

  while :; do
    # check for probably LaTeX loop (e.g. varioref)
    if test $cycle -eq "$max_iters"; then
      error 0 "Maximum of $max_iters cycles exceeded"
      break
    fi

    # report progress
    cycle=`expr $cycle + 1`
    verbose "Cycle $cycle for $command_line_filename"

    xref_files_save

    # We run bibtex first, because I can see reasons for the indexes
    # to change after bibtex is run, but I see no reason for the
    # converse.
    run_bibtex
    run_index
    run_core_conversion

    xref_files_changed || break
  done

  # If we were using thumbpdf and producing PDF, then run thumbpdf
  # and TeX one last time.
  run_thumbpdf

  # If we are using tex4ht, call it.
  run_tex4ht

  # Install the result if we didn't already (i.e., if the output is
  # dvipdf or ps).
  case $latex2html:$out_lang in
    *:dvipdf)
      run_dvipdf "$in_noext.`out_lang_tex`"
      move_to_dest "$in_noext.`out_lang_ext`"
      ;;
    *:ps)
      : ${DVIPS:=dvips}
      run $DVIPS -o "$in_noext.`out_lang_ext`" "$in_noext.`out_lang_tex`"
      move_to_dest "$in_noext.`out_lang_ext`"
      ;;
  esac

  cd_orig
}

## -------------------------------- ##
## TeX processing auxiliary tools.  ##
## -------------------------------- ##


# A sed script that preprocesses Texinfo sources in order to keep the
# iftex sections only.  We want to remove non TeX sections, and comment
# (with `@c _texi2dvi') TeX sections so that makeinfo does not try to
# parse them.  Nevertheless, while commenting TeX sections, don't
# comment @macro/@end macro so that makeinfo does propagate them.
# Unfortunately makeinfo --iftex --no-ifinfo doesn't work well enough
# (yet), makeinfo can't parse the TeX commands, so work around with sed.
#
# We assume that `@c _texi2dvi' starting a line is not present in the
# document.
#
comment_iftex=\
'/^@tex/,/^@end tex/{
  s/^/@c _texi2dvi/
}
/^@iftex/,/^@end iftex/{
  s/^/@c _texi2dvi/
  /^@c _texi2dvi@macro/,/^@c _texi2dvi@end macro/{
    s/^@c _texi2dvi//
  }
}
/^@ifnottex/,/^@end ifnottex/{
  s/^/@c (_texi2dvi)/
}
/^@ifinfo/,/^@end ifinfo/{
  /^@node/p
  /^@menu/,/^@end menu/p
  t
  s/^/@c (_texi2dvi)/
}
s/^@ifnotinfo/@c _texi2dvi@ifnotinfo/
s/^@end ifnotinfo/@c _texi2dvi@end ifnotinfo/'

# Uncommenting is simpler: remove any leading `@c texi2dvi'; repeated
# copies can sneak in via macro invocations.
uncomment_iftex='s/^@c _texi2dvi\(@c _texi2dvi\)*//'


# run_makeinfo ()
# ---------------
# Expand macro commands in the original source file using Makeinfo.
# Always use `end' footnote style, since the `separate' style
# generates different output (arguably this is a bug in -E).  Discard
# main info output, the user asked to run TeX, not makeinfo.
run_makeinfo ()
{
  test $in_lang = texinfo \
    || return 0

  # Unless required by the user, makeinfo expansion is wanted only
  # if texinfo.tex is too old.
  if $expand; then
    makeinfo=${MAKEINFO:-makeinfo}
  else
    # Check if texinfo.tex performs macro expansion by looking for
    # its version.  The version is a date of the form YEAR-MO-DA.
    # We don't need to use [0-9] to match the digits since anyway
    # the comparison with $txiprereq, a number, will fail with non
    # digits.
    # Run in a temporary directory to avoid leaving files.
    version_test_dir=$t2ddir/version_test
    ensure_dir "$version_test_dir"
    (
       cd "$version_test_dir"
       echo '\input texinfo.tex @bye' >txiversion.tex
       # Be sure that if tex wants to fail, it is not interactive:
       # close stdin.
       $TEX txiversion.tex </dev/null >txiversion.out 2>txiversion.err
    )
    if test $? != 0; then
      cat "$version_test_dir/txiversion.out"
      cat "$version_test_dir/txiversion.err" >&2
      error 1 "texinfo.tex appears to be broken, quitting."
    fi
    eval `sed -n 's/^.*\[\(.*\)version \(....\)-\(..\)-\(..\).*$/txiformat=\1 txiversion="\2\3\4"/p' "$version_test_dir/txiversion.out"`
    verbose "texinfo.tex preloaded as \`$txiformat', version is \`$txiversion' ..."
    if test "$txiprereq" -le "$txiversion" >&6 2>&1; then
      makeinfo=
    else
      makeinfo=${MAKEINFO:-makeinfo}
    fi
    # If TeX is preloaded, offer the user this convenience:
    if test "$txiformat" = Texinfo; then
      escape=@
    fi
  fi

  if test -n "$makeinfo"; then
    # in_src: the file with macros expanded.
    # Use the same basename to generate the same aux file names.
    work_src=$workdir/src
    ensure_dir "$work_src"
    in_src=$work_src/$in_base
    local miincludes
    miincludes=`list_prefix includes -I`
    verbose "Macro-expanding $command_line_filename to $in_src ..."
    # eval $makeinfo because it might be defined as something complex
    # (running missing) and then we end up with things like '"-I"',
    # and "-I" (including the quotes) is not an option name.  This
    # happens with gettext 0.14.5, at least.
    sed "$comment_iftex" "$command_line_filename" \
      | eval $makeinfo --footnote-style=end -I "$in_dir" $miincludes \
        -o /dev/null --macro-expand=- \
      | sed "$uncomment_iftex" >"$in_src"
    # Continue only if everything succeeded.
    if test $? -ne 0 \
       || test ! -r "$in_src"; then
      verbose "Expansion failed, ignored...";
    else
      in_input=$in_src
    fi
  fi
}

# insert_commands ()
# ------------------
# Used most commonly for @finalout, @smallbook, etc.
insert_commands ()
{
  if test -n "$textra"; then
    # _xtr.  The file with the user's extra commands.
    work_xtr=$workdir/xtr
    in_xtr=$work_xtr/$in_base
    ensure_dir "$work_xtr"
    verbose "Inserting extra commands: $textra"
    local textra_cmd
    case $in_lang in
      latex)   textra_cmd=1i;;
      texinfo) textra_cmd='/^@setfilename/a';;
      *)       error 1 "internal error, unknown language: $in_lang";;
    esac
    sed "$textra_cmd\\
$textra" "$in_input" >"$in_xtr"
    in_input=$in_xtr
  fi

  case $in_lang:$latex2html:`out_lang_tex` in
    latex:tex4ht:html)
      # _tex4ht.  The file with the added \usepackage{tex4ht}.
      work_tex4ht=$workdir/tex4ht
      in_tex4ht=$work_tex4ht/$in_base
      ensure_dir "$work_tex4ht"
      verbose "Inserting \\usepackage{tex4ht}"
      perl -pe 's<\\documentclass(?:\[.*\])?{.*}>
                 <$&\\usepackage[xhtml]{tex4ht}>' \
        "$in_input" >"$in_tex4ht"
      in_input=$in_tex4ht
      ;;
  esac
}

# run_recode ()
# -------------
# If this is a Texinfo file with a specified input encoding, and
# recode is available, then recode to plain 7 bit Texinfo.
run_recode ()
{
  local from
  local to

  if test $in_lang = texinfo; then
    pgm='s/^ *@documentencoding  *\([^ ][^ ]*\) *$/\1/
        t found
        d
        :found
        q'
    encoding=`sed -e "$pgm" "$in_input"`
    if $recode && test -n "$encoding" && findprog recode; then
      if test -n "$recode_from"; then
        from=$recode_from
        to=$encoding
      else
        from=$encoding
        to=$texinfo
      fi
      verbose "Recoding from $from to $to."
      # _rcd.  The Texinfo file recoded in 7bit.
      work_rcd=$workdir/recode
      in_rcd=$work_rcd/$in_base
      ensure_dir "$work_rcd"
      if recode "$encoding..$to" <"$in_input" >"$in_rcd" \
         && test -s "$in_rcd"; then
        in_input=$in_rcd
      else
        verbose "Recoding failed, using original input."
      fi
    fi
  fi
}

# compute_language FILENAME
# -------------------------
# Return the short string describing the language in which FILENAME
# is written: `texinfo' or `latex'.
compute_language ()
{
  # If the user explicitly specified the language, use that.
  # Otherwise, if the first line is \input texinfo, assume it's texinfo.
  # Otherwise, guess from the file extension.
  if test -n "$set_language"; then
    echo $set_language
  elif sed 1q "$1" | grep 'input texinfo' >&6; then
    echo texinfo
  else
    # Get the type of the file (latex or texinfo) from the given language
    # we just guessed, or from the file extension if not set yet.
    case $1 in
      *.ltx | *.tex | *.drv | *.dtx) echo latex;;
      *)                             echo texinfo;;
    esac
  fi
}


# run_hevea (MODE)
# ----------------
# Convert to HTML/INFO/TEXT.
#
# Don't pass `-noiso' to hevea: it's useless in HTML since anyway the
# charset is set to latin1, and troublesome in other modes since
# accented characters loose their accents.
#
# Don't pass `-o DEST' to hevea because in that case it leaves all its
# auxiliary files there too...  Too bad, because it means we will need
# to handle images some day.
run_hevea ()
{
  local hevea="${HEVEA:-hevea}"
  local run_hevea="$hevea"

  case $1 in
    html) ;;
    text|info) run_hevea="$run_hevea -$1";;
    *) error 1 "run_hevea: invalid argument: $1";;
  esac

  # Compiling to the tmp directory enables to preserve a previous
  # successful compilation.
  run_hevea="$run_hevea -fix -O -o '$out_base'"
  run_hevea="$run_hevea `list_prefix includes -I` -I '$orig_pwd' "
  run_hevea="$run_hevea '$in_input'"

  if $debug; then
    run_hevea="$run_hevea -v -v"
  fi

  verbose "running $run_hevea"
  if eval "$run_hevea" >&5; then
    # hevea leaves trailing white spaces, this is annoying.
    case $1 in text|info)
      perl -pi -e 's/[ \t]+$//g' "$out_base"*;;
    esac
    case $1 in
    html|text) move_to_dest "$out_base";;
    info) # There can be foo.info-1, foo.info-2 etc.
               move_to_dest "$out_base"*;;
    esac
  else
    error 1 "$hevea exited with bad status, quitting."
  fi
}


# run_core_conversion ()
# ----------------------
# Run the TeX (or HeVeA).
run_core_conversion ()
{
  case $in_lang:$latex2html:`out_lang_tex` in
    *:dvi|*:pdf|latex:tex4ht:html)
        run_tex;;
    latex:*:html|latex:*:text|latex:*:info)
        run_hevea $out_lang;;
    *)
        error 1 "invalid input/output combination: $in_lang/$out_lang";;
  esac
}


# compile ()
# ----------
# Run the full compilation chain, from pre-processing to installation
# of the output at its expected location.
compile ()
{
  # Source file might include additional sources.
  # We want `.:$orig_pwd' before anything else.  (We'll add `.:' later
  # after all other directories have been turned into absolute paths.)
  # `.' goes first to ensure that any old .aux, .cps,
  # etc. files in ${directory} don't get used in preference to fresher
  # files in `.'.  Include orig_pwd in case we are in clean build mode, where
  # we have cd'd to a temp directory.
  common="$orig_pwd$path_sep$in_dir$path_sep"
  #
  # If we have any includes, put those at the end.
  # Keep a final path_sep to get the default (system) TeX directories included.
  txincludes=`list_infix includes $path_sep`
  test -n "$txincludes" && common="$common$txincludes$path_sep"
  #
  for var in $tex_envvars; do
    eval val="\$common\$${var}_orig"
    # Convert relative paths to absolute paths, so we can run in another
    # directory (e.g., in clean build mode, or during the macro-support
    # detection). ".:" is added here.
    val=`absolute_filenames "$val"`
    eval $var="\"$val\""
    export $var
    eval verbose \"$var=\'\$${var}\'\"
  done

  # --expand
  run_makeinfo

  # --command, --texinfo
  insert_commands

  # --recode
  run_recode

  # Run until a fix point is reached.
  run_tex_suite
}


# remove FILES
# ------------
remove ()
{
  verbose "Removing" "$@"
  rm -rf "$@"
}


# mostly_clean
# ------------
# Remove auxiliary files and directories.  Changes the current directory.
mostly_clean ()
{
  cd_orig
  set X "$t2ddir"
  shift
  $tidy || {
    local log="$work_build/$in_noext.log"
    set X ${1+"$@"} "$log" `generated_files_get "$work_build/$in_noext"`
    shift
  }
  remove ${1+"$@"}
}


# cleanup ()
# ----------
# Remove what should be removed according to options.
# Called at the end of each compilation cycle, and at the end of
# the script.  Changes the current directory.
cleanup ()
{
  case $build_mode in
    local) cd_orig; remove "$t2ddir";;
    clean) mostly_clean;;
    tidy)  ;;
  esac
}



## ---------------------- ##
## Command line parsing.  ##
## ---------------------- ##

# Push a token among the arguments that will be used to notice when we
# ended options/arguments parsing.
# Use "set dummy ...; shift" rather than 'set - ..." because on
# Solaris set - turns off set -x (but keeps set -e).
# Use ${1+"$@"} rather than "$@" because Digital Unix and Ultrix 4.3
# still expand "$@" to a single argument (the empty string) rather
# than nothing at all.
arg_sep="$$--$$"
set dummy ${1+"$@"} "$arg_sep"; shift

# 
# Parse command line arguments.
while test x"$1" != x"$arg_sep"; do

  # Handle --option=value by splitting apart and putting back on argv.
  case "$1" in
    --*=*)
      opt=`echo "$1" | sed -e 's/=.*//'`
      val=`echo "$1" | sed -e 's/[^=]*=//'`
      shift
      set dummy "$opt" "$val" ${1+"$@"}; shift
      ;;
  esac

  # This recognizes --quark as --quiet.  Oh well.
  case "$1" in
    -@ ) escape=@;;
    -~ ) catcode_special=false;;
    # Silently and without documentation accept -b and --b[atch] as synonyms.
    -b | --batch) batch=true;;
         --build)      shift; build_mode=$1;;
         --build-dir)  shift; build_dir=$1; build_mode=tidy;;
    -c | --clean) build_mode=clean;;
    -D | --debug) debug=true;;
    -e | -E | --expand) expand=true;;
    -h | --help) usage;;
    -I)   shift; list_concat_dirs includes "$1";;
    -l | --lang | --language) shift; set_language=$1;;
    --mostly-clean) action=mostly-clean;;
    --no-line-error) line_error=false;;
    --max-iterations) shift; max_iters=$1;;
    -o | --out  | --output)
      shift
      # Make it absolute, just in case we also have --clean, or whatever.
      oname=`absolute "$1"`;;

    # Output formats.
    -O|--output-format) shift; out_lang_set "$1";;
       --dvi|--dvipdf|--html|--info|--pdf|--ps|--text)
       out_lang_set `echo "x$1" | sed 's/^x--//'`;;

    -p) out_lang_set pdf;;
    -q | -s | --quiet | --silent) quiet=true; batch=true;;
    -r | --recode) recode=true;;
    --recode-from) shift; recode=true; recode_from="$1";;
    --src-specials) src_specials=--src-specials;;
    --shell-escape) shell_escape=--shell-escape;;  
    --tex4ht) latex2html=tex4ht;;
    -t | --texinfo | --command ) shift; textra="$textra\\
"`echo "$1" | sed 's/\\\\/\\\\\\\\/g'`;;
    --translate-file ) shift; translate_file="$1";;
    --tidy) build_mode=tidy;;
    -v | --vers*) version;;
    -V | --verb*) verb=true;;
    --) # What remains are not options.
      shift
      while test x"$1" != x"$arg_sep"; do
        set dummy ${1+"$@"} "$1"; shift
        shift
      done
      break;;
    -*)
      error 1 "Unknown or ambiguous option \`$1'." \
              "Try \`--help' for more information."
      ;;
    *) set dummy ${1+"$@"} "$1"; shift;;
   esac
   shift
done
# Pop the token
shift

# $tidy:  compile in a t2d directory.
# $clean: remove all the aux files.
case $build_mode in
  local) clean=false; tidy=false;;
  tidy)  clean=false; tidy=true;;
  clean) clean=true;  tidy=true;;
      *) error 1 "invalid build mode: $build_mode";;
esac

# Interpret remaining command line args as filenames.
case $# in
 0)
  error 2 "Missing file arguments." "Try \`--help' for more information."
  ;;
 1) ;;
 *)
  if test -n "$oname"; then
    error 2 "Can't use option \`--output' with more than one argument."
  fi
  ;;
esac


# We can't do much without tex.
#
if findprog ${TEX:-tex}; then :; else cat <<EOM
You don't have a working TeX binary (${TEX:-tex}) installed anywhere in
your PATH, and texi2dvi cannot proceed without one.  If you want to use
this script, you'll need to install TeX (if you don't have it) or change
your PATH or TEX environment variable (if you do).  See the --help
output for more details.

For information about obtaining TeX, please see http://www.tug.org.  If
you happen to be using Debian, you can get it with this command:
  apt-get install tetex-bin
EOM
  exit 1
fi


# We want to use etex (or pdftex) if they are available, and the user
# didn't explicitly specify.  We don't check for elatex and pdfelatex
# because (as of 2003), the LaTeX team has asked that new distributions
# use etex by default anyway.
#
# End up with the TEX and PDFTEX variables set to what we are going to use.
if test -z "$TEX"; then
  if findprog etex; then TEX=etex; else TEX=tex; fi
fi
#
if test -z "$PDFTEX"; then
  if findprog pdfetex; then PDFTEX=pdfetex; else PDFTEX=pdftex; fi
fi


# File descriptor usage:
# 0 standard input
# 1 standard output (--verbose messages)
# 2 standard error
# 3 some systems may open it to /dev/tty
# 4 used on the Kubota Titan
# 5 tools output (turned off by --quiet)
# 6 tracing/debugging (set -x output, etc.)


# Main tools' output (TeX, etc.) that TeX users are used to seeing.
#
# If quiet, discard, else redirect to the message flow.
if $quiet; then
  exec 5>/dev/null
else
  exec 5>&1
fi


# Enable tracing, and auxiliary tools output.
#
# Should be used where you'd typically use /dev/null to throw output
# away.  But sometimes it is convenient to see that output (e.g., from
# a grep) to aid debugging.  Especially debugging at distance, via the
# user.
if $debug; then
  exec 6>&1
  set -x
else
  exec 6>/dev/null
fi

# 

# input_file_name_decode
# ----------------------
# Decode COMMAND_LINE_FILENAME, and compute:
# - COMMAND_LINE_FILENAME clean of TeX commands
# - IN_DIR
#   The directory to the input file, possibly absolute if needed.
# - IN_DIR_ABS
#   The absolute directory of the input file.
# - IN_BASE
#   The input file base name (no directory part).
# - IN_NOEXT
#   The input file name without extensions (nor directory part).
# - IN_INPUT
#   Defaults to COMMAND_LINE_FILENAME, but might change if the
#   input is preprocessed (recode etc.).  With directory, possibly absolute.
input_file_name_decode ()
{
  # See if we are run from within AUC-Tex, in which case we are
  # passed `\input{FOO.tex}' or even `\nonstopmode\input{FOO.tex}'.
  case $command_line_filename in
    *\\nonstopmode*)
      batch=true;;
  esac
  case $command_line_filename in
    *\\input{*}*)
      # Let AUC-TeX error parser deal with line numbers.
      line_error=false
      command_line_filename=`\
        expr X"$command_line_filename" : X'.*input{\([^}]*\)}'`
      ;;
  esac

  # If the COMMAND_LINE_FILENAME is not absolute (e.g., --debug.tex),
  # prepend `./' in order to avoid that the tools take it as an option.
  echo "$command_line_filename" | LC_ALL=C $EGREP '^(/|[A-Za-z]:/)' >&6 \
  || command_line_filename="./$command_line_filename"

  # See if the file exists.  If it doesn't we're in trouble since, even
  # though the user may be able to reenter a valid filename at the tex
  # prompt (assuming they're attending the terminal), this script won't
  # be able to find the right xref files and so forth.
  test -r "$command_line_filename" ||
    error 1 "cannot read $command_line_filename, skipping."

  # Get the name of the current directory.
  in_dir=`func_dirname "$command_line_filename"`
  in_dir_abs=`absolute "$in_dir"`
  # In a clean build, we `cd', so get an absolute file name.
  if $tidy; then
    in_dir=$in_dir_abs
  fi

  # Strip directory part but leave extension.
  in_base=`basename "$command_line_filename"`
  # Strip extension.
  in_noext=`noext "$in_base"`

  # The normalized file name to compile.  Must always point to the
  # file to actually compile (in case of recoding, macro-expansion etc.).
  in_input=$in_dir/$in_base


  # Compute the output file name.
  if test x"$oname" != x; then
    out_name=$oname
  else
    out_name=$in_noext.`out_lang_ext`
  fi
  out_dir=`func_dirname "$out_name"`
  out_dir_abs=`absolute "$out_dir"`
  out_base=`basename "$out_name"`
  out_noext=`noext "$out_base"`
}


## -------------- ##
## TeXify files.  ##
## -------------- ##

for command_line_filename
do
  verbose "Processing $command_line_filename ..."

  input_file_name_decode

  # `texinfo' or `latex'?
  in_lang=`compute_language "$command_line_filename"`

  # An auxiliary directory used for all the auxiliary tasks involved
  # in compiling this document.
  case $build_dir in
      '' | . ) t2ddir=$out_noext.t2d ;;
      *) # Avoid collisions between multiple occurrences of the same
         # file, so depend on the output path.  Remove leading `./',
         # at least to avoid creating a file starting with `.!', i.e.,
         # an invisible file. The sed expression is fragile if the cwd
         # has active characters.  Transform / into ! so that we don't
         # need `mkdir -p'.  It might be something to reconsider.
         t2ddir=$build_dir/`echo "$out_dir_abs/$out_noext.t2d" |
             sed "s,^$orig_pwd/,,;s,^\./,,;s,/,!,g"`
  esac
  # Remove it at exit if clean mode.
  trap "cleanup" 0 1 2 15

  ensure_dir "$build_dir" "$t2ddir"

  # We will change directory, better work with an absolute path...
  t2ddir=`absolute "$t2ddir"`
  # Sometimes there are incompatibilities between auxiliary files for
  # DVI and PDF.  The contents can also change whether we work on PDF
  # and/or DVI.  So keep separate spaces for each.
  workdir=$t2ddir/`out_lang_tex`
  ensure_dir "$workdir"

  # _build.  In a tidy build, where the auxiliary files are output.
  if $tidy; then
    work_build=$workdir/build
  else
    work_build=.
  fi

  # _bak.  Copies of the previous auxiliary files (another round is
  # run if they differ from the new ones).
  work_bak=$workdir/bak

  # Make those directories.
  ensure_dir "$work_build" "$work_bak"

  case $action in
    compile)
      # Compile the document.
      compile
      cleanup
      ;;

    mostly-clean)
      mostly_clean
      ;;
  esac
done

verbose "done."
exit 0 # exit successfully, not however we ended the loop.


==> share/bin/texloganalyser <==
#!/usr/bin/env perl
# This is texloganalyser, for parsing of TeX logs
# Copyright (c) 2006-2009 Thomas van Oudenhove
# All rights reserved

# README - important notice:
# you should feed the first line with the path of your Perl executable
# (on *nix systems, the output of 'which perl')
#
# (this program works at least with perl 5.8.8)
# Getopt::Long MUST be installed on your system for this program to work

# License:
# Redistribution and use in source and binary forms, with or without
# modification, are permitted provided that the following conditions
# are met:
# 1. Redistributions of source code must retain the above copyright
#    notice, this list of conditions and the following disclaimer.
# 2. Redistributions in binary form must reproduce the above copyright
#    notice, this list of conditions and the following disclaimer in the
#    documentation and/or other materials provided with the distribution.
#
# THIS SOFTWARE IS PROVIDED BY THE AUTHOR AND CONTRIBUTORS ``AS IS''
# AND ANY EXPRESS OR IMPLIED WARRANTIES, INCLUDING, BUT NOT LIMITED
# TO, THE IMPLIED WARRANTIES OF MERCHANTABILITY AND FITNESS FOR A
# PARTICULAR PURPOSE ARE DISCLAIMED.  IN NO EVENT SHALL THE AUTHOR OR
# CONTRIBUTORS BE LIABLE FOR ANY DIRECT, INDIRECT, INCIDENTAL,
# SPECIAL, EXEMPLARY, OR CONSEQUENTIAL DAMAGES (INCLUDING, BUT NOT
# LIMITED TO, PROCUREMENT OF SUBSTITUTE GOODS OR SERVICES; LOSS OF
# USE, DATA, OR PROFITS; OR BUSINESS INTERRUPTION) HOWEVER CAUSED AND
# ON ANY THEORY OF LIABILITY, WHETHER IN CONTRACT, STRICT LIABILITY,
# OR TORT (INCLUDING NEGLIGENCE OR OTHERWISE) ARISING IN ANY WAY OUT
# OF THE USE OF THIS SOFTWARE, EVEN IF ADVISED OF THE POSSIBILITY OF
# SUCH DAMAGE.

use warnings;
use strict;
use Getopt::Long;
Getopt::Long::Configure ("bundling");

my $version = "0.7";
my $copyright = "2006-2010";
my $opt = {
	   help => '',
	   version => '',
	   h => '',
	   o => '',
	   u => '',
	   v => '',
	   p => '',
	   f => '',
	   w => '',
	   e => '',
	   i => '',
	   s => '',
	   r => '',
	   t => '',
	  };

GetOptions(
	   'help' => \$opt->{help},
	   'version' => \$opt->{version},
	   'h' => \$opt->{h},
	   'o' => \$opt->{o},
	   'u' => \$opt->{u},
	   'v' => \$opt->{v},
	   'p' => \$opt->{p},
	   'f' => \$opt->{f},
	   'w' => \$opt->{w},
	   'e' => \$opt->{e},
	   'i' => \$opt->{i},
	   't' => \$opt->{t},
	   's' => \$opt->{s},
	   'r' => \$opt->{r},
	  );

my $abstract = {
		warnings => 0,
	       };

my $texlog = $ARGV[-1];

die "Usage: $0 ".options()." <TeX log>\n"
  if (not defined $texlog and (not $opt->{help} and
			       not $opt->{version}));

if ($opt->{help}) {
  printhelp();
  exit();
}

if ($opt->{version}) {
  printversion();
  exit();
}

analyze();

sub analyze {
  my $line;
  my $output;
  my $test = 0;

  open my $source, "<", $texlog;
  while (defined ($line = <$source>)) {
    undef $output;
    # display summary and page numbers (default)
    summary($line);
    pagenumber($line);

    if ($opt->{e}) {
      if ($line =~ m/Here is how much/) {
	$test = 1;
	$output = "\n";
      }
      $output .= $line if $test;
    }
    # look for boxes warnings
    if ($opt->{o} and $opt->{h}) {
      $output = $line if ($line =~ m/\\hbox/ and
			   $line =~ m/Overfull/);
    } elsif ($opt->{u} and $opt->{h}) {
      $output = $line if ($line =~ m/\\hbox/ and
			   $line =~ m/Underfull/);
    } elsif ($opt->{o} and $opt->{v}) {
      $output = $line if ($line =~ m/\\vbox/ and
			   $line =~ m/Overfull/);
    } elsif ($opt->{u} and $opt->{v}) {
      $output = $line if ($line =~ m/\\vbox/ and
			   $line =~ m/Underfull/);
    } elsif ($opt->{h} and $opt->{v}) {
      $output = $line if ($line =~ m/\\vbox/ or
			   $line =~ m/\\hbox/);
    } elsif ($opt->{o} and $opt->{u}) {
      $output = $line if ($line =~ m/Underfull/ or
			   $line =~ m/Overfull/);
    } elsif ($opt->{h}) {
      $output = $line if ($line =~ m/\\hbox/);
    } elsif ($opt->{v}) {
      $output = $line if ($line =~ m/\\vbox/);
    } elsif ($opt->{o}) {
      $output = $line if ($line =~ m/Overfull/);
    } elsif ($opt->{u}) {
      $output = $line if ($line =~ m/Underfull/);
    }
    # look for LaTeX Font Info
    if ($opt->{f}) {
      $output = $line if ($line =~ m/Font Info/);
    }
    # packages infos
    if ($opt->{p}) {
      $output = $line if ($line =~ m/Package/);
    }
    # references warnings
    if ($opt->{r}) {
      $output = $line if ($line =~ m/Reference/ or
			  $line =~ m/Label(.*)/ and $1 =~ m/multiply defined/);
    }
    # TeX files used
    if ($opt->{t}) {
      scannedtexfiles($line, "tex");
    }
    # sty and cls files used
    if ($opt->{s}) {
      scannedfiles($line, "sty");
      scannedfiles($line, "cls");
    }
    # images (pdf, ps, jpg, png)
    if ($opt->{i}) {
      foreach my $t ('pdf', 'eps', 'ps', 'png', 'jpg') {
	scannedfiles($line, $t);
      }
    }
    # display all warnings
    if ($opt->{w}) {
      $output = $line if ($line =~ m/Warning/);
    }
    print "$output" if defined $output;
  }
  print "\n";
  print_abstract();
  close $source;
}

sub pagenumber {
  my $logline = shift;
  if ($logline =~ m/.*(\[[0-9]+)/) {
    print $1."]";
  }
}

sub scannedfiles {
  my ($logline, $filetype) = @_;
    if ($logline =~ m/^\((.*\.$filetype)/i) {
    print "(".$1.")";
  }
}

sub scannedtexfiles {
  my ($logline, $filetype) = @_;
  if ($logline =~ m/\((.*\.$filetype)/i) {
    print "(".$1.")";
  }
}

sub summary {
  my $line = shift;
  # prints log summary ()
  $abstract->{warnings} += 1 if ($line =~ m/Warning/);
}

sub options {
  my $stropts = "[";
  my $multopt = '';
  foreach my $k (sort keys %{$opt}) {
    if ($k eq 'version') {
      $stropts .= "--version|";
    } elsif ($k eq 'help') {
      $stropts .= "--help|";
    } else {
      $multopt .= $k;
    }
  }
  $stropts .= '-'.$multopt.']';
  return $stropts;
}

sub print_abstract {
  print "The log contained ".$abstract->{warnings}." warnings.\n";
}

sub printversion {
  print "This is texloganalyser, version $version\n";
  print "\t Copyright $copyright Thomas van Oudenhove\n";
}

sub printhelp {
  printversion();
  print "Usage: texloganalyser ".options()." <TeX log>\n";
  print "\t Displays selective infos of LaTeX logs\n";
  print "These flags may be used:\n";
  print "\t e: displays the end of the log\n";
  print "\t f: outputs the LaTeX Font Infos\n";
  print "\t h: outputs only warnings about horizontal boxes\n";
  print "\t i: displays 'images' (pdf, [e]ps, png, jpg) used\n";
  print "\t o: outputs only warnings about overfull boxes\n";
  print "\t p: outputs the LaTeX Packages infos\n";
  print "\t r: displays warnings about references\n";
  print "\t s: displays .sty and .cls files used\n";
  print "\t t: displays .tex files used\n";
  print "\t u: outputs only warnings about underfull boxes\n";
  print "\t v: outputs only warnings about vertical boxes\n";
  print "\t w: displays all Warnings\n";
  print "You may want to have a look at `perldoc texloganalyser`.\n";
}

__END__


=pod

=head1 texloganalyser Documentation

=head2 NAME

texloganalyser -- displays selective infos from TeX log files

=head2 SYNOPSIS

texloganalyser [-efhioprstuvw] tex_log_file

texloganalyser [--version]

texloganalyser [--help]

=head2 DESCRIPTION

Various options may be used to select which information from the TeX log you want to see/analyze (see next section). The default is to display only page numbers (page numbers are B<always> displayed).

=head2 OPTIONS

=over 1

=item B<--version>: displays version information.

=item B<--help>: displays help as a summary of options.

=item B<-e>: displays the end of the log, about the TeX's memory.

=item B<-f>: outputs the LaTeX Font Infos warnings and calculations.

=item B<-h>: outputs only warnings about horizontal boxes.

=item B<-i>: displays 'images' (pdf, [e]ps, png, jpg) used.

=item B<-o>: outputs only warnings about overfull boxes.

=item B<-p>: outputs the LaTeX Packages infos and warnings.

=item B<-r>: displays warnings about references (missing or multiply-defined).

=item B<-s>: displays .sty and .cls files used.

=item B<-t>: displays .tex files used. This option is B<very> useful when you parse logs of master files, to know in which file to look to correct errors/warnings.

=item B<-u>: outputs only warnings about underfull boxes.

=item B<-v>: outputs only warnings about vertical boxes.

=item B<-w>: displays all TeX, LaTeX and font Warnings.

=back

=head2 BUGS

None yet identified. However, the display should be improved...

=head2 HISTORY

This program was first released in 2006. Its purpose was to display selective information of my PhD's TeX log.

=head3 Changelog

=over

=item v0.7: bug patch for .tex files (-t option)

=item v0.6: default displays number of warnings (and page numbers).

  added option: references and label warnings

=item v0.5: use of GetOpt::Long and code cleaning

  added options: display of files used
  improved documentation

=item v0.4: added features and bugs corrections (options h, v, o and u)

=item v0.3: display of Warnings and last lines of the log

=item v0.2: display of "Font Info" and "Packages" added

=item v0.1: first version, displays only warnings about boxes

=back

=head2 AUTHORS

I<texloganalyser> is a program by Thomas van Oudenhove (L<vanouden@enstimac.fr>). Feel free to contact him for features requests or bugs.

=cut


==> share/bin/update-bib <==
#! /bin/sh

set -e

BIB_EXTERNALS="kernighan.bib richie.bib strategoxt.bib visser.bib"

fetch()
{
  local url=http://$1
  local bib=$2
  if test "x$bib" = x; then
      bib=$(basename "$1")
  fi
  wget "$url" -O "$bib"

  # Missing commas.
  perl -pi -e 's/(.\})$/\1,/g' "$bib"

  # Useless empty fields.
  perl -ni -e 'print unless /^\s*\w+\s*=\s*\{\},/' "$bib"
}

(
    cd bib
    chmod a+w $BIB_EXTERNALS
    fetch netlib.bell-labs.com/cm/cs/bib/bwk.bib kernighan.bib
    fetch cm.bell-labs.com/cm/cs/bib/dmr.bib richie.bib
    fetch buildfarm.st.ewi.tudelft.nl/releases/strategoxt/publications-unstable-latest/publications/strategoxt/strategoxt.bib
    perl -pi -e 's/Benoît/Beno{\^i}t/' strategoxt.bib

    fetch buildfarm.st.ewi.tudelft.nl/releases/strategoxt/publications-unstable-latest/publications/visser/visser.bib

    fetch tom.loria.fr/bibtex.php tom.bib
    # This one has actually html mark up.
    perl -ni -e 'print unless /^\s*</' tom.bib


    # Avoid accidental edition.
    chmod a-w $BIB_EXTERNALS
)


==> share/bin/update-cite <==
#! /usr/bin/perl -w

use strict;
use IO::File;
use File::Glob ':glob';
use Getopt::Long qw(GetOptions);

sub help ()
{
  print <<EOF;
Usage: $0 [OPTIONS] FILES

Update the (LaTeX) files citations to newer BibTeX keys.  A copy of
the original file is left with a ~ appended.

The BibTeX files are looked for in share.  They must have an oldkeys
entry listing the previous keys.  For instance:

\@Book{muchnick.97.advanced,
  oldkeys =      {Muchnick97, muchnick.97},
  ...

Options:
  -h, --help        Display this message and exit successfully
  -s, --share=DIR   Specify the path to the share directory [share]
EOF
  exit 0;
}

# Location of the share directory.
my $share = 'share';

# The sed program to update old cite keys.
my $updater = '';

# contents ($FILE_NAME)
# ---------------------
sub contents ($)
{
  my ($file) = @_;
  local $/;			# Turn on slurp-mode.
  my $f = new IO::File "< $file" or die "$file";
  my $contents = $f->getline or die "$file";
  $f->close;
  return $contents;
}

# Extend UPDATER given this FILE.
sub learn_from_bib ($)
{
  my ($file) = @_;
  my $fh = new IO::File $file;
  my $key;
  while ($_ = $fh->getline)
    {
      if (/^@\w+\{\s*(\S+?),$/)
	{
	  $key = $1;
	}
      elsif (/oldkeys\s*=\s*\{(.+?)\}/)
	{
	  my $older = '\Q' . join ('\E|\Q', split (/,\s*/, $1)) . '\E';
	  $updater = $updater
	    # Unfortunately look-behinds must be fixed width.
	    . "s!(?<=[{, ])(?:${older})(?=[.}])!$key!gm;\n";
	}
    }
  print "$updater\n";
}

# Backup this FILE.
sub backup ($)
{
  my ($from) = @_;
  my $SIMPLE_BACKUP_SUFFIX = $ENV{'SIMPLE_BACKUP_SUFFIX'} || '~';
  my $to = "$from$SIMPLE_BACKUP_SUFFIX";
  use File::Copy;
  move ($from, $to)
    or die "cannot backup $from: $!";
  return $to;
}

# Update this FILE.
sub update ($)
{
  my ($file) = @_;
  my $backup = backup ($file);

  # Update.
  $_ = contents ($backup);
  eval $updater;
  my $out = new IO::File ">$file" or die;
  print $out $_;
}

# Parse ARGV, return the list of files to update.
sub parse_options ()
{
  use Getopt::Long;
  Getopt::Long::config ("bundling", "pass_through");
  Getopt::Long::GetOptions
    (
     's|share=s' => \$share,
     'h|help'    => sub { help; },
    )
    or die;

  foreach my $arg (@ARGV)
    {
      if ($arg =~ /^-./)
	{
	  print STDERR "$0: unrecognized option `$arg'\n";
	  print STDERR "Try `$0 --help' for more information.\n";
	  exit (1);
	}
    }
  return @ARGV;
}

my @tex = parse_options ();
learn_from_bib ($_)
  foreach bsd_glob ('share/bib/*.bib');
update ($_)
  foreach @tex;

### Setup "GNU" style for perl-mode and cperl-mode.
## Local Variables:
## perl-indent-level: 2
## perl-continued-statement-offset: 2
## perl-continued-brace-offset: 0
## perl-brace-offset: 0
## perl-brace-imaginary-offset: 0
## perl-label-offset: -2
## cperl-indent-level: 2
## cperl-brace-offset: 0
## cperl-continued-brace-offset: 0
## cperl-label-offset: -2
## cperl-extra-newline-before-brace: t
## cperl-merge-trailing-else: nil
## cperl-continued-statement-offset: 2
## End:


==> share/bin/vaucanson-g-to-tikz <==
#! /usr/bin/perl

# Usage: vaucanson-g-to-tikz FILES
#
# Convert all the FILES to use TikZ instead of Vaucanson-G.  Copies of
# the original FILES are left as *.bak.
#
# The main motivation for such a conversion is to get rid of PSTricks
# which (i) has portability issues bw versions, (ii) requires passing
# via DVI.  TikZ does not have these limitations.
#
# In THL the whole lecture notes + exams were converted using this
# script, and the following preamble:
# 
# \usepackage{pgf,tikz}
# \usetikzlibrary{automata}
# \usetikzlibrary{arrows}
# \tikzstyle{automaton}=[shorten >=1pt,
#                        node distance=2cm,
#                        pos=.4,
#                        >=stealth',
#                        initial text=]
# \tikzstyle{accepting}=[accepting by arrow]
# 
# %% Support more angles for initial/accepting states.
# %% From Alexandre Duret-Lutz.
# \tikzoption{initial angle}{\tikzaddafternodepathoption{\def\tikz@initial@angle{#1}}}
# \tikzoption{accepting angle}{\tikzaddafternodepathoption{\def\tikz@accepting@angle{#1}}}


# geo
# ---
sub geo ($)
{
    my ($geo) = @_;
    $geo =~ s/[\[\]]//g;
    # Forget about the case, so that we can convert LoopN, LoopS
    # etc. too.
    return lc $geo;
}

# geo2rel ($direction)
# --------------------
# Convert NSEW in the corresponding above/below etc.
sub geo2rel ($)
{
    my ($geo) = @_;
    my $res = "";
    $geo = geo($geo);

    $res = "above" if $geo eq "n";
    $res = "below" if $geo eq "s";
    $res = "left"  if $geo eq "w";
    $res = "right" if $geo eq "e";

    $res;
}

# convert_state ($kind, $geo)
# ---------------------------
# $kind is Initial|Final
# $geo is (n|s|...)
# Helper for \State etc. conversion.
sub convert_state ($$)
{
    my ($kind, $geo) = @_;
    my $res = "";
    $res = "initial" if $kind eq "Initial";
    $res = "accepting" if $kind eq "Final";

    if (defined $geo)
    {
	$geo = geo($geo);

	# Handle NSEW.
	my $rel = geo2rel($geo);
	$res .= " $rel"
	    if $rel ne '';

	# Yes, we need to repeat: "accepting, accepting angle = XX".
	$res .= ", $res angle = 45"  if $geo eq "ne";
	$res .= ", $res angle = 135" if $geo eq "nw";
	$res .= ", $res angle = 225" if $geo eq "sw";
	$res .= ", $res angle = 315" if $geo eq "se";
    }
    print STDERR "@_ -> $res\n";
    return $res;
}

# convert_vcpicture ($prefix, $contents)
# --------------------------------------
# $contents is the contents of a {VCPicture} environment, and $prefix
# is everything that is between the beginning of the line that
# contains the previous \VCDraw and the \begin{VCPicture}.  It is used
# both to compute the output indentation, and to see if there are
# prefix-commands such as \MediumScale.
#
# Returns a TikZ environment.
sub convert_vcpicture ($$)
{
    my ($prefix, $input) = @_;
    local $_ = $input;

    # The prefix may contain request to change the scale.  The
    # following is extracted from the soureces of Vaucanson-G:
    #
    # \newcommand{\LargeScale}{0.85}
    # \newcommand{\MediumScale}{0.6}
    # \newcommand{\SmallScale}{0.5}
    # \newcommand{\TinyScale}{0.42}
    print STDERR "                   Prefix: {$prefix}\n";

    my $scale = "";
    $scale = ", scale = 0.85" if $prefix =~ /LargePicture/;
    $scale = ", scale = 0.6"  if $prefix =~ /MediumPicture/;
    $scale = ", scale = 0.5"  if $prefix =~ /SmallPicture/;
    $scale = ", scale = 0.42" if $prefix =~ /TinyPicture/;

    # Gather initial/final states.

    # \Initial, \Final
    # ----------------
    # In Vaucanson the fact that a state is initial/final is separated
    # from the declaration of the state.  That's not the case in TikZ,
    # so first gather information about declared initial/final states.
    my %state;
    s{\\(Initial|Final)(\[.*?\])?\{(.*?)\}}
     {$state{$3} .= ", " . convert_state($1, $2);
      ""}ge;

    # \State, \StateVar
    # -----------------
    # StateVar means that the frame of the state can grow to cope
    # with large content.
    s{\\State(?:Var)?\[(.*?)\]\{(.*?)\}\{(.*?)\}}
     {\\node[state$state{$3}] ($3) at $2 {\$$1\$};\n}g;
    s{\\State(?:Var)?\{(.*?)\}\{(.*?)\}}
     {\\node[state$state{$2}] ($2) at $1 {};\n}g;

    # \EdgeL, \EdgeR
    # --------------
    # L means that the node information is on the left.
    # I know that TikZ supports above/below, I don't know about left/right.
    s{\\EdgeL\{(.*?)\}\{(.*?)\}\{(.*?)\}}
     {\\path[->] ($1) edge node[above] {\$$3\$} ($2);\n}g;
    s{\\EdgeR\{(.*?)\}\{(.*?)\}\{(.*?)\}}
     {\\path[->] ($1) edge node[below] {\$$3\$} ($2);\n}g;

    # \ArcL, \ArcR
    # --------------
    # The initial L changes the starting angle (Arc = 15 degre, LArc = 30).
    # The optional [pos] specifies the position of the label (defaults to .45).
    s{\\L?ArcL(?:\[.*?\])?\{(.*?)\}\{(.*?)\}\{(.*?)\}}
     {\\path[->] ($1) edge [bend left] node[above] {\$$3\$} ($2);\n}g;
    s{\\L?ArcR(?:\[.*?\])?\{(.*?)\}\{(.*?)\}\{(.*?)\}}
     {\\path[->] ($1) edge [bend right] node[above] {\$$3\$} ($2);\n}g;

    # \LoopX
    # ------
    my $rel;
    s{\\Loop([NSEW]*)(?:\[.*?\])?\{(.*?)\}\{(.*?)\}}
     {$rel = geo2rel($1);
      "\\path[->] ($2) edge [loop $rel] node[$rel] {\$$3\$} ($2);\n"}ge;

    # Check how much space there is in the prefix (before the \VCDraw).
    my $space = $prefix;
    $space =~ s/^(\s+).*/$1/;

    # Remove all the indentation, and reindent.
    s{^\s*}{  }gm;

    # Add the TikZ environment call, and indent.
    $_ = "\\begin{tikzpicture}[automaton$scale]\n$_\\end{tikzpicture}";
    s{^}{$space}gm;

    "% $prefix\n$_";
}


sub convert_file($)
{
    my ($file) = @_;
    my ($bak) = "$file.bak";
    rename ($file, $bak);
    use IO::File;
    my $in = new IO::File($bak);
    my $out = new IO::File(">$file");
    local $/ = undef;

    $_ = $in->getline;
    s{^([^\n]*)\\VCDraw\s*\{\s*\\begin\{VCPicture\}\{(.*?)\}(.*?)\\end\{VCPicture\}\}?}
     {convert_vcpicture($1, $3)}gesm;
    print $out $_;
}

for my $file (@ARGV)
{
    convert_file($file);
}


==> share/bin/xhtex <==
#! /bin/sh

# This file is part of tex4ht, but many distros
# (https://trac.macports.org/ticket/30270,
# http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=118090) forget to
# include it.  So just have your PATH _end_ with share/bin so that the
# mouseover option of tex4ht works.

        tex '\def\Link#1.a.b.c.{\expandafter\def\csname tex4ht\endcsname{\expandafter\def\csname tex4ht\endcsname{#1,xhtml}\input tex4ht.sty }}\def\HCode{\futurelet\HCode\HChar}\def\HChar{\ifx"\HCode\def\HCode"##1"{\Link##1}\expandafter\HCode\else\expandafter\Link\fi}\HCode '$2'.a.b.c.\input ' $1
        tex '\def\Link#1.a.b.c.{\expandafter\def\csname tex4ht\endcsname{\expandafter\def\csname tex4ht\endcsname{#1,xhtml}\input tex4ht.sty }}\def\HCode{\futurelet\HCode\HChar}\def\HChar{\ifx"\HCode\def\HCode"##1"{\Link##1}\expandafter\HCode\else\expandafter\Link\fi}\HCode '$2'.a.b.c.\input ' $1
        tex '\def\Link#1.a.b.c.{\expandafter\def\csname tex4ht\endcsname{\expandafter\def\csname tex4ht\endcsname{#1,xhtml}\input tex4ht.sty }}\def\HCode{\futurelet\HCode\HChar}\def\HChar{\ifx"\HCode\def\HCode"##1"{\Link##1}\expandafter\HCode\else\expandafter\Link\fi}\HCode '$2'.a.b.c.\input ' $1
        tex4ht -f/$1 -i~/tex4ht.dir/ht-fonts/$3
        t4ht -f/$1 $4 ## -d~/WWW/temp/ -m644

# Local Variables:
# mode: shell-script
# End:


==> share/styles/FinalStateVar.tex <==
%%%%% macro FinalStateVar %%%%%%%%%%%%%%%%%%%
\newcommand{\StateLineDblTemp}{0}
\newcommand{\FinalStateVar}[3][]%
    {\ifStateLineDbl
        \renewcommand{\StateLineDblTemp}{1}
     \else
        \renewcommand{\StateLineDblTemp}{0}
     \fi
     \StateLineDouble
     \StateVar[#1]{#2}{#3}
     \ifthenelse{\equal{\StateLineDblTemp}{0}}%
                {\StateLineSimple}{}%
    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> share/styles/VCPref-beamer.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  This files contains initial values
%  of Vaucanson's parameter for slides
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%
% State aspect
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetStateLabelColor{Sepia}
\SetStateLabelScale{1.7}
\SetStateLineWidth{2pt}
\SetStateLineColor{blue}
\SetStateFillColor{blue}%Cyan}
\FixDimState{solid}{YellowOrange}{1}{YellowOrange}{white}
%%%%%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetEdgeLabelColor{green}%OliveGreen}
\SetEdgeLabelScale{1.7}
\SetEdgeLineWidth{1.2pt}
\SetEdgeLineColor{brown}%Mahogany}
\FixDimEdge{dashed}{1.2}{Apricot}{Apricot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\LargeScale}{1.5}
\renewcommand{\MediumScale}{1.16}
\renewcommand{\SmallScale}{0.92}
\renewcommand{\TinyScale}{0.75}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\HideFrame
\HideGrid
\MediumPicture
\HideName
\RigidLabel
\FullState
\MediumState


==> share/styles/VCPref-gastex.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  This files contains initial values
%  of Vaucanson's parameter
%  Modify it to create your own style
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
% State aspect
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetStateLabelColor{black}		%% color
\SetStateLabelScale{1}		%% float
\SetStateLineStyle{solid}		%% aspect (other values: none, dashed, dotted)
\SetStateLineWidth{.14mm}		%% length
\SetStateLineColor{black}		%% color
\SetStateFillStatus{none}		%% aspect
\SetStateFillColor{black}		%% color
\FixDimState{solid}{gray}{1}{gray}{white}  %% LineStyle,LineColor,LineCoef (*\StateLineWidth),LabelColor,FillColor
\FixStateLineDouble{2}{5}               %% Double style: \StateLineDblCoef, \StateLineDblSep, coeffs applied to \StateLineWidth
%%%%%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetEdgeLabelColor{black}		%% color
\SetEdgeLabelScale{1}		        %% float
\SetEdgeLineStyle{solid}		%% aspect
\SetEdgeLineWidth{.14mm}			%% length
\SetEdgeLineColor{black}		%% color
\SetArcAngle{17}			%% int (degree)
\SetLArcAngle{30}			%% int (degree)
\SetArcCurvature{0.7}			%% float
\SetEdgeOffset{0pt}                     %% length
\SetArcOffset{1pt}			%% length
\SetLoopOffset{0pt}			%% length
\renewcommand{\ForthBackEdgeOffset}{5}	%% float : coef*\EdgeLineWidth -> offset
\FixDimEdge{solid}{1.2}{gray}{gray}     %% LineStyle,LineCoef,LineColor,LabelColor
\FixEdgeBorder{2}{white}		%% int,color : coef*\EdgeLineWidth -> width of border
\FixEdgeLineDouble{1.5}{2}		%% float : coefs*\EdgeLineWidth -> (width of lines, distance)
%%%%%%%%%%%%%%
% ZZ aspect
%%%%%%%%%%%%%%
\setlength{\ZZSize}{.9cm}		% length : apparent diameter
\renewcommand{\ZZShape}{0.5}		% coef: opening of the ZZ
\SetZZLineWidth{1.7}			% float
\renewcommand{\TransLabelZZCoef}{0.6}	% float : coef*\ZZSize -> distance added for labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\LargeScale}{1.2}        %float : argument of a \scalebox
\renewcommand{\MediumScale}{1}        %float
\renewcommand{\SmallScale}{.7}		%float
\renewcommand{\TinyScale}{0.5}		%float
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% State parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\MediumStateDiameter}{.8cm}		%length
\setlength{\SmallStateDiameter}{.6cm}		%length
\setlength{\LargeStateDiameter}{1.2cm}		%length
\setlength{\VerySmallStateDiameter}{.3cm}	%length
\renewcommand{\VSStateLineCoef}{.6}    		%float : coef *\StateLineWidth
\renewcommand{\StateDblDimen}{outer}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\ArrowOnMediumState}{1}		%float : coef *\StateDiameter for size of initial and final arrows
\renewcommand{\ArrowOnSmallState}{1} 		%float
\renewcommand{\ArrowOnLargeState}{1}		%float
\renewcommand{\ArrowOnVerySmallState}{5} 	%float
\renewcommand{\LoopOnMediumState}{7}		%float : curvature
\renewcommand{\LoopOnSmallState}{9} 		%float
\renewcommand{\LoopOnLargeState}{5.5} 		%float
\renewcommand{\LoopOnVariableState}{4.5} 		%float
\renewcommand{\CLoopOnMediumState}{8}		%float
\renewcommand{\CLoopOnSmallState}{12}		%float
\renewcommand{\CLoopOnLargeState}{6}		%float
\renewcommand{\CLoopOnVariableState}{5.2}		%float
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\EdgeLabelPosit}{.5}   %per cent (use \Fix..LabelPosit with values in [10;90])
\renewcommand{\EdgeLabelRevPosit}{.5}
\renewcommand{\ArcLabelPosit}{.5}
\renewcommand{\ArcLabelRevPosit}{.5}
\renewcommand{\LArcLabelPosit}{.5}
\renewcommand{\LArcLabelRevPosit}{.5}
\renewcommand{\LoopLabelPosit}{.5}
\renewcommand{\LoopLabelRevPosit}{.5}
\renewcommand{\CLoopLabelPosit}{.5}
\renewcommand{\CLoopLabelRevPosit}{.5}
\renewcommand{\InitStateLabelPosit}{.10}
\renewcommand{\InitStateLabelRevPosit}{.90}
\renewcommand{\FinalStateLabelPosit}{.90}
\renewcommand{\FinalStateLabelRevPosit}{.10}
\SetEdgeArrowWidth{1.03mm}			%width of the edge arrow
\SetEdgeArrowLengthCoef{1.37}				%float : coef*\EdgeArrowSizeDim length of EA
\setlength{\EdgeDblArrowWidth}{1.3mm}		%width : size of EA for double transitions
\renewcommand{\EdgeDblArrowLengthCoef}{1.09}	% 
\SetEdgeArrowInsetCoef{0}				%float : coef*\EdgeArrowSizeDim
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetVCDirectory{}        %default dir=current dir
\HideFrame
\HideGrid
\MediumPicture
\HideName
\RigidLabel
\FullState				%% PlainState
\MediumState


==> share/styles/VCPref-main.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  This files contains initial values
%  of Vaucanson's parameter
%  Modify it to create your own style
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
% State aspect
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetStateLabelColor{black}		%% color
\SetStateLabelScale{1.7}		%% float
\SetStateLineStyle{solid}		%% aspect (other values: none, dashed, dotted)
\SetStateLineWidth{1.8pt}		%% length
\SetStateLineColor{black}		%% color
\SetStateFillStatus{solid}		%% aspect
\SetStateFillColor{white}		%% color
\FixDimState{solid}{gray}{1}{gray}{white}  %% LineStyle,LineColor,LineCoef (*\StateLineWidth),LabelColor,FillColor
\FixStateLineDouble{0.6}{0.4}               %% Double style: \StateLineDblCoef, \StateLineDblSep, coeffs applied to \StateLineWidth
%%%%%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetEdgeLabelColor{black}		%% color
\SetEdgeLabelScale{1.7}		        %% float
\SetEdgeLineStyle{solid}		%% aspect
\SetEdgeLineWidth{1pt}			%% length
\SetEdgeLineColor{black}		%% color
\SetArcAngle{15}			%% int (degree)
\SetLArcAngle{30}			%% int (degree)
\SetArcCurvature{0.8}			%% float
\SetEdgeOffset{0pt}                     %% length
\SetArcOffset{1pt}			%% length
\SetLoopOffset{0pt}			%% length
\renewcommand{\ForthBackEdgeOffset}{5}	%% float : coef*\EdgeLineWidth -> offset
\FixDimEdge{solid}{1.2}{gray}{gray}     %% LineStyle,LineCoef,LineColor,LabelColor
\FixEdgeBorder{2}{white}		%% int,color : coef*\EdgeLineWidth -> width of border
\FixEdgeLineDouble{0.5}{0.6}		%% float : coefs*\EdgeLineWidth -> (width of lines, distance)
%%%%%%%%%%%%%%
% ZZ aspect
%%%%%%%%%%%%%%
\setlength{\ZZSize}{.9cm}		% length : apparent diameter
\renewcommand{\ZZShape}{0.5}		% coef: opening of the ZZ
\SetZZLineWidth{1.7}			% float
\renewcommand{\TransLabelZZCoef}{0.6}	% float : coef*\ZZSize -> distance added for labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\LargeScale}{0.85}        %float : argument of a \scalebox
\renewcommand{\MediumScale}{0.6}        %float
\renewcommand{\SmallScale}{0.5}		%float
\renewcommand{\TinyScale}{0.42}		%float
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% State parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\MediumStateDiameter}{.9cm}		%length
\setlength{\SmallStateDiameter}{.6cm}		%length
\setlength{\LargeStateDiameter}{1.2cm}		%length
\setlength{\VerySmallStateDiameter}{.3cm}	%length
\renewcommand{\VSStateLineCoef}{.6}    		%float : coef *\StateLineWidth
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\ArrowOnMediumState}{1.5}		%float : coef *\StateDiameter for size of initial and final arrows
\renewcommand{\ArrowOnSmallState}{1.7} 		%float
\renewcommand{\ArrowOnLargeState}{1.3}		%float
\renewcommand{\ArrowOnVerySmallState}{5} 	%float
\renewcommand{\LoopOnMediumState}{7}		%float : curvature
\renewcommand{\LoopOnSmallState}{9.6} 		%float
\renewcommand{\LoopOnLargeState}{5.8} 		%float
\renewcommand{\LoopOnVariableState}{5.1} 		%float
\renewcommand{\CLoopOnMediumState}{8}		%float
\renewcommand{\CLoopOnSmallState}{12}		%float
\renewcommand{\CLoopOnLargeState}{6}		%float
\renewcommand{\CLoopOnVariableState}{5.2}		%float
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\EdgeLabelPosit}{.45}   %per cent (use \Fix..LabelPosit with values in [10;90])
\renewcommand{\EdgeLabelRevPosit}{.55}
\renewcommand{\ArcLabelPosit}{.40}
\renewcommand{\ArcLabelRevPosit}{.60}
\renewcommand{\LArcLabelPosit}{.40}
\renewcommand{\LArcLabelRevPosit}{.60}
\renewcommand{\LoopLabelPosit}{.25}
\renewcommand{\LoopLabelRevPosit}{.75}
\renewcommand{\CLoopLabelPosit}{.25}
\renewcommand{\CLoopLabelRevPosit}{.75}
\renewcommand{\InitStateLabelPosit}{.10}
\renewcommand{\InitStateLabelRevPosit}{.90}
\renewcommand{\FinalStateLabelPosit}{.90}
\renewcommand{\FinalStateLabelRevPosit}{.10}
\SetEdgeArrowWidth{5pt}		%length of the edge arrow
\SetEdgeArrowLengthCoef{1.4}		%float : coef*\EdgeArrowSizeDim width of EA
\setlength{\EdgeDblArrowWidth}{5.5pt}		%length : size of EA for double transitions
\renewcommand{\EdgeDblArrowLengthCoef}{1.7}	%int 
\SetEdgeArrowInsetCoef{0.1}			%float : coef*\EdgeArrowSizeDim
\SetEdgeArrowStyle{->}				%style (other styles : <-, |-|, -|,...)
\renewcommand{\EdgeRevArrowStyle}{<-}           %style for reverse transitions
\renewcommand{\StateDimen}{outer}		%side of the boundary of states that corresponds to the diameter
\renewcommand{\StateDblDimen}{middle}		%idem for states with double line (values: outer, middle or inner)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetVCDirectory{}        %default dir=current dir
\HideFrame
\HideGrid
\MediumPicture
\HideName
\RigidLabel
\FullState				%% PlainState
\MediumState


==> share/styles/VCPref-slides.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  This files contains initial values
%  of Vaucanson's parameter for slides
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%
% State aspect
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetStateLabelColor{Sepia}
\SetStateLabelScale{1.7}
\SetStateLineWidth{2pt}
\SetStateLineColor{blue}
\SetStateFillColor{Cyan}
\FixDimState{solid}{YellowOrange}{1}{YellowOrange}{white}
%%%%%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetEdgeLabelColor{OliveGreen}
\SetEdgeLabelScale{1.7}
\SetEdgeLineWidth{1.2pt}
\SetEdgeLineColor{Mahogany}
\FixDimEdge{dashed}{1.2}{Apricot}{Apricot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\LargeScale}{1.5}
\renewcommand{\MediumScale}{1.16}
\renewcommand{\SmallScale}{0.92}
\renewcommand{\TinyScale}{0.75}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\HideFrame
\HideGrid
\MediumPicture
\HideName
\RigidLabel
\FullState
\MediumState


==> share/styles/VCpatch-pstricks-1-10.tex <==
\renewenvironment{VCPicture}[2][0]%
  {\settoheight{\VertShiftH}{$\{$}%
   \settodepth{\VertShiftD}{$\{$}%
   \setlength{\VertShift}{.5\VertShiftD-.5\VertShiftH}%
   \begin{pspicture}[shift=#1]#2%
   \ifVCFrame \FrameStyle \psframe#2\fi%
   \ifVCGrid \FrameStyle\GridStyle \psgrid#2\fi}%
  {\RstState\RstEdge%
   \end{pspicture}}


==> share/styles/Vaucanson-G.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                           
%                  Vaucanson-G.tex                      
%                                                           
%       Automata drawer based on Pstricks
%                       
%                V 0.2 - 03/05/09
%  modification of StateVar
%  Chg*LabelScale is relative w.r.t Set*LabelScale
%  Chg Vaucanson to Vaucanson-G
%                V 0.3 - 03/09/10
%  VCPref-main is no more required to initialize VC-G
%                V 0.3.1 - 06/07/06
%  Remove ``\ifVCName\makebox[0pt][r]{\fbox{{\scriptsize #2}}}\fi%''
%  in the definition of \VCDraw
%                V 0.3.2 - 06/07/06
%  Replace \renewcommand{\StateLabelCol} by \renewcommand{\StateLabelColor}
%  in \SetStateLabelColor
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Commands for geometric constructions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% constants 
\newcommand{\SQRTwo}{0.717}
\newcommand{\SQRThree}{1.732}
\newcommand{\GoldMean}{0.618}
\newcommand{\GoldMeanI}{1.618}
\newcommand{\SQRGoldMeanI}{1.272}
\newcommand{\Vaucanson}{\textsc{V$\overline{\text{au}}$C%
\raisebox{.3ex}{$\underline{\text{an}}$}S$\overline{\text{on}}$-G}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label drawing macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Separator in compound labels (eg \IOL{input}{output})
\newcommand{\IOL}[2]{#1\!\mid\! #2}
%%% Stacked labels
\newcommand{\StackTwoLabels}[2]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ #2 \end{array}%
   \renewcommand{\arraystretch}{1.333}}
\newcommand{\StackThreeLabels}[3]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ #2 \\ #3 \end{array}%
   \renewcommand{\arraystretch}{1.333}}
%%% Stacked labels with +
\newcommand{\StackTwoLabelsP}[2]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ + \\ #2 \end{array}%
   \renewcommand{\arraystretch}{1.333}}
\newcommand{\StackThreeLabelsP}[3]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ + \\ #2 \\ + \\ #3 \end{array}% 
   \renewcommand{\arraystretch}{1.333}}
%%% Lined up labels (with +)
\newcommand{\LineTwoLabelsP}[2]{#1 + #2} 
\newcommand{\LineThreeLabelsP}[3]{#1 + #2 + #3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\LargeScale}{0.85}
\newcommand{\MediumScale}{0.6}
\newcommand{\SmallScale}{0.5}
\newcommand{\TinyScale}{0.42}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% State parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Size = StateDiameter
%%% The preset sizes are given in cm, and not in "psunits".
%%% This allows to use different scales for the whole figure 
%%% and for the "drawing grid".
\newlength{\MediumStateDiameter}
\newlength{\SmallStateDiameter}
\newlength{\LargeStateDiameter}
\newlength{\VerySmallStateDiameter}
\setlength{\MediumStateDiameter}{.9cm}
\setlength{\SmallStateDiameter}{.6cm}
\setlength{\LargeStateDiameter}{1.2cm}
\setlength{\VerySmallStateDiameter}{.3cm}
%%% Border line = StateLine
\newlength{\StateLineWidth}        % width
\setlength{\StateLineWidth}{1.8pt}
\newcommand{\StateLineStyle}{solid} % style
\newcommand{\StateLineColor}{black}
\newif\ifStateLineDbl \StateLineDblfalse 
\newcommand{\StateLineDblCoef}{0.6} 
\newcommand{\StateLineDblSep}{0.4} 
\newcommand{\VSStateLineCoef}{.6} % coef. for very small state
%%% State background and label
\newcommand{\StateFillStatus}{solid} 
\newcommand{\StateFillColor}{white}
\newcommand{\StateLabelColor}{black}
\newcommand{\StateLabelScale}{1.7}
\newcommand{\SmallStateFillStatus}{solid} %
\newcommand{\SmallStateFillColor}{white} %
   % As they have usually no labels it useful
   % to have a coloring facility for the "SmallState"
%%%  Dimmed states (e.g. for non accessible states)
\newcommand{\DimStateLineStyle}{solid} 
\newcommand{\DimStateLineCoef}{1} % 
\newcommand{\DimStateLineColor}{gray}
\newcommand{\DimStateLabelColor}{gray}
\newcommand{\DimStateFillColor}{white}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge drawing parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% line
\newlength{\EdgeLineWidth}
\setlength{\EdgeLineWidth}{1pt}
\newcommand{\EdgeLineStyle}{solid}
\newif\ifEdgeLineDbl \EdgeLineDblfalse 
%\newcommand{\EdgeLineDblStatus}{false} 
\newcommand{\EdgeLineDblCoef}{0.5} 
\newcommand{\EdgeLineDblSep}{0.6} 
\newcommand{\EdgeLineColor}{black}
% arrow
\newlength{\EdgeArrowWidth}\setlength{\EdgeArrowWidth}{5pt}
\newlength{\EdgeDblArrowWidth}\setlength{\EdgeDblArrowWidth}{5.5pt}
\newcommand{\EdgeArrowLengthCoef}{1.4}
\newcommand{\EdgeDblArrowLengthCoef}{1.7}
\newcommand{\EdgeArrowInset}{0.1}
\newcommand{\EdgeArrowStyle}{->}
\newcommand{\EdgeRevArrowStyle}{<-}
% border
\newcommand{\EdgeLineBorderCoef}{2}
\newcommand{\EdgeLineBorderColor}{white}
% label
\newcommand{\EdgeLabelColor}{black}
\newcommand{\EdgeLabelScale}{1.7}
%%% Dimmed edges 
\newcommand{\DimEdgeLineCoef}{1.2} 
\newcommand{\DimEdgeLineStyle}{solid} 
\newcommand{\DimEdgeLineColor}{gray}
\newcommand{\DimEdgeLabelColor}{gray}
%%% Zigzag edges parameter
\newlength{\ZZSize}
\setlength{\ZZSize}{.9cm}%\MediumStateDiameter
\newcommand{\ZZShape}{0.5}
\newcommand{\ZZLineWidth}{1.7}% coefficient multiplicateur
\newcommand{\TransLabelZZCoef}{0.6}% coefficient multiplicateur
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge geometric parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Edge 
\newlength{\EdgeOffset}
\setlength{\EdgeOffset}{0pt}
\newcommand{\ForthBackEdgeOffset}{5}% coef
% Arc parameters
\newcommand{\VaucArcAngle}{15}
\newcommand{\VaucArcCurvature}{0.8}
\newlength{\VaucArcOffset}
\setlength{\VaucArcOffset}{1pt}
% Large Arc parameters
\newcommand{\VaucLArcAngle}{30}
\newcommand{\VaucLArcCurvature}{0.8}
\newlength{\LoopOffset}\setlength{\LoopOffset}{0pt}
\newlength{\LoopVarOffset}\setlength{\LoopVarOffset}{.7pt}
\newcommand{\LoopAngle}{30}
\newcommand{\CLoopAngle}{22}
\newcommand{\LoopVarAngle}{28}
% Size of loops (depending on the size of the state)
\newcommand{\LoopOnMediumState}{7}
\newcommand{\LoopOnSmallState}{9.6} 
\newcommand{\LoopOnLargeState}{5.8} 
\newcommand{\LoopOnVariableState}{5.1} 
\newcommand{\LoopOnVerySmallState}{15} 
\newcommand{\CLoopOnMediumState}{8}
\newcommand{\CLoopOnSmallState}{12}
\newcommand{\CLoopOnLargeState}{6}
\newcommand{\CLoopOnVariableState}{5.2}
%\newcommand{\CLoopOnVerySmallState}{14} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label parameters --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% label distance from transition
\newlength{\TransLabelSep}\setlength{\TransLabelSep}{3.5pt}
% label position on transitions
\newcommand{\EdgeLabelPosit}{.45}\newcommand{\EdgeLabelRevPosit}{.55}
\newcommand{\ArcLabelPosit}{.4}\newcommand{\ArcLabelRevPosit}{.6}
\newcommand{\LArcLabelPosit}{.4}\newcommand{\LArcLabelRevPosit}{.6}
\newcommand{\LoopLabelPosit}{.25}\newcommand{\LoopLabelRevPosit}{.75}
\newcommand{\CLoopLabelPosit}{.25}\newcommand{\CLoopLabelRevPosit}{.75}
% label position on initial-final arrow
\newcommand{\InitStateLabelPosit}{.1}\newcommand{\InitStateLabelRevPosit}{.9}
\newcommand{\FinalStateLabelPosit}{.9}\newcommand{\FinalStateLabelRevPosit}{.1}
%%% Size of initial and final arrow
% the size is relative to the diameter
% and the coefficient varies with the diameter
\newcommand{\ArrowOnStateCoef}{}
\newcommand{\ArrowOnMediumState}{1.5}
\newcommand{\ArrowOnSmallState}{1.7} 
\newcommand{\ArrowOnLargeState}{1.3}
\newcommand{\ArrowOnVerySmallState}{5} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Shift for aligned labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\VertShiftH} \settoheight{\VertShiftH}{$\{$}
\newlength{\VertShiftD} \settodepth{\VertShiftD}{$\{$}
\newlength{\VertShift}
\setlength{\VertShift}{.5\VertShiftD-.5\VertShiftH}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% flags 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifVCFrame
\newcommand{\HideFrame}{\VCFramefalse}
\newcommand{\ShowFrame}{\VCFrametrue}
\newif\ifVCGrid
\newcommand{\HideGrid}{\VCGridfalse}
\newcommand{\ShowGrid}{\VCGridtrue}
\newif\ifVCRigidLabel
\newcommand{\RigidLabel}{\VCRigidLabeltrue}
\newcommand{\SwivelLabel}{\VCRigidLabelfalse}
\newif\ifVCStateLabelBaseLine
\newcommand{\AlignedLabel}{\VCStateLabelBaseLinetrue}
\newcommand{\FloatingLabel}{\VCStateLabelBaseLinefalse}
\HideFrame
\HideGrid
\RigidLabel
\FloatingLabel
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   style for the frame around the picture
\psset{unit=1cm}
\newpsstyle{VaucFrameStyle}{arrows=-,framesep=0pt,%                   
                     linewidth=0.6pt,linecolor=black,%
                                         linestyle=solid,%
                                         doubleline=false,%
                                         fillcolor=white,fillstyle=none,%
                                         cornersize=relative,framearc=0}
\newcommand{\FrameStyle}{\psset{style=VaucFrameStyle}}
\newpsstyle{VaucGridStyle}{%
      gridwidth=0.6pt,griddots=10,subgriddiv=1,%
          gridlabels=7pt}
\newcommand{\GridStyle}{\psset{style=VaucGridStyle}}
% figure, vertically centered by default
% draw frame according to VCFrame flag
% Set the shift for aligned label w.r.t the current size of characters
\newenvironment{VCPicture}[2][.5]%
  {\settoheight{\VertShiftH}{$\{$}%
   \settodepth{\VertShiftD}{$\{$}%
   \setlength{\VertShift}{.5\VertShiftD-.5\VertShiftH}%
   \begin{pspicture}[#1]#2%
   \ifVCFrame \FrameStyle \psframe#2\fi%
   \ifVCGrid \FrameStyle\GridStyle \psgrid#2\fi}%
  {\RstState\RstEdge%
   \end{pspicture}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scaling matters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% The "sizes" (for states) and the "line widths" are given 
%%% as "lengthes" in a fixed unit (cm or pt), whereas the positions 
%%% are supposed to be given in "psunits".
%%% This allows to use different scaling parameters 
%%% for the whole figure and for the "drawing grid".
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scaling commands
\newcommand{\VCScale}{0.6}% Global scale parameter
\newcommand{\VCGridScale}{1}% Global scale parameter
% 
\newcommand{\FixVCScale}[1]{\renewcommand{\VCScale}{#1}}% v4 pour 
%                                              % cause de syntaxe
\newcommand{\LargePicture}{\FixVCScale{\LargeScale}}
\newcommand{\MediumPicture}{\FixVCScale{\MediumScale}}
\newcommand{\SmallPicture}{\FixVCScale{\SmallScale}}
\newcommand{\TinyPicture}{\FixVCScale{\TinyScale}}
%%% Grid scale commands
% \newcommand{\VCGridScale}{}% Grid scale parameter
% 
\newcommand{\FixVCGridScale}[1]{\renewcommand{\VCGridScale}{#1}}% v4 pour 
% "grid unit"
%%%%% Typical figure would look like
%   \scalebox{\VCScale}{%
%     \begin{VCPicture}{(x0,y0)(x1,y1)}
%     %  figure description
%     \end{VCPicture}%
%    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Using a special directory for the figure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\VCDirectory}{}
\newcommand{\SetVCDirectory}[1]{\renewcommand{\VCDirectory}{#1}}
% flag for printing the name of the figure file
\newif\ifVCName
\newcommand{\HideName}{\VCNamefalse}
\newcommand{\ShowName}{\VCNametrue}
\newcommand{\VCDraw}[2][\VCGridScale]{%
\psset{unit=#1cm}%
\scalebox{\VCScale}{#2}%
\psset{unit=1cm}}%
\newcommand{\VCCall}[2][\VCGridScale]{%
\psset{unit=#1cm}%
\ifVCName\makebox[0pt][r]{\fbox{{\scriptsize #2}}}\fi%
\scalebox{\VCScale}{\input{\VCDirectory #2}}%
\psset{unit=1cm}}%
%%% commands
\newcommand{\VCPut}[3][0]{\rput{#1}#2{#3}}% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% State internal parameters  --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\StateLineWid}
\setlength{\StateLineWid}{\StateLineWidth}
\newcommand{\StateLineSty}{\StateLineStyle} 
\newcommand{\StateLineCol}{\StateLineColor}
%\newcommand{\StateLineDblSta}{\StateLineDblStatus}
\newcommand{\StateLineDblWid}{\StateLineDblWidth}
\newcommand{\StateLineDblSp}{\StateLineDblSep}
\newcommand{\StateFillCol}{\StateFillColor}
\newcommand{\StateFillSta}{\StateFillStatus} 
\newcommand{\StateLabelSca}{1}
\newcommand{\StateLabelCol}{\StateLabelColor}
\newcommand{\StateDimen}{outer}
\newcommand{\StateDblDimen}{middle}
%%%  Initial-final quality
\newcommand{\VCIFflag}{2}\newcommand{\VCIFflagtemp}{2}
\newcommand{\PlainState}%
  {\renewcommand{\VCIFflag}{0}\renewcommand{\VCIFflagtemp}{0}}
\newcommand{\FullState}%
  {\renewcommand{\VCIFflag}{2}\renewcommand{\VCIFflagtemp}{2}}
\newcommand{\IFState}{\renewcommand{\VCIFflag}{1}}
\newcommand{\IFXState}{\renewcommand{\VCIFflag}{2}}
\newcommand{\RstVCIF}{\renewcommand{\VCIFflag}{\VCIFflagtemp}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  State drawing style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% flag for hiding -- showing states (used for overlays in slides)
% the trick is to have two different styles and instead of 
% saving\restoring parameters
\newif\ifVCShowState
\newcommand{\HideState}{\VCShowStatefalse}
\newcommand{\ShowState}{\VCShowStatetrue}
\ShowState % initialisation
% the only difference between the two styles is the linestyle
\newpsstyle{VaucStateStyle}{framesep=0pt,%                   
         linewidth=\StateLineWid,linecolor=\StateLineCol,%
         linestyle=\StateLineSty,doubleline=false,%
         fillcolor=\StateFillCol,fillstyle=\StateFillSta,% 
         border=0pt,dimen=\StateDimen,%
         cornersize=relative,framearc=1,framesep=0pt}
\newpsstyle{VaucStateDblStyle}{framesep=0pt,%                   
         linewidth=\StateLineDblCoef\StateLineWid,linecolor=\StateLineCol,%
         linestyle=\StateLineSty,doubleline=true,doublesep=\StateLineDblSep\StateLineWid,%
         fillcolor=\StateFillCol,fillstyle=\StateFillSta,% 
         border=0pt,dimen=\StateDblDimen,%
         cornersize=relative,framearc=1,framesep=0pt}
\newpsstyle{VaucHiddenStateStyle}{framesep=0pt,%                   
         linewidth=\StateLineWid,linecolor=\StateLineCol,%
         linestyle=none,%
         fillcolor=\StateFillCol,fillstyle=none,% 
         border=0pt,dimen=outer,%
         cornersize=relative,framearc=1,framesep=0pt}
\newcommand{\StateStyle}{%
   \ifVCShowState%
         \ifStateLineDbl\psset{style=VaucStateDblStyle}\else\psset{style=VaucStateStyle}\fi%
   \else\psset{style=VaucHiddenStateStyle}\fi}
\newcommand{\VaucStateRBLabel}[1]{%
    \textcolor{\StateLabelCol}{\scalebox{\StateLabelSca}{\scalebox{\StateLabelScale}{\rput[B]{0}(0,\VertShift){$ #1 $}}}}}%
\newcommand{\VaucStateLabel}[1]%
    {\ifVCShowState%
        \ifVCRigidLabel%
           \ifVCStateLabelBaseLine%
                 \textcolor{\StateLabelCol}{\scalebox{\StateLabelSca}{\scalebox{\StateLabelScale}{\rput[B]{*0}(0,\VertShift){$ #1 $}}}}%
           \else
                 \textcolor{\StateLabelCol}{\scalebox{\StateLabelSca}{\scalebox{\StateLabelScale}{\rput{*0}(0,0){$ #1 $}}}}%
           \fi
        \else
                 \textcolor{\StateLabelCol}{\scalebox{\StateLabelSca}{\scalebox{\StateLabelScale}{$ #1 $}}}%
        \fi
     \else%
                 \textcolor{white}{\scalebox{\StateLabelSca}{\scalebox{\StateLabelScale}{$ #1 $}}}%
     \fi}
\newcommand{\VCPutStateLabel}[2]%
    {\rput#1{\scalebox{\StateLabelSca}{$ #2 $}}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  State parameter changing and setting macros 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% line style
\newcommand{\ChgStateLineStyle}[1]{\renewcommand{\StateLineSty}{#1}}
\newcommand{\RstStateLineStyle}{\ChgStateLineStyle{\StateLineStyle}}
\newcommand{\SetStateLineStyle}[1]%
   {\renewcommand{\StateLineStyle}{#1}\RstStateLineStyle}%
%%% doubleline status
\newcommand{\StateLineDouble}{\StateLineDbltrue}
\newcommand{\StateLineSimple}{\StateLineDblfalse}
%%% line width
\newcommand{\ChgStateLineWidth}[1]{\setlength{\StateLineWid}{#1\StateLineWidth}}%  
\newcommand{\RstStateLineWidth}{\ChgStateLineWidth{1}}%
\newcommand{\SetStateLineWidth}[1]% ATTN the parameter is a length
   {\setlength{\StateLineWidth}{#1}\RstStateLineWidth}
%%% line color
\newcommand{\ChgStateLineColor}[1]{\renewcommand{\StateLineCol}{#1}}
\newcommand{\RstStateLineColor}{\ChgStateLineColor{\StateLineColor}}
\newcommand{\SetStateLineColor}[1]%
   {\renewcommand{\StateLineColor}{#1}\RstStateLineColor}
%%% background fill status
\newcommand{\ChgStateFillStatus}[1]{\renewcommand{\StateFillSta}{#1}}
\newcommand{\RstStateFillStatus}{\ChgStateFillStatus{\StateFillStatus}}
\newcommand{\SetStateFillStatus}[1]% 
    {\renewcommand{\StateFillStatus}{#1}\RstStateFillStatus}
%%% backgroud color
\newcommand{\ChgStateFillColor}[1]{\renewcommand{\StateFillCol}{#1}}
\newcommand{\RstStateFillColor}{\ChgStateFillColor{\StateFillColor}}
\newcommand{\SetStateFillColor}[1]% 
    {\renewcommand{\StateFillColor}{#1}\RstStateFillColor}%
%%% label color
\newcommand{\ChgStateLabelColor}[1]{\renewcommand{\StateLabelCol}{#1}}
\newcommand{\RstStateLabelColor}{\ChgStateLabelColor{\StateLabelColor}}
\newcommand{\SetStateLabelColor}[1]%
    {\renewcommand{\StateLabelColor}{#1}\RstStateLabelColor}
%%% label scale
\newcommand{\ChgStateLabelScale}[1]{\renewcommand{\StateLabelSca}{#1}}
\newcommand{\RstStateLabelScale}{\ChgStateLabelScale{1}}
\newcommand{\SetStateLabelScale}[1]%
   {\renewcommand{\StateLabelScale}{#1}\RstStateLabelScale}
\newcommand{\FixStateLineDouble}[2]{%
    \renewcommand{\StateLineDblCoef}{#1}%
    \renewcommand{\StateLineDblSep}{#2}}
\newcommand{\FixDimState}[5]{%
    \renewcommand{\DimStateLineStyle}{#1}%
    \renewcommand{\DimStateLineCoef}{#3}%
    \renewcommand{\DimStateLineColor}{#2}%
    \renewcommand{\DimStateLabelColor}{#4}%
    \renewcommand{\DimStateFillColor}{#5}}%
%%% restoring state parameters
\newcommand{\RstState}{%
   \RstStateLineStyle\RstStateLineWidth%
   \RstStateLineColor%
   \RstStateFillStatus\RstStateFillColor%
   \RstStateLabelColor\RstStateLabelScale}%
%%% establishing the dimmed style
\newcommand{\DimState}{%
    \ChgStateLineStyle{\DimStateLineStyle}%
    \ChgStateLineWidth{\DimStateLineCoef}%
    \ChgStateLineColor{\DimStateLineColor}%
        \ChgStateFillColor{\DimStateFillColor}%
    \ChgStateLabelColor{\DimStateLabelColor}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% State drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% preparation
\newlength{\StateDiam}
\newlength{\VaucAOS}\newlength{\VaucAOSdiag}
%%%  A flag to remember the current size of state
\newcommand{\StateSizeFlag}{}
%
\newcommand{\SetAOS}{%
   \setlength{\VaucAOS}{\ArrowOnStateCoef\StateDiam}%
   \setlength{\VaucAOSdiag}{\SQRTwo\VaucAOS}}
%% parameter for variable width states
\newlength{\VariableStateIntDiam}
\newlength{\VariableStateWidth}
\newlength{\VariableStateITPos}
\newcommand{\SetStateIntDiam}{%
   \setlength{\VariableStateIntDiam}{\StateDiam}%
   \addtolength{\VariableStateIntDiam}{-2\StateLineWid}%
}%
% Loop parameters
\newcommand{\LoopSize}{}\newcommand{\LoopSi}{}
\newcommand{\LoopVarSize}{}\newcommand{\LoopVarSi}{}
\newcommand{\CLoopSize}{}\newcommand{\CLoopSi}{}
%
\newcommand{\ChgLoopSize}[1]{\renewcommand{\LoopSi}{#1}}
\newcommand{\RstLoopSize}{\ChgLoopSize{\LoopSize}}
\newcommand{\SetLoopSize}[1]%
   {\renewcommand{\LoopSize}{#1}\RstLoopSize}
%
\newcommand{\ChgCLoopSize}[1]{\renewcommand{\CLoopSi}{#1}}
\newcommand{\RstCLoopSize}{\ChgCLoopSize{\CLoopSize}}
\newcommand{\SetCLoopSize}[1]%
   {\renewcommand{\CLoopSize}{#1}\RstCLoopSize}
%
\newcommand{\ChgLoopVarSize}[1]{\renewcommand{\LoopVarSi}{#1}}
\newcommand{\RstLoopVarSize}{\ChgLoopVarSize{\LoopVarSize}}
\newcommand{\SetLoopVarSize}[1]%
   {\renewcommand{\LoopVarSize}{#1}\RstLoopVarSize}
%
%%% setting state diameter -- internal command
\newcommand{\SetStateDiam}[4]{%
   \setlength{\StateDiam}{#1}%
   \renewcommand{\ArrowOnStateCoef}{#2}%
   \SetLoopSize{#3}%
   \SetLoopVarSize{#3}%
   \SetCLoopSize{#4}%
   \SetAOS\SetStateIntDiam}
%%% setting state diameter -- external command
\newcommand{\FixStateDiameter}[1]%  v4 pour cause de syntaxe
   {\setlength{\StateDiam}{#1}\SetStateIntDiam \SetAOS}
%%%
\newcommand{\MediumState}%
   {\SetStateDiam{\MediumStateDiameter}{\ArrowOnMediumState}%
         {\LoopOnMediumState}{\CLoopOnMediumState}%
                  \renewcommand{\StateSizeFlag}{0}}
\newcommand{\SmallState}%
   {\SetStateDiam{\SmallStateDiameter}{\ArrowOnSmallState}%
         {\LoopOnSmallState}{\CLoopOnSmallState}%
                  \renewcommand{\StateSizeFlag}{1}}
\newcommand{\LargeState}%
   {\SetStateDiam{\LargeStateDiameter}{\ArrowOnLargeState}%
         {\LoopOnLargeState}{\CLoopOnLargeState}%
                  \renewcommand{\StateSizeFlag}{2}}
%
\newcommand{\RstStateSize}%
  {\ifthenelse{\equal{\StateSizeFlag}{0}}%
              {\MediumState}%
              {\ifthenelse{\equal{\StateSizeFlag}{1}}%
                              {\SmallState}{\LargeState}}}%
%%% Initialization
\MediumState
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\VaucState}[3][{}]%
   {\rput#2{%
      \Cnode[radius=.5\StateDiam](0,0){#3}%
          \ifVCShowState%
      \nput[labelsep=-.5\StateDiam]{0}{#3}%
        {\makebox[0pt]{\VaucStateLabel{#1}}}%
      \fi%
      \ifthenelse{\equal{\VCIFflag}{0}}{}{%
        \pnode(-\VaucAOS,0){#3w}\pnode(\VaucAOS,0){#3e}%
        \pnode(0,\VaucAOS){#3n}\pnode(0,-\VaucAOS){#3s}%
           \ifthenelse{\equal{\VCIFflag}{1}}{}{%
          \pnode(-\VaucAOSdiag,\VaucAOSdiag){#3nw}%
           \pnode(\VaucAOSdiag,\VaucAOSdiag){#3ne}%
           \pnode(-\VaucAOSdiag,-\VaucAOSdiag){#3sw}%
           \pnode(\VaucAOSdiag,-\VaucAOSdiag){#3se}%
                   }%
            }%
     }%
}
%
\newcommand{\State}[3][{}]{\StateStyle\VaucState[#1]{#2}{#3}}
%
\newcommand{\FinalState}[3][{}]%
   {\psset{style=VaucStateDblStyle}\VaucState[#1]{#2}{#3}}
%%% ecological commands   
\newcommand{\StateIF}[3][{}]{\IFState\State[#1]{#2}{#3}\RstVCIF}%
\newcommand{\StateIFX}[3][{}]{\IFXState\State[#1]{#2}{#3}\RstVCIF}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Very Small State   
\newcommand{\VSState}[2]%
    {\renewcommand{\ArrowOnStateCoef}{\ArrowOnVerySmallState}%
         \FixStateDiameter{\VerySmallStateDiameter}%
     \ChgStateLineWidth{\VSStateLineCoef}%
         \State{#1}{#2}%
         \RstStateLineWidth\RstStateSize}% mod 020201
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% white brace, of no width, used to place the label vertically
%\newlength{\BraceLength}
\newcommand{\WB}{%
   \textcolor{white}{\{\!\!\!}}%
\newcommand{\HS}{}
\newlength{\ExtraSpace}
\setlength{\ExtraSpace}{1em}
%
\newcommand{\StateVar}[3][]%
 {\StateStyle %
  \settowidth{\VariableStateWidth}{\scalebox{\StateLabelSca}{\scalebox{\StateLabelScale}{$#1$}}}%
  \addtolength{\VariableStateWidth}{\ExtraSpace}
  \ifthenelse{\lengthtest{\VariableStateWidth < \VariableStateIntDiam}}%
        {\setlength{\VariableStateWidth}{\VariableStateIntDiam}}{}%
  \setlength{\VariableStateITPos}{\ArrowOnStateCoef\StateDiam}%
  \addtolength{\VariableStateITPos}{0.5\VariableStateWidth}%
  \addtolength{\VariableStateITPos}{-0.5\StateDiam}%
  \rput#2{\pnode(\VariableStateITPos,0){#3e}%
          \pnode(-\VariableStateITPos,0){#3w}%
          \pnode(0,\ArrowOnStateCoef\StateDiam){#3n}%
          \pnode(0,-\ArrowOnStateCoef\StateDiam){#3s}}%
  \rput#2{\rnode{#3}{\psframebox{\protect\rule[-.5\VariableStateIntDiam]{0pt}{\VariableStateIntDiam}\protect\rule{\VariableStateWidth}{0pt}}}}
  \rput#2{\VaucStateRBLabel{#1}}%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\VarLoopOn}{\ChgLoopOffset{\LoopVarOff}%
   \ChgLoopSize{\LoopVarSi}%
   \ChgLoopAngle{\LoopVarAng}}
\newcommand{\VarLoopOff}{\RstLoopOffset \RstLoopSize \RstLoopAngle}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge drawing parameters  --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\EdgeLineWid}
\setlength{\EdgeLineWid}{\EdgeLineWidth}
\newcommand{\EdgeLineSty}{\EdgeLineStyle}
\newcommand{\EdgeLineCol}{\EdgeLineColor}
% label
\newcommand{\EdgeLabelSca}{1}
\newcommand{\EdgeLabelCol}{\EdgeLabelColor}
% arrow
\newlength{\EdgeArrowSZDim}
\setlength{\EdgeArrowSZDim}{\EdgeArrowWidth}
\newcommand{\EdgeArrowSZNum}{\EdgeArrowLengthCoef}
\newcommand{\EdgeArrowSty}{\EdgeArrowStyle}
\newcommand{\EdgeArrowIns}{\EdgeArrowInset}
% border 
\newlength{\EdgeLineBord}\setlength{\EdgeLineBord}{0pt}
%%% Zigzag edge parameter
\newlength{\ZZSiZ}
\setlength{\ZZSiZ}{\ZZSize}%
\newcommand{\ZZLineWid}{\ZZLineWidth}% coefficient multiplicateur
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge geometric parameters  --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Edge 
\newlength{\EdgeOff}
\setlength{\EdgeOff}{\EdgeOffset}
% Arc
\newcommand{\VaucArcAng}{\VaucArcAngle}
\newcommand{\VaucLArcAng}{\VaucLArcAngle}
\newlength{\VaucArcOff}\setlength{\VaucArcOff}{\VaucArcOffset}
% Loop
\newcommand{\VaucArcCurv}{\VaucArcCurvature}
\newcommand{\VaucLArcCurv}{\VaucLArcCurvature}
\newcommand{\LoopAng}{\LoopAngle}
\newcommand{\CLoopAng}{\CLoopAngle}
\newcommand{\LoopVarAng}{\LoopVarAngle}
\newlength{\LoopOff}\setlength{\LoopOff}{\LoopOffset}
\newlength{\LoopVarOff}\setlength{\LoopVarOff}{\LoopVarOffset}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label parameters --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% label distance from transition
\newlength{\TransLabelSP}\setlength{\TransLabelSP}{\TransLabelSep}
% label position on transitions
\newcommand{\EdgeLabelPos}{\EdgeLabelPosit}
\newcommand{\ArcLabelPos}{\ArcLabelPosit}
\newcommand{\LArcLabelPos}{\LArcLabelPosit}
\newcommand{\LoopLabelPos}{\LoopLabelPosit}
\newcommand{\CLoopLabelPos}{\CLoopLabelPosit}
% label position on initial-final arrow
\newcommand{\InitStateLabelPos}{\InitStateLabelPosit}
\newcommand{\FinalStateLabelPos}{\FinalStateLabelPosit}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Transition styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpsstyle{VaucEdgeStyle}%
    {arrows=\EdgeArrowSty,arrowsize=\EdgeArrowSZDim,arrowlength=\EdgeArrowSZNum,%
         arrowinset=\EdgeArrowIns,%
     linewidth=\EdgeLineWid,linecolor=\EdgeLineCol,linestyle=\EdgeLineSty,%
     doubleline=false,%
         bordercolor=\EdgeLineBorderColor,border=\EdgeLineBord,%
     fillstyle=none,offset=\EdgeOff,%
     labelsep=\TransLabelSP,nodesep=0pt}
\newpsstyle{VaucEdgeDblStyle}%
    {arrows=\EdgeArrowSty,arrowsize=\EdgeArrowSZDim,arrowlength=\EdgeArrowSZNum,%
         arrowinset=\EdgeArrowIns,%
     linewidth=\EdgeLineDblCoef\EdgeLineWid,linecolor=\EdgeLineCol,linestyle=\EdgeLineSty,%
     doubleline=true,doublesep=\EdgeLineDblSep\EdgeLineWid,%
         bordercolor=\EdgeLineBorderColor,border=\EdgeLineBord,%
     fillstyle=none,offset=\EdgeOff,%
     labelsep=\TransLabelSP,nodesep=0pt}
%%% Arc
\newpsstyle{VaucArcR}{ncurv=\VaucArcCurv,arcangle=-\VaucArcAng,%
     labelsep=\TransLabelSP,offset=-\VaucArcOff}
\newpsstyle{VaucArcL}{ncurv=\VaucArcCurv,arcangle=\VaucArcAng,%
     labelsep=\TransLabelSP,offset=\VaucArcOff}
\newpsstyle{VaucLArcR}{ncurv=\VaucLArcCurv,arcangle=-\VaucLArcAng,%
     labelsep=\TransLabelSP,offset=-\VaucArcOff}
\newpsstyle{VaucLArcL}{ncurv=\VaucLArcCurv,arcangle=\VaucLArcAng,%
     labelsep=\TransLabelSP,offset=\VaucArcOff}
%%% zig-zag
\newpsstyle{VaucZigzagStyle}%
   {linewidth=\ZZLineWid\EdgeLineWid,%
    labelsep=\TransLabelSP,nodesep=0pt,%
    coilwidth=1.2\ZZSiZ,coilarmA=0.1\ZZSiZ,%
    coilarmB=0.3\ZZSiZ,coilheight=\ZZShape,linearc=1.6pt}
%%%
\newcommand{\EdgeStyle}{\ifEdgeLineDbl\psset{style=VaucEdgeDblStyle}%
        \else\psset{style=VaucEdgeStyle}\fi}
\newcommand{\ZigzagStyle}%
   {\addtolength{\TransLabelSP}{\TransLabelZZCoef\ZZSiZ}%
    \psset{style=VaucZigzagStyle}%
        \addtolength{\TransLabelSP}{-\TransLabelZZCoef\ZZSiZ}%
        }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Transition parameter changing and setting macros 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% geometric parameters
\newcommand{\ChgEdgeOffset}[1]{\setlength{\EdgeOff}{#1}}
\newcommand{\RstEdgeOffset}{\ChgEdgeOffset{\EdgeOffset}}
\newcommand{\SetEdgeOffset}[1]%
   {\setlength{\EdgeOffset}{#1}\RstEdgeOffset}
\newcommand{\ForthBackOffset}{%
   \setlength{\EdgeOff}{\ForthBackEdgeOffset\EdgeLineWid}}
%
\newcommand{\ChgArcAngle}[1]{\renewcommand{\VaucArcAng}{#1}}
\newcommand{\RstArcAngle}{\ChgArcAngle{\VaucArcAngle}}
\newcommand{\SetArcAngle}[1]%
   {\renewcommand{\VaucArcAngle}{#1}\RstArcAngle}
%
\newcommand{\ChgLArcAngle}[1]{\renewcommand{\VaucLArcAng}{#1}}
\newcommand{\RstLArcAngle}{\ChgLArcAngle{\VaucLArcAngle}}
\newcommand{\SetLArcAngle}[1]%
   {\renewcommand{\VaucLArcAngle}{#1}\RstLArcAngle}
%
\newcommand{\ChgArcCurvature}[1]{\renewcommand{\VaucArcCurv}{#1}}
\newcommand{\RstArcCurvature}{\ChgArcCurvature{\VaucArcCurvature}}
\newcommand{\SetArcCurvature}[1]%
   {\renewcommand{\VaucArcCurvature}{#1}\RstArcCurvature}
%
\newcommand{\ChgLArcCurvature}[1]{\renewcommand{\VaucLArcCurv}{#1}}
\newcommand{\RstLArcCurvature}{\ChgLArcCurvature{\VaucLArcCurvature}}
\newcommand{\SetLArcCurvature}[1]%
   {\renewcommand{\VaucLArcCurvature}{#1}\RstLArcCurvature}
%
\newcommand{\ChgArcOffset}[1]{\setlength{\VaucArcOff}{#1}}
\newcommand{\RstArcOffset}{\setlength{\VaucArcOff}{\VaucArcOffset}}
\newcommand{\SetArcOffset}[1]%
   {\renewcommand{\VaucArcOffset}{#1}\RstArcOffset}
%
\newcommand{\ChgLoopOffset}[1]{\setlength{\LoopOff}{#1}}
\newcommand{\RstLoopOffset}{\setlength{\LoopOff}{\LoopOffset}}
\newcommand{\SetLoopOffset}[1]%
   {\renewcommand{\LoopOffset}{#1}\RstLoopOffset}
%
\newcommand{\ChgLoopAngle}[1]{\renewcommand{\LoopAng}{#1}}
\newcommand{\RstLoopAngle}{\ChgLoopAngle{\LoopAngle}}
\newcommand{\SetLoopAngle}[1]%
   {\renewcommand{\LoopAngle}{#1}\RstLoopAngle}
%
\newcommand{\ChgCLoopAngle}[1]{\renewcommand{\CLoopAng}{#1}}
\newcommand{\RstCLoopAngle}{\ChgCLoopAngle{\CLoopAngle}}
\newcommand{\SetCLoopAngle}[1]%
   {\renewcommand{\CLoopAngle}{#1}\RstCLoopAngle}
%
%%% drawing parameters
\newcommand{\ChgEdgeLineColor}[1]{\renewcommand{\EdgeLineCol}{#1}}
\newcommand{\RstEdgeLineColor}{\ChgEdgeLineColor{\EdgeLineColor}}
\newcommand{\SetEdgeLineColor}[1]%
   {\renewcommand{\EdgeLineColor}{#1}\RstEdgeLineColor}
%
\newcommand{\ChgEdgeLineStyle}[1]{\renewcommand{\EdgeLineSty}{#1}}  
\newcommand{\RstEdgeLineStyle}{\ChgEdgeLineStyle{\EdgeLineStyle}}
\newcommand{\SetEdgeLineStyle}[1]%
   {\renewcommand{\EdgeLineStyle}{#1}\RstEdgeLineStyle}
%
\newcommand{\ChgEdgeLineWidth}[1]% coefficient !
   {\setlength{\EdgeLineWid}{#1\EdgeLineWidth}}
\newcommand{\RstEdgeLineWidth}{\ChgEdgeLineWidth{1}}
\newcommand{\SetEdgeLineWidth}[1]% length !
   {\setlength{\EdgeLineWidth}{#1}\RstEdgeLineWidth}
%
\newcommand{\EdgeLineDouble}%
        {\EdgeLineDbltrue%
    \ChgEdgeArrowWidth{\EdgeDblArrowWidth}
    \ChgEdgeArrowLengthCoef{\EdgeDblArrowLengthCoef}}
\newcommand{\EdgeLineSimple}%
   {\EdgeLineDblfalse \RstEdgeArrowWidth \RstEdgeArrowLengthCoef}
%
\newcommand{\ChgEdgeLabelColor}[1]{\renewcommand{\EdgeLabelCol}{#1}}
\newcommand{\RstEdgeLabelColor}{\ChgEdgeLabelColor{\EdgeLabelColor}}
\newcommand{\SetEdgeLabelColor}[1]%
   {\renewcommand{\EdgeLabelColor}{#1}\RstEdgeLabelColor}
%
\newcommand{\ChgEdgeLabelScale}[1]{\renewcommand{\EdgeLabelSca}{#1}}
\newcommand{\RstEdgeLabelScale}{\ChgEdgeLabelScale{1}}
\newcommand{\SetEdgeLabelScale}[1]%
   {\renewcommand{\EdgeLabelScale}{#1}\RstEdgeLabelScale}
\newcommand{\FixDimEdge}[4]{%
    \renewcommand{\DimEdgeLineStyle}{#1}%
    \renewcommand{\DimEdgeLineCoef}{#2}%
    \renewcommand{\DimEdgeLineColor}{#3}%
    \renewcommand{\DimEdgeLabelColor}{#4}}%
%
\newcommand{\ChgEdgeArrowStyle}[1]{\renewcommand{\EdgeArrowSty}{#1}}
\newcommand{\RstEdgeArrowStyle}{\ChgEdgeArrowStyle{\EdgeArrowStyle}}
\newcommand{\SetEdgeArrowStyle}[1]%
   {\renewcommand{\EdgeArrowStyle}{#1}\RstEdgeArrowStyle}
%
\newcommand{\ChgEdgeArrowWidth}[1]%
   {\setlength{\EdgeArrowSZDim}{#1}} % !! length !!
\newcommand{\RstEdgeArrowWidth}{\ChgEdgeArrowWidth{\EdgeArrowWidth}}
\newcommand{\SetEdgeArrowWidth}[1]%
   {\setlength{\EdgeArrowWidth}{#1} \RstEdgeArrowWidth}
%
\newcommand{\ChgEdgeArrowLengthCoef}[1]{\renewcommand{\EdgeArrowSZNum}{#1}}
\newcommand{\RstEdgeArrowLengthCoef}{\ChgEdgeArrowLengthCoef{\EdgeArrowLengthCoef}}
\newcommand{\SetEdgeArrowLengthCoef}[1]%
   {\renewcommand{\EdgeArrowLengthCoef}{#1}\RstEdgeArrowLengthCoef}
%
\newcommand{\ChgEdgeArrowInsetCoef}[1]{\renewcommand{\EdgeArrowIns}{#1}}
\newcommand{\RstEdgeArrowInsetCoef}{\ChgEdgeArrowInsetCoef{\EdgeArrowInset}}
\newcommand{\SetEdgeArrowInsetCoef}[1]%
   {\renewcommand{\EdgeArrowInset}{#1}\RstEdgeArrowInsetCoef}
%
\newcommand{\ReverseArrow}%
   {\ChgEdgeArrowStyle{\EdgeRevArrowStyle}%
    \renewcommand{\EdgeLabelPos}{\EdgeLabelRevPosit}%
    \renewcommand{\ArcLabelPos}{\ArcLabelRevPosit}%
    \renewcommand{\LArcLabelPos}{\LArcLabelRevPosit}%
    \renewcommand{\LoopLabelPos}{\LoopLabelRevPosit}%
    \renewcommand{\CLoopLabelPos}{\CLoopLabelRevPosit}%
    \renewcommand{\InitStateLabelPos}{\InitStateLabelRevPosit}%
    \renewcommand{\FinalStateLabelPos}{\FinalStateLabelRevPosit}}
\newcommand{\StraightArrow}%
   {\ChgEdgeArrowStyle{\EdgeArrowStyle}%
    \renewcommand{\EdgeLabelPos}{\EdgeLabelPosit}%
    \renewcommand{\ArcLabelPos}{\ArcLabelPosit}%
    \renewcommand{\LArcLabelPos}{\LArcLabelPosit}%
    \renewcommand{\LoopLabelPos}{\LoopLabelPosit}%
    \renewcommand{\CLoopLabelPos}{\CLoopLabelPosit}%
    \renewcommand{\InitStateLabelPos}{\InitStateLabelPosit}%
    \renewcommand{\FinalStateLabelPos}{\FinalStateLabelPosit}}
% Double
\newcommand{\FixEdgeLineDouble}[2]{%
    \renewcommand{\EdgeLineDblCoef}{#1}%
    \renewcommand{\EdgeLineDblSep}{#2}}
% border
\newcommand{\FixEdgeBorder}[2]{%
    \renewcommand{\EdgeLineBorderCoef}{#1}%
    \renewcommand{\EdgeLineBorderColor}{#2}}
\newcommand{\EdgeBorder}%
  {\setlength{\EdgeLineBord}{\EdgeLineBorderCoef\EdgeLineWid}}
\newcommand{\EdgeBorderOff}{\setlength{\EdgeLineBord}{0pt}}
%%%
\newcommand{\DimEdge}{%
    \ChgEdgeLineStyle{\DimEdgeLineStyle}%
    \ChgEdgeLineWidth{\DimEdgeLineCoef}%
    \ChgEdgeLineColor{\DimEdgeLineColor}%
        \ChgEdgeLabelColor{\DimEdgeLabelColor}}
%%%
\newcommand{\ChgZZSize}[1]{\setlength{\ZZSiZ}{#1}}
\newcommand{\RstZZSize}{\setlength{\ZZSiZ}{\ZZSize}}
\newcommand{\SetZZSize}[1]{\setlength{\ZZSiZe}{#1}\RstZZSize}
%%%\ZZLineWidth
\newcommand{\ChgZZLineWidth}[1]{\renewcommand{\ZZLineWid}{#1}}
\newcommand{\RstZZLineWidth}{\ChgZZLineWidth{\ZZLineWidth}}
\newcommand{\SetZZLineWidth}[1]%
   {\renewcommand{\ZZLineWidth}{#1}\RstZZLineWidth}
%
%%% label of transitions
\newcommand{\VaucEdgeLabel}[1]{%
        \textcolor{\EdgeLabelCol}{\scalebox{\EdgeLabelSca}{\scalebox{\EdgeLabelScale}{$ #1 $}}}}
%%%
\newcommand{\RstEdge}{%
   \RstEdgeOffset\RstArcAngle\RstLArcAngle%
   \RstArcCurvature\RstLArcCurvature%
   \RstArcOffset\RstLoopOffset\RstLoopSize%
   \RstEdgeLineColor\RstEdgeLineStyle\RstEdgeLineWidth\EdgeLineSimple%
   \StraightArrow%\EdgeBorderOff%
   \RstEdgeLabelScale\RstEdgeLabelColor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Initial-final arrow drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% implicit parameter
\newcommand{\InitialDir}{w}\newcommand{\FinalDir}{e}
% without label
\newcommand{\Initial}[2][\InitialDir]{\EdgeStyle\ncline{#2#1}{#2}}
\newcommand{\Final}[2][\FinalDir]{\EdgeStyle\ncline{#2}{#2#1}}
% with label
%  NB modified syntax eg \InitialL[pos]{dir}{statename}{label}
\newcommand{\InitialL}[4][{\InitStateLabelPos}]%
   {\EdgeStyle\ncline{#3#2}{#3}\naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\InitialR}[4][{\InitStateLabelPos}]%
   {\EdgeStyle\ncline{#3#2}{#3}\nbput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\FinalL}[4][{\FinalStateLabelPos}]%
   {\EdgeStyle\ncline{#3}{#3#2}\naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\FinalR}[4][{\FinalStateLabelPos}]%
   {\EdgeStyle\ncline{#3}{#3#2}\nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Transition drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EdgeL}[4][{\EdgeLabelPos}]%
   {\EdgeStyle \ncline{#2}{#3} \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\EdgeR}[4][{\EdgeLabelPos}]%
   {\EdgeStyle \ncline{#2}{#3} \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%
\newcommand{\ArcL}[4][{\ArcLabelPos}]%
   {\EdgeStyle \psset{style=VaucArcL}% 
    \ncarc{#2}{#3} \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\ArcR}[4][{\ArcLabelPos}]%
   {\EdgeStyle \psset{style=VaucArcR}% 
    \ncarc{#2}{#3} \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\LArcL}[4][{\LArcLabelPos}]%
   {\EdgeStyle \psset{style=VaucLArcL}% 
    \ncarc{#2}{#3} \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\LArcR}[4][{\LArcLabelPos}]%
   {\EdgeStyle \psset{style=VaucLArcR}% 
    \ncarc{#2}{#3} \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%
\newcounter{anglea}\newcounter{angleb}
\newcommand{\LoopXR}[7]%
   {{\setcounter{anglea}{#2-#4}}%
    {\setcounter{angleb}{#2+#4}}%
    {\EdgeStyle \psset{angleA=\theanglea,angleB=\theangleb,offset=#5,ncurv=#6}% 
    \nccurve{#3}{#3} \nbput[npos=#1]{\VaucEdgeLabel{#7}}}}
\newcommand{\LoopXL}[7]%
   {{\setcounter{anglea}{#2+#4}}%
    {\setcounter{angleb}{#2-#4}}%
    {\EdgeStyle \psset{angleA=\theanglea,angleB=\theangleb,offset=-#5,ncurv=#6}% 
    \nccurve{#3}{#3} \naput[npos=#1]{\VaucEdgeLabel{#7}}}}
\newcommand{\LoopR}[4][{\LoopLabelPos}]%
   {\LoopXR{#1}{#2}{#3}{\LoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\LoopL}[4][{\LoopLabelPos}]%
   {\LoopXL{#1}{#2}{#3}{\LoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\CLoopR}[4][{\CLoopLabelPos}]%
   {\LoopXR{#1}{#2}{#3}{\CLoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\CLoopL}[4][{\CLoopLabelPos}]%
   {\LoopXL{#1}{#2}{#3}{\CLoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\LoopVarR}[4][{\LoopLabelPos}]%
   {\LoopXR{#1}{#2}{#3}{\LoopVarAng}{\LoopVarOff}{\LoopVarSi}{#4}}
\newcommand{\LoopVarL}[4][{\LoopLabelPos}]%
   {\LoopXL{#1}{#2}{#3}{\LoopVarAng}{\LoopVarOff}{\LoopVarSi}{#4}}
\newcommand{\LoopW}[3][{\LoopLabelPos}]{\LoopR[#1]{180}{#2}{#3}}
\newcommand{\LoopE}[3][{\LoopLabelPos}]{\LoopL[#1]{0}{#2}{#3}}
\newcommand{\LoopN}[3][{\LoopLabelPos}]{\LoopL[#1]{90}{#2}{#3}}
\newcommand{\LoopS}[3][{\LoopLabelPos}]{\LoopR[#1]{-90}{#2}{#3}}
\newcommand{\LoopNW}[3][{\LoopLabelPos}]{\LoopR[#1]{135}{#2}{#3}}
\newcommand{\LoopNE}[3][{\LoopLabelPos}]{\LoopL[#1]{45}{#2}{#3}}
\newcommand{\LoopSW}[3][{\LoopLabelPos}]{\LoopL[#1]{-135}{#2}{#3}}
\newcommand{\LoopSE}[3][{\LoopLabelPos}]{\LoopR[#1]{-45}{#2}{#3}}
\newcommand{\CLoopW}[3][{\CLoopLabelPos}]{\CLoopR[#1]{180}{#2}{#3}}
\newcommand{\CLoopE}[3][{\CLoopLabelPos}]{\CLoopL[#1]{0}{#2}{#3}}
\newcommand{\CLoopN}[3][{\CLoopLabelPos}]{\CLoopL[#1]{90}{#2}{#3}}
\newcommand{\CLoopS}[3][{\CLoopLabelPos}]{\CLoopR[#1]{-90}{#2}{#3}}
\newcommand{\CLoopNW}[3][{\CLoopLabelPos}]{\CLoopR[#1]{135}{#2}{#3}}
\newcommand{\CLoopNE}[3][{\CLoopLabelPos}]{\CLoopL[#1]{45}{#2}{#3}}
\newcommand{\CLoopSW}[3][{\CLoopLabelPos}]{\CLoopL[#1]{-135}{#2}{#3}}
\newcommand{\CLoopSE}[3][{\CLoopLabelPos}]{\CLoopR[#1]{-45}{#2}{#3}}
\newcommand{\LoopVarN}[3][{\CLoopLabelPos}]{\LoopVarL[#1]{90}{#2}{#3}}
\newcommand{\LoopVarS}[3][{\CLoopLabelPos}]{\LoopVarR[#1]{-90}{#2}{#3}}
%
\newcommand{\ZZEdge}[2]%
   {\EdgeStyle\ZigzagStyle\nczigzag{#1}{#2}}%
\newcommand{\ZZEdgeL}[4][{\EdgeLabelRevPosit}]%
   {\EdgeStyle\ZigzagStyle\nczigzag{#2}{#3}%
    \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\ZZEdgeR}[4][{\EdgeLabelRevPosit}]%
   {\EdgeStyle\ZigzagStyle\nczigzag{#2}{#3}%
    \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Reprise des macros pstricks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Point}[2]{\pnode#1{#2}}
\newcommand{\Edge}[2]{\EdgeStyle\ncline{#1}{#2}}
%
\newcommand{\VArcL}[5][{\ArcLabelPos}]%
   {\EdgeStyle \psset{style=VaucLArcL}% 
    \ncarc[#2]{#3}{#4} \naput[npos=#1]{\VaucEdgeLabel{#5}}}
\newcommand{\VArcR}[5][{\ArcLabelPos}]%
   {\EdgeStyle \psset{style=VaucLArcR}% 
    \ncarc[#2]{#3}{#4} \nbput[npos=#1]{\VaucEdgeLabel{#5}}}
%
\newcommand{\VCurveL}[5][{\ArcLabelPos}]%
   {\EdgeStyle \psset{angleA=0,angleB=180,ncurv=1}% 
    \nccurve[#2]{#3}{#4} \naput[npos=#1]{\VaucEdgeLabel{#5}}}
\newcommand{\VCurveR}[5][{\ArcLabelPos}]%
   {\EdgeStyle \psset{angleA=0,angleB=0,ncurv=1}% 
    \nccurve[#2]{#3}{#4} \nbput[npos=#1]{\VaucEdgeLabel{#5}}}
%
\newcommand{\LabelL}[2][{\EdgeLabelPos}]%
   {\naput[npos=#1]{\VaucEdgeLabel{#2}}}
\newcommand{\LabelR}[2][{\EdgeLabelPos}]%
   {\nbput[npos=#1]{\VaucEdgeLabel{#2}}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> share/styles/pgfsubpic.tex <==
%    pgfsubpic.tex
%    Version 1.1, 25 Dec 2009

%    Copyright 2009 by David Chiang

%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.

%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.

%    You should have received a copy of the GNU General Public License along
%    with this program; if not, write to the Free Software Foundation, Inc.,
%    51 Franklin Street, Fifth Floor, Boston, MA 02110-1301 USA.

% New in version 1.1:
% - the ability to save a subpicture in local variables
% - nodes in subpictures are tracked if the subpicture is placed with arbitrary transforms
% - new \pgffitsubpicture macro to transform a subpicture (preserving aspect) to fit in a desired box

% To do: 
% - speed up interpictureshift hook by promoting subsubpictures

\newdimen\pgf@subpicminx
\newdimen\pgf@subpicminy
\newdimen\pgf@subpicmaxx
\newdimen\pgf@subpicmaxy

% Special virtual node for current subpicture's bounding box
\expandafter\def\csname pgf@sh@ns@current subpicture\endcsname{rectangle}
\expandafter\def\csname pgf@sh@np@current subpicture\endcsname{%
  \def\southwest{\pgfqpoint{\pgf@subpicminx}{\pgf@subpicminy}}%
  \def\northeast{\pgfqpoint{\pgf@subpicmaxx}{\pgf@subpicmaxy}}%
}
\expandafter\def\csname pgf@sh@nt@current subpicture\endcsname{{\pgf@pt@aa}{\pgf@pt@ab}{\pgf@pt@ba}{\pgf@pt@bb}{\the\pgf@pt@x}{\the\pgf@pt@y}} % the transformation at invocation time
\expandafter\def\csname pgf@sh@pi@current subpicture\endcsname{\pgfpictureid}

% Create a pgfpicture inside an hbox for delayed placement
\def\pgfsubpicture{%
\expandafter\global\expandafter\setbox\pgf@hbox=\hbox\bgroup
\pgfinterruptpicture
\pgfpicture
\relax % not sure why. otherwise a curly brace immediately after causes an error
}

\def\endpgfsubpicture{
\global\pgf@subpicminx=\pgf@picminx
\global\pgf@subpicminy=\pgf@picminy
\global\pgf@subpicmaxx=\pgf@picmaxx
\global\pgf@subpicmaxy=\pgf@picmaxy
\global\edef\subpictureid{\pgfpictureid}%
\pgfsetbaseline{\pgf@picminy}%
\endpgfpicture%
\endpgfinterruptpicture%
\egroup
}

% Allocate registers for saving a subpicture. #1 is text, not a control sequence.
\def\pgfnewsubpicture#1{%
\expandafter\newbox\csname pgf@subpic@hbox@#1\endcsname
\expandafter\newdimen\csname pgf@subpic@minx@#1\endcsname
\expandafter\newdimen\csname pgf@subpic@miny@#1\endcsname
\expandafter\newdimen\csname pgf@subpic@maxx@#1\endcsname
\expandafter\newdimen\csname pgf@subpic@maxy@#1\endcsname
}

% saved subpictures are local to the current group
\def\pgfsavesubpicture#1{%
\expandafter\setbox\csname pgf@subpic@hbox@#1\endcsname\copy\pgf@hbox
\csname pgf@subpic@minx@#1\endcsname\pgf@subpicminx
\csname pgf@subpic@miny@#1\endcsname\pgf@subpicminy
\csname pgf@subpic@maxx@#1\endcsname\pgf@subpicmaxx
\csname pgf@subpic@maxy@#1\endcsname\pgf@subpicmaxy
\expandafter\edef\csname pgf@subpic@id@#1\endcsname{\subpictureid}
}

\def\pgfrestoresubpicture#1{%
\edef\act{\global\noexpand\setbox\pgf@hbox\noexpand\copy\csname pgf@subpic@hbox@#1\endcsname}\act
\expandafter\global\expandafter\pgf@subpicminx\csname pgf@subpic@minx@#1\endcsname
\expandafter\global\expandafter\pgf@subpicminy\csname pgf@subpic@miny@#1\endcsname
\expandafter\global\expandafter\pgf@subpicmaxx\csname pgf@subpic@maxx@#1\endcsname
\expandafter\global\expandafter\pgf@subpicmaxy\csname pgf@subpic@maxy@#1\endcsname
\xdef\subpictureid{\csname pgf@subpic@id@#1\endcsname}
}

% Place a previously-created subpicture, lining up its origin with the current origin
\def\pgfplacesubpicture{
\pgfscope
% expand current bounding box to accommodate subpicture
\pgfpathrectanglecorners{\pgfpoint{\the\pgf@subpicminx}{\the\pgf@subpicminy}}{\pgfpoint{\the\pgf@subpicmaxx}{\the\pgf@subpicmaxy}}%
\pgfusepath{use as bounding box}%
%
% make the subpicture a node in the containing picture
\expandafter\gdef\csname pgf@sh@ns@\subpictureid\endcsname{rectangle}
\expandafter\xdef\csname pgf@sh@np@\subpictureid\endcsname{%
  \noexpand\def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@subpicminx}{\the\pgf@subpicminy}}%
  \noexpand\def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@subpicmaxx}{\the\pgf@subpicmaxy}}%
}%
\pgfgettransform\pgf@temp
\expandafter\xdef\csname pgf@sh@nt@\subpictureid\endcsname{\pgf@temp}%
\expandafter\xdef\csname pgf@sh@pi@\subpictureid\endcsname{\pgfpictureid}%
%
% align origin of subpicture with origin
\pgftransformshift{\pgfpoint{\the\pgf@subpicminx}{\the\pgf@subpicminy}}%
\pgfqboxsynced{\pgf@hbox}%
\endpgfscope
}

% Hook onto existing macro \pgf@shape@interpictureshift.
% This is called whenever we look up an anchor of a node.
% This hook recursively checks to see if the node's picture
% is a subpicture of another, and if so, adjusts its position accordingly.

% This is slow. It makes drawing trees O(n^2) in the depth of the tree.
% The alternative is to store, for each picture, a list of the nodes
% inside it. But this way doesn't require us to hijack \pgfnode, and
% is robust to re-placement of a subpicture. A compromise would be
% to store, for each picture, a list of the *subpictures* inside it.

\let\orig@pgf@shape@interpictureshift\pgf@shape@interpictureshift
\def\unwind@subpic#1{%
% is #1 the current picture?
\edef\subpicid{#1}%
\ifx\subpicid\pgfpictureid
% yes, we're done
\else
% does #1 have a parent picture?
\expandafter\ifx\csname pgf@sh@pi@#1\endcsname\relax
% no, the original node was not inside the current picture
\fallback
\else
% yes, apply transform and move up to parent picture
{%
  \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
  \pgf@pos@transform{\pgf@x}{\pgf@y}%
  \global\pgf@x=\pgf@x
  \global\pgf@y=\pgf@y
}%
\unwind@subpic{\csname pgf@sh@pi@#1\endcsname}%
\fi
\fi
}
\def\pgf@shape@interpictureshift#1{%
\edef\fallback{\pgf@x=\the\pgf@x\pgf@y=\the\pgf@y\noexpand\orig@pgf@shape@interpictureshift{#1}}%
\unwind@subpic{\csname pgf@sh@pi@#1\endcsname}%
}

% \pgffitsubpicture{sw}{ne}
% Make the subpicture fit in the rectangle from sw to ne, preserving its aspect ratio.
\def\pgffitsubpicture#1#2{%
% current size
\pgfpointdiff{\pgfpointanchor{current subpicture}{south west}}{\pgfpointanchor{current subpicture}{north east}}%
\pgf@xa=\pgf@x \pgf@ya=\pgf@y
% desired size
\pgf@process{\pgfpointdiff{#1}{#2}}%
\pgf@xb=\pgf@x \pgf@yb=\pgf@y
\pgfmathparse{min(\pgf@xb/\pgf@xa,\pgf@yb/\pgf@ya)}%
\pgfmathparse{min(1,\pgfmathresult)}%
\pgftransformscale{\pgfmathresult}%
%
% current position
\pgfpointanchor{current subpicture}{center}%
\pgf@xa=\pgf@x \pgf@ya=\pgf@y
% desired position
% we scaled transform, so apply reverse scaling to argument
\pgfmathparse{1/\pgfmathresult}%
\pgf@process{\pgfpointscale{\pgfmathresult}{\pgfpointlineattime{0.5}{#1}{#2}}}%
\pgf@xb=\pgf@x \pgf@yb=\pgf@y
\pgfpointdiff{\pgfpoint{\pgf@xa}{\pgf@ya}}{\pgfpoint{\pgf@xb}{\pgf@yb}}%
\pgftransformshift{\pgfpoint{\pgf@x}{\pgf@y}}%
}

% utility functions -- not currently used

\def\pgfnodedelete#1{%
\expandafter\global\expandafter\let\csname pgf@sh@ns@#1\endcsname\relax
\expandafter\global\expandafter\let\csname pgf@sh@np@#1\endcsname\relax
\expandafter\global\expandafter\let\csname pgf@sh@nt@#1\endcsname\relax
\expandafter\global\expandafter\let\csname pgf@sh@pi@#1\endcsname\relax
\expandafter\global\expandafter\let\csname pgf@sh@ma@#1\endcsname\relax
}

\def\pgfnodeifexists#1#2#3{%
\expandafter\ifx\csname pgf@sh@ns@#1\endcsname\relax#3\else#2\fi
}



==> share/styles/pgftree.tex <==
%    pgftree.tex
%    Version 1.1, 25 Dec 2009

%    Copyright 2009 by David Chiang

%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.

%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.

%    You should have received a copy of the GNU General Public License along
%    with this program; if not, write to the Free Software Foundation, Inc.,
%    51 Franklin Street, Fifth Floor, Boston, MA 02110-1301 USA.

% New in version 1.1:
% - major restructuring to not do arbitrary nesting of subpicture environments
% - sideways trees

% To do:
% - trees with all leaves at same level
% - if \nodename does not exist as desired, wrap inside a rectangle node
% - don't use pgfsubpic internals

\newdimen\levelsep \levelsep=30pt
\newdimen\subtreesep \subtreesep=2pt

\def\leveldirection{down}
\def\siblingdirection{right}

% definitions of growing directions
\def\pgftree@levelshift{\csname pgftree@levelshift@\leveldirection\endcsname}
\def\pgftree@parentanchor{\csname pgftree@parentanchor@\leveldirection\endcsname}
\def\pgftree@childanchor{\csname pgftree@childanchor@\leveldirection\endcsname}
% these assume that the current subpicture is the child
\def\pgftree@presiblingshift{\csname pgftree@presiblingshift@\siblingdirection\endcsname}
\def\pgftree@postsiblingshift{\csname pgftree@postsiblingshift@\siblingdirection\endcsname}

\def\pgftree@levelshift@down{\pgfpoint{0}{-\levelsep}}
\def\pgftree@parentanchor@down{south}
\def\pgftree@childanchor@down{north}

\def\pgftree@levelshift@up{\pgfpoint{0}{\levelsep}}
\def\pgftree@parentanchor@up{north}
\def\pgftree@childanchor@up{south}

\def\pgftree@levelshift@right{\pgfpoint{\levelsep}{0}}
\def\pgftree@parentanchor@right{east}
\def\pgftree@childanchor@right{west}

\def\pgftree@levelshift@left{\pgfpoint{-\levelsep}{0}}
\def\pgftree@parentanchor@left{west}
\def\pgftree@childanchor@left{east}

\def\pgftree@presiblingshift@right{\pgf@process{\pgf@x-\pgf@subpicminx \advance\pgf@x\subtreesep \pgf@y 0pt}}
\def\pgftree@postsiblingshift@right{\pgf@process{\pgf@x\pgf@subpicmaxx \pgf@y 0pt}}

\def\pgftree@presiblingshift@left{\pgf@process{\pgf@x-\pgf@subpicmaxx \advance\pgf@x-\subtreesep \pgf@y 0pt}}
\def\pgftree@postsiblingshift@left{\pgf@process{\pgf@x\pgf@subpicminx \pgf@y 0pt}}

\def\pgftree@presiblingshift@up{\pgf@process{\pgf@x 0pt \pgf@y-\pgf@subpicminy \advance\pgf@y\subtreesep}}
\def\pgftree@postsiblingshift@up{\pgf@process{\pgf@x 0pt \pgf@y\pgf@subpicmaxy}}

\def\pgftree@presiblingshift@down{\pgf@process{\pgf@x 0pt \pgf@y-\pgf@subpicmaxy \advance\pgf@y-\subtreesep}}
\def\pgftree@postsiblingshift@down{\pgf@process{\pgf@x 0pt \pgf@y\pgf@subpicminy}}

% for convenience if you are using \pgftree directly
\def\drawnode#1{\pgfnode{rectangle}{base}{#1}{\nodename}{\pgfusepath{discard}}}
\def\drawedge{%
\pgfpathmoveto{\pgfpointanchor{\parentnodename}{\pgftree@parentanchor}}%
\pgfpathlineto{\pgfpointanchor{\nodename}{\pgftree@childanchor}}%
\pgfusepath{stroke}}

% local variables that we need to assign to inside a \pgfforeach
\newdimen\pgftree@childx
\newdimen\pgftree@savechildx
\newdimen\pgftree@childy
\newdimen\pgftree@savechildy
\newcount\pgftree@childi
\newcount\pgftree@savechildi

%%% \pgftree{subtree}

\def\pgftree#1{%
\def\nodename{r}%
#1
\pgfplacesubpicture
}

%%% \pgfsubtree{root}{subtrees}
% The first argument draws the root node using PGF/TikZ commands.
% The node must be named \nodename.

% The second argument is an even-length sequence of tokens.
% Token 2n-1 in the sequence draws the nth edge. It should draw an edge from \parentnodename to \nodename.
% Token 2n in the sequence draws the nth subtree. Its root must be named \nodename.

\pgfnewsubpicture{children}
\pgfnewsubpicture{child}
\newdimen\pgftree@lastchildx
\newdimen\pgftree@lastchildy

\def\pgfsubtree#1#2{%
\let\parentnodename\nodename
\pgftree@savechildx=\pgftree@childx
\pgftree@savechildy=\pgftree@childy
\pgftree@savechildi=\pgftree@childi
% Build subpicture with all the children and their subtrees. Save it in "children"
{\pgftree@childx=0pt%
\pgftree@childy=0pt%
\pgftree@childi=0%
\process@children #2}%
\ifnum\pgftree@childi>0%
\begin{pgfsubpicture}%
% Create root node
#1
% Place children
% move down \levelsep
{\pgftransformshift{\pgftree@levelshift}%
% center so that parent is midway between origins of first and last children
\pgftransformshift{\pgfpointscale{-0.5}{\pgfpoint{\the\pgftree@childx}{\the\pgftree@childy}}}%
\pgfplacesubpicture}
% Draw the edges
{\pgftree@childi=0%
\process@edges #2}%
\end{pgfsubpicture}%
\else % leaf node
\begin{pgfsubpicture}%
#1
\end{pgfsubpicture}%
\fi
\global\pgftree@childi=\pgftree@savechildi
\global\pgftree@childx=\pgftree@savechildx
\global\pgftree@childy=\pgftree@savechildy
}

\def\process@children{%
\pgfutil@ifnextchar\egroup
{% No more children, step back to origin of last child
\global\pgftree@childx\pgftree@lastchildx
\global\pgftree@childy\pgftree@lastchildy
\global\pgftree@childi\pgftree@childi
\pgfrestoresubpicture{children}% pass children back to caller
}%
{\@process@children}%
}
\def\@process@children#1#2{% #1 is the edge, #2 is the child
% Build the current child and save it as "child"
{\edef\nodename{\parentnodename-\the\pgftree@childi}%
#2}%
\pgfsavesubpicture{child}%
\begin{pgfsubpicture}
% Place previous children (if any)
\ifnum\pgftree@childi>0%
\pgfrestoresubpicture{children}%
\pgfplacesubpicture
\fi
% Place current child
\pgfrestoresubpicture{child}%
\ifnum\pgftree@childi>0% the first child is always at 0
\pgftree@presiblingshift \global\advance\pgftree@childx\pgf@x \global\advance\pgftree@childy\pgf@y
\fi
\global\pgftree@lastchildx\pgftree@childx
\global\pgftree@lastchildy\pgftree@childy
{\pgftransformshift{\pgfpoint{\the\pgftree@childx}{\the\pgftree@childy}}%
\pgfplacesubpicture}%
\pgftree@postsiblingshift \global\advance\pgftree@childx\pgf@x \global\advance\pgftree@childy\pgf@y
\end{pgfsubpicture}%
% Save the augmented row of children back into "children"
\pgfsavesubpicture{children}%
\advance\pgftree@childi by 1%
\process@children
}

\def\process@edges{%
\pgfutil@ifnextchar\egroup
{}%
{\@process@edges}%
}
\def\@process@edges#1#2{%
\edef\nodename{\parentnodename-\the\pgftree@childi}%
#1%
\advance\pgftree@childi by 1%
\process@edges
}

\def\subtreeof#1{%
% the subpicture which contains a node also contains exactly its subtree
\csname pgf@sh@pi@#1\endcsname
}


==> share/styles/tikz-qtree.tex <==
%    tikz-qtree.tex
%    Version 1.1, 25 Dec 2009

%    Copyright (C) 2002, 2009 by David Chiang

%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.

%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.

%    You should have received a copy of the GNU General Public License along
%    with this program; if not, write to the Free Software Foundation, Inc.,
%    51 Franklin Street, Fifth Floor, Boston, MA 02110-1301 USA.

% New in version 1.1:

% - sideways trees

%% These macros facilitate building up an object recursively before
%% putting it into the input stream.

\newtoks\@result
\def\@call#1#2{\let\@cont=#2\bgroup\@result={}#1}
\def\@return{\global\@result=\@result\egroup\@cont}

\def\@ifequal#1#2{\edef\testa{#1}\edef\testb{#2}\ifx\testa\testb}

%% scan a tree: this just scans a subtree and then puts it onto the
%% input stream

\def\Tree{\@call\@subtree\@Tree}
\def\@Tree{%
%\showthe\@result %debug
\ifpgfpicture % is there a test for tikzpicture?
\pgftree{\the\@result}%
\else
\tikzpicture[baseline]\pgftree{\the\@result}\endtikzpicture
\fi
}

%% scan a subtree
\newtoks\child@list
\newtoks\root@node

\def\@subtree[{%
\root@node={}%
\pgfutil@ifnextchar.{\@call\@interior\@@subtree}{\@@@subtree}}
\def\@@subtree{%
\root@node=\@result
\@@@subtree
}
\def\@@@subtree{%
\@call\@children\@@@@subtree
}
\def\@@@@subtree]{%
\child@list=\@result
\pgfutil@ifnextchar.{\@call\@interior\@@@@@subtree}{\@@@@@@subtree}}
\def\@@@@@subtree{%
%%% Check for mismatch.
\@ifequal{\the\root@node}{\pgfutil@empty}%
  \root@node=\@result
\fi
\@ifequal{\the\root@node}{\the\@result}\else
  \message{Warning: mismatched labels, \the\root@node{} and \the\@result.}%
\fi
\@@@@@@subtree
}
\def\@@@@@@subtree{%
\@ifequal{\the\root@node}{\pgfutil@empty}
\edef\act{\noexpand\@result={\noexpand\pgfsubtree{\noexpand\path coordinate (\noexpand\nodename);}{\the\child@list}}}%
\else
\edef\act{\noexpand\@result={\noexpand\pgfsubtree{\the\root@node}{\the\child@list}}}%
\fi
\act
\@return}

%% scan a sequence of subtrees or leaves

\newif\ifscanned@edge

\def\@children{%
\scanned@edgefalse
\child@list{}%
\@@children}
\def\@@children{%
\pgfutil@ifnextchar]{\@result\child@list\@return}{% end of children
\pgfutil@ifnextchar\edge{% explicit edge
\ifscanned@edge
\message{Warning: more than one edge given for a single child}\let\next\@@children % ignore
\else
\scanned@edgetrue\let\next\@@@children
\fi
\@call\@edge\next}{%
% else, a real node is next
\ifscanned@edge\else % no explicit edge, supply default
\expandafter\child@list\expandafter{\the\child@list{\edge@adapter{}}}%
\fi
\scanned@edgefalse
\pgfutil@ifnextchar[{\@call\@subtree\@@@children}% subtree
{\@call\@leaf\@@@children} % leaf
}}}
\def\@@@children{%
% wrap child inside curly braces
\expandafter\@result\expandafter{\expandafter{\the\@result}}
\edef\act{\noexpand\child@list{\the\child@list \the\@result}}\act
\@@children
}

\def\@interior.{\@result{\node[alias=\nodename][every tree node,every internal node]}\@label}

\def\@leaf{\@call\@label\@@leaf}
\def\@@leaf{\edef\act{\noexpand\@result{\noexpand\pgfsubtree{\noexpand\node[alias=\noexpand\nodename][every tree node,every leaf node]\the\@result}{}}}\act\@return}

\def\@edge\edge #1;{%
\@result{\edge@adapter{#1}}%
\@return}
\def\edge@adapter#1{%
\let\tikzparentnode\parentnodename
\let\tikzchildnode\nodename
\path edge from parent #1;%
}

% a label is either text or PGF/TikZ code starting with \node
\def\@label{\pgfutil@ifnextchar\node{\@litlabel}{\@@label}}
\def\@@label#1 {%
\expandafter\@result\expandafter{\the\@result{#1};}%
\@return}

% try to copy \node command into \@result without stripping braces
\def\@litlabel\node{\@@litlabel}
\def\@@litlabel{\pgfutil@ifnextchar\bgroup{\@@@litlabel}{\@@@@litlabel}}
\def\@@@litlabel#1{\expandafter\@result\expandafter{\the\@result {#1}}\@@litlabel}
\def\@@@@litlabel#1;{\expandafter\@result\expandafter{\the\@result #1;}\@return}

% predefined edges

\def\tree@edge#1#2{(#1.\pgftree@parentanchor) -- (#2.\pgftree@childanchor)}

\def\roof@edge#1#2{\csname roof@edge@\leveldirection\endcsname{#1}{#2}}
\def\roof@edge@down#1#2{(#1.south) -- (#2.north west) -- (#2.north east) -- cycle}
\def\roof@edge@up#1#2{(#1.north) -- (#2.south west) -- (#2.south east) -- cycle}
\def\roof@edge@left#1#2{(#1.west) -- (#2.north east) -- (#2.south east) -- cycle}
\def\roof@edge@right#1#2{(#1.east) -- (#2.north west) -- (#2.south west) -- cycle}

%%% Options

\tikzoption{level distance}{\pgfmathsetlength\levelsep{#1}}
\tikzoption{sibling distance}{\pgfmathsetlength\subtreesep{#1}} % different semantics

% I don't really like this scheme
\tikzoption{grow}{\csname grow@#1\endcsname}
\tikzoption{grow'}{\csname growprime@#1\endcsname}
\def\grow@up{\def\leveldirection{up}\def\siblingdirection{left}}
\def\grow@down{\def\leveldirection{down}\def\siblingdirection{right}}
\def\growprime@up{\def\leveldirection{up}\def\siblingdirection{right}}
\def\growprime@down{\def\leveldirection{down}\def\siblingdirection{left}}
\def\grow@left{\def\leveldirection{left}\def\siblingdirection{down}}
\def\grow@right{\def\leveldirection{right}\def\siblingdirection{up}}
\def\growprime@left{\def\leveldirection{left}\def\siblingdirection{up}}
\def\growprime@right{\def\leveldirection{right}\def\siblingdirection{down}}

% defaults appropriate for linguistic trees
\tikzset{every tree node/.style={anchor=base}}
\tikzset{every leaf node/.style={}}
\tikzset{every internal node/.style={}}
\def\tikz@edge@to@parent@path{\tree@edge{\tikzparentnode}{\tikzchildnode}}

% predefined roof style
\tikzset{roof/.style={edge from parent path=\roof@edge{\tikzparentnode}{\tikzchildnode}}}


